Computing Simple Mechanisms: Lift-and-Round over Marginal Reduced Forms

We study revenue maximization in multi-item multi-bidder auctions under the natural item-independence assumption - a classical problem in Multi-Dimensional Bayesian Mechanism Design. One of the biggest challenges in this area is developing algorithms to compute (approximately) optimal mechanisms that are not brute-force in the size of the bidder type space, which is usually exponential in the number of items in multi-item auctions. Unfortunately, such algorithms were only known for basic settings of our problem when bidders have unit-demand [CHMS10,CMS15] or additive valuations [Yao15]. In this paper, we significantly improve the previous results and design the first algorithm that runs in time polynomial in the number of items and the number of bidders to compute mechanisms that are $O(1)$-approximations to the optimal revenue when bidders have XOS valuations, resolving an open problem raised in [CM16,CZ17]. Moreover, the computed mechanism has a simple structure: It is either a posted price mechanism or a two-part tariff mechanism. As a corollary of our result, we show how to compute an approximately optimal and simple mechanism efficiently using only sample access to the bidders' value distributions. Our algorithm builds on two innovations that allow us to search over the space of mechanisms efficiently: (i) a new type of succinct representation of mechanisms - the marginal reduced forms, and (ii) a novel Lift-and-Round procedure that concavifies the problem.

==> arXiv/abstract.tex <==
We study revenue maximization in multi-item multi-bidder auctions under the natural \emph{item-independence} assumption -- a classical problem in Multi-Dimensional Bayesian Mechanism Design. One of the biggest challenges in this area is developing algorithms to compute (approximately) optimal mechanisms that are not brute-force in the size of the bidder type space, which is usually exponential in the number of items in multi-item auctions. Unfortunately, such algorithms were only known for basic settings of our problem when bidders have unit-demand ~\cite{ChawlaHMS10,ChawlaMS15} or additive valuations~\cite{Yao15}. 

In this paper, we significantly improve the previous results and design the first algorithm that runs in time \emph{polynomial in the number of items and the number of bidders} to compute mechanisms that are $O(1)$-approximations to the optimal revenue when bidders have XOS valuations, resolving an open problem raised in~\cite{ChawlaM16,CaiZ17}. Moreover, the computed mechanism has a simple structure: It is either a posted price mechanism or a two-part tariff mechanism. As a corollary of our result, we show how to compute an approximately optimal and simple mechanism efficiently using \emph{only sample access} to the bidders' value distributions. Our algorithm builds on two innovations that allow us to search over the space of mechanisms efficiently: (i) a new type of succinct representation of mechanisms -- the \emph{marginal reduced forms}, and (ii) a novel \emph{Lift-and-Round procedure} that concavifies the problem.%Our algorithm is enabled by a novel LP relaxation over a new type of succinct description of mechanisms -- the \emph{marginal reduced forms}, which allows us to search over the space of mechanisms efficiently.

%A recent line of works~\cite{ChawlaHK07,ChawlaHMS10,Alaei11,HartN12,KleinbergW12,CaiH13, BILW14,Yao15,RubinsteinW15,CaiDW16,ChawlaM16,CaiZ17} show that, by exploiting \emph{item-independence} assumption, there exist simple mechanisms that are $O(1)$-approximations to the optimal revenue in general settings. However, these results are largely non-constructive in multi-bidder settings except for basic cases, either when bidders are symmetric or when they have additive or unit-demand valuations. 

%In this paper, we make significant progress in transforming these simple vs. optimal results to be \emph{constructive}, that is, we provide the first polynomial time algorithm to compute simple mechanisms that are $O(1)$-approximations to the optimal revenue in multi-item auctions when bidders have constrained-additive valuations. This is also the first efficient algorithm to achieve an $O(1)$-approximation in this setting even without the simplicity requirement. As a corollary of our result, we show how to compute an approximately optimal and simple mechanism efficiently, when we only have sample access to the bidders' value distributions. Our algorithm is enabled by a novel LP relaxation over the \emph{marginal reduced forms}, which allows us to search over the space of simple mechanisms efficiently.

 %In this paper, we make these simple vs. optimal results \emph{constructive}, that is, we provide the first polynomial time algorithm to compute simple mechanisms that are $O(1)$-approximations to the optimal revenue in multi-item auctions when bidders have XOS valuations, matching the state of the art existential result by Cai and Zhao~\cite{CaiZ17}. This is also the first efficient algorithm to achieve an $O(1)$-approximation in this setting even without the simplicity requirement. As a corollary of our result, we show how to compute an approximately optimal and simple mechanism efficiently with only sample access to the bidders' value distributions. Our algorithm is enabled by a novel LP relaxation over the \emph{marginal reduced forms}, which allows us to search over the space of simple mechanisms efficiently.


%A key component of our LP is what we call the \emph{marginal reduced form} representations of mechanisms.%, which can be viewed as the marginals of the reduced form representation of a mechanism, hence the name.

%To solve our LP, it is necessary to optimize over the polytope $P$ that contains all \emph{feasible marginal reduced forms}, but to the best of our knowledge, $P$ does not have a succinct description or an efficient separation oracle. We provide an efficient separation oracle for a different polytope $Q$ that is sandwiched between $P$ and $c\cdot P$ for some absolute constant $c$ when the bidders have constrained-additive valuations.



%We study the multi-buyer multi-item auction and provide an \emph{efficient} and \emph{simple} mechanism that approximates the optimal revenue. Cai and Zhao~\cite{CaiZ17} proved that a two-part tariff mechanism achieves a constant factor of the optimal revenue, for multiple buyers with XOS valuations. In this paper, we show that we can compute efficiently a two-part tariff that achieves an $O(1)$-approximation, with access to the buyers' value distributions and the demand oracle for buyers' valuations.
%a way to efficiently learn simple mechanisms whose revenue is a constant factor of the optimal one for buyers with XOS valuation when their types for different items are independent. 
%More specifically, we show how to compute an anonymous sequential posted price mechanism with an entry fee when (i) we know the agents' distributions and (ii) we have access to a demand oracle for each agent.


%Our result is enabled by combining the following three new insights: (i) We construct an LP over a set of new polytopes called \emph{marginal reduced form}. When each buyer $i$ has constrained-additive valuations, the $i$-th polytope contains the marginal probabilities that buyer $i$ receives each item $j$ for every realized type $t_{ij}$ for this item, in a feasible allocation. Our program is constructed via a relaxation that searches over a product space of the dual parameters. 
%constructing a multiplicative factor approximation of the polytope of each buyer's Marginal Reduced Forms. When the buyer valuation is constrained additive, this polytope contains for each item the probability that the buyer gets this item under any possible realised type for this item, under any feasible allocation.  Cai and Zhao \cite{CaiZ17} showed how to bound the revenue of a BIC mechanism M, using a set of dual parameters that were tailored-made for $\cM$. 
%(ii) To efficiently compute an approximately-optimal solution to the LP, we prove a multiplicative approximation to the marginal reduced form;  (iii) We robustify the analysis in Cai and Zhao~\cite{CaiZ17} by showing that for any feasible solution of the LP, its objective can be bounded by two-part tariff mechanisms.
%we can still bound the revenue of BIC mechanism $\cM$, under a richer class of dual parameters. 
%In order to compute the simple mechanism, we search over the space of Marginal Interim Forms and the space of dual parameters. Our method is called Marginal Reduced Form Relaxation.

%Moreover, applying the robustness results from Cai, Daskalakis \cite{CaiD17}, we can compute approximately optimal simple mechanism when we have sample access to the agent’s distribution and the agents have constraint additive valuation, by introducing an additive error that tends to $0$ as the number of samples increases. Combining with the result by Cai and Daskalakis~\cite{CaiD17}, we also show that the simple mechanism can be computed efficiently with only sample access to the buyers' distributions.





\notshow{

\argyrisnote{
Notes:
	Should we mention that the results hold with high probability?
	Should we mention that for XOS we need an adjusted demand oracle? We haven't named it yet.
}
\mingfeinote{I think we can mention that in the intro.}




\mingfeinote{

A note for the abstract:

Result: We can compute simple mechanisms.

Technique: 
1. Marginal Reduced Form (Define it) + Relaxation

Cai and Zhao proved that for any mechanism, there exists a set of dual parameters such that the revenue is bounded.

We search over the product space of the dual parameters.

2. Multiplicative approximation for the Marginal Reduced Form.

3. Robustify the analysis from Cai and Zhao, to prove that any feasible solution of the LP can be bounded using simple mechanism. 

Make the learnable result from C-D constructive.

}

}

==> arXiv/appx_exampled_adjustable_oracle.tex <==
\section{Counterexample for Adjustable Demand Oracle}\label{sec:example_adjustable_oracle}

%\todo[inline]{Make the notation consistent. Maybe put the index r to the superscript?}

For XOS valuations, our algorithm for constructing the simple mechanism requires access to a special adjustable demand oracle $\adem_i(\cdot,\cdot,\cdot)$. Readers may wonder if this enhanced oracle (rather than a demand oracle) is necessary to prove our result. In this section we show that (even an approximation of) $\adem_i$ can not be implemented using polynomial number of queries from the value oracle, demand oracle and a classic XOS oracle. All the oracles are defined as follows. Throughout this section, we only consider a single buyer and thus drop the subscript $i$. %For simplicity, we fix any buyer's type $t$ and consider the oracles for this type. One can also think of the distribution $D$ containing a single support $t$. 
Recall that the XOS valuation $v(\cdot)$ satisfies that $v(S)=\max_{k\in [K]}\left\{\sum_{j\in S}\alpha_j^{(k)}\right\}$ for every set $S$, where $\{\alpha_j^{(k)}\}_{j\in [m]}$ is the $k$-th additive function.
\begin{itemize}
    \item Demand Oracle ($\dem$): takes a price vector $p\in \mathbb{R}^m$ as input, and outputs\\ $S^*\in \argmax_{S\subseteq [m]} \left(v(S) - \sum_{j\in S}p_j\right)$.
    \item XOS Oracle (\xos): takes a set $S\subseteq [m]$ as input, and outputs the $k^*$-th additive function $\{\alpha_j^{(k^*)}\}_{j\in [m]}$, where $k^*\in \argmax_{k\in [K]}\left\{\sum_{j\in S}\alpha_j^{(k)}\right\}$.
\item Value Oracle: takes a set $S\subseteq [m]$ as input, and outputs $v(S)$. We notice that a value oracle can be easily simulated with an XOS oracle. Thus we focus on XOS oracles for the rest of this section.
  %  \todo[inline]{People also usually allow value oracles. We should mention that we can simulate a value oracle using an XOS oracle easily. So the result holds even if value oracles are allowed.}
    \item Adjustable Demand Oracle (\adem): takes a coefficient vector $b\in \mathbb{R}^m$ and a price vector $p\in \mathbb{R}^m$ as inputs, and outputs $(S^*,\{\alpha_j^{(k^*)}\}_{j\in [m]})$ where $(S^*,k^*) \in \argmax_{S\subseteq [m],k\in[K]} \left\{\sum_{j\in S}b_j \alpha_{j}^{(k)}- \sum_{j\in S}p_j\right\}$. 
    %\argyrisnote{Argyris: Maybe we change it to:
%$
%(S^*,\{\alpha_{ij}^{(k^*)}(t_{ij})\}_{j\in S^*}) \in \argmax_{S\subseteq [m],k\in[K]} \left\{\sum_{j\in S}b_j \alpha_{ij}^{(k)}(t_{ij}) - \sum_{j\in S}p_j\right\}$.}
\end{itemize}

An (approximate) implementation of $\adem$ is an algorithm that takes inputs $b,p\in \mathbb{R}^m$, and outputs a set $S\subseteq [m]$ and $k\in [K]$. The algorithm has access to the demand oracle and XOS oracle of $v$. We denote $\alg(v,b,p)$ the output of the algorithm. For any $\alpha>1$, $\alg$ is an $\alpha$-approximation to $\adem$ if for every XOS valuation $v$ and every $b,p\in \mathbb{R}^m$, the algorithm outputs $(S',k')$ that satisfies:
$$\max_{S\subseteq [m],k\in[K]} \left\{\sum_{j\in S}b_j \alpha_{j}^{(k)}- \sum_{j\in S}p_j\right\}\leq \alpha\cdot \left(\sum_{j\in S}b_j \alpha_{j}^{(k')}- \sum_{j\in S'}p_j\right)$$


In Theorem~\ref{lem:example_adjustable_oracle} we show that we cannot approximate the output of an Adjustable Demand Oracle within any finite factor,
if we are permitted to query polynomial many times the XOS, Value and Demand Oracle.
%We postpone the proof of Theorem~\ref{lem:example_adjustable_oracle} to Appendix~\ref{sec:appx_example_adjustable_oracle}.

\begin{theorem}\label{lem:example_adjustable_oracle}%\argyrisnote{Argyris: Should we also add a remark saying that the XOS valuation had poly many additive functions? I am a bit worried that it might confuse someone.} \yangnote{Yang: I think it is important to say how we can access an XOS valuation. We assume that one can only access it via demand and XOS queries. Even though the valuations all have poly description size, the algorithm does not see the description.}
Given any $\alpha>1$, there \textbf{does not exist} an implementation of $\adem$ (denoted as $\alg$) that satisfies both of the following properties:
\begin{enumerate}
    \item For any XOS valuation $v$ over $m$ items, $\alg$ makes $\poly(m)$ queries to the value oracle, the demand oracle and XOS oracle of $v$, and runs in time $\poly(m, b)$. Here $b$ is the bit complexity of the problem instance (See Definition~\ref{def:bit complexity}).%\footnote{In this scenario, $b$ is the maximum bit complexity among all $\{\alpha_j^{(k)}\}_{j\in [m], k\in [K]}$.} %\mingfeinote{Mingfei: Maybe also take into account the bit complexity of the problem instance?}
    \item $\alg$ is an $\alpha$-approximation to $\adem$.
\end{enumerate}
\end{theorem}





%\begin{prevproof}{Theorem}{lem:example_adjustable_oracle}
\begin{proof}
Recall that a value oracle can be easily simulated with an XOS oracle. Thus we only argue for demand queries and XOS queries. For the sake of contradiction, assume there exists such an algorithm $\alg$. Let $\ell>e^{2\alpha}$ be an arbitrary even integer. Let $m=2\ell$.
%and any $\eps<(\alpha m)^{-1}$. 
Denote by $L = {\ell \choose \ell/2}$.
We decompose the items into two sets $S_1 = \left\{1,\ldots,\ell \right\}$ and $S_2=\left\{\ell+1,\ldots,m \right\}$. 


We consider an XOS valuation $\widehat{v}$ generated by $2\ell$ additive functions denoted by $\{\widehat{\alpha}_j^{(k)}\}_{j\in[m],k\in[2\ell]}$ parameterized by variables $\eps',\eps$ such that $0 < (\ell+1)\eps' < \eps < \frac{1}{2}$. For $k=1,\ldots,\ell$ and $j\in [m]$:
\notshow{
$$
\widehat{\alpha}_{j}^{(k)}
=
\begin{cases}
j + \eps+ \left(1 - \frac{1}{\ell} \right) \eps' \quad &\text{if $j=k$} \\
0 &\text{if $j\in S_1$ and $j\not=k$} \\
0 \quad &\text{if $j\in S_2$} \\
\end{cases}
$$
}

{$$
\widehat{\alpha}_{j}^{(k)}
=
\begin{cases}
j + \eps+ \left(1 - \frac{1}{\ell} \right) \eps' \quad &\text{if $j=k$} \\
0 &\text{otherwise} \\
\end{cases}
$$}

For $k=\ell + 1,\ldots,2\ell$ and $j\in [m]$, define
$$
\widehat{\alpha}_{j}^{(k)}
=
\begin{cases}
j \quad &\text{if $j=k-\ell$} \\
0 \quad &\text{if $j\in S_1$ and $j\not=k-\ell$}\\
\frac{2}{\ell}\cdot\eps \quad &\text{if $j\in S_2$} \\
\end{cases}
$$


Next, we introduce a family of XOS valuations $\{v_r\}_{r\in [L]}$ over $m$ items. For every $r$, the valuation $v_r$ is generated by $K=2\ell + 1$ additive functions, denoted as $\{\alpha_{r, j}^{(k)}\}_{j\in [m]}, \forall k\in [K]$. We define all the additive functions as follows (and hence $v_r$ is defined as $v_r(S)=\max_{k\in [K]}\sum_{j\in S}\alpha_{r,j}^{(k)}, \forall S\subseteq [m]$):



\paragraph{For $k\in[2\ell]$:}  For every $r\in [L]$ and $j\in[m]$, define
$$
\alpha_{r, j}^{(k)}
=
\widehat{\alpha}_{j}^{(k)}
$$
\paragraph{For $k=2\ell + 1$:} Take any bijective mapping $\mathcal{C}$ between $[L]$ and subsets of $S_2$ of size $\frac{\ell}{2}$. 
For every $r\in [L]$, define
$$
\alpha_{r, j}^{(2\ell+1)}
=
\begin{cases}
1\quad &\text{if $j\in S_1$ and $j\not=\ell$}\\
1+\eps \quad &\text{if $j = \ell$}\\
\frac{2}{\ell}\cdot\eps' \quad &\text{if $j\in \mathcal{C}(r)$} \\
0 \quad &\text{if $j\in S_2\backslash \mathcal{C}(r)$} 
\end{cases}
$$

In the following lemmas, we prove that given access to both the XOS and Demand oracle, the algorithm can not distinguish between valuations $v_r$ and $\widehat{v}$, unless the algorithm knows $\mathcal{C}(r)$ (or $r$).
%In the following lemmas, we formalize this statement.


%\begin{lemma}\label{lem:output-XOS-oracle}
%For any $r\in 2^{[\ell]}$ and input set $S\subseteq [m]$ such that $S\cap S_2 \neq \mathcal{C}(r)$, then $\adem(v_r,S) = \adem(\widehat{v},S)$.
%\end{lemma}




\begin{lemma}\label{lem:v_r val}
For any $r\in [L]$ and any nonempty set $S\subseteq [m]$,
%if $S_1\not\subseteq S$ or $S\cap S_2 \neq \mathcal{C}(r)$ there exists an additive function with index $k^*\in[2\ell]$ such that $\sum_{j\in S}\alpha_{r,j}^{(k^*)} > \sum_{j\in S}\alpha_{r,j}^{(2\ell+1)}$. If $S_1\subseteq S$ and $S\cap S_2 = \mathcal{C}(r)$, then for any $k\in [2\ell]$,$\sum_{j\in S}\alpha_{r,j}^{(2\ell+1)} > \sum_{j\in S}\alpha_{r,j}^{(k)} $. 
$
\sum_{j\in S}\alpha_{r,j}^{(2\ell+1)} > \sum_{j\in S}\alpha_{r,j}^{(k)} 
$ for all $k\in [2\ell]$ if and only if $S=S_1\cup \mathcal{C}(r)$.
Hence for any $r\in [\ell]$ and any nonempty set $S\subseteq [m]$,
$$\xos(v_r,S)=
\begin{cases}
\{\alpha_{r,j}^{(2\ell+1)}\}_{j\in[m]} \quad & \text{if $S=S_1\cup \mathcal{C}(r)$ %S_1\subseteq S$ and $S\cap S_2 = \mathcal{C}(r)$
}\\
\xos(\widehat{v},S) \quad & \text{otherwise}
\end{cases}$$
\end{lemma}


\begin{proof}
%Observe that valuation $v_r$ and $\widehat{v}$ do not have only additive valuation $\{\alpha_{r,j}^{(2\ell+1)}\}_{j\in[m]}$ in common.
%Thus, it is enough to show $\adem(v_r,S)$ returns $\{\alpha_{r,j}^{(2\ell+1)}\}_{j\in[m]}$ if and only if $S\cap S_1 = S_1$ and $S\cap S_2= \mathcal{C}(r)$.
Let $j^* = \max\{j: j\in S_1\cap S\}$ (define it to be 0 if $S\cap S_1=\emptyset$). We consider the following cases:

\begin{itemize}
\item Case 1: $S\cap S_1=\emptyset$. Then $S\subseteq S_2$. For any $k^*=\ell + 1,\ldots,2\ell$,
$$
\sum_{j\in S} \alpha_{r,j}^{(k^*)} = \sum_{j\in S}  \frac{2}{\ell}\eps
> \sum_{j\in S} \frac{2}{\ell}\eps'\geq \sum_{j\in S\cap \mathcal{C}(r)} \frac{2}{\ell}\eps'= \sum_{j\in S} \alpha_{r,j}^{(2\ell+1)}
$$

\item Case 2: $S\cap S_2=\emptyset$. Then $S\subseteq S_1$ and $S\cap S_1 \neq \emptyset$, which implies that $j^* > 0$. We have
$$
\sum_{j\in S} \alpha_{r,j}^{(j^*)} = j^* + \eps+ \left(1 - \frac{1}{\ell} \right) \eps'
> j^* + \eps
\geq \sum_{j=1}^{j^*} \alpha_{r,j}^{(2\ell+1)}
\geq 
\sum_{j\in S} \alpha_{r,j}^{(2\ell+1)}
$$
Here the second last inequality follows from the fact that $S\subseteq S_1$ and $\alpha_{r,j}^{(2\ell+1)}=1$ for every $j\in S_1/\{\ell\}$ and $\alpha_{r,\ell}^{(2\ell+1)}=1+\eps$. The last inequality follows from the definition of $j^*$. 

\item Case 3: $S_1\not\subseteq S$, $S\cap S_1\neq \emptyset$ and $S\cap S_2 \neq \emptyset$. We have that

$$
\sum_{j\in S} \alpha_{r,j}^{(\ell+j^*)} = j^* + \sum_{j\in S_2\cap S}\frac{2}{\ell}\eps 
>
j^* +  \sum_{j\in S_2\cap S}\frac{2}{\ell}\eps'
\geq 
\sum_{j\in S} \alpha_{r,j}^{(2\ell+1)}
$$

The last inequality follows from the fact that $\sum_{j\in S\cap S_1}\alpha_{r,j}^{(2\ell+1)}\leq j^*$: If $j^*\not=\ell$, then $\alpha_{r,j}^{(2\ell+1)}=1,\forall j\in S\cap S_1$; If $j^*=\ell$, since $S_1\not\subseteq S$, $\sum_{j\in S\cap S_1}\alpha_{r,j}^{(2\ell+1)}=|S\cap S_1|+\eps\leq (\ell-1)+\eps<\ell$. 

\item Case 4: $S_1\subseteq S$ and $S\cap S_2 \neq \mathcal{C}(r)$. We have

$$
\sum_{j\in S} \alpha_{r,j}^{(\ell)} = \alpha_{r,\ell}^{(\ell)}=
\ell+ \eps+ \left(1 - \frac{1}{\ell} \right) \eps'
>
\left(\ell + \eps\right) +  \sum_{j\in \mathcal{C}(r)\cap S}\frac{2}{\ell}\eps'
= 
\sum_{j\in S} \alpha_{r,j}^{(2\ell+1)}
$$
Here the inequality is because: $\mathcal{C}(r)\cap S \neq \mathcal{C}(r)$, then $|\mathcal{C}(r)\cap S| \leq \frac{\ell}{2} - 1$,
which implies that $\sum_{j\in \mathcal{C}(r)\cap S}\frac{2}{\ell}\eps' \leq \left(\frac{\ell}{2}-1\right)\frac{2}{\ell}\eps' < \left(1-\frac{1}{\ell}\right)\eps'$.

\item Case 5: $S_1\subseteq S$ and $S\cap S_2 = \mathcal{C}(r)$. Recall that $|\mathcal{C}(r)|=\frac{\ell}{2} $. We notice that $\sum_{j\in S}  \alpha_{r,j}^{(2\ell+1)} = \ell + \eps + \eps'
$. On the other hand,
$$
\max_{k\in [\ell]} \sum_{j\in S}  \alpha_{r,j}^{(k)} 
= \sum_{j\in S} \alpha_{r,j}^{(\ell)}= \ell + \eps+ \left(1 - \frac{1}{\ell} \right) \eps' < \sum_{j\in S}  \alpha_{r,j}^{(2\ell+1)} 
$$

and

$$
\max_{\ell< k\leq 2\ell} \sum_{j\in S}  \alpha_{r,j}^{(k)} 
= \sum_{j\in S} \alpha_{r,j}^{(2\ell)}
= \ell + \sum_{j\in \mathcal{C}(r)} \alpha_{r,j}^{(2\ell)}= \ell + \eps < \sum_{j\in S}  \alpha_{r,j}^{(2\ell+1)} 
$$
\end{itemize}

We have proved the first part of the statement. The second part of the statement then follows by noticing that the first $2\ell$ additive functions of $v_r$ and $\widehat{v}$ are exactly the same.  
\end{proof}

%\Cref{cor:output-XOS-oracle} follows directly from \Cref{lem:v_r val}.

%\begin{corollary}\label{cor:output-XOS-oracle}
%For any $r\in [\ell]$ and input set $S\subseteq [m]$,
%then
%$$\xos(v_r,S)=
%\begin{cases}
%\{\alpha_{r,j}^{(2\ell+1)}\}_{j\in[m]} \quad & \text{if $S_1\subseteq S$ and $S\cap S_2 = \mathcal{C}(r)$}\\
%\xos(\widehat{v},S) \quad & \text{otherwise}
%\end{cases}$$
%\end{corollary}

\begin{lemma}\label{lem:output-Demand-oracle}
For any $r\in [L]$ and any set of prices $\bm{p} \in \mathbb{R}^m_{\geq 0}$ such that $\{j\in S_2: p_j \leq \frac{2}{\ell}\eps'\}\neq \mathcal{C}(r)$, we have $\dem(v_r,\bm{p})= \dem(\widehat{v},\bm{p})$.
\end{lemma}

\begin{proof}
Recall that

$$ \dem(v_r,\bm{p}) \in \argmax_{S\subseteq [m]} \left\{v_r(S) - \sum_{j\in S} p_j\right\} = \argmax_{S\subseteq [m]}\left\{\max_{k \in [K]}  \sum_{j\in S} (\alpha_{r,j}^{(k)} - p_j)\right\}$$

We notice that valuations $v_r$ and $\widehat{v}$ differ only in the $(2\ell+1)$-th additive valuation (with coefficients $\{\alpha_{r,j}^{(2\ell+1)}\}_{j\in[m]}$). Thus by \Cref{lem:v_r val}, $\dem(v_r,\bm{p})= \dem(\widehat{v},\bm{p})$ unless $S^*=S_1\cup \mathcal{C}(r)$ is the favorite bundle for valuation $v_r$ at price $\bm{p}$, i.e. 
$$\sum_{j\in S_1\cup \mathcal{C}(r)}(\alpha_{r,j}^{(2\ell+1)} - p_j) = \max_{S\subseteq [m], k \in [K]}  \sum_{j\in S} (\alpha_{r,j}^{(k)} - p_j)$$

Let $S_0= \{j\in S_2 : p_j \leq \frac{2}{\ell}\eps'\}$.
%First we are going to prove that when $S \cap \mathcal{C}(r) \subset \mathcal{C}(r)$,
%then $\dem(v_r,p)= \dem(\widehat{v},p)$.
Firstly, if $\mathcal{C}(r)\not\subseteq S_0$, then there exists $j\in S_2$ such that $p_j>\frac{2}{\ell}\eps'$. Since $\alpha_{r,j}^{(2\ell+1)}=\frac{2}{\ell}\eps',\forall j\in \mathcal{C}(r)$, we have  
$$\sum_{j\in S_1\cup \mathcal{C}(r)}(\alpha_{r,j}^{(2\ell+1)} - p_j)
<
\sum_{j\in S_1\cup({\mathcal{C}(r)\cap} S_0)}(\alpha_{r,j}^{(2\ell+1)} -  p_j)
\leq \max_{S\subseteq [m], k \in [K]}  \sum_{j\in S} (\alpha_{r,j}^{(k)} - p_j),$$
%\argyrisnote{Argyris: Maybe change the above two sentences to: Let $S_0= \{j\in S_2 : p_j \leq \frac{2}{\ell}\eps'\}$.
%First we are going to prove that when $S \cap \mathcal{C}(r) \subset \mathcal{C}(r)$,
%then $\dem(v_r,p)= \dem(\widehat{v},p)$.
%Firstly, if $\mathcal{C}(r)\not\subseteq S_0$, then there exists $j\in S_2 \backslash \mathcal{C}(r)$ such that $p_j>\frac{2}{\ell}\eps'$. Since $\alpha_{r,j}^{(2\ell+1)}=\frac{2}{\ell}\eps',\forall j\in \mathcal{C}(r)$, we have  
%$$\sum_{j\in S_1\cup \mathcal{C}(r)}(\alpha_{r,j}^{(2\ell+1)} - p_j)<\sum_{j\in S_1\cup (\mathcal{C}(r)\cap S_0)}(\alpha_{r,j}^{(2\ell+1)} -  p_j)\leq \max_{S\subseteq [m], k \in [K]}  \sum_{j\in S} (\alpha_{r,j}^{(k)} - p_j),$$}

which implies that $\dem(v_r,\bm{p})=\dem(\widehat{v},\bm{p})$. It remains to consider the case where $\mathcal{C}(r)\subseteq S_0$ and $\mathcal{C}(r)\not=S_0$. We have
$$\sum_{j\in S_1\cup \mathcal{C}(r)}(\alpha_{r,j}^{(2\ell+1)} - p_j)
\leq \ell +\eps - \sum_{j\in S_1}p_j 
+ \sum_{j \in \mathcal{C}(r)} \alpha_{r,j}^{(2\ell+1)} 
= \ell +\eps - \sum_{j\in S_1}p_j 
+ \eps'
$$
Here the first inequality follows from $\sum_{j\in S_1}\alpha_{r,j}^{(2\ell+1)}=\ell+\eps$ and $p_j\geq 0,\forall j\in \mathcal{C}(r)$. And the equality follows from $\sum_{j \in \mathcal{C}(r)} \alpha_{r,j}^{(2\ell+1)}= |\mathcal{C}(r)|\cdot \frac{2}{\ell}\eps'=\ell/2\cdot \frac{2}{\ell}\eps'=\eps'$. %since $|\mathcal{C}(r)| = \frac{\ell}{2}$ and $\alpha_{r,j}^{(2\ell+1)} = \frac{2}{\ell}\eps'$ for $j\in \mathcal{C}(r)$.
On the other hand, %let $T=S_0\backslash \mathcal{C}(r)$.

\begin{align*}
\sum_{j\in S_1\cup S_0}(\alpha_{r,j}^{(2\ell)} -  p_j)
&= \ell  - \sum_{j\in S_1}p_j 
+ \sum_{j \in S_0} \left(\alpha_{r,j}^{(2\ell)} - p_j\right) \\
&\geq \ell  - \sum_{j\in S_1}p_j 
+ \sum_{j \in S_0} \left(\frac{2}{\ell}\eps - \frac{2}{\ell}\eps'\right) \\
&\geq  \ell  - \sum_{j\in S_1}p_j 
+  \left( \frac{\ell}{2}+1\right)\left(\frac{2}{\ell}\eps - \frac{2}{\ell}\eps'\right)\\
&=  \ell  - \sum_{j\in S_1}p_j 
+ \eps -\eps' + \frac{2}{\ell}\left( \eps - \eps'\right) \\
&> \ell  - \sum_{j\in S_1}p_j 
+ \eps -\eps' + \frac{2}{\ell}\left( (\ell+1)\eps' - \eps'\right) \\
&=  \ell + \eps + \eps' - \sum_{j\in S_1}p_j
\end{align*}
Here the first inequality follows from $p_j \leq \frac{2}{\ell}\eps'$, $\alpha_{r,j}^{(2\ell)}=\frac{2}{\ell}\eps$ for $j\in {S_0}$. The second inequality follows from $|S_0| \geq \frac{\ell}{2}+1$, since $|\mathcal{C}(r)|=\frac{\ell}{2}$, $\mathcal{C}(r)\subseteq S_0$, and $\mathcal{C}(r)\not=S_0$. The third inequality follows from our choice of $\eps$ and $\eps'$ such that $\eps > (\ell+1)\eps'$. Thus,
$$
\sum_{j\in S_1\cup \mathcal{C}(r)}(\alpha_{r,j}^{(2\ell+1)} - p_j) < \sum_{j\in S_1\cup S_0}(\alpha_{r,j}^{(2\ell)} - p_j) \leq \max_{S\subseteq [m], k \in [K]}  \sum_{j\in S} (\alpha_{r,j}^{(k)} - p_j)
$$
which implies that $\dem(v_r,\bm{p})=\dem(\widehat{v},\bm{p})$.
%Thus if $C(r) \neq S$, then $\dem(v_r,\bm{p})=\dem(\widehat{v},\bm{p})$.
\end{proof}


\begin{comment}
In the following lemma, we analyze the possible outputs of its XOS oracle for any fixed $v_r$. A direct implication of \Cref{lem:output-XOS-oracle} is that none of the above $2^\ell+\ell$ additive functions is redundant. 


\begin{lemma}\label{lem:output-XOS-oracle}
For any valuation $v_r$ and input set $S\subseteq [m]$, let $k^*$ be the index of the output additive function from the XOS oracle. We have
\begin{enumerate}
    \item If $S\cap S_2\not=\emptyset$, then $k^*$ is the (unique) $k$ that satisfies  $\mathcal{C}(k)=S\cap S_2$. 
    \item If $S\cap S_2=\emptyset$, then $k^*=2^\ell+\max\{j:j\in S\}$. 
\end{enumerate}
\end{lemma}

\begin{proof}
First suppose the input set $S$ satisfies $S\cap S_2\not=\emptyset$. Note that $\alpha_{r,j}^{(k)}\leq 2\ell$ for any $j\in S_1$. We calculate $\sum_{j\in [m]}\alpha_{r,j}^{(k)}$ for $k\in [2^\ell]$ by a case study. Let $x=|S\cap S_2|\leq \ell$.
\begin{enumerate}
    \item $\mathcal{C}(k)=S\cap S_2$: Now $\sum_{j\in S}\alpha_{r,j}^{(k)}\geq \sum_{j\in S\cap S_2}\alpha_{r,j}^{(k)}=\gamma x(2\ell-x)$.
    \item $|\mathcal{C}(k)|=x$ and $\mathcal{C}(k)\not=S\cap S_2$: Now $$\sum_{j\in S}\alpha_{r,j}^{(k)}=\sum_{j\in S\cap S_1}\alpha_{r,j}^{(k)}+\sum_{j\in S\cap S_2}\alpha_{r,j}^{(k)}\leq 2\ell\cdot \ell+\gamma(x-1)(2\ell-x)<\gamma x(2\ell-x),$$ where the last inequality follows from $\gamma> 2\ell^2$ and $2\ell-x\geq 1$. 
    \item $|\mathcal{C}(k)|<x$: Now $\sum_{j\in S}\alpha_{r,j}^{(k)}\leq 2\ell\cdot \ell+\gamma|\mathcal{C}(k)|\cdot (2\ell-|\mathcal{C}(k)|)\leq 2\ell^2+\gamma(x-1)(2\ell-x+1)<\gamma x(2\ell-x)$, since $\gamma>2\ell^2$ and $x\leq \ell$.  
    \item $|\mathcal{C}(k)|>x$: Now $\sum_{j\in S}\alpha_{r,j}^{(k)}\leq 2\ell\cdot \ell+\gamma x\cdot (2\ell-|\mathcal{C}(k)|)\leq 2\ell^2+\gamma x(2\ell-x-1)<\gamma x(2\ell-x)$, since $\gamma>2\ell^2$ and $x\geq 1$ because $S\cap S_2\not=\emptyset$. 
\end{enumerate}
Thus the output $k^*$ of the XOS oracle is the (unique) $k$ that satisfies  $\mathcal{C}(k)=S\cap S_2$.

The other case is simpler. Consider any $S$ such that $S\cap S_2=\emptyset$, i.e. $S\subseteq S_1$. Let $j^*=\max\{j:j\in S\}\leq \ell$ be the largest index of items in $S$. Then $|S|\leq j^*$. If $k\in [2^\ell]$, then $\sum_{j\in S}\alpha_{r,j}^{(k)}\leq |S|\leq j^*$. If $k\in (2^\ell,2^\ell+j^*]$, $\sum_{j\in S}\alpha_{r,j}^{(k)}=2(k-2^\ell)$. If $k>2^\ell+j^*$, then $\sum_{j\in S}\alpha_{r,j}^{(k)}=0$. Thus the output $k^*$ of the XOS oracle is $k^*=2^\ell+j^*$. 
\end{proof} 
\end{comment}

To complete the proof of \Cref{lem:example_adjustable_oracle}, set $\eps = 0.1$ and $\eps' = \frac{0.1}{2(\ell+1)}$. We notice that the bit complexity of our input is $b=O(\poly(\ell))$ for any valuation $v_r$.
Now consider the coefficient vector $\bm{c}=(1, 1/2,\ldots, 1/\ell, 0, \ldots, 0)$ with price vector $\bm{p}=\textbf{0}$. For any valuation $v_r$ in the family, clearly $\adem$ will select the whole set $[m]$ since all coefficients are non-negative. 

For any $k\in [2\ell]$, $\sum_{j\in [m]}c_j\alpha_{r,j}^{(k)}\leq 1 + \eps + \left(1-\frac{1}{\ell}\right)\eps'<2$. 
%$$\sum_{j\in [m]}b_j\alpha_{r,j}^{(k)}=\sum_{j\in [\ell]}(1-\eps)^{j-1}\cdot (1-\eps)^{\ell-j}=\ell\cdot (1-\eps)^{\ell-1}\leq \ell\cdot e^{-(\ell-1)\eps}$$
%For any $k\in \{2^\ell+1,\ldots,2^{\ell}+\ell\}$, $\sum_{j\in [m]}b_j\alpha_{r,j}^{(k)}=\frac{1}{k-2^\ell}\cdot 2(k-2^\ell)=2$. 
%we notice that $b_{a_{k,i}}\leq (1-\eps)^{i-1}$ since $a_{k,i}$ is larger than at least $i-1$ elements in $S_1$. Thus  
%$$\sum_{j\in [m]}b_j\alpha_{r,j}^{(k)}\leq\sum_{i=1}^{|T_k|}(1-\eps)^{i-1}\cdot (1-\eps)^{|T_k|-i}=|T_k|\cdot (1-\eps)^{|T_k|-1}\leq \max_{x\in [\ell]}\{x\cdot e^{-(x-1)\eps}\}=\ell\cdot e^{-(\ell-1)\eps}$$
%Here the last inequality follows from $1-y<e^{-y}$ for $y\in (0,1)$. The last equality follows from taking derivative of $x\cdot e^{-(x-1)\eps}$ and $\ell\eps<1$ \mingfeinote{Mingfei: Here we use the fact that $\ell\eps<1$. If $\ell\eps>1$, choosing $x=1/\eps$ will maximize the above term.}. 
On the other hand, when $k=2\ell+1$, since $\ell>e^{2\alpha}$ we have
$$\sum_{j\in [m]}c_j\alpha_{r,j}^{(2\ell+1)}\geq\sum_{j\in [\ell]}\frac{1}{j}\cdot 1>\log(\ell)>2\alpha>\alpha\cdot \max_{k\not=2\ell+1}\left\{\sum_{j\in [m]}c_j\alpha_{r,j}^{(k)}\right\}=\alpha\cdot \max_{k}\left\{\sum_{j\in [m]}c_j\widehat{\alpha}_{j}^{(k)}\right\}$$
%$$\sum_{j\in [m]}b_j\alpha_{r,j}^{(r)}=\sum_{j\in [\ell]}(1-\eps)^{2(j-1)}=\frac{1-(1-\eps)^{2\ell}}{1-(1-\eps)^2}\geq \frac{1-(1-\eps)^{2\ell}}{2\eps}\geq \frac{1-e^{-2\ell\eps}}{2\eps}$$

%Hence we have 

%$$\frac{\sum_{j\in [m]}b_j\alpha_{r,j}^{(r)}}{\max_{k\not=r}\left\{\sum_{j\in [m]}b_j\alpha_{r,j}^{(k)}\right\}}\geq \frac{1}{2\ell\eps}\cdot\frac{1-e^{-2\ell\eps}}{e^{-(\ell-1)\eps}}$$

%\mingfeinote{Mingfei: Let $\ell\eps=x$, then the ratio $1/x\cdot \frac{1-e^{-x}}{e^{-x/2}}$ goes to 1 when $x\to 0$. If $\ell\eps>1$, then $\max_{x\in [\ell]}\{x\cdot e^{-(x-1)\eps}\}$ is maximized when $x=1/\eps$, which becomes comparable to $\sum_{j\in [\ell]}(1-\eps)^{2(j-1)}$.}

Thus informally speaking, to obtain an $\alpha$-approximation to $\adem$ for every valuation $v_r$, the algorithm needs to distinguish $v_r$ from $\widehat{v}$ by identifying the $(2\ell+1)$-th additive function. %, among $2\ell+1$ additive functions. 
%However, each XOS query returns at most one additive function, while demand queries do not return any information about the additive function. %By setting $\eps = 0.1$ and $\eps' = \frac{0.1}{2(\ell+1)}$ We notice that $b=O(\log\ell)$ for any valuation $v_r$.
By Lemmas~\ref{lem:v_r val} and \ref{lem:output-Demand-oracle}, the algorithm must be able to identify $r$ or $\mathcal{C}(r)$. However, there are $L = {\ell \choose \ell/2}$ different valuations in the family $\{v_r\}_{r\in [L]}$. Thus there must exist one $v_r$ such that the algorithm can not distinguish $v_r$ from $\widehat{v}$ within $poly(\ell)=poly(m,b)$ queries to both oracles. 

%Formally, consider another XOS valuation $\widehat{v}$. $\widehat{v}(S)=\max_{k\in [K]}\sum_{j\in S}\widehat{\alpha}_{j}^{(k)}, \forall S\subseteq [m]$. $\widehat{\alpha}_{j}^{(k)}=0$ if $k\in [2^\ell]$ and $j\in S_1$; otherwise, pick any $r\in [2^\ell]$ and let $\widehat{\alpha}_{j}^{(k)}=\alpha_{r,j}^{(k)}$. In other words, $\widehat{\alpha}_{j}^{(k)}$ differs from any $\alpha_{r,j}^{(k)}$ only when $j\in S_1$ and $k=r$. 
Formally, consider the execution of $\alg$ on valuation $\widehat{v}$. Let $Q$ be the total number of queries during the execution and define set $S^{(1)},\ldots,S^{(Q)}\subseteq [m]$ as follows: For every $q\in [Q]$, if the $q$-th query is an XOS query, define $S^{(q)}$ as the input set to the XOS oracle; If it's a demand query, let $S^{(q)}=\{j\in S_2: p_j^{(q)} \leq \frac{2}{\ell}\eps'\}$, where $\bm{p}^{(q)}=\{p_j^{(q)}\}_{j\in [m]}$ is the input price vector to the demand oracle.  
%be all the input queries to the XOS oracle and $\bm{p}^{(1)},\ldots,\bm{p}^{(Q)}$ be the input queries to the Demand Oracle during the execution of $\alg$ on input $\widehat{v}$.
%Since the number of queries 
Recall that $m=2\ell$ and $b=\poly(\ell)$, we have $Q=\poly(m, b)<L = {\ell \choose \ell/2}$ for sufficiently large $\ell$. Thus there exists some $r^*\in [L]$ such that $\mathcal{C}(r^*)\not=S_2\cap S^{(q)}$ %and $\mathcal{C}(r^*) \not= \{j\in S_2: \bm{p}^{(q)}_j \leq \frac{2}{\ell}\eps'\}$ 
for any $q\in [Q]$.
By \Cref{lem:v_r val}, we have that $\xos(\widehat{v},S^{(q)})=\xos(v_r,S^{(q)})$ and by \Cref{lem:output-Demand-oracle} we have that $\dem(\widehat{v},\bm{p}^{(q)}) = \dem(v_r,\bm{p}^{(q)})$ for any $q\in [Q]$. 
This implies that the execution (and thus output) of $\alg$ on input valuation $\widehat{v}$ is exactly the same as its execution on $v_{r^*}$.  
%$\alg$ can not distinguish $v_{r^*}$ from $\widehat{v}$. 

We notice that from the above calculation, $\max_{k}\left\{\sum_{j\in [m]}c_j\alpha_{r^*,j}^{(k)}\right\}\geq\sum_{j\in [\ell]}\frac{1}{j}>\log(\ell)>2\alpha$, while
$\max_{k}\left\{\sum_{j\in [m]}c_j\widehat{\alpha}_{j}^{(k)}\right\}=\max_{k\not=2\ell+1}\left\{\sum_{j\in [m]}c_j\alpha_{r^*,j}^{(k)}\right\}<2$. Thus on input $(v_{r^*},\bm{c})$, $\alg$ achieves less than a $\frac{1}{\alpha}$-fraction of the optimal objective from $\adem$, contradicting with the fact that $\alg$ is an $\alpha$-approximation to $\adem$. 
\end{proof}
%\end{prevproof}





==> arXiv/appx_polytope.tex <==
%\section{Missing Details from Section~\ref{sec:multi-approx-polytope}}\label{sec:appx_polytope}

\section{Multiplicative Approximation of Down-Monotone and Boxable Polytopes}\label{sec:multi-approx-polytope}

In this section, we provide a proof of \Cref{thm:multiplicative approx for constraint additive-main body} and prove \Cref{thm:main XOS-main body} for constrained-additive valuations using \Cref{thm:multiplicative approx for constraint additive-main body}. We restate the theorem here.

\begin{theorem}\label{thm:main}
(Restatement of \Cref{thm:main XOS-main body} for constrained-additive valuations) Let $T=\sum_{i,j}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance (\Cref{def:bit complexity}).
%~\footnote{For any instance of our problem, define \emph{the bit complexity of the problem instance}, as the maximum bit complexity of $n$,$m$,$f_{ij}(t_{ij})$ and $t_{ij}$ %(or $\alpha_{ij}^{(k)}(t_{ij})$ for XOS buyers) 
%over all $i,j,t_{ij}\in \cT_{ij}$.
%See \Cref{def:bit complexity} for more details.} 
For constrained-additive buyers, for any $\delta>0$, there exists an algorithm that computes a rationed posted price mechanism or a two-part tariff mechanism, such that the revenue of the mechanism is at least $c\cdot \opt$ for some absolute constant $c>0$ with probability $1-\delta-\frac{2}{n}$. Our algorithm assumes query access to a value oracle and a demand oracle of buyers' valuations, and has running time $\poly(n,m,T,b,\log (1/\delta))$.
\end{theorem}


For \Cref{thm:multiplicative approx for constraint additive-main body}, we indeed prove a result for a natural family of polytopes. Throughout this section, we assume that the polytope we consider is  \emph{down-monotone}. Formally, a polytope $\cP\subseteq [0,1]^d$ is down-monotone if and only if for every $\bx\in \cP$ and $\textbf{0}\leq \bx'\leq \bx$, we have $\bx'\in \cP$.
To state our result, we need the following definitions.

\begin{definition}
For any two sets $A,B \subseteq \mathbb{R}^d$,
we denote by $A+B$ the \emph{Minkowski addition} of set $A$ and set $B$ where:
$$A+B = \{a + b : a \in A\text{ and } b \in B\}
$$

Note that if both $A$ and $B$ are convex, then $A+B$ is also convex.
\end{definition}

\begin{definition}
Let $\cP$ be a convex polytope, we define $a\cdot \cP:=\{a\bx: \bx\in\cP\}$ for any $a\geq 0$.
\end{definition}

\begin{definition}\label{def:mixture}
Let $\ell$ be a finite integer. For any set of convex sets $\{\cP_i\}_{i\in [\ell]}$ and a distribution $\cD=\{q_i\}_{i\in[\ell]}$, %over the elements in $[N]$.
 the set $\cP = \sum_{i\in[\ell]}q_i \cP_i$
is called the mixture of $\{\cP_i\}_{i\in [\ell]}$ over distribution $\cD$.
\end{definition}


\begin{definition}\label{def:truncated polytope}
%\argyrisnote{Argyris: I don't think downward closed refer to polytopes? I named it lower-closed instead}
Let $\cP,\cQ\subseteq [0,1]^d$ be down-monotone polytopes. For each coordinate $j\in[d]$,
we define the width of $\cP$ at coordinate $j$ as $l_j(\cP)=\max_{\bx\in \cP}x_j$.
%{$l_j(\cP)=\sup_{\bx\in \cP}x_j$.}
%We say that $\cP$ is lower-closed if for each $p \in \cP$,
%then for $p'\in [0,1]^d$ such that
%$$
%0\leq p'(j)\leq p(j) \quad \forall j \in[d]
%$$
%we have that $p' \in \cP$.
%Moreover w
For any $\eps>0$, we define the {($\eps,\cQ$)-truncated polytope of $\cP$ (denoted as $\cP^{tr(\eps,\cQ)}$)} in the following way: $\bx\in \cP^{tr(\eps,\cQ)}$ if and only if there exists $\bx'\in \cP$ such that $x_j=x_j'\cdot \ind[l_j(\cQ)\geq \eps],\forall j\in [d]$.
%For each $\bx\in \cP$, then for the element $p'\in [0,1]^d$ such that
%$$
%p'(i)=
%\begin{cases}
%p(i) \quad &\text{if $\eps \leq l_i(\cP)$} \\
%0 & \text{o.w.}
%\end{cases}\quad \forall i\in[d]
%$$
%Note that if $\cP$ is lower-closed,
%then for each $\eps>0$, $\cP_\eps^t \subseteq \cP$.
We notice that since $\cP$ is down-monotone, $\cP^{tr(\eps,\cQ)}\subseteq \cP$. Moreover, $\cP^{tr(\eps,\cQ)}$ is convex if $\cP$ is convex.
We also use $\cP^{tr(\eps)}$ to denote $\cP^{tr(\eps,\cP)}$.
\end{definition}


\begin{definition}\label{def:box polytope}
Let $\cP\subseteq [0,1]^d$.
%First we are going to describe a way to partition the coordinates of $\cP$.
%For each $i\in[d]$,
%we say that the $i$-th coordinate of $\cP$ is $\eps$-good if $l_j(\cP) \geq \eps$. 
%We say that the $i$-th coordinate of $\cP$ is $\eps$-bad if it is not $\eps$-good.
For any $\eps>0$, define the $\eps$-box polytope $\pbox$ of $\cP$ as follows: 
{$\pbox=\{\bx\subseteq [0,1]^d: x_j\leq \min\left( \eps,l_j(\cP)\right),\forall j\in [d]\}$.} Clearly, $\pbox$ is convex.
%For any element $p\in [0,\eps]^d$ such that:
%$$
%p(i) \leq
%\min\left( \eps,l_i(\cP)\right) \quad \forall i \in[d]
%$$
%then $p\in \cP^b_\eps$.
%Under some natural polytopes $\cP$,
%we can prove that for sufficiently small $\eps$,
%then $\cP_\eps^b \subseteq \cP$.
%This property is going to be very usefull.
%\mingfeinote{Mingfei: What does this sentence mean?}
\end{definition}


\Cref{thm:special case of multiplicative approx} is the main theorem of this section. We prove that if $\cP$ is a mixture of a set of down-monotone, convex polytopes $\{\cP_i\}_{i\in[\ell]}$, and $\cP$ contains the polytope $c\cdot\pbox$ for some {$c\leq1$}, then there exists another down-monotone, convex polytope $\widehat{\cP}$ sandwiched between $c/6\cdot \cP$ and $\cP$. {And more importantly, we have an efficient separation oracle for $\widehat{\cP}$, whose running time is \emph{independent of $\ell$}, as long as we can efficiently optimize any linear objective for every $\cP_i$. The key feature of our separation oracle for $\widehat{\cP}$ is that its running time does not depend on $\ell$, as in our applications, $\ell$ is usually exponential in the input size.}


\begin{theorem}\label{thm:special case of multiplicative approx}%[(Concrete Version of \Cref{thm:special case of multiplicative approx-main body})]
Let $\ell$ be a positive integer, and $\cP \subseteq [0,1]^d$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in [\ell]}$,
where for each $i\in[\ell]$, $\cP_i\subseteq [0,1]^d$ is a convex and down-monotone polytope. 
%Let $b_l$ be an upper bound on the bit complexity of vector $\{l_j(\cP)\}_{j\in[d]}$.
%Let $b$ be an upper bound on the bit complexity of all corners in $\cP_i$ for each $i\in [\ell]$.
Suppose for every $i\in [\ell]$, %the bit complexity of every corner in $\cP_i$ is at most $b$, and 
{there exists an oracle $\cQ_i(\cdot)$, whose output $\cQ_i(\bm{a})\in \argmax\{\bm{a}\cdot \bx:\bx\in \cP_i\}$ for any input $\bm{a}\in \mathbb{R}^d$. % that solves the optimization problem $\max\{\mathbf{a}\cdot \bx:\bx\in \cP_i\}$ for any $\mathbf{a}\in \mathbb{R}^d$.
Given $\{l_j(\cP)\}_{j\in[d]}$, suppose $c\cdot\pbox\subseteq \cP$ for some $\eps>0$ and $c\in (0,1]$. Let $b$ be an upper bound on the bit complexity of $\cQ_i(\bm{a})$ for all $i\in[\ell]$ and $\bm{a}\in \mathbb{R}^d$, as well as on the bit complexity of $l_j(\cP)$ for all $j\in [d]$.} %\footnote{\yangnote{Yang: I removed the assumption that the bit complexity of a corner is at most $b$. I think the bit complexity of the output of $\cQ_i$ implies that the corners all have bit complexity at most $b$. We also need the bit complexity of $l_j(\cP)$.}}
%\argyrisnote{instead of:}there exists an algorithm with running time \mingfeinote{Add time}, that solves the optimization program $\text{max}\{\mathbf{a}\cdot \bx\mid\bx\in \cP_i\}$
%, for any $\mathbf{a}\in \mathbb{R}^d$.
%\begin{align*}
%    \text{max}\quad& \mathbf{a}\cdot \bx\\
%    \text{s.t.}\quad& \bx\in \cP_i
%\end{align*}
%Let $\widehat{\cP}^t_{\eps}$ be the mixture of $\{\cP_{i,\eps}^t\}_{i\in[L]}$ over the empirical distribution induced by \argyrisnote{$k(\delta)\geq sth$} independent samples from $\cD$,
%where $\cP_{i,\eps}^t$ is the $\eps$-truncated of the lowered-closed polytope $\cP_i$ (See Definition~\ref{def:truncated polytope}).
 %and let $b_\eps$ be an upper bound on the bit complexity of $\eps$ and 
%Let $b=\max(b_l,b_{\cP})$.
Let the parameter {$k\geq \Omega\left(d^4\left(b + \log\left( \frac{1}{\eps}\right)\right)\right)$.} %$k \geq \max\left(\log\left( \frac{1}{\eps} \right), \Omega(d^4(b + \log\left( \frac{1}{\eps}\right))\right)$. %\argyrisnote{Argyris: why not just $k \geq \Omega\left(d^4\left( b_\cP + \log\left( \frac{1}{1-\eps T}\right)\right)\right)$?}.
 We can construct a convex and down-monotone  polytope $\widehat{\cP}$ using $N = \left\lceil\frac{8kd}{\eps^2}\right\rceil$ samples from $\cD$ such that with probability at least {$1-2de^{-2dk}$}, the following guarantees hold:
%\argyrisnote{The polytope exists with probability 1, but the guarantees are satisfied with some probability}
\begin{enumerate}
%    \item For every $\bx\in \cP$, there exists an $\hat{\bx}\in \widehat{\cP}$ such that $\hat{x}_j\in [(1-\delta)x_j,(1+\delta)x_j]$, $\forall j\in [d]$.
%    \item For every $\hat{\bx}\in \widehat{\cP}$, there exists an $\bx\in \cP$ such that $x_j\in [(1-\delta)\hat{x}_j,(1+\delta)\hat{x}_j]$, $\forall j\in [d]$.
\item $\frac{c}{6}\cdot\cP\subseteq \widehat{\cP}\subseteq \cP$. 
\item There exists a separation oracle $SO$ for $\widehat{\cP}$,
whose running time on input with bit complexity $b'$, is $\poly\left(b,b',k,d,\frac{1}{\eps}\right)$ and requires $\poly\left(b,b', k,d,\frac{1}{\eps}\right)$ queries to oracles in  $\{\cQ_i\}_{i\in[\ell]}$ with inputs of bit complexity at most $\poly\left(b, b',k,d,\frac{1}{\eps}\right)$.
%\todo{define bit complexity of separation oracle}
%\argyrisnote{runs in time \mingfeinote{Add time}.}
\end{enumerate}
%For every $0 < \eps$ such that $\cP_\eps^b \subseteq \cP$ and $\delta$ with probability \argyrisnote{smt}, 
%let $\widehat{D}$ be the empirical distribution induced by $k\geq $ \mingfeinote{sth.} independent samples from $D_i$.
%Let $\widehat{\cP}^t{\eps'}$ be the mixture of $\{\cP_{i,\eps}^t\}_{t_i\in T_i}$ over the empirical distribution $\widehat{D}_i$.
%Let $\widehat{W}_i = \frac{1}{2}\widehat{\cP}_{\eps}^t + \frac{1}{2}\cP_{\eps'}^$. Then with probability  
%\begin{enumerate}
%    \item For each $\widetilde{p} \in \frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b$,
%there exists a $p \in \frac{1}{2}\cP_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b$ such that for all $j\in[d]$:
%$$\frac{p(j)}{\widetilde{p}(j)}\in \left[1-\delta,1+ \delta\right]$$
%\item For each $p \in \frac{1}{2}\cP^b_{\eps} +\frac{1}{2}\cP^t_{\eps}$,
%there exists a $\widetilde{p} \in \frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b$ such that for all $j\in[d]$:

%$$\frac{p(j)}{\widetilde{p}(j)}\in \left[1-\delta,1+\delta\right]$$
%\end{enumerate}

%Moreover consider $\widehat{\cP}= (1-\delta)\left(\frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b \right)$.
\end{theorem}



\notshow{
\begin{theorem}\label{thm:special case of multiplicative approx-main body}
Let $\ell$ be a positive integer. Let $\cP \subseteq [0,1]^d$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in [\ell]}$,
where for each $i\in[\ell]$, $\cP_i\subseteq [0,1]^d$ is a convex and down-monotone polytope. 
Assume for all $i$,
the bit complexity of each corner of $\cP_i$ is at most $b$. Suppose for every $i\in [\ell]$, there is an algorithm $\mathcal{A}$ that can maximize any linear objective over $\cP_i$, i.e. solve $\max\{\mathbf{a}\cdot \bx:\bx\in \cP_i\}$ for any $\mathbf{a}\in \mathbb{R}^d$ with bit complexity $y$, in time $RT_{\mathcal{A}}(y)$.
Suppose $c\cdot\pbox\subseteq \cP$ for some $\eps>0$ and absolute constant $c\in (0,1]$, then for any $\delta\in (0,1)$ there is an algorithm (with running time $\poly(d,\frac{1}{\eps},\log(1/\delta))$) that with probability at least $1-\delta$, constructs a convex and down-monotone polytope $\widehat{\cP}\in [0,1]^{d}$ using $\poly(d,\frac{1}{\eps},\log(1/\delta))$ samples from $\cD$, such that
\begin{enumerate}
\item $\frac{c}{6}\cdot\cP\subseteq \widehat{\cP}\subseteq \cP$. 
\item There exists a separation oracle $SO$ for $\widehat{\cP}$. The running time of $SO$ on any input with bit complexity $b'$ is $\poly(d,b,b',\frac{1}{\eps},\log(1/\delta),RT_{\mathcal{A}}(\poly(d,b,b',\frac{1}{\eps},\log(1/\delta))))$.
\end{enumerate}
\end{theorem}
}

%\yangnote{Yang: I think the statement of \Cref{thm:special case of multiplicative approx-main body} is inaccurate. Why not directly state \Cref{thm:special case of multiplicative approx}.
%}
%\mingfeinote{Mingfei: Maybe it's a good idea to first verify that $W_i$ satisfies all the constraints and apply it to solve our problem, before giving the proof.}
%\argyrisnote{Argyris: I agree, maybe we can create a subsection for the proof of the theorem and devote the rest of this section for its application to contraint additive.}


The complete proof of \Cref{thm:special case of multiplicative approx} is postponed to \Cref{subsec:proof_general_polytope}. Here we give a sketch of the proof. We first prove that if the polytope $\cP$ contains $c$ times the $\eps$-box polytope, then the convex set $\frac{c}{2}(\ptruncated + \pbox)$ is sandwiched between $\frac{c}{2}\cP$ and $\cP$ (\Cref{lem:boxable polytope contained} in \Cref{subsec:proof_general_polytope}). Next, we construct the polytope $\widehat{\cP}$ that is close to $\frac{c}{2}(\ptruncated + \pbox)$. For $\eps>0$ and every $i\in [\ell]$, let $\ptruncatedI$ be the $(\eps,\cP)$-truncated polytope of $\cP_i$. It is clear that $\ptruncated$ is a mixture of $\{\ptruncatedI\}_{i\in [\ell]}$ over distribution $\cD$. We  construct our polytope $\widehat{\cP}$ using $\ptruncatedEmp$, the mixture of $\{\ptruncatedI\}_{i\in [\ell]}$ over an empirical distribution $\widehat{\cD}$ of $\cD$. Cai et al.~\cite{CaiDW12b,CaiDW13a} proved that with polynomially many samples from $\cD$, $\ptruncatedEmp$ and $\ptruncated$ are close within an additive error $\eps$ in the $\ell_\infty$-norm (\Cref{thm:approx mixture} in \Cref{subsec:proof_general_polytope}). By choosing $\widehat{\cP}=\frac{c}{3}(\ptruncatedEmp + \pbox)$, we show that $\widehat{\cP}$ is a multiplicative approximation to $\cP$.
%$\frac{c}{2}(\ptruncated +\pbox)$. %\mingfeinote{pin down the constant here when reading the proof.}
%within a multiplicative factor, in any direction.     

To apply \Cref{thm:special case of multiplicative approx} to the single-bidder marginal reduced form polytope $W_i$, we first show that $W_i$ is a mixture of a set of polytopes $\{W_{i,t_i}\}_{t_i\in \cT_i}$ over $D_i$, where each $W_{i,t_i}$ contains {``all feasible single-bidder marginal reduced forms'' for a specific type $t_i$ (\Cref{def:W_i-t_i} in \Cref{sec:mrf for constraint additive}).}
%since the marginal reduced form $\widehat{w}_i$ is implemented by a feasible allocation $\{\sigma_S(t_i)\}_S$ where $t_i\sim D_i$.  
For every $t_i$, we can maximize any linear objective over $W_{i,t_i}$ via a query to the demand oracle. % (or a scalable demand oracle for XOS buyers).
Finally, we prove that $W_i$ contains ($c$ times) the $\eps$-box polytope of itself, for some $c\in (0,1)$ and $\eps>0$. 



\subsection{Proof of \Cref{thm:special case of multiplicative approx}}\label{subsec:proof_general_polytope}

In this section we give a proof of \Cref{thm:special case of multiplicative approx}. We first prove the following observation about the Minkowski addition of down-monotone polytopes.  

\begin{observation}
Let $\cP\subseteq [0,1]^d$ be any down-monotone polytope. Then for every $0\leq a\leq b$, $a\cdot \cP\subseteq b\cdot \cP$. Let $\cP_1,\cP_2\subseteq [0,1]^d$ both be down-monotone polytopes. Then for every $0\leq a_1'\leq a_1$ and $0\leq b_1'\leq b_1$, $a_1'\cP_1+b_1'\cP_2\subseteq a_1\cP_1+b_1\cP_2$.  
\end{observation}
\begin{proof}
For the first half of the statement, for every $\bx\in a\cdot \cP$, $\frac{\bx}{a}\in \cP$. Since $\cP$ is down-monotone, $\frac{\bx}{b}\in \cP$. Thus $\bx\in b\cdot\cP$. As $a'_1\cdot \cP\subseteq a_1\cdot \cP$ and $b'_1\cdot \cP\subseteq b_1\cdot \cP$, the second half of the statement follows from the definition of the Minkowski addition.%for every $\bx\in a_1'\cP_1+b_1'\cP_2$. Then there exist $\bx_1\in \cP_1, \bx_2\in \cP_2$ such that $\bx=a_1'\bx_1+b_1'\bx_2$. We then have $\bx=a_1'\bx_1+b_1'\bx_2\leq a_1\bx_1+b_1\bx_2\in a_1\cP_1+b_1\cP_2$. 
\end{proof}

%The following theorem is a more concrete version of \Cref{thm:special case of multiplicative approx-main body}.

\notshow{
\begin{theorem}\label{thm:special case of multiplicative approx}[(Concrete Version of \Cref{thm:special case of multiplicative approx-main body})]
Let $\ell$ be a positive integer, and $\cP \subseteq [0,1]^d$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in [\ell]}$,
where for each $i\in[\ell]$, $\cP_i\subseteq [0,1]^d$ is a convex and down-monotone polytope. 
%Let $b_l$ be an upper bound on the bit complexity of vector $\{l_j(\cP)\}_{j\in[d]}$.
%Let $b$ be an upper bound on the bit complexity of all corners in $\cP_i$ for each $i\in [\ell]$.
Suppose for every $i\in [\ell]$, %the bit complexity of every corner in $\cP_i$ is at most $b$, and 
\yangnote{there exists an oracle $\cQ_i(\cdot)$, whose output $\cQ_i(\mathbf{a})\in \argmax\{\mathbf{a}\cdot \bx:\bx\in \cP_i\}$ for any input $\mathbf{a}\in \mathbb{R}^d$. % that solves the optimization problem $\max\{\mathbf{a}\cdot \bx:\bx\in \cP_i\}$ for any $\mathbf{a}\in \mathbb{R}^d$.
Given $\{l_j(\cP)\}_{j\in[d]}$, suppose $c\cdot\pbox\subseteq \cP$ for some $\eps>0$ and $c\in (0,1]$. Let $b$ be an upper bound on the bit complexity of $\cQ_i(a)$ for all $i\in[\ell]$ and $\mathbf{a}\in \mathbb{R}^d$, as well as on the bit complexity of $l_j(\cP)$ for all $j\in [d]$.} \footnote{\yangnote{Yang: I removed the assumption that the bit complexity of a corner is at most $b$. I think the bit complexity of the output of $\cQ_i$ implies that the corners all have bit complexity at most $b$. We also need the bit complexity of $l_j(\cP)$.}}
%\argyrisnote{instead of:}there exists an algorithm with running time \mingfeinote{Add time}, that solves the optimization program $\text{max}\{\mathbf{a}\cdot \bx\mid\bx\in \cP_i\}$
%, for any $\mathbf{a}\in \mathbb{R}^d$.
%\begin{align*}
%    \text{max}\quad& \mathbf{a}\cdot \bx\\
%    \text{s.t.}\quad& \bx\in \cP_i
%\end{align*}
%Let $\widehat{\cP}^t_{\eps}$ be the mixture of $\{\cP_{i,\eps}^t\}_{i\in[L]}$ over the empirical distribution induced by \argyrisnote{$k(\delta)\geq sth$} independent samples from $\cD$,
%where $\cP_{i,\eps}^t$ is the $\eps$-truncated of the lowered-closed polytope $\cP_i$ (See Definition~\ref{def:truncated polytope}).
 %and let $b_\eps$ be an upper bound on the bit complexity of $\eps$ and 
%Let $b=\max(b_l,b_{\cP})$.
Let the parameter \yangnote{$k\geq \Omega\left(d^4\left(b + \log\left( \frac{1}{\eps}\right)\right)\right)$.} %$k \geq \max\left(\log\left( \frac{1}{\eps} \right), \Omega(d^4(b + \log\left( \frac{1}{\eps}\right))\right)$. %\argyrisnote{Argyris: why not just $k \geq \Omega\left(d^4\left( b_\cP + \log\left( \frac{1}{1-\eps T}\right)\right)\right)$?}.
 We can construct a convex and down-monotone  polytope $\widehat{\cP}$ using $N = \left\lceil\frac{8kd}{\eps^2}\right\rceil$ samples from $\cD$ such that with probability at least {$1-2de^{-2dk}$}, the following guarantees hold:
%\argyrisnote{The polytope exists with probability 1, but the guarantees are satisfied with some probability}
\begin{enumerate}
%    \item For every $\bx\in \cP$, there exists an $\hat{\bx}\in \widehat{\cP}$ such that $\hat{x}_j\in [(1-\delta)x_j,(1+\delta)x_j]$, $\forall j\in [d]$.
%    \item For every $\hat{\bx}\in \widehat{\cP}$, there exists an $\bx\in \cP$ such that $x_j\in [(1-\delta)\hat{x}_j,(1+\delta)\hat{x}_j]$, $\forall j\in [d]$.
\item $\frac{c}{6}\cdot\cP\subseteq \widehat{\cP}\subseteq \cP$. 
\item There exists a separation oracle $SO$ for $\widehat{\cP}$,
whose running time on input with bit complexity $b'$, is $\poly\left(b,b',k,d,\frac{1}{\eps}\right)$ and requires $\poly\left(b,b', k,d,\frac{1}{\eps}\right)$ queries to oracles in  $\{\cQ_i\}_{i\in[\ell]}$ with inputs of bit complexity at most $\poly\left(b, b',\yangnote{k},d,\frac{1}{\eps}\right)$.
%\todo{define bit complexity of separation oracle}
%\argyrisnote{runs in time \mingfeinote{Add time}.}
\end{enumerate}
%For every $0 < \eps$ such that $\cP_\eps^b \subseteq \cP$ and $\delta$ with probability \argyrisnote{smt}, 
%let $\widehat{D}$ be the empirical distribution induced by $k\geq $ \mingfeinote{sth.} independent samples from $D_i$.
%Let $\widehat{\cP}^t{\eps'}$ be the mixture of $\{\cP_{i,\eps}^t\}_{t_i\in T_i}$ over the empirical distribution $\widehat{D}_i$.
%Let $\widehat{W}_i = \frac{1}{2}\widehat{\cP}_{\eps}^t + \frac{1}{2}\cP_{\eps'}^$. Then with probability  
%\begin{enumerate}
%    \item For each $\widetilde{p} \in \frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b$,
%there exists a $p \in \frac{1}{2}\cP_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b$ such that for all $j\in[d]$:
%$$\frac{p(j)}{\widetilde{p}(j)}\in \left[1-\delta,1+ \delta\right]$$
%\item For each $p \in \frac{1}{2}\cP^b_{\eps} +\frac{1}{2}\cP^t_{\eps}$,
%there exists a $\widetilde{p} \in \frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b$ such that for all $j\in[d]$:

%$$\frac{p(j)}{\widetilde{p}(j)}\in \left[1-\delta,1+\delta\right]$$
%\end{enumerate}

%Moreover consider $\widehat{\cP}= (1-\delta)\left(\frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b \right)$.
\end{theorem}

}

%\argyrisnote{Maybe we should state a lemma saying that for down-monotone polytopes, minkowski sum has the property that $aP_1 + bP_2 \subseteq a' P_1 + b' P_2$ when $a'\geq a$ and $b'\geq b$?}

%\argyrisnote{I changed slightly Lemma~\ref{lem:boxable polytope contained}}

We use the following result from an unpublished manuscript by Cai et al.~\cite{CaiDW21}. A special case of the result appeared as Theorem 4 in~\cite{CaiDW12bfull} (conference version by the same authors). In particular, the result we use here is stated for a mixture of polytopes, while Theorem 4 in~\cite{CaiDW12bfull} is only for the polytope of all feasible reduced forms, but the proof is essentially the same. Interested readers are welcome to email the first author for a proof of~\Cref{thm:approx mixture}.%based on a series of works by the same authors~\cite{CaiDW12a,CaiDW12bfull,CaiDW13a,CaiDW13b}.


\begin{theorem}[\cite{CaiDW21}]\label{thm:approx mixture}
Let $\ell$ be a positive integer. Let $\cP$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in [\ell]}$,
where $\cP_i\subseteq \mathbb{R}^d$ is a convex polytope for every $i\in[\ell]$. Assume for all $i$,
the bit complexity of each corner of $\cP_i$ is at most $b$. For any $\eps > 0$ and integer %$k \geq \max\left(\log\left( \frac{1}{\eps} \right), \Omega(d^4(b + \log\left( \frac{1}{\eps}\right))\right)$
{$k \geq \ \Omega\left(d^4\left(b + \log\left( \frac{1}{\eps}\right)\right)\right)$},
let $\cD'$ be the empirical distribution induced by $\lceil\frac{8kd}{\varepsilon^2}\rceil$ samples from $\cD$.
Let $\cP$ be the mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD'$. With probability at least $1-2de^{-2dk}$ we have that
\begin{enumerate}
    \item For all $\bx\in \cP$,
    there exists an $\bx'\in \cP'$ such that $||\bx-\bx'||_\infty \leq \eps$.
    \item For all $\bx'\in \cP'$,
    there exists an $\bx\in \cP$ such that $||\bx-\bx'||_\infty \leq \eps$.
\end{enumerate}
\end{theorem}


To prove \Cref{thm:special case of multiplicative approx}, we need the following lemmas.

\begin{lemma}\label{lem:boxable polytope contained}
Let $\cP\subseteq [0,1]^d$ be a convex and down-monotone polytope. If $c\cdot \pbox\subseteq \cP$ for some $\eps>0$ and $c\in(0,1]$, 
%and $\cP$ is a lowered-closed convex set
then $\frac{c}{2}\cP \subseteq \frac{c}{2}\ptruncated + \frac{c}{2}\pbox \subseteq \cP$.
\end{lemma}

\begin{proof}
First we prove that $\frac{c}{2}\cP \subseteq \frac{c}{2}\ptruncated + \frac{c}{2}\pbox$.
Note that it is enough to prove that $\cP \subseteq \ptruncated + \pbox$.
For any $\bx\in \cP$,
we consider the vectors $\bx',\bx''\in [0,1]^d$ such that
$$\bx_j'=\bx_j\cdot \ind[l_j(\cP)\geq \eps],\forall j\in [d]$$
$$\bx_j''=\bx_j\cdot \ind[l_j(\cP)<\eps],\forall j\in [d]$$
%$$
%p^t(i) =
%\begin{cases}
%p(i) \quad &\text{if $l_i(\cP)\geq \eps$}\\
%0 & \text{o.w.}
%\end{cases} \quad \forall i \in[d]
%$$
%and
%$$
%p^b(i) =
%\begin{cases}
%p(i) \quad &\text{if $l_i(\cP) < \eps$}\\
%0 & \text{o.w.}
%\end{cases} \quad \forall i %\in[d]
%$$
Note that $\bx = \bx' + \bx''$.
By the definition of $\ptruncated$, $\bx' \in \ptruncated$. For $\bx''$, we notice that for every $j\in [d]$, $\bx_j''=\bx_j\cdot \ind[l_j(\cP)<\eps]\leq l_j(\cP)\cdot \ind[l_j(\cP)<\eps]$. By the definition of $\pbox$,
%we have that 
$\bx''\in \pbox$. Thus $\bx = \bx' + \bx''\in \ptruncated +\pbox$.
%which concludes the first part of the proof.

For the other direction, note that $\ptruncated\subseteq \cP$ by \Cref{def:truncated polytope} and $c \cdot \pbox\subseteq \cP$ by assumption, so $\frac{c}{2}\pbox + \frac{c}{2}\ptruncated \subseteq \frac{1}{2}\cP + \frac{1}{2}\cP= \cP$.
%By a well-known of Minkowski sum over convex polytopes we have that 
%The proof is done by a forklore that $\frac{1}{2}\cP + \frac{1}{2}\cP= \cP$ for convex polytope $\cP$.
%which concludes the proof.\argyrisnote{Argyris: I found it in notes online and in Wikipedia and the proof sounds easy.}
%Thus, it is enough to prove that $\frac{1}{2}\cP_\eps^b + \frac{1}{2}\cP_{\eps}^t \subseteq \frac{1}{2}\cP + \frac{1}{2}\cP \subseteq \cP$.
\end{proof}


\begin{lemma}\label{lem:mixture of truncated distribution}
Let $\ell$ be a positive integer and $\cP \subseteq [0,1]^d$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in [\ell]}$,
where for each $i\in[\ell]$, $\cP_i\subseteq [0,1]^d$ is a convex and down-monotone polytope.
%For each $i\in [\ell]$,
%define as $\ptruncatedI$ the polytope such that $\bx^{tr}\in\cP_i^{tr,\eps}$ if there exists $\bx\in \cP_i$ such that for each $j\in[d]$
%$$
%\bx^{tr}_j = \bx_j \ind[l_j(\cP)\geq \eps]
%$$
Then $\ptruncated$ is a mixture of $\{\ptruncatedI\}$ over $\cD$,
where for each $i\in [\ell]$, $\ptruncatedI\subseteq \cP_i$ is the $(\eps,\cP)$-truncated polytope of $\cP_i$ (\Cref{def:truncated polytope}).
\end{lemma}

\begin{proof}
To prove our statement, we first show that for each $\widehat{\bx}\in \ptruncated$,
there exist $\{\widehat{\bx}^{(i)}\in \ptruncatedI\}_{i\in[\ell]}$ such that $\widehat{\bx}= \sum_{i\in[\ell]}q_i \widehat{\bx}^{(i)}$.
By definition of $\ptruncated$,
%if $\bx^{(tr,\eps)}\in \ptruncated$,then 
there exists $\bx \in \cP$ such that for each $j\in[d]$, $\widehat{\bx}_j = \bx_j\cdot \ind[l_j(\cP)\geq \eps]$.


Since $\bx \in \cP$ and $\cP$ is a mixture of $\{\cP_i\}_{i\in [\ell]}$ over $\cD$, there exist $\{\bx^{(i)} \in \cP_i\}_{i\in[\ell]}$ such that $\bx = \sum_{i\in[\ell]}q_i \bx^{(i)}$.
For each $i\in [\ell]$,
consider $\widehat{\bx}^{(i)}$ be defined such that for all $j\in[d]$:
$$\widehat{\bx}_j^{(i)} = \bx_j^{(i)}\ind[l_j(\cP)\geq \eps]
$$
Clearly, $\widehat{\bx}^{(i)}\in \ptruncatedI$ and $\widehat{\bx}=\sum_{i\in[\ell]}q_i \widehat{\bx}^{(i)}$. Similarly, we can argue that  any point $\widehat{\bx}$ that lies in the mixture of $\{\ptruncatedI\}$ over $\cD$ must also lie in $\ptruncated$, which concludes the proof.
\end{proof}


\begin{lemma}\label{lem:mixture of lower-closed}
Let $\ell$ be a positive integer, and $\cP\subseteq [0,1]^d$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in[\ell]}$,
where $\cP_i$ is a convex and down-monotone polytope in $[0,1]^d$ for every $i$. Then $\cP$ is a convex and down-monotone polytope.
\end{lemma}

\begin{proof}
For every $\bx\in \cP$, there exists a set of vectors $\{\bx^{(i)}\}_{i\in [\ell]}$ such that $\bx^{(i)}\in \cP_i,\forall i$, and $\bx = \sum_{i\in[\ell]}q_i \cdot \bx^{(i)}$. Now consider any $\hat{\bx}$ such that $\mathbf{0}\leq \hat{\bx}\leq \bx$.
%Now we are going to prove that any element $p'$ such that
%$$
%p'(i) \leq p(i)
%$$
%then $p'\in \cP$.
For each $i \in [\ell]$, let $\hat{\bx}^{(i)}\in [0,1]^d$ be the vector such that $\hat{\bx}^{(i)}_j=\bx^{(i)}_j\cdot \hat{\bx}_j/\bx_j,\forall j\in [d]$.
Clearly, $0\leq \hat{x}^{(i)}_j\leq x^{(i)}_j$ for all $j\in[d]$. %$\mathbf{0}\leq \hat{\bx}^{(i)}\leq \bx^{(i)}$.
Since $\cP_i$ is down-monotone, we have $\hat{\bx}^{(i)}\in \cP_i$. Note that for every $j\in [d]$, $\sum_{i}q_i\cdot\hat{\bx}^{(i)}_j=(\sum_{i\in[\ell]} q_i\bx^{(i)}_j)\cdot \hat{\bx}_j/\bx_j=\hat{\bx}_j$. Thus $\hat{\bx}=\sum_{i\in[\ell]} q_i\cdot\hat{\bx}^{(i)}\in \cP$.
%we consider the point $p_i''$ such that:
%$$
%p_i''(j) =
%\begin{cases}
%0 \quad & \text{if $p'(j)=0$} \\
%\frac{p'(j)}{p(j)}p_i(j) \quad & %\text{o.w.}
%\end{cases}
%$$
%Note that $p'(j) \leq p(j)$,
%which implies that for any $i\in[L]$ and $j\in[d]$, $p_i''(j) \leq p_i(j)$.
%Since each $\cP_i$ is lower-closed and $p_i\in \cP_i$,
%then $p_i' \in \cP_i$.
%Consider the point $p'' = \sum_{i\in[L]}q_i p_i''$, for which $p''\in \cP$.
%Then for any $j\in[d]$:
%\begin{align*}
%p''(j) =& \sum_{i\in[L]}q_i p_i''(j) \\
%   =& \frac{p'(j)}{p(j)}\sum_{i\in [L]} q_i p_i(j) \\
%   =& p'(j)
%\end{align*}
%Where $\sum_{i\in [L]} q_i p_i(j)= p(j)$ because $\cP$ is a mixture of $\{\cP_i\}_{i\in[L]}$ over $\cD$.
%Thus $p'=p'' \in \cP$.
\end{proof}





\notshow{
\begin{prevproof}{Theorem}{thm:special case of multiplicative approx}
We condition on the probability \todo{say probability}.
We are only going to prove that for each $p\in \frac{1}{2}\cP^t_{\eps} +\frac{1}{2}\cP^b_{\eps}$,
then there exists a $\widetilde{p}\in \frac{1}{2}\widehat{\cP}^t_{\eps} +\frac{1}{2}\cP^b_{\eps}$ such that:
$$\frac{p(j)}{\widetilde{p}(j)}\in \left[1-\delta,1+\delta\right]$$
since the other case is similar.
Any $p\in \frac{1}{2}\cP^b_{\eps} +\frac{1}{2}\cP^t_{\eps}$,
can be decomposed into $p = \frac{1}{2}p^b+ \frac{1}{2}p^t$ such that $p^b \in \cP^b_{\eps}$ and $p^t \in \cP^t_{\eps}$.
By Theorem~\ref{thm:approx mixture} we know that there exists a $\widehat{p}\in \widehat{\cP}_{\eps}^t$ such that for each $j\in[d]$:
\begin{align}
|\widehat{p}^t(j) - p^t(j)| \leq \delta \eps\label{eq:additive error}
\end{align}
We partition the coordinates of $p$ into four disjoint sets.
\begin{align*}
    S^1 =& \{j\in[d]: l_j(\cP) \geq \eps \land p(j) \geq \eps\} \\
    S^2 =& \{j\in[d]:l_j(\cP) \geq \eps \land  p(j) < \eps \land p^t(j) \leq \widehat{p}^t(j)\} \\
    S^3 =& \{j\in[d]:l_j(\cP) \geq \eps \land  p(j) < \eps \land p^t(j) > \widehat{p}^t(j)\}\\
    S^4 =& \{j\in[d]:l_j(\cP) < \eps\}\\
\end{align*}
We consider the point $\widetilde{p}^t$ such that:
$$
\widetilde{p}^t(j) = 
\begin{cases}
\widehat{p}^t(j) \quad & \text{if $j\in S^1$}\\
{p}^t(j) \quad & \text{if $j\in S^2$}\\
\widehat{p}^t(j) & \text{if $j\in S^3$} \\
0 & \text{if $j\in S^4$} 
\end{cases}
$$
Since for each $i\in[L]$, $\cP_i$ is a lower closed polytpe,
then also $\cP_{\eps,i}^t$ is a lowered closed polytope.
Thus by Lemma~\ref{lem:mixture of lower-closed} 
$\widehat{\cP}_{\eps}^t$ is a lowered-closed polytope.
Notice that for each $j\in[d]$, $\widetilde{p}^t(j) \leq \widehat{p}^t(j)$,
which implies that $\widetilde{p}^t\in \widehat{\cP}_{\eps}^t$.
We also consider the point $\widetilde{p}^b\in [0,1]^d$:
$$
\widetilde{p}^b(j) = 
\begin{cases}
p^b(j) \quad & \text{if $j\in S^1$}\\
p^b(j) \quad & \text{if $j\in S^2$}\\
\min(\eps, p^b(j) + p^t(j) - \widehat{p}^t(j)) & \text{if $j\in S^3$} \\
p^b(j) & \text{if $j\in S^4$}
\end{cases}
$$
Observe that for $j\in S^1 \cup S^2 \cup S^4$,
the elements of $\widetilde{p}^b$ are the same as $p^b\in \cP_{\eps}^b$.
Notice that for $j\in S^2$,
$h_j(\cP)\geq \eps$ and $\widetilde{p}^b(j) \leq \eps$,
which implies that $\widetilde{p}^b \in \cP_{\eps}^b$.

We consider the element $\widetilde{p}=\frac{1}{2}\widetilde{p}^b + \frac{1}{2}\widetilde{p}^t $Now we are going to show that $\widetilde{p} \in \frac{1}{2}\widehat{\cP}_{\eps}^b  +\frac{1}{2}\cP_{\eps}^t$,
we have that for each $j\in [d]$:
$$\frac{p(j)}{\widetilde{p}(j)}\in \left[1-\delta,1+\delta\right]$$
For $j\in S^1$,
note that by Equation~\eqref{eq:additive error} and that for $j\in S^1$,then $p(j) \geq \eps$
\begin{align*}
&-\frac{\delta}{2}p(j)\leq -\frac{\delta \eps}{2} \leq \widetilde{p}(j) - p(j) \leq \frac{\delta \eps}{2} \leq \frac{\delta}{2}p(j) \\
\Rightarrow & \frac{p(j)}{\widetilde{p}(j)}\in \left[1-\frac{\delta}{2},1+\frac{\delta}{2} \right]
\end{align*}

For $j\in S^2$,
observe that 
$$\widetilde{p}(j) = \frac{1}{2}\widetilde{p}^t(j)+ \frac{1}{2}\widetilde{p}^b(j) =
\frac{1}{2}{p}^t(j)+ \frac{1}{2}{p}^b(j) = p(j)$$

For $j\in S^3$,
if $\eps\geq p^b(j) + p^t(j) - \widehat{p}^t(j)$,
then 
%$$\widetilde{p}(j) = \frac{1}{2}\widetilde{p}^t(j)+ \frac{1}{2}\widetilde{p}^b(j) =
%\frac{1}{2}{p}^t(j)+ \frac{1}{2}{p}^b(j) = p(j)$$
\begin{align*}
\widetilde{p}(j) = & \frac{1}{2}\widetilde{p}^t(j)+ \frac{1}{2}\widetilde{p}^b(j)  \\
=& \frac{\widehat{p}^t(j)}{2}+ \frac{p^b(j) + p^t(j) - \widehat{p}^t(j)}{2}\\
=&\frac{1}{2}{p}^t(j)+ \frac{1}{2}{p}^b(j) = p(j)
%\geq p(j) -\frac{\eps'}{2\eps}p(j)
\end{align*}

if $\eps< p^b(j) + p^t(j) - \widehat{p}^t(j)$,
then
\begin{align*}
\widetilde{p}(j) = & \frac{1}{2}\widetilde{p}^t(j)+ \frac{1}{2}\widetilde{p}^b(j)  \\
=& \frac{\widehat{p}^t(j)}{2}+ \frac{\eps}{2}\\
<& \frac{\widehat{p}^t(j)}{2}+ \frac{p^b(j) + p^t(j) - \widehat{p}^t(j)}{2}\\
=&\frac{1}{2}{p}^t(j)+ \frac{1}{2}{p}^b(j) = p(j)
\end{align*}
Observe that by combining the fact that for each $j\in [d]$ since $p^b\in \cP_{\eps}^b$ then $p^b(j)\leq \eps$ and Equation~\eqref{eq:additive error}, we get that
$$
p^b(j) + p^t(j) - \widehat{p}^t(j)\leq \eps+\delta \eps=(1+\delta)\eps
$$
thus
\begin{align*}
\widetilde{p}(j) = & \frac{1}{2}\widetilde{p}^t(j)+ \frac{1}{2}\widetilde{p}^b(j)  \\
=& \frac{\widehat{p}^t(j)}{2}+ \frac{\eps}{2}\\
\geq& \frac{\widehat{p}^t(j)}{2(1+\delta)}+ \frac{p^b(j) + p^t(j) - \widehat{p}^t(j)}{2(1+\delta)}\\
=&\frac{1}{1+\delta}\left(\frac{1}{2}{p}^t(j)+ \frac{1}{2}{p}^b(j)\right)\\
=&  \frac{1}{1+\delta}p(j)
\end{align*}
which implies that 
$$\frac{p(j)}{\widetilde{p}(j)}\in \left[1,1+\delta\right]$$
For $j\in S^4$,
since $h_j(\cP) < \eps$,
note that $p^t(j) = \widetilde{p}^t(j) = 0$,
which implies that 
$$\widetilde{p}(j) = \frac{1}{2}\widetilde{p}^b(j) = \frac{1}{2}{p}^b(j)= p(j)$$



Now we are going to prove that $\frac{(1-\delta)^2}{2}\cP \subseteq \widehat{\cP}\subseteq \cP$,
where $\widehat{\cP} = (1-\delta)\left( \frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b\right)$.
For each $\widetilde{p}\in\widehat{\cP}=(1-\delta)\left(\frac{1}{2}\widehat{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b\right)$,
we can decompose $\widetilde{p}=\frac{1-\delta}{2}\widehat{p}^t + \frac{1-\delta}{2}\widehat{p}^b$
such that $\widehat{p}^t\in \widehat{\cP}_{\eps}^t$ and $\widehat{p}^b\in \cP^b$.
By what we proved before,
we know that there exists a $p^t\in{\cP}_{\eps}^t$ such that  for each $j\in[d]$
$$
\frac{p^t(j)}{\widehat{p}^t(j)} \in \left[1-\delta,1+\delta \right]
$$
Consider the point $p = \frac{1}{2}p^t + \frac{1}{2}p^b \in \left(\frac{1}{2}{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b\right)$.
For for each $j\in[d]$
$$
\widetilde{p}(j)= \frac{1-\delta}{2}\widehat{p}^t(j) + \frac{1-\delta}{2}\widehat{p}^b(j) \leq \frac{1}{2}p(j)+ \frac{1}{2}\widehat{p}^b(j) = p(j)
$$
Since $\cP_\eps^b\subseteq \cP$ and $\cP$ is a lowered-closed polytope,
by Lemma~\ref{lem:boxable polytope contained}, we know that $p \in \frac{1}{2}{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b \subseteq \cP$
Since $\cP$ is a lowered closed polytope, $p \in \cP$ and for each $j\in[d]$ $\widetilde{p}(j) \leq p(j)$,
then $\widetilde{p}\in \cP$,which implies that $\widehat{\cP} \subseteq \cP$.


For any ${p} \in (1-\delta)^2\left( \frac{1}{2}{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b\right)$,
%there exists a point $p \in \left( \frac{1}{2}{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b\right)$.
we can decompose ${p}=\frac{(1-\delta)^2}{2}{p}^t + \frac{(1-\delta)^2}{2}{p}^b$
such that ${p}^t\in {\cP}_{\eps}^t$ and ${p}^b\in \cP^b$.
By what we have proved before,
we know that there exists a $\widehat{p}^t$ such that for each $j\in[d]$:
$$
\frac{p^t(j)}{\widehat{p}^t(j)} \in \left[1-\delta,1+\delta \right]
$$
Consider the point $\widehat{p} = \frac{1-\delta}{2}\widehat{p}^t + \frac{1-\delta}{2}p^b \in \left(\frac{1-\delta}{2}{\cP}_{\eps}^t  +\frac{1-\delta}{2}\cP_{\eps}^b\right)$.
For each $j\in[d]$ note that
$$p(j) = \frac{(1-\delta)^2}{2}{p}^t(j) + \frac{(1-\delta)^2}{2}{p}^b(j) \leq \frac{1-\delta}{2}\widehat{p}^t(j) + \frac{1-\delta}{2}{p}^b(j)=\widehat{p}(j)$$

We know that $\cP_\eps^b$ is lowered-closed and by Lemma~\ref{lem:mixture of lower-closed} we know that $\widehat{\cP}_\eps^t$ is lowered-closed.
Thus $\widehat{\cP}$ is a lowered-closed polytope,
as the Minkowski sum of lowered-closed polytopes $\frac{(1-\delta)^2}{2}\widehat{\cP}_\eps^t$ and $\frac{(1-\delta)^2}{2}\cP_\eps^b$.
Since for each $p \in (1-\delta)^2\left(\frac{1}{2}\cP_\eps^t +\frac{1}{2}\cP_\eps^b\right)$ and for each $j\in[d]$,
there exists a $\widehat{p}\in \widehat{\cP}$ such that for each $j\in[d]$,
it holds that $p(j) \leq \widehat{p}(j)$, implies that since $\cP$ is lowered-closed  $p \in \widehat{\cP}$.
Thus $(1-\delta)^2\left(\frac{1}{2}\cP_\eps^t +\frac{1}{2}\cP_\eps^b\right)\subseteq \widehat{\cP}$.



By Lemma~\ref{lem:boxable polytope contained},
we know that $\frac{(1-\delta)^2}{2}\cP\subseteq (1-\delta)^2\left( \frac{1}{2}{\cP}_{\eps}^t  +\frac{1}{2}\cP_{\eps}^b\right) \subseteq \widehat{\cP}$.

\end{prevproof}


}



%\begin{theorem}\label{thm:special case of multiplicative approx}
%Let $\ell$ be a positive integer.
%Let $\cP \subseteq [0,1]^d$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in [\ell]}$,
%where for each $i\in[\ell]$, $\cP_i\subseteq [0,1]^d$ is a down-monotone convex polytope. 
%Suppose $c\cdot \pbox\subseteq \cP$ for some $1\leq c,\eps>0$. And suppose for every $i\in [\ell]$,
%there exists an algorithm with running time \mingfeinote{Add time}, that solves the optimization program $\text{max}\{\mathbf{a}\cdot \bx\mid\bx\in \cP_i\}$
%, for any $\mathbf{a}\in \mathbb{R}^d$.
%Then there exists a convex polytope $\widehat{\cP}$ such that with probability at least \mingfeinote{$1-o(1)$}, both of the following guarantees hold:
%\todo{fix constant}
%\begin{enumerate}
%\item $\frac{c}{6}\cP\subseteq \widehat{\cP}\subseteq \cP$. \mingfeinote{What is $\delta$.}
%\item There exists a separation oracle for $\widehat{\cP}$ that runs in time \mingfeinote{Add time}.
%\end{enumerate}
%\end{theorem}


To prove \Cref{thm:special case of multiplicative approx},
we will also need the celebrated result of the equivalence between optimization and separation.

\begin{theorem}[\cite{KarpP80,GrotschelLS81}]\label{thm:equivalence of opt and sep}
Let $\cP\subseteq \mathbb{R}^d$ be a convex polytope and suppose we have access to an algorithm $\mathcal{A}(\bm{a}):\mathbb{R}^d\rightarrow\cP$, that takes input vector $\bm{a}\in \mathbb{R}^d$,
outputs a vector $\bx^* \in \cP$ with bit complexity at most $b$,
such that $\bx^* \in \text{argmax}\{\bm{a}\cdot \bx:\bx\in \cP\}$.
Then we can construct a separation oracle $SO$ for $\cP$, where on {any input $\bm{a}\in \mathbb{R}^d$ with bit complexity at most $b'$, $SO$ makes at most $\poly(d,b,b')$ queries to $\mathcal{A}$, and the input of each query has bit complexity no more than $\poly(d,b,b')$.} Moreover, the running time of $SO$ on $\bm{a}$ is at most  $\poly(d,b,b',RT_{\mathcal{A}}(\poly(d,b,b')))$. Here $RT_{\mathcal{A}}(c)$ is the running time of $\mathcal{A}$ with input whose bit complexity is at most $c$. 
%where the running time of $SO$ for a vector $\mathbf{a}\in \mathbb{R}^d$ with bit complexity at most $b'$ is $\poly(d,b,b',RT_{\mathcal{A}}(\poly(d,b,b')))$. Here $RT_{\mathcal{A}}(c)$ is the running time of $\mathcal{A}$ with input whose bit complexity is at most $c$. 
\end{theorem}



\begin{prevproof}{Theorem}{thm:special case of multiplicative approx}

Consider the polytopes $\ptruncated$ and $\pbox$.
By Lemma~\ref{lem:mixture of truncated distribution}, $\ptruncated$ is a mixture of $\{\ptruncatedI\}_{i\in[\ell]}$ over distribution $\cD$. %(where $\cP_i^{tr,\eps}$ is defined in Lemma~\ref{lem:mixture of truncated distribution}) over $\cD$. 
Let $\widehat{\cD}$ be the empirical distribution induced by $N=\lceil\frac{8kd}{\eps^2}\rceil$ samples from $\cD$.  
Let $\ptruncatedEmp$ be the mixture of 
$\{\ptruncatedI\}_{i\in[\ell]}$ over $\widehat{\cD}$.
%the empirical distribution induced by $N=\lceil\frac{8kd}{\eps^2}\rceil$ samples from $\cD$. 
By Theorem~\ref{thm:approx mixture},
we have that with probability at least {$1-2de^{-2dk}$}, both of the two following conditions hold:
\begin{enumerate}
    \item For each $\widehat{p}\in \ptruncatedEmp$,
    there exists a $p\in \ptruncated$ such that $||p-\widehat{p}||_\infty \leq \eps$.
    \item For each ${p}\in {\ptruncated}$,
    there exists a $\widehat{p}\in \ptruncatedEmp$ such that $||p-\widehat{p}||_\infty \leq \eps$.
\end{enumerate}
For the rest of the proof, we condition on the event that both conditions hold.
We consider the polytope $\widehat{\cP}=\frac{c}{3}\left(\ptruncatedEmp+\pbox\right)$.
First we are going to prove that $\widehat{\cP}\subseteq \cP$.
%Any $\widehat{p}\in\widehat{\cP}$,
%can be decomposed as $\widehat{p}=\frac{c}{2}\widehat{p}^{tr}+\frac{c}{2}\widehat{p}^{box}$,
%such that $\widehat{p}^{tr}\in \widehat{\ptruncated}$ and ${p}^{box}\in {\pbox}$.
By condition 1, we have that for any $\widehat{p}^{tr}\in \ptruncatedEmp$,
there exists a ${p}^{tr}\in {\ptruncated}$ such that $||p^{tr}-\widehat{p}^{tr}||_{\infty}\leq \eps$.
Consider the vector $\tilde{p}^{tr}$ defined such that for each $j\in[d]$,
$$
\tilde{p}^{tr}_j = \min\left( \widehat{p}^{tr}_j, p^{tr}_j\right).
$$
Since for each $j\in[d]$, $\tilde{p}^{tr}_j \leq {p}^{tr}_j$ and $\ptruncated$ is down-monotone (\Cref{lem:mixture of lower-closed}),
we have $\tilde{p}^{tr}\in \ptruncated$.
Let vector $\tilde{p}^{box}$ be such that for every $j\in[d]$,
$$
\tilde{p}^{box}_j = \widehat{p}^{tr}_j - \tilde{p}^{tr}_j=\widehat{p}^{tr}_j -\min(\widehat{p}^{tr}_j, {p}^{tr}_j).
%\leq
%\begin{cases}
%\eps \quad &\text{if $l_j(\cP)\geq \eps$} \\
%0 & \text{o.w}
%\end{cases} 
$$
Notice that for every $\bx\in \ptruncatedI$, $x_j=0$ for all $j$ such that $l_j(\cP)<\eps$. Since $\ptruncated$ and $\ptruncatedEmp$ are both mixtures of $\{\ptruncatedI\}_{i\in[\ell]}$, we have for every $\bx\in \ptruncated$ and $\widehat{\bx}\in \ptruncatedEmp$, $x_j=\widehat{x}_j=0$ for all $j$ such that $l_j(\cP)<\eps$. Therefore, we have $\tilde{p}^{box}_j\leq \eps\cdot \ind[l_j(\cP)\geq \eps]\leq \min(\eps,l_j(\cP))$, for every $j\in [d]$. The first inequality follows from the fact that $||p^{tr}-\widehat{p}^{tr}||_{\infty}\leq \eps$, 
%by the choice of $p^{tr}_j$ for which Property (1) holds and from the fact 
and that if $l_j(\cP) < \eps$,
then $\widehat{p}^{tr}_j=p^{tr}_j=0$.
Thus $\tilde{p}^{box}\in \pbox$.

%Thus for each $\widehat{p}^{tr} \in \widehat{\ptruncated}$,
%there exists a ${p}^{tr}\in \ptruncated$ and $p^{box}\in \pbox$ such that for each $j\in[d]$:
%$$
%\widehat{p}^{tr}_j \leq p^{tr}_j + p^{box}_j
%$$
%which implies that

For every $\widehat{p}^{tr}\in \ptruncatedEmp$, we have found $\tilde{p}^{tr}\in \ptruncated$ and $\tilde{p}^{box}\in \pbox$ such that $\widehat{p}^{tr}=\tilde{p}^{tr}+\tilde{p}^{box}$. Thus

\begin{equation}\label{equ:proof-hatp}
\begin{aligned}
&\ptruncatedEmp\subseteq \ptruncated + \pbox \\
\Rightarrow & \ptruncatedEmp+\pbox \subseteq \ptruncated + 2\pbox\subseteq \frac{3}{c}\cdot\cP \\
\Rightarrow & \widehat{\cP}=\frac{c}{3}\left(\ptruncatedEmp+\pbox\right)\subseteq \cP
\end{aligned}
\end{equation}

The second line follows from the assumption that $c\pbox \subseteq \cP$ and $\ptruncated\subseteq \cP$ (by \Cref{def:truncated polytope} and the fact that $\cP$ is down-monotone), and $c\leq 1$. 
%and since for each $i\in [L]$, $\cP_i$ is down-monotone, then by Lemma~\ref{lem:mixture of lower-closed} $\ptruncated$ is also down-monotone and by Definition~\ref{def:truncated polytope} we know that $\ptruncated\subseteq \cP$.
Similarly, by switching the role of $\ptruncated$ and $\ptruncatedEmp$, with condition 2, we also have ${\ptruncated}\subseteq \ptruncatedEmp + \pbox$. Thus
\begin{align*}
&{\ptruncated} + \pbox \subseteq \ptruncatedEmp + 2\pbox \\ %2\left(\ptruncatedEmp + \pbox \right)\\
\Rightarrow& \cP \subseteq {\ptruncated} + \pbox \subseteq 2\left(\ptruncatedEmp + \pbox \right)=\frac{6}{c}\widehat{\cP}\\
\Rightarrow & \frac{c}{6}\cP \subseteq \widehat{\cP}
\end{align*}
The second line follows from $\cP \subseteq {\ptruncated} + \pbox$ (Lemma~\ref{lem:boxable polytope contained}), {the origin $\mathbf{0}\in \ptruncatedEmp$}, and the definition of $\widehat{\cP}$. Thus $\frac{c}{6}\cP \subseteq \widehat{\cP}\subseteq \cP$.

%\argyrisnote{We need to assume }
To construct a separation oracle for $\widehat{\cP}$, it is sufficient to optimize any linear objective over $\widehat{\cP}$. For every $\bm{a}\in \mathbb{R}^d$, we are going to solve the maximization problem $\max\{\bm{a}\cdot \bx:~\bx\in \widehat{\cP}\}$.

Let $\{i_1,...,i_N\}$
be the $N$ samples from $\cD$, where $i_k\in [\ell]$ for $k\in [N]$.
We notice that
$$
\widehat{\cP} = \sum_{k\in[N]}\frac{c}{3N}\cdot\cP^{tr(\eps,\cP)}_{i_k} + \frac{c}{3}\pbox 
$$
%Since $\widehat{P}$ is the Minkowski sum of polytope $\widehat{\ptruncated}$ and $\pbox$,
%where polytope $\widehat{\ptruncated}$ is the Minkowski sum of $\frac{8kd}{\eps^2}$ polytopes in $\{\ptruncatedI\}_{i\in[L]}$,
is the Minkowski addition of a set of polytopes. Thus in order to maximize over $\widehat{\cP}$, it's sufficient to maximize over each polytope. In other words, it is sufficient to solve
%find an element in 
$\max\{\bm{a}\cdot \bx:\bx\in \pbox\}$ and 
%to be able to find an element in
$\max\{\bm{a}\cdot \bx:\bx\in \cP^{tr(\eps,\cP)}_{i_k}\}$ for each $k\in [N]$.
First consider $\pbox$. Since the polytope is a ``box'' where the constraint for each coordinate $j$ is separate: $x_j\leq \min(\eps,l_j(\cP))$.  Thus the optimum $\bx^{box}\in \pbox$ satisfies that $x^{box}_j =\min(l_j(\cP),\eps)\cdot \ind[a_j>0]$. 
%the element $\bx^{box}\in [0,\eps]^d$ such that for each $j\in[d]$, $x^{box}_j = a_j^+\cdot\min(l_j(\cP),\eps)$.
%Then $\bx^{box}\in \text{argmax}\{\mathbf{a}\cdot \bx\mid\bx\in \pbox\}$.
%\yangnote{Since $l_j(\cP)=\max_{\bx\in\cP}x_j$, the bit complexity of $l_j(\cP)$ must be at most $b$.}
Thus the optimum $\bx^{box}$ can be computed in time {$O(d\cdot(b+\log 1/\eps+b'))$} %$O(d\cdot b)$
and its bit complexity is at most {$O(d\cdot(b+\log 1/\eps))$, where $b'$ is the bit complexity of $\bm{a}$.} %$O(d \cdot b)$.


Now we show how to %use $\text{max}\{\mathbf{a}\cdot \bx\mid\bx\in \cP_i\}$ in order to 
solve $\max\{\bm{a}\cdot \bx:\bx\in \cP_{i_k}^{tr(\eps,\cP)}\}$
using a single query to $\cQ_{i_k}(\cdot)$, for every $k\in [N]$.
Consider the vector $\bm{a}'\in \mathbb{R}^d$ such that $a_j'=a_j\cdot \ind[l_j(\cP)\geq \eps], \forall j\in [d]$.
%$$
%\mathbf{a}'_j=
%\begin{cases}
%\mathbf{a}_j \quad & \text{if $l_j(\cP)\geq %\eps$} \\
%0 & \text{o.w.}
%\end{cases}
%$$
%We remind that $\bx' \in \ptruncatedI$ if there exists a $\bx \in \cP_i$ such that for each $j\in[d]$
%$$
%\bx_j' =
%\begin{cases}
%\bx_j \quad & \text{if $l_j(\cP)\geq \eps$} \\
%0 & \text{o.w.}
%\end{cases}
%$$
%Observe that:
Then clearly
$$\max\{\bm{a}\cdot \bx:\bx\in \cP_{i_k}^{tr(\eps,\cP)}\} = \max\{\bm{a}'\cdot \bx:\bx\in \cP_{i_k}\}$$
Let $\widehat{\bx}^{(i_k)}$ be the output from oracle $\cQ_{i_k}(\bm{a}')$,
then $\widehat{\bx}^{(i_k)}\in \text{argmax}\{\bm{a}'\cdot \bx:\bx\in \cP_{i_k}\}$.
Consider the element $\bx^{(i_k)}\in [0,1]^d$ such that for each $j\in [d]$, $x^{(i_k)}_j=\widehat{x}^{(i_k)}_j\cdot\ind[l_j(\cP)\geq \eps]$.
%$$
%\bx^{(i)}=
%\begin{cases}
%\widehat{\bx}^{(i)} \quad & \text{if $l_j(\cP)\geq \eps$} \\
%0 & \text{o.w.}
%\end{cases}
%$$
Then $\bx^{(i_k)}\in \text{argmax}\{\bm{a}'\cdot \bx:\bx\in \cP^{tr(\eps,\cP)}_{i_k}\}$ and its bit complexity is at most the bit complexity of $\widehat{\bx}^{(i_k)}$, which is at most $b$, {by our assumption on $\cQ_i(\cdot)$}.
%\argyrisnote{Not sure if needed: Since by assumption the bit complexity of vertices in $P_i$ is at most $b$,
%then the bit complexity of $\cQ_i(\mathbf{a}')$ is at most $b$.}

%Observe the following:

%$$
%\sum_{j\in[n]}\frac{c}{6n}\bx^{(i)} + \frac{c}{6}\bx^{box} \in  \text{argmax}\{\mathbf{a}\cdot \bx\mid\bx\in \widehat{\cP}\}
%$$
%Notice that in order to calculate an element in $\text{argmax}\{\mathbf{a}\cdot \bx\mid\bx\in \widehat{\cP}\}$,
%it is enough to take the Minkowski sum of the elements we described above.

Thus we have
$$\sum_{k\in[N]}\frac{c}{3N}\cdot \bx^{(i_k)} + \frac{c}{3}\cdot \bx^{box}\in\text{argmax}\{\bm{a}\cdot \bx:\bx\in \widehat{\cP}\}$$

{To sum up, we provide an algorithm to optimize any linear objective over $\widehat{\cP}$. Moreover, the output of our optimization algorithm always has bit complexity $\poly(b, k,d, 1/\eps)$. For any $\bm{a}\in \mathbb{R}^d$ with bit complexity $b'$, our optimization algorithm runs in time $\poly(b, b', k,d, 1/\eps)$ and make $N=\left\lceil \frac{8kd}{\eps^2}\right\rceil$ queries to the oracles in $\{\cQ_i\}_{i\in[\ell]}$. Using Theorem~\ref{thm:equivalence of opt and sep}, we can construct a separation oracle for $\widehat{\cP}$ that satisfies the properties in the statement of \Cref{thm:special case of multiplicative approx}.}


%The total running time is $\poly\left(b,k,d,\frac{1}{\eps}\right)$ and we require $N=\left\lceil \frac{8kd}{\eps^2}\right\rceil$ queries to oracles in $\{\cQ_i\}_{i\in[\ell]}$ with bit complexity at most the bit complexity of $\bx$ and the bit complexity of the final answer, which is $\poly\left(b,k,d,\frac{1}{\eps}\right)$. Thus by Theorem~\ref{thm:equivalence of opt and sep},
%Thus by the equivalence between optimization and separation~\cite{KarpP80,GrotschelLS81}, 
%we can construct the separation oracle mentioned in the statement.
\end{prevproof}

%\yangnote{Yang: Do we want to keep \Cref{thm:special case of multiplicative approx-main body}? It seems that we do not use it anywhere.}

%\begin{prevproof}{Theorem}{thm:special case of multiplicative approx-main body}
%For any $\delta\in (0,1)$, by applying \Cref{thm:special case of multiplicative approx} with parameter\\ $k\geq \max\left(\log\left( \frac{1}{\eps} \right), \Omega(d^4(b + \log\left( \frac{1}{\eps}\right)),\log(\frac{1}{\delta})\right)$, the probability that the algorithm successfully constructs a polytope is at least $1-\delta$. The running time of the algorithm and SO directly follows from the statement of \Cref{thm:special case of multiplicative approx}. 
%\end{prevproof}


\subsection{Approximating Single-Bidder Marginal Reduced Form Polytope for Constrained-Additive Buyers}\label{sec:mrf for constraint additive}

In this section,
we prove \Cref{thm:multiplicative approx for constraint additive-main body} using \Cref{thm:special case of multiplicative approx}.
%apply Theorem~\ref{thm:special case of multiplicative approx} in order to construct a polytope that contains a constant fraction of the marginal reduced form polytope for a bidder with constraint additive valuation. 
The goal is to show that the single-bidder marginal reduced form polytope $W_i$ satisfies the requirements of Theorem~\ref{thm:special case of multiplicative approx}.
%Throughout this section,
%our goal is to estimate the marginal reduced form polytope of an agent $W_i$, with a constrained additive valuation,
Recall that for every buyer $i$, the support of her type is $\cT_i$ and the support of her value for each item $j$ is $\cT_{ij}$. Additionally, $W_i$ is a subset of $[0,1]^{\sum_{j\in[m]}|\cT_{ij}|}$, and there is a coordinate for every $j\in [m]$ and every $t_{ij}\in \cT_{ij}$. To ease the notation, we will use $t_{ij}$'s to index the coordinates throughout this section. Since each buyer is constrained-additive, we denote $\cF_i$ the feasibility constraint of buyer $i$, and drop the subscript if the buyer is fixed or clear from context.

\begin{lemma}\label{obs:constraint additive length}
%Let $W_i$ be the marginal reduced form polytope when the buyer's valuation is constraint additive.
For each $i\in[n],j\in[m]$ and $t_{ij}\in\cT_{ij}$, $l_{t_{ij}}(W_i)=f_{ij}(t_{ij})$. Recall that $l_{t_{ij}}(W_i)$ is the width of $W_i$ at coordinate $t_{ij}$ (\Cref{def:truncated polytope}).
\end{lemma}

\begin{proof}
For every $i\in [n]$ and every $\widehat{w}_i\in W_i$, by \Cref{def:W_i-constrained-add}, there exists a number $\sigma_S(t_i)\in [0,1]$ for every $t_i\in \cT_i, S\in \cF_i$ such that
\begin{enumerate}
    \item $\sum_{S\in \cF_i}\sigma_S(t_i)\leq 1$, $\forall t_i\in \cT_i$.
    \item $\widehat{w}_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S\in \cF_i:j\in S}\sigma_S(t_i)$, for all $j\in[m]$ and $t_{ij}\in \cT_{ij}$.
\end{enumerate}

Thus for every $j,t_{ij}$, by combining both properties above, we have $$\widehat{w}_{ij}(t_{ij})\leq f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot 1=f_{ij}(t_{ij}).$$

Moreover, for every $j,t_{ij}$, choosing $\widehat{\sigma}$ such that:~\footnote{$\widehat{\sigma}$ is simply the allocation that gives buyer $i$ item $j$ when her value for item $j$ is $t_{ij}$ and does not give her anything otherwise.}
$$
\widehat{\sigma}_S(t_i') =
\begin{cases}
1 \quad & \text{if $t_{ij}'=t_{ij} \land S=\{j\}$} \\
0 & \text{o.w.}
\end{cases}
$$
induces an element $\widetilde{w}_i\in W_i$ such that 
%that corresponds to this allocation has 
$\widetilde{w}_{ij}(t_{ij})=f_{ij}(t_{ij})$.
Thus $l_{t_{ij}}(W_i)=f_{ij}(t_{ij})$.


%For each $i\in[n],j\in[m],t_{ij}\in\cT_{ij}$

\notshow{
$$l_{t_{ij}}(W_i) \leq \max_{\widehat{\sigma}_i\in \widehat{\Sigma}_i} f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{i}((t_{ij},t_{i,-j}),S)\leq f_{ij}(t_{ij})$$
where $\Sigma_i$ is the set such that $\sigma \in \Sigma_i$ if
\begin{align*}
    \sum_{S\subseteq 2^{[m]}} \sigma_i(t_i,S) \leq 1 \quad \forall t_i \in \cT_i \\
    \sigma_i(t_i,S) \geq 0 \quad \forall t_i\in \cT_i, S \subseteq 2^{[m]}
\end{align*}

Moreover observe that when we use the allocations $\widehat{\sigma}_{i}$ such that:
$$
\widehat{\sigma}_{i}(t_i',S) =
\begin{cases}
1 \quad & \text{if $t_{ij}'=t_{ij} \land S=\{j\}$} \\
0 & \text{o.w.}
\end{cases}
$$
the element $\widetilde{w}\in W_i$ that corresponds to this allocation has $\widetilde{w}_{ij}(t_{ij})=f_{ij}(t_{ij})$.
Thus $l_{t_{ij}}(W_i)=f_{ij}(t_{ij})$.
}


\end{proof}

\begin{definition}\label{def:W_i-t_i}
For any buyer $i$ and type $t_i\in \cT_i$, consider $W_{t_i}\subseteq [0,1]^{\sum_{j\in[m]}|\cT_{ij}|}$ defined as follows: $w_i \in W_{t_i}$ if and only if there exists a collection of non-negative numbers $\{\sigma_{S}\}_{S\in \cF_i}$ such that
%there exists a distribution over feasible allocation $\sigma_i \in \Delta^{|\cF|}$,
%where for each $S \in \cF$ we index an element of $\sigma_i$ by $\sigma_i(S)$, such that:
\begin{enumerate}
    \item $\sum_{S\in \cF_i}\sigma_S\leq 1$.
    \item $w_{ij}(t_{ij}')=\sum_{S\in \cF_i, j\in S}\sigma_S\cdot \ind[t_{ij}'=t_{ij}],\forall j\in [m],t_{ij}'\in \cT_{ij}$.
\end{enumerate}
%$$
%w_{ij}(t_{ij}')=
%\begin{cases}
%\sum_{\substack{S\subseteq \cF\\j \in S}}\sigma_i(S) \quad &\text{if $t_{ij}'=t_{ij}$} \\
%0 & \text{o.w.}
%\end{cases}
%$$
\end{definition}

The following observation directly follows from \Cref{def:W_i-constrained-add} and \Cref{def:W_i-t_i}. 

\begin{observation}\label{obs:mix constraint additive}
$W_{i}$ is mixture of $\{W_{t_i}\}_{t_i\in \cT_i}$ over distribution $D_i$. Recall that $D_i$ is the distribution for buyer $i$'s type $t_i$.
%$\{f_i(t_i)\}_{t_i \in T_i}$.
\end{observation}

\begin{lemma} \label{lem:monotone-closed polytope W}
For every $i$ and $t_i \in \cT_i$, $W_{t_i}$ is %closed, 
a convex and down-monotone polytope. Moreover, given access to a demand oracle $\dem_i(t_i,\cdot)$ for buyer $i$, we can calculate an element $$w_i^*\in \text{argmax}_{w_i\in W_{t_i}} \bm{a}\cdot w_i,$$
for any $\bm{a}\in \mathbb{R}^{\sum_{j\in[m]}|\cT_{ij}|}$ with a single query to the demand oracle. Moreover, the bit complexity of $w_i^*$ is at most $\sum_{j\in[m]}|\cT_{ij}|$.
%we can optimize over any $\eps$-boxed polytope $W_{t_i,\eps}^t$ of $W_{t_i}$ for any $\eps>0$.
\end{lemma}
\begin{proof}
{For every feasible set $S\in \cF_i$, consider allocation $\lambda^{(S)}=\{\ind[S'=S]\}_{S'\in\cF_i}$. The set of $\sigma=\{\sigma_S\}_{S\in\cF_i}$ that satisfy property 1 of \Cref{def:W_i-t_i} is equivalent to the set of all convex combinations of the $\lambda^{(S)}$'s and the origin $\mathbf{0}$.
%\footnote{\yangnote{Yang: Is there any specific reason for us to allow the sum of $\sigma_S$ to be $<1$? Note that $\emptyset$ is in $\cF_i$.}} 
More specifically, $\sigma = \sum_{S\in \cF_i} \sigma_S\cdot \lambda^{(S)}+(1-\sum_{S\in\cF_i}\sigma_S)\cdot \mathbf{0}$. Hence, the set of $\sigma$'s is a convex polytope $P$ in $[0,1]^{|\cF_i|}$. Since $W_{t_i}$ is a projection of $P$ to $[0,1]^{\sum_{j\in[m]}|\cT_{ij}|}$, $W_{t_i}$ is also a convex polytope.}

%$W_{t_i}$ is closed because of its definition. For every $w_1,w_2\in W_{t_i}$ and $x\in (0,1)$, let $\{\sigma_S\}_{S\in \cF_i}$, $\{\sigma_S'\}_{S\in \cF_i}$ be the two vectors associated with $w_1$ and $w_2$ accordingly. Then consider $\{x\sigma_S+(1-x)\sigma_S'\}_{S\in \cF_i}$ and we have $xw_1+(1-x)w_2\in W_{t_i}$. Thus $W_{t_i}$ is convex.

Next, we prove $W_{t_i}$ is down-monotone. Consider any $w_i\in W_{t_i}$. By \Cref{def:W_i-t_i}, $w_{ij}(t_{ij}')=0$ for all $j,t_{ij}'$ such that $t_{ij}'\not=t_{ij}$. To prove that $W_{t_i}$ is down-monotone, it suffices to prove that for every $j_0\in [m]$, any vector $\widetilde{w}_i$, achieved by only decreasing the coordinate $t_{ij_0}$ from $w_i$, is still in $W_{t_i}$. Formally, $\widetilde{w}_i$ satisfies
\begin{itemize}
    \item $\widetilde{w}_{ij_0}(t_{ij_0})<w_{ij_0}(t_{ij_0})$.
    \item $\widetilde{w}_{ij}(t_{ij})=w_{ij}(t_{ij})$, if $j\not=j_0$.
    \item 
    $\widetilde{w}_{ij}(t_{ij}')=0$, for any $j\in[m]$, if $t_{ij}'\not=t_{ij}$.
\end{itemize}

Let $\{\sigma_S\}_{S\in \cF_i}$ be the vector of numbers associated with $w_i$ in \Cref{def:W_i-t_i}. Let $\alpha=\frac{\widetilde{w}_{ij_0}(t_{ij_0})}{w_{ij_0}(t_{ij_0})}<1$. Consider another vector $\{\widetilde{\sigma}_S\}_{S\in \cF_i}$ where for every $S\in \cF_i$, $$\widetilde{\sigma}_S=
\begin{cases}
\alpha\cdot\sigma_S+(1-\alpha)\cdot (\sigma_{S\cup\{j_0\}}+\sigma_S), & j_0\not\in S\wedge S\cup\{j_0\}\in \cF_i\\
\alpha\cdot \sigma_S, & j_0\in S\\
\sigma_S, & \text{o.w.}
\end{cases}$$

We notice that the above definition is well-defined because $S\in \cF_i$ as long as $S\cup\{j_0\}\in \cF_i$. {Also $\sum_{S\in \cF_i}\widetilde{\sigma}_S\leq 1$. Intuitively, $\sigma=\{\sigma_S\}_{S\in \cF_i}$ represents a randomized allocation of sets $S\in \cF_i$ to the bidder. Then $\{\widetilde{\sigma}_S\}_{S\in \cF_i}$ represents another randomized allocation: choose a set $S$ according to the the randomized allocation  $\sigma$, if $S$ contains $j_0$, then throw away $j_0$ with probability $1-\alpha$.} 

Now we have $\sum_{S\in \cF_i, j_0\in S}\widetilde{\sigma}_S=\alpha\sum_{S\in \cF_i, j_0\in S}\sigma_S=\widetilde{w}_{ij_0}(t_{ij_0})$ and $\sum_{S\in \cF_i, j\in S}\widetilde{\sigma}_S=w_{ij}(t_{ij})$, for all $j\not=j_0$. Thus $\widetilde{w}_i\in W_{t_i}$, and $W_{t_i}$ is down-monotone.

\begin{comment}
First we are going to prove that $W_{t_i}$ is down-monotone.
Consider a point $w_i\in W_{t_i}$ and a point $w_i'$ such that for each $t_{ij}\in \cT_{ij}$:
$$
0\leq w_{ij}'(t_{ij}) \leq w_{ij}(t_{ij})
$$
Because $w_i\in W_{t_i}$,
there exists a $\sigma_i\in \Delta^{|\cF|}$ such that
$$
w_{ij}(t_{ij}')=
\begin{cases}
\sum_{\substack{S\subseteq \cF\\j \in S}}\sigma_i(S) \quad &\text{if $t_{ij}'=t_{ij}$} \\
0 & \text{o.w.}
\end{cases}
$$

We consider the following $\widehat{\sigma}_i \in \Delta^{|\cF|}$:
$$
\widehat{\sigma}_{i}(S)=
\begin{cases}
\prod_{k\in S}\left(\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})} \right)\sum_{S \subseteq T\subseteq \cF}\sigma_i(T) \prod_{k\in T\backslash S}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right) \quad &\text{if $t_{ij}'=t_{ij}$} \\
0 & \text{o.w.}
\end{cases}
$$



First we are going to prove that $\widehat{\sigma}_i \in \Delta^{|\cF|}$.
\begin{align*}
    \sum_{S\subseteq \cF} \widehat{\sigma}_i(S)
    = &\sum_{S\subseteq \cF} \sum_{S \subseteq T \subseteq \cF} \sigma_i(T) \prod_{k\in S}\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\prod_{k\in T\backslash S}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right) \\
    = &  \sum_{T \subseteq \cF} \sigma_i(T) \sum_{S\subseteq T} \prod_{k\in S}\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\prod_{k\in T\backslash S}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right)
\end{align*}

For any set $T\subseteq \cF$,
consider that we choose each a subset of $T$ independently at random and we choose item $k\in T$ with probability $\frac{w'_{ik}}{w_{ik}}\leq 1$.
Note that the probability of choosing exactly subset $S \subseteq T$ is $\prod_{k\in S}\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\prod_{k\in T\backslash S}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right)$.
Thus:
$$\sum_{S\subseteq T} \prod_{k\in S}\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\prod_{k\in T\backslash S}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right)=1$$
which implies that
\begin{align*}
    \sum_{S\subseteq \cF} \widehat{\sigma}_i(S)
    = &  \sum_{T \subseteq \cF} \sigma_i(T) \sum_{S\subseteq T} \prod_{k\in S}\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\prod_{k\in T\backslash S}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right) \\
    = & \sum_{T \subseteq \cF} \sigma_i(T) \leq 1
\end{align*}
which proves that $\widehat{\sigma}_i \in \Delta^{|\cF|}$.
Now we are going to show that when we use allocation $\widehat{\sigma}_i$,
then 
$$
w_{ij}'(t_{ij}')=
\begin{cases}
\sum_{\substack{S\subseteq \cF\\j \in S}}\widehat{\sigma}_i(S) \quad &\text{if $t_{ij}'=t_{ij}$} \\
0 & \text{o.w.}
\end{cases}
$$
Note that for $t_{ij}\in t_i$ then:
\begin{align*}
\sum_{\substack{S\subseteq \cF\\j \in S}}\widehat{\sigma}_i(S)
=&    \sum_{\substack{S\subseteq \cF\\j \in S}} \prod_{k\in S}\left(\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})} \right)\sum_{S \subseteq T\subseteq \cF}\sigma_i(T) \prod_{k\in T\backslash S}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right) \\
=&\frac{w_{ij}'(t_{ij})}{w_{ij}(t_{ij})}\sum_{\substack{T\subseteq \cF\\j \in T}}\sigma_i(T) \sum_{S\subseteq T} \prod_{k\in S\backslash\{j\}}\left(\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})} \right)  \prod_{k\in T\backslash \{S\cup \{j\}\}}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right) \\
\end{align*}

Similar to what we argued above,
we can prove that
$$\sum_{S\subseteq T} \prod_{k\in S\backslash\{j\}}\left(\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})} \right)  \prod_{k\in T\backslash \{S\cup \{j\}\}}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right)=1$$
by thinking that $\prod_{k\in S\backslash\{j\}}\left(\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})} \right)  \prod_{k\in T\backslash \{S\cup \{j\}\}}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right)$ is the probability when we choose a subset of $T\backslash \{j\}$ where we include item $j$ in the set independently at random with probability $\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\leq 1$. 
Thus we have that
\begin{align*}
\sum_{\substack{S\subseteq \cF\\j \in S}}\widehat{\sigma}_i(S)
=&\frac{w_{ij}'(t_{ij})}{w_{ij}(t_{ij})}\sum_{\substack{T\subseteq \cF\\j \in T}}\sigma_i(T) \sum_{S\subseteq T} \prod_{k\in S\backslash\{j\}}\left(\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})} \right)  \prod_{k\in T\backslash \{S\cup \{j\}\}}\left(1-\frac{w_{ik}'(t_{ik})}{w_{ik}(t_{ik})}\right) \\
= & \frac{w_{ij}'(t_{ij})}{w_{ij}(t_{ij})}\sum_{\substack{T\subseteq \cF\\j \in T}}\sigma_i(T)\\
=& w_{ij}'(t_{ij})
\end{align*}
For $t_{ij}' \neq t_{ij}$,
then $w_{ij}(t_{ij}')= w_{ij}'(t_{ij}')=0$.

\end{comment}


It remains to show that we can find an element in $\text{argmax}_{w_i\in W_{t_i}} \bm{a}\cdot w_i$ for any $\bm{a}\in \mathbb{R}^{\sum_{j\in[m]}|\cT_{ij}|}$, given access to a demand oracle.
%\argyrisnote{Argyris: we change the bit complexity of the input by this assumption.} 
W.l.o.g. we assume that for each $j\in[m]$ and $t_{ij}\in \cT_{ij}$,
$a_{ij}(t_{ij})\leq \frac{1}{2}\cdot t_{ij}$ (by scaling and the fact that $t_{ij}>0$).
Observe that any corner $w_i$ of the polytope $W_{t_i}$ corresponds to the choice of $\{\sigma_S\}_{S\in \cF_i}$ such that $\sigma_S=\ind[S=T]$ for some particular $T\in \cF_i$, i.e. $w_{ij}(t_{ij}')=\ind[j\in T\wedge t_{ij}'=t_{ij}]$.

Since 
%we know that over any polytope,
$w_i^*\in \text{argmax}_{w_i\in W_{t_i}} \bm{a}\cdot w_i$ is a corner of $W_{t_i}$. We have
%can be one of the corners,
%we can see that
\begin{align*}
    & \text{max}_{w_i\in W_{t_i}} \bm{a}\cdot w_i\\
    =& \max_{S\in\cF_i} {\sum_{j\in S}} a_{ij}(t_{ij})\\ %\text{\yangnote{Yang: Where did $a_{ij}(t_{ij})$ go? Why are you multiplying $w_{ij}$ with $t_{ij}$?}}\\
    =& \max_{S\in\cF_i} {\sum_{j\in S}} a_{ij}(t_{ij})^+\\
    =& \max_{S\in\cF_i} {\sum_{j\in S}} (t_{ij}-(t_{ij}-a_{ij}(t_{ij})^+))\\
%    =& \max_{S\subseteq \cF} \left\{\sum_{j\in S} (t_{ij}-(1- w_{ij}(t_{ij})^+)t_{ij})\right\}\\
\end{align*}


Here $x^+=\max\{x,0\}$. The second equality holds because $\cF_i$ is downward-closed.
%Since we assumed that for each $j\in[m]$ and $t_{ij}\in\cT_{ij}$, $w_{ij}(t_{ij})\leq 1$,
%then $(1-w_{ij}(t_{ij}))t_{ij} \geq 0$.
%Thus we can intepret $\max_{S\subseteq \cF} {\sum_{j\in S}} (t_{ij}-(1- w_{ij}(t_{ij})^+)t_{ij})$ as the maximizing utility that an agent with type $t_i$ has,
%when we participates in a posted price mechanism,
%where the price of the $j$-th item is $(1- w_{ij}(t_{ij})^+)t_{ij}$.
%Let $S^* = \arg\max_{S\subseteq \cF} {\sum_{j\in S}} (t_{ij}-(1- w_{ij}(t_{ij})^+)t_{ij})$ and consider $w\in [0,1]^{\sum_{j\in[m]}|\cT_{ij}|}$ such that for each $j\in[m]$ and $t_{ij}'\in \cT_{ij}$ we set $w_{ij}(t_{ij}')=\ind[j\in S \land t_{ij}'=t_{ij}]$.
Notice that $a_{ij}(t_{ij})^+\leq \frac{1}{2}t_{ij}$. Thus with a single query to the demand oracle, with type $t_i$ and prices $p_{ij}=t_{ij}-a_{ij}(t_{ij})^+\geq 0,\forall j$, we can find $\text{argmax}_{w_i\in W_{t_i}} \bm{a}\cdot w_i$. The bit complexity of $w_i^*$ is at most $\sum_{j\in[m]}|\cT_{ij}|$. %$\log(\sum_{j\in[m]}|\cT_{ij}|)$.
%\todo{Does demand query outputs utility or maximizing bundle?}\argyrisnote{Argyris: That's how I defined it.}
\end{proof}

\begin{lemma}\label{lem:box polytope constraint additive}
Let $T = \sum_{j\in[m]}|\cT_{ij}|$. For any $\eps < \frac{1}{T}$, $(1-\eps T)W_{i}^{box(\eps)}\subseteq W_i$.
\end{lemma}

%Lemma~\ref{lem:box polytope constraint additive} is a special case of Lemma~\ref{lem:welfare rare}. We refer the readers to the proof of Lemma~\ref{lem:welfare rare}.
\begin{proof}

For any $w_i\in (1-\eps T )W_i^{box(\eps)}$, we prove that $w_i\in W_i$. 
%Then $(\pi_i,w_i)\in W_i$ since $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})$ for any $j,t_{ij}$.

Consider the following set of numbers $\{\sigma_{S}(t_i)\}_{t_i,S}$ (see \Cref{{def:W_i-constrained-add}}): For each $j\in [m], t_{ij}\in \cT_{ij}$, let $c_j(t_{ij})=\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right)$ and
$$p_j(t_{ij})=\frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})c_j(t_{ij})\cdot \sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))}.$$ 

{Note that for every $j'\in[m]$, there exists a value $t_{ij'}\in\cT_{ij'}$ such that $f_{ij'}(t_{ij'})\geq 1/|\cT_{ij'}|$. Due to our choice of $\eps$, the corresponding $c_{j'}(t_{ij'})<1$. Hence, $\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))>0$, and $p_j(t_{ij})$  is well-defined.}

For every $t_i$, define
\begin{align*}
\sigma_{S}(t_i)=
\begin{cases}
p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'})), &\text{if  $S=\{j\}$ for some $j\in[m]$}\\
0, &\text{o.w.}
\end{cases}
\end{align*}

For every $j$ and $t_{ij}$, let $C_j(t_{ij})$ be the independent Bernoulli random variable that is $1$ with probability $c_j(t_{ij})$. Then for every $j$, 
$$
\Pr_{C_j(t_{ij}), t_{ij}\sim D_{ij}}\left[C_j(t_{ij})=1\right]=\sum_{t_{ij}\in \cT_{ij}} f_{ij}(t_{ij})\cdot\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right) \leq \eps \cdot |\cT_{ij}|
$$

By the union bound,
\begin{align*}\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))=&\Pr_{\substack{t_{i,-j}\sim D_{i,-j}\\\forall j' \neq j, C_k(t_{ij'})}}[C_{j'}(t_{ij'}) =0,\forall j'\not=j]\\
=&1- \Pr_{\substack{t_{i,-j}\sim D_{i,-j}\\\forall j' \neq j, C_k(t_{ij'})}}[C_{j'}(t_{ij'}) =1,\exists j'\not=j]\\
\geq & 1-\sum_{j\neq j'}\Pr_{\substack{t_{ij}\sim D_{ij}\\ C_j(t_{ij}) }}[C_j(t_{ij})=1]\\
\geq & 1-\eps\cdot T
\end{align*}


Now we show that $w_i\in W_i$ by verifying both properties in \Cref{def:W_i-constrained-add}. {For the first property, since $w_i\in (1-\eps T)W_{i}^{box(\eps)}$, $0 \leq w_{ij}(t_{ij}) \leq \left(1-\eps \cdot T \right)\cdot\min\{\eps,l_{t_{ij}}(W_i)\}= \left(1-\eps \cdot T \right)\cdot f_{ij}(t_{ij})\cdot c_j(t_{ij})$. The equality is due to the definition of $c_j(t_{ij})$ and \Cref{obs:constraint additive length}.} Thus $p_j(t_{ij})\leq 1$ for every $j$ and $t_{ij}$.
{We have that $\sum_{S}\sigma_S(t_i)=\sum_{j\in[m]} p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))\leq \sum_{j\in[m]} c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))\leq \prod_{j\in[m]}\left(c_j(t_{ij})+(1-c_j(t_{ij})\right)=1$.}% We notice that $\sum_j c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))$ is exactly the probability of there exists a unique $C_j(t_{ij})=1$.  Thus $\sum_{S}\sigma_S(t_i)\leq 1$.

The second property: 
\begin{align*}
&f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sigma_S(t_{ij},t_{i,-j})\\
=&f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))=w_{ij}(t_{ij})
\end{align*}
\notshow{
The third inequality:
\begin{align*}
&f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S(t_{ij},t_{i,-j})\cdot \frac{\alpha_{ij}(t_{ij})}{V_{ij}(t_{ij})}\\
=&f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))\cdot \frac{\max_k\alpha_{ij}(t_{ij})}{V_{ij}(t_{ij})}=\pi_{ij}(t_{ij})=w_{ij}'(t_{ij})
\end{align*}
}
Thus by \Cref{def:W_i-constrained-add}, $w_i\in W_i$. %We finish our proof.
%. Thus $(\pi_i,w_i)\in W_i$. We finish our proof.

\notshow{
The old proof:

We consider the following allocation rule $\sigma_{S}^k(t_i)$ parametrised by variables $\{p_{j,t_{ij}}\in[0,1]\}_{j\in[m],t_{ij}\in T_{ij}}$.
We are going to prove that $W_{i,\epsilon}^r\subseteq W_i$.
When an agent with type $t_i$ appears, the mechanism works in the following way.
For each $j\in[m]$, let 
$$C(j) \sim Ber\left( \min\left(\frac{\epsilon}{f_{ij}(t_{ij})},1 \right)\right)$$
If there exists only one $j^*\in[m]$ such that $C(j^*)=1$,
then allocate only the $j^*$-th item to the agent activating the additive function $k^*\in[K]$ such that $\alpha^{k*}_{j^*}=V_{ij}(t_{ij})$.
%with probability $p_{j,t_{ij}}$.
Note that:
$$
\Pr_{\substack{t_{ij}\sim D_{ij}\\C(j) \sim Ber\left( \min\left(\frac{\epsilon}{f_{ij}(t_{ij})},1) \right)\right) }}\left[C_j=1  \right] \leq \sum_{t_{ij}\in \cT_{ij}} f_{ij}(t_{ij})\cdot\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right) \leq \eps \cdot |\cT_{ij}|
$$
Thus by union bound, $\Pr[C_j=0,\forall j]\geq 1-\sum_j\Pr[C_j=1]\geq 1-\eps\cdot T$.
%the probability that there is no $j\in[m]$ such that $C(j)=1$ is at least $1-\epsilon \cdot M$.
Thus under this allocation we have that
\begin{align*}
    w_{ij}(t_{ij}) = \pi_{ij}(t_{ij}) \geq (1-\epsilon\cdot M)  \min\left(\frac{\epsilon}{f_{ij}(t_{ij})}, 1 \right)f_{ij}(t_{ij}) =
    (1-\epsilon\cdot M)  \min\left(\epsilon, f_{ij}(t_{ij})\right)
\end{align*}
Thus for any target 
$$\{\hat{\pi}_{ij}(t_{ij})\leq (1-\epsilon \cdot M)\min(\epsilon,f_{ij}(t_{ij})\}_{j\in[m],t_{ij}\in T_{ij}}$$ 
there exists a set of variables $\{p_{j,t_{ij}} \in [0,1]\}_{j\in[m],t_{ij}\in T_{ij}}$ such that when the agent has type $t_{i}$, then with probability $p_{j,t_{ij}}$ we set $C(j)=0$ and then run the mechanism as we described it.
This allocation distribution ensures that:
\begin{align*}
    w_{ij}(t_{ij}) = \pi_{ij}(t_{ij}) =\hat{\pi}_{ij}(t_{ij})
\end{align*}
Thus we proved that for every $(\pi,w)$ such that:
\begin{align*}
    w_{ij}(t_{ij}) = \pi_{ij}(t_{ij}) \leq
    (1-\epsilon\cdot M)  \min\left(\epsilon, f_{ij}(t_{ij})\right)
\end{align*}
$(\pi,w_i)\in  W_i$.
Observe that for each $(\pi',w_i')$ such that:
\begin{align*}
    w_{ij}'(t_{ij})\leq w_{ij}(t_{ij}) \\
    \pi_{ij}'(t_{ij})\geq \pi_{ij}(t_{ij})
\end{align*}

then $(\pi',w')\in W_i$.
This concludes that $W_{i,\eps}^r \subseteq W_i$ for all $\epsilon < \frac{1}{T}$.}
\end{proof}


\notshow{

\begin{theorem}\label{thm:multiplicative approx for constraint additive}
%[Restatement of \Cref{thm:multiplicative approx for constraint additive-main body}]
Let $T = \sum_{j\in[m]}|\cT_{ij}|$ and consider parameters $\eps <\frac{1}{T}$ and \\
$k\geq\max \left(\log\left(\frac{1}{\eps}\right),\Omega\left(d^4\left( b + \log\left( \frac{1}{\eps}\right)\right)\right)\right)$.
Let $b$ be an upper bound on the bit complexity of each element in $\{f_{ij}(t_{ij})\}_{j\in[m],t_{ij}\in\cT_{ij}}$.
Then with probability at least $1-2T\exp(-2Tk)$,
having access to $\left\lceil\frac{8kT}{(1-\eps T)^2}\right\rceil$ samples from $\cD_i$,
we can construct a convex polytope $\widehat{W}_i$ such that
\begin{enumerate}
\item $\frac{1-\eps T}{6}W_i\subseteq \widehat{W}_i\subseteq W_i$

\item There exists a separation oracle $SO$ for $\widehat{W}_i$,
whose running time on input with bit complexity $b''$, is $\poly\left(b,b'',k,d,\frac{1}{\eps}\right)$ and performs $\poly\left(b,b'', k,d,\frac{1}{\eps}\right)$ queries to demand oracle $\dem_i(\cdot,\cdot)$ with inputs of bit complexity $\poly\left(b, b'',d,\frac{1}{\eps}\right)$.
\end{enumerate} 
\end{theorem}


\begin{proof}
%The proof follows since:
We notice that:
\begin{enumerate}
\item By \Cref{obs:constraint additive length}, we have that the bit complexity of each element in $\{l_j(W_i)\}$ is $b'$.
\item By Observation~\ref{obs:mix constraint additive}, we have that $W_{i}$ is mixture of $\{W_{t_i}\}_{t_i\in \cT_i}$ over distribution $D_i$.
%
\item By Lemma~\ref{lem:monotone-closed polytope W}, for each $t_i\in\cT_i$, $W_{t_{i}}$ is lowered-closed and given access to demand oracle $\dem_i(t_i,\cdot)$ we can find an element in $\text{argmax}\{\bm{a}\cdot w_i\mid w_i\in W_{t_i}\}$.
Note that each output of the demand oracle has bit complexity at most $T$. 
%
\item By Lemma~\ref{lem:box polytope constraint additive}, $(1-\eps T)W_i^{box(\eps)}\subseteq W_i$ 
\end{enumerate}
%We apply Theorem~\ref{thm:special case of multiplicative approx} to our problem, which concludes the proof.
The proof then follows directly by applying \Cref{thm:special case of multiplicative approx} to $W_i$ for every $i$.
\end{proof}

}

%\yangnote{Yang: Check the statement of \Cref{thm:multiplicative approx for constraint additive-main body} and see if it matches what \Cref{thm:special case of multiplicative approx} guarantees.}

\begin{prevproof}{Theorem}{thm:multiplicative approx for constraint additive-main body}

We simply verify that $W_i$ satisfies all assumptions in \Cref{thm:special case of multiplicative approx}. Recall that $T=\sum_{i,j}|\cT_{ij}|$ and {$b$ is an upper bound of the bit complexity of all $f_{ij}(t_{ij})$'s and all $t_{ij}$'s.} We have the following: 

\begin{enumerate}
\item By \Cref{obs:mix constraint additive}, we have that $W_{i}$ is a mixture of $\{W_{t_i}\}_{t_i\in \cT_i}$ over distribution $D_i$.

\item By Lemma~\ref{lem:monotone-closed polytope W}, for each $t_i\in\cT_i$, $W_{t_{i}}$ is a convex and down-monotone polytope. Given access to the demand oracle $\dem_i(t_i,\cdot)$, we can find an element in $\argmax\{\bm{a}\cdot w_i: w_i\in W_{t_i}\}$ in time {$poly(b',b,T)$ and a single query to $\dem_i(t_i,\cdot)$}, where $b'$ is the bit complexity of the input $\bm{a}$. Note that each output of the demand oracle has bit complexity at most $T$. 

\item By \Cref{obs:constraint additive length}, {$l_{t_{ij}}(W_i)=f_{ij}(t_{ij})$,for all $j$ and $t_{ij}$.  Thus, each $l_{t_{ij}}(W_i)$ has bit complexity at most $b$.} %Thus every corner of $W_i$ has bit complexity $poly(n,m,T,b)$. 

%we have that the bit complexity of each element in $\{l_j(W_i)\}$ is $b'$.

%

%
\item By Lemma~\ref{lem:box polytope constraint additive}, $(1-\eps T)W_i^{box(\eps)}\subseteq W_i$ for any $\eps<\frac{1}{T}$. Choosing $\eps=\frac{1}{2T}$ obtains $\frac{1}{2}W_i^{box(\frac{1}{2T})}\subseteq W_i$.

%\yangnote{Yang: It will be useful to compute an explicit constant $c$ in \Cref{thm:multiplicative approx for constraint additive-main body}.}
\end{enumerate}

%\yangnote{The statement of~\Cref{thm:multiplicative approx for constraint additive-main body} then follows from \Cref{thm:special case of multiplicative approx}.}
For any $\delta\in (0,1)$, we apply \Cref{thm:special case of multiplicative approx} with parameter $k=poly(n,m,T,b,\log(1/\delta))$, $c=\frac{1}{2}$ and $\eps=\frac{1}{2T}$. The probability that the algorithm successfully constructs a polytope that satisfies both properties of \Cref{thm:special case of multiplicative approx} is at least $1-\delta$. We have $\frac{1}{12}\cdot W_i\subseteq \widehat{W}_i\subseteq W_i$ by the first property of \Cref{thm:special case of multiplicative approx} with $c=\frac{1}{2}$. Since the  vertex-complexity of $W_{t_i}$ for each $t_i$ is no more than $T$, and the vertex-complexity for $W_i^{box(\frac{1}{2T})}$ is no more than $\poly(b,T)$, the vertex-complexity for $\widehat{W}_i$ is no more than $poly(n,m,T,b,\log(1/\delta))$. The running time of the algorithm and the separation oracle $SO$ for $\widehat{W}_i$ follows from the second property of \Cref{thm:special case of multiplicative approx}. 

%For any $\delta\in (0,1)$, by applying \Cref{thm:multiplicative approx for constraint additive-main body} with parameter\\ $k\geq \max \left(\log\left(\frac{1}{\eps}\right),\Omega\left(d^4\left( b + \log\left( \frac{1}{\eps}\right)\right)\right),\log(\frac{1}{\delta})\right)$, the probability that the algorithm successfully constructs a polytope is at least $1-\delta$. The running time of the algorithm and SO directly follows from the statement of \Cref{thm:multiplicative approx for constraint additive}. 
%The proof is done by applying \Cref{thm:multiplicative approx for constraint additive-main body}.
\end{prevproof}



At last, we give the proof of \Cref{thm:main} by combining \Cref{thm:bounding-lp-simple-mech} and \Cref{thm:multiplicative approx for constraint additive-main body}.

\begin{prevproof}{Theorem}{thm:main}
Fix any $\delta\in (0,1)$. Recall that in the LP of \Cref{fig:bigLP}, we use an estimation of $\prev$, which is $\estprev$, according to \Cref{thm:chms10}. Denote $\cE_1$ the event that an RPP mechanism is successfully computed and $\cE_2$ the event that the algorithm in \Cref{thm:multiplicative approx for constraint additive-main body} successfully constructs a convex polytope $\widehat{W}_i$ that satisfies both properties in the statement of \Cref{thm:multiplicative approx for constraint additive-main body} {for each buyer $i\in [n]$}. Note that $\cE_1$ happens with probability at least $1-\frac{2}{n}$ and {we take enough samples to make sure that} $\cE_2$ happens with probability at least $1-\delta$, by the union bound, the probability that both $\cE_1$ and $\cE_2$ happen is at least $1-\delta-\frac{2}{n}$. From now on, we will condition on both events $\cE_1$ and $\cE_2$.

Now in the LP of \Cref{fig:bigLP}, we replace $W_i$ by $\widehat{W}_i$ for every $i$ (we will call it the modified LP). By property 1 and 2 of \Cref{thm:multiplicative approx for constraint additive-main body}, we can solve the modified LP using the separation oracle for $\widehat{W}_i$, in time $\poly(b,n,m,T,\log(1/\delta))$ (recall that $T=\sum_{i,j}|\cT_{ij}|$) according to \Cref{thm:ellipsoid}. Let $x^*=(w^*,\lambda^*,\hat\lambda^*,\textbf{d}^*)$ be an optimal solution of the modified LP. Then $w_i^*\in \widehat{W}_i$ for every $i$ according to Constraint {\Wconstraint} in the modified LP. By property 1 of \Cref{thm:multiplicative approx for constraint additive-main body}, we have $\widehat{W}_i\subseteq W_i$. Thus $w_i^*\in W_i,\forall i$ and hence $x^*$ is also a feasible solution of the original LP in \Cref{fig:bigLP}.

Recall that $\optlp$ is the optimum objective of the original LP. Denote $\optlp'$ the optimum objective of the modified LP. Thus in order to prove that $(w^*,\lambda^*,\hat\lambda^*,\textbf{d}^*)$ is an approximately-optimal solution in the original LP, it suffices to show that $\optlp'\geq c\cdot \optlp$. Take any feasible solution $(w,\lambda,\hat\lambda,\textbf{d})$ of the original LP. We have that $w_i\in W_i$ for every $i$. Now consider another set of variables $(w',\lambda',\hat\lambda,\textbf{d})$ such that $w'_{ij}(t_{ij})=c\cdot w_{ij}(t_{ij})$ and $\lambda'_{ij}(t_{ij},\beta_{ij},\delta_{ij})=c\cdot \lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$, for all $i,j,t_{ij},\beta_{ij},\delta_{ij}$, where $c=1/12$. %$c\in(0,1)$ is the constant in the first property of \Cref{thm:multiplicative approx for constraint additive-main body}.
We verify that $(w',\lambda',\hat\lambda,\textbf{d})$ is a feasible solution for the modified LP. For Constraint {\Wconstraint}, since $c\cdot W_i\subseteq \widehat{W}_i$ (property 1 of \Cref{thm:multiplicative approx for constraint additive-main body}), we have that $w'_i\in \widehat{W}_i$, for all $i$. For Constraint {\LambdaMarginalConstraint}, it holds since we multiply both $\lambda$ and $w$ by $c$. Constraint {\PiConstraint}, {\CompareMarginalConstraint} and {\MarginalToGlobalConstraint} hold, as for each of them their LHS is smaller while the RHS remains unchanged. Every other constraint holds since both of their LHS and RHS remain the same. Thus $(w',\lambda',\hat\lambda,\textbf{d})$ is a feasible solution for the modified LP.

%\todo{Add the correct labels for the constraints.}

Now notice that the objective of the solution $(w',\lambda',\hat\lambda,\textbf{d})$ is exactly $c$ times the objective of the solution $(w,\lambda,\hat\lambda,\textbf{d})$. By choosing $(w,\lambda,\hat\lambda,\textbf{d})$ to be the optimal solution of the original LP, we have that $\optlp'\geq c\cdot \optlp$. It implies that the objective of $(w^*,\lambda^*,\hat\lambda^*,\textbf{d}^*)$ is at least $c\cdot \optlp$. Thus if we compute the simple mechanisms using the decision variables $(w^*,\lambda^*,\hat\lambda^*,\textbf{d}^*)$. By \Cref{thm:multiplicative approx for constraint additive-main body}, we have    $$c_1\cdot \rev(\Mpp)+c_2\cdot\rev(\Mtpt)\geq\optlp'\geq c\cdot \optlp\geq c\cdot \opt$$
We finish our proof by noticing that the simple mechanisms can be computed in time $\poly(n,m,T)$ given the solution $(w^*,\lambda^*,\hat\lambda^*,\textbf{d}^*)$.
\end{prevproof}



==> arXiv/appx_prelim.tex <==
\section{Additional Preliminaries}\label{appx:prelim}
\begin{definition}~\cite{RubinsteinW15}\label{def:subadditive independent}
Let $\cD_i$ be the type distribution of bidder $i$ and denote by $\cV_i$ her distribution over valuations $v_i(t_i,\cdot)$ where $t_i\sim \cD_i$. We say that $\cV_i$ is subadditiver over independent items if
\begin{itemize}
\item $v_i(\cdot,\cdot)$ has no externalities, that is for any $S\subseteq[m]$, $t_i,t_i' \in \cT_i$ such that $t_{ij}=t_{ij}'$ for $j\in S$,
then $v_i(t_i,S)=v_i(t_i',S)$.
\item $v_i(\cdot,\cdot)$ is monotone, that is for each $t_i\in \cT_i$ and $S\subseteq T \subseteq[m]$, $v_i(t_i,S)\leq v_i(t_i,T)$
\item $v_i(\cdot,\cdot)$ is subadditive function, that is for all $t_i\in \cT_i$ and $S_1,S_2\subseteq [m]$, $v_i(t_i,S_1 \cup S_2)\leq v_i(t_i,S_1)+ v_i(t_i,S_2)$ 
\end{itemize}
\end{definition}

\paragraph{Mechanisms:} A mechanism $M$ in multi-item auctions can be described as a tuple $(x,p)$. For every type profile $t$, buyer $i$ and bundle $S\subseteq [m]$, $x_{iS}(t)$ is the probability of buyer $i$ receiving the exact bundle $S$ at profile $t$, $p_i(t)$ is the payment for buyer $i$ at the same type profile. To ease notations, for every buyer $i$ and types $t_i$, we use $p_i(t_i)=\E_{t_{-i}}[p_i(t_i,t_{-i})]$ as the interim price paid by buyer $i$ and $\sigma_{iS}(t_i)=\E_{t_{-i}}[x_{iS}(t_i,t_{-i})]$ as the interim probability of receiving the exact bundle $S$.

\paragraph{IC and IR constraints:} A mechanism $M=(x,p)$ is BIC if:
$$\sum_{S\subseteq [m]}\sigma_{iS}(t_i)\cdot v_i(t_i,S)-p_i(t_i)\geq \sum_{S\subseteq [m]}\sigma_{iS}(t_i')\cdot v_i(t_i,S)-p_i(t_i'), \forall i,t_i,t_i'\in \cT_i.$$

The mechanism is DSIC if:
$$\sum_{S\subseteq [m]}x_{iS}(t_i,t_{-i})\cdot v_i(t_i,S)-p_i(t_i,t_{-i})\geq \sum_{S\subseteq [m]}x_{iS}(t_i',t_{-i})\cdot v_i(t_i,S)-p_i(t_i',t_{-i}), \forall i,t_i,t_i'\in \cT_i,t_{-i}\in \cT_{-i}.$$

The mechanism is (interim) IR if:
$$\sum_{S\subseteq [m]}\sigma_{iS}(t_i)\cdot v_i(t_i,S)-p_i(t_i)\geq 0, \forall i,t_i\in \cT_i.$$

The mechanism is ex-post IR if:
$$\sum_{S\subseteq [m]}x_{iS}(t_i,t_{-i})\cdot v_i(t_i,S)-p_i(t_i,t_{-i})\geq 0, \forall i,t_i\in \cT_i,t_{-i}\in \cT_{-i}.$$



\begin{definition}[Separation Oracle for Convex Polytope $\cP$]
A Separation Oracle $SO$ for a convex polytope $\cP\subseteq \mathbb{R}^d$,
takes as input a point $\bx \in \mathbb{R}^d$ and if $\bx \in \cP$,
then the oracle says that the point is in the polytope.
If $\bx \notin \cP$,
then the oracle output a separating hyperplane,
that is it outputs a vector $\textbf{y}\in \mathbb{R}^d$ and $c\in \mathbb{R}$ such that $\textbf{y}^T x \leq c$,
but for $\textbf{z} \in \cP$, $\textbf{y}^T \textbf{z} > c$.
\end{definition}

%\paragraph{Access to the Buyers' Valuations.}
\notshow{
\begin{definition}[Scalable Demand Oracle for XOS Valuations]\label{def:scalable demand oracle}
%Consider a set of non-negative coefficients $\{b_j\}_{j\in[m]}$, non-negative  prices $\{p_j\}_{j\in[m]}$ and a type $t_i\in \cT_i$ for bidder $i$.
For every buyer $i$, a scalable demand oracle with input $\dem_i(t_i,\{b_j\}_{j\in[m]},\{p_j\}_{j\in[m]} )$ for an XOS valuation $v_i(\cdot,\cdot)$,
takes an input the bidder's type $t_i$, the non-negative coefficient vector $\{b_j\}_{j\in[m]}$ and the non-negative price vector $\{p_j\}_{j\in[m]}$, and outputs a subset of items $S^*\subseteq[m] $ and $k^*\in[K]$ such that
$$
(S^*,k^*) \in \arg\max_{S\subseteq [m],k\in[K]} \sum_{j\in S}b_j \alpha_{ij}^{(k)}(t_{ij}) - \sum_{j\in S}p_j
$$
%Note that the scalable demand oracle multiplies the value that each item contributes to the total value of the agent by a different coefficient.
\end{definition}

%Moreover we will need access to a slightly modified version of the value oracle defined below.

\begin{definition}[Value Oracle for XOS Valuation $v_i(\cdot,\cdot)$]
Consider a type $t_i\in \cT_i$ for bidder $i$ and a $k\in[K]$.
A value oracle $\val(\cdot,\cdot)$ for XOS valuation $v_i(\cdot,\cdot)$,
takes an input the bidder's type, and a $k\in[K]$ and outputs $\{a_{ij}^{(k)}(t_{ij})\}_{j\in[m]}$.
\end{definition}
}


\begin{definition}[Polytopes and Facet-Complexiy]\label{def:facet-complexity} We say $P$ has \emph{facet-complexity} at most $b$ if it can be written as $P:= \{\vec{x}\mid \vec{x} \cdot \vec{w}^{(i)} \leq c_i,\ \forall i \in \mathcal{I}\}$, where each $\vec{w}^{(i)}$ and $c_i$ has bit complexity at most $b$ for all $i \in \mathcal{I}$. We use the term \emph{convex polytope} to refer to a set of points that is closed, convex, bounded,\footnote{$P\subseteq \mathbb{R}^d$ is bounded if it is contained in $[-x,x]^d$ for some $x \in \mathbb{R}$.} and has finite facet-complexity.
\end{definition}


\begin{definition}[Vertex-Complexity]\label{def:vertex-complexity}
We use the term \emph{corner} to refer to non-degenerate extreme points of a convex polytope. In other words, $\vec{y}$ is a corner of the $d$-dimensional convex polytope $P$ if $\vec{y} \in P$ and there exist $d$ linearly independent directions $\vec{w}^{(1)},\ldots,\vec{w}^{(d)}$ such that $\vec{x} \cdot \vec{w}^{(i)} \leq \vec{y} \cdot \vec{w}^{(i)}$ for all $\vec{x} \in P, 1 \leq i \leq d$. We use \textbf{$\Cor(P)$} to denote the set of corners of a convex polytope $P$. We say $P$ has vertex-complexity at most $b$ if all vectors in $\Cor(P)$ have bit complexity no more than $b$.
\end{definition}

The following fact states that the vertex-complexity and facet-complexity of a polytope in $\mathbb{R}^d$ are off by at most a $d^2$ multiplicative factor.

\begin{fact}[Lemma 6.2.4 of~\cite{grotschel2012geometric}]\label{fact:corners2}
Let $P$ be a convex polytope in $\mathbb{R}^d$. If $P$ has facet-complexity at most $b$, its vertex-complexity is at most $O(b\cdot d^2)$. Similarly, if $P$ has vertex-complexity at most $\ell$, its facet-complexity is at most $O(\ell\cdot d^2)$.
\end{fact}

\begin{theorem}\label{thm:ellipsoid}[Ellipsoid Algorithm for Linear Programming~\cite{grotschel2012geometric}\footnote{Properties 1 and 2 follow from Theorem 6.4.9 of~\cite{grotschel2012geometric} and Property 3 follows from Remark 6.5.2 of~\cite{grotschel2012geometric}.}]
Let $P$ be a convex polytope in $\mathbb{R}^d$ specified via a separation oracle $SO$, and $\vec{c}$ is any fixed vector in $\mathbb{R}^d$. %Assume that all $\vec{w}$ and $h$, for all separation hyperplanes $\vec{w}\cdot\vec{x}\leq h$ possibly output by $SO$ 
Assume that $P$'s facet-complexity and the bit complexity of $\vec{c}$ are no more than $b$. Then we can run the ellipsoid algorithm to optimize $\vec{c}\cdot\vec{x}$ over $P$, maintaining the following properties:
\begin{enumerate}
\item The algorithm will only query $SO$ on rational points with bit complexity $\poly(d,b)$.
\item The algorithm will solve the linear program in time $\poly(d, b,\rt_{SO}(\poly(d,b)))$, where $\rt_{SO}(x)$ is the running time of the SO on any input of bit complexity $x$.
\item The output optimal solution is a corner of $P$.
\end{enumerate}
\end{theorem}


==> arXiv/appx_program.tex <==
\section{Missing Details from Section~\ref{sec:program}}\label{sec:appx_program}

%\subsection{Overview of this Section and Discussion about XOS Valuations}

In this section, we provide a proof of \Cref{thm:bounding-lp-simple-mech}. Indeed, we prove a generalization that works for XOS buyers (\Cref{thm:bounding-lp-simple-mech-XOS}), with the generalized of the single-bidder marginal reduced form polytope~\Cref{def:W_i} and a generalized LP (\Cref{fig:XOSLP}). 

\begin{theorem}\label{thm:bounding-lp-simple-mech-XOS}
Let $(w,\lambda,\hat\lambda, \bd)$ (or  $(\pi,w,\lambda,\hat\lambda, \bd)$) be any feasible solution of the LP in \Cref{fig:bigLP} (or \Cref{fig:XOSLP}).
%Then for sufficiently small $\epsilon_r$, 
Let $\Mpp$ be the rationed posted price mechanism computed in \Cref{thm:chms10}. Let $\Mtpt$ be the two-part tariff mechanism shown in Mechanism~\ref{def:constructed-SPEM} with prices $\{Q_j\}_{j\in[m]}$ (\Cref{def:Q_j-XOS}). Then the objective function of the solution $2\cdot \sum_{j\in [m]}Q_j$ is bounded by $c_1\cdot \rev(\Mpp)+c_2\cdot \rev(\Mtpt)$, for some constant $c_1,c_2>0$. 
%for some \mingfeinote{restricted SPM} $\cM_1$ and some \mingfeinote{SPEM} $\cM_2$. 
Moreover, both $\Mpp$ and $\Mtpt$ can be computed in time $\poly(n,m,\sum_{i,j}|\cT_{ij}|)$, 
%and require $\poly(n,m,\sum_{i,j}|\cT_{ij}|)$ queries 
with access to the demand oracle for the buyers' valuations. 
%(for constrained-additive valuations) or \todo{the scalable demand oracle} (for XOS valuations). 
\end{theorem}



%We notice that with \Cref{thm:bounding-lp-simple-mech-XOS}, we can compute simple mechanisms efficiently given any feasible solution to the LP, even for XOS valuations. Thus the only part that is missing from a complete construction for XOS buyers, is to find efficiently an approximately-optimal solution to the LP in \Cref{fig:XOSLP}. Recall that in the constrained-additive case, we prove that we can efficiently construct another polytope $\widehat{W}_i$ sandwiched between $c\cdot W_i$ and $W_i$ for some absolute constant $c\in (0,1)$. The proof heavily relies on the fact that $W_i$ is down-monotone (see \Cref{sec:multi-approx-polytope}), which is not the case for the XOS marginal reduced form polytope $W_i$ due to the correlation between $\pi$ and $w$. 
%Thus our result for the constrained-additive case does not directly generalize to XOS valuations. Nonetheless, we believe that a similar approach may allow us to efficiently find an approximate solution of the LP in Figure~\ref{fig:XOSLP}, which can be combined with \Cref{thm:bounding-lp-simple-mech-XOS} to resolve the problem for the XOS case.
%the only non-constructed part is to get an efficient separation oracle for the (generalized) marginal reduced form polytope $W_i$.

%The proof of Theorem~\ref{thm:bounding-lp-simple-mech} is proved for XOS functions using the definition of marginal reduced form polytope for XOS bidders as stated in Definition~\ref{def:W_i}.

%However we cannot apply \Cref{thm:special case of multiplicative approx-main body} in order to construct a proxy polytope for the reduced form polytope as we did when the bidders are constrained-additive.


%In this section,
%we make some notes about Theorem~\ref{thm:bounding-lp-simple-mech}
%stated again below.


\subsection{Result by Cai and Zhao~\cite{CaiZ17} for XOS Valuations}\label{appx_cai-zhao}

The result by Cai and Zhao~\cite{CaiZ17} applies also to XOS valuations. Here we state their result for this general case. Note that this is a generalized definition and lemma for \Cref{def:core-constrained-additive} and \Cref{lem:caiz17-constrained-additive}.

\begin{definition}\label{def:core}
For any $i\in [n],j\in [m]$, let $\cV_{ij}^0 = \{ V_{ij}(t_{ij}): t_{ij} \in \cT_{ij}\}$. For any feasible interim allocation $\sigma$, and non-negative numbers {$\tilde{\vBeta}=\{\tilde{\beta}_{ij}\in \cV_{ij}^0\}_{i\in[n],j\in[m]}$, $\vC=\{c_i\}_{i\in[n]}$} and $\vr=\{r_{ij}\}_{i\in [n],j\in [m]}\in [0,1]^{nm}$ (which we refer to as the dual parameters), %~\footnote{$\tilde{\vBeta}$, $\vC$, and $r$ are the dual parameters that we refer to in the introduction.}
define $\core(\sigma,\tilde{\vBeta},\vC,\vr)$ as the welfare under allocation $\sigma$ truncated at $\tilde{\beta}_{ij}+c_i$ for every $i,j$.
%, with rebate ratio $r$ (see the remark below). 
Formally, $$\core(\sigma,\tilde{\vBeta},\vC,\vr)=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \left(\ind[t_{ij}< \tilde{\beta}_{ij}+c_i]+r_{ij}\cdot \ind[t_{ij}= \tilde{\beta}_{ij}+c_i] \right)$$
if the buyers have constrained-additive valuations, and
$$\core(\sigma,\tilde{\vBeta},\vC,\vr)=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}\gamma_{ij}^S(t_i)\cdot \left(\ind[V_{ij}(t_{ij})< \tilde{\beta}_{ij}+c_i]+r_{ij}\ind[V_{ij}(t_{ij})= \tilde{\beta}_{ij}+c_i] \right)$$ if the buyers have XOS valuations.
Here $\gamma_{ij}^S(t_i)=\alpha_{ij}^{k^*(t_i,S)}(t_{ij})$, where $\displaystyle k^*(t_i,S)=\arg\max_{k\in[K]}\big(\sum_{j\in S}\alpha^k_{ij}(t_{ij})\big)$.
\end{definition}

\begin{lemma}\cite{CaiZ17}\label{lem:caiz17}
Given any BIC and IR mechanism $\cM$, there exists \textbf{(i)} a feasible interim allocation $\sigma$,\footnote{Note that when buyers have constrained-additive valuations, it suffice to take $\sigma$ to be the interim allocation rule of $\cM$. For XOS valuations, $\sigma$ will be the interim allocation of a modified version of $\cM$. See Section~5 in~\cite{CaiZ16a} for details.} where $\sigma_{iS}(t_i)$ is the interim probability for buyer $i$ to receive exactly bundle $S$ when her type is $t_i$, \textbf{(ii)} non-negative numbers {$\tilde{\vBeta}^{(\sigma)}=\{\tilde{\beta}_{ij}^{(\sigma)}\in \cV_{ij}^0\}_{i\in[n],j\in[m]}$, $\vC^{(\sigma)}=\{c_i^{(\sigma)}\}_{i\in[n]}$} %\argyrisnote{can we say instead $\{\tilde{\beta}_{ij}\in \cV_{ij}^0\}_{i,j}, \{c_i\}_{i\in[n]}$?}
 and $\vr^{(\sigma)}\in [0,1]^{nm}$ that depend on $\sigma$, and \textbf{(iii)} a two-part tariff mechanism $\cM_1^{(\sigma)}$ such that %\yangnote{Yang: We need to make sure all the $\tilde{\beta}_{ij}$ are in $\cV_{ij}$ and all $c_i$ are in $\Delta_i$. I think it's fine to say $\tilde{\beta}_{ij}\in \cV^0_{ij}$, and we only choose $c_i$'s such that for at least one item $j$, $\tilde{\beta}_{ij}+c_i \in \cV^0_{ij}$.}
\begin{enumerate}
    \item $\sum_{i\in[n]} \left(\Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde\beta_{ij}^{(\sigma)}]+r_{ij}^{(\sigma)}\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde\beta_{ij}^{(\sigma)}]\right)\leq \frac{1}{2}$.
    \item $\frac{1}{2}\cdot\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\sigma_{iS}(t_i)\leq \Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde\beta_{ij}^{(\sigma)}]+r_{ij}^{(\sigma)}\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde\beta_{ij}^{(\sigma)}],\forall i,j$.
    \item $\rev(\cM)\leq 28\cdot \prev+4\cdot\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$.
    \item $\sum_{i\in [n]} c_i^{(\sigma)}\leq 8\cdot \prev$.
    \item $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})\leq 64\cdot \prev + 8\cdot \rev(\cM_1^{(\sigma)})$.
\end{enumerate}
\end{lemma}



\subsection{Single-Bidder Marginal Reduced Form Polytope for XOS Valuations}\label{sec:mrf-XOS}
In Definition~\ref{def:W_i} we define the single-bidder marginal reduced form polytope $W_i$ for XOS buyers, which differs from the single-bidder marginal reduced form polytope for constrained-additive valuation is several ways.
In Definition~\ref{def:W_i},
we define a distribution $\sigma_S^k$ over all possible subset of items $S\subseteq [m]$ and over the finite number $k\in[K]$ over additive functions that can be chosen when we evaluate the value that the buyer has for a set of items. In Definition~\ref{def:W_i-constrained-add}, the distribution $\sigma_S$ was only over sets in the set of feasible allocations. 
%A difference in Definition~\ref{def:W_i} is that we force the sum over $\sigma_S^{(k)}$ to be equal to $1$,
%while in Definition~\ref{def:W_i-constrained-add} we loosen the constraint to be less or equal than $1$.
%The change in the constraint is without loss of generality since if the mentioned sum is not equal to $1$, we can push any remainder probability to the empty set.

Similar to Definition~\ref{def:W_i-constrained-add},
$\pi_{ij}(t_{ij})$ is equal to $f_{ij}(t_{ij})$ times the probability that the $i$-th buyer receives the $j$-th item.
%However $w_{ij}(t_{ij})$ is equal to $\frac{f_{ij}(t_{ij})}{V_{ij}(t_{ij})}$ times or we receive get the $j$-th the item.
In contrast to Definition~\ref{def:W_i-constrained-add},
in Definition~\ref{def:W_i},
the value of $w_{ij}(t_{ij})$ is $\frac{f_{ij}(t_{ij})}{V_{ij}(t_{ij})}$ times the expected value that the buyer has for the item when we are allowed to choose which additive functions in $k\in[K]$ we count the value of the buyer, or we are even allowed to allocate an item to the buyer but count zero value for it (that is equivalent to just throwing away the item).


\begin{definition}[XOS valuations: single-bidder marginal reduced form polytope]\label{def:W_i}
%\argyrisnote{We can assume that we also have $\emptyset\in [m]$, so that we can make the first constraint equality.}
For every $i\in [n]$, the single-bidder marginal reduced form polytope $W_i\subseteq [0,1]^{2\cdot \sum_j|\cT_{ij}|}$ is defined as follows. Let $\pi_i=(\pi_{ij}(t_{ij}))_{j,t_{ij}\in \cT_{ij}}$ and $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}\in \cT_{ij}}$. Then $(\pi_i,w_i)\in W_i$ if and only if there exist a number $\sigma_S^{(k)}(t_i)\in [0,1]$ for every $t_i\in \cT_i, S\subseteq [m],k\in [K]$, such that
\begin{enumerate}
    \item $\sum_{S,k}\sigma_S^{(k)}(t_i)\leq 1 $, $\forall t_i\in \cT_i$.
    \item $%f_{ij}(t_{ij})\geq\pi_{ij}(t_{ij})\geq 
    {\pi_{ij}(t_{ij})=}f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})$, for all $i,j,t_{ij}\in \cT_{ij}$.
    \item ${w_{ij}(t_{ij})\leq} f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}$, for all $i,j,t_{ij}\in \cT_{ij}$.
\end{enumerate}
\end{definition}



\subsection{The Linear Program for XOS valuations}\label{sec:program-XOS}

%\mingfeinote{LP for the XOS valuations. Move it to the appendix later.}

\begin{figure}[H]
\colorbox{MyGray}{
\begin{minipage}{.98\textwidth}
\small
$$\quad\textbf{max  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}} 
 f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta}} \lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})\leq \beta_{ij} + \delta_{ij}]$$
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
\vspace{-.3in}
  \begin{align*}
 & \textbf{s.t.}\\
 &\quad\textbf{Allocation Feasibility Constraints:}\\
 &\quad\Wconstraint \quad (\pi_i,w_i) \in W_i & \forall i \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
&\quad\PiConstraint \quad \sum_i\sum_{t_{ij}\in \cT_{ij}}\pi_{ij}(t_{ij})\leq 1 & \forall j\\  
 &\quad\textbf{Natural Feasibility Constraints:}\\
    &\quad\LambdaMarginalConstraint\quad f_{ij}(t_{ij})\cdot\sum_{\beta_{ij}\in \cV_{ij}}\sum_{\delta_{ij}\in \Delta} \lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij}) = w_{ij}(t_{ij}) & \forall i,j,t_{ij}\in \cT_{ij}\\
    &\quad\CompareMarginalConstraint\quad\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}(\beta_{ij}, \delta_{ij}) & \forall i,j, t_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}\\
    &\quad\HatLambdaDistributionConstraint\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta}} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) = 1 & \forall i,j\\
    &\quad\textbf{Problem Specific Constraints:}\\
    &\quad\ReduceDemandConstaint \quad \sum_{i\in[n]}\sum_{\beta_{ij} \in \cV_{ij}}\sum_{\delta_{ij}\in \Delta} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}] \leq \frac{1}{2}& \forall j\\
    %& (5)\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \lambda_{ij}(t_{ij},\beta_{ij}) \leq  \hat\lambda_{ij}(\beta_{ij}^+) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})> \beta_{ij}] & \forall i,j,\beta_{ij}\in \cV_{ij}\\
    %&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad+\hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq\beta_{ij}]\\
    & \quad\MarginalToGlobalConstraint\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \left(\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})+ \lambda_{ij}(t_{ij},\beta_{ij}^+,\delta_{ij})\right) \leq \\
    &\qquad\qquad\qquad\hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}]+\hat\lambda_{ij}(\beta_{ij}^+,\delta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq\beta_{ij}^+] & \forall i,j,\beta_{ij}\in \cV_{ij}^0,\delta_{ij}\in \Delta\\
    %& \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) &\forall i\in[n], j \in[m] \\
    &\quad\BoundMeanDeltaConstraint\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\ \delta_{ij} \in \Delta}} \delta_{ij}\cdot \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \leq d_i  & \forall i,j\\
    &\quad\BoundSumDeltaConstraint\quad\sum_{i\in[n]} d_i \leq %\yangnote{16}\cdot \prev \\
    {111\cdot \estprev}\\
     & \lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}(\beta_{ij},\delta_{ij})\geq 0,\pi_{ij}(t_{ij})\geq 0, w_{ij}(t_{ij})\geq 0, d_i\geq 0 & \forall i,j,t_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}
\end{align*}
\end{minipage}}
\caption{LP for XOS Valuations }~\label{fig:XOSLP}
\end{figure}

The LP for XOS valuations can be found in \Cref{fig:XOSLP}. Here $V_{ij}^0=\{V_{ij}(t_{ij}):t_{ij}\in \cT_{ij}\}$, $\cV_{ij}^+ = \{V_{ij}(t_{ij}) + \eps_r: t_{ij} \in \cT_{ij}\}$ and $\cV_{ij} = \cV^0_{ij} \cup \cV^+_{ij}$. We notice that this is consistent with our LP for constrained-additive buyers (\Cref{fig:bigLP}), as $V_{ij}(t_{ij})=t_{ij}$ for constrained-additive buyers.

%\todo{Argue that $W$ is a polytope}
%Note that $W$ is the convex hull of finite many deterministic allocation rules and deterministic choice of the activated additive function.
%Thus $W$ is a convex polytope.
%\todo{We have to argue that when the function is XOS we really have polytopes? I think it is enough to note that this is true, since we have finite many types and finite many possible allocations.}





Denote $\optlp$ the optimum objective of the LP in \Cref{fig:XOSLP}. Similar to the constrained-additive case, we have the following lemma.

\begin{lemma}\label{lem:bound rev by opt-XOS}
%For sufficiently small $\varepsilon_r$ \todo{fix the value $\varepsilon_r$} and 
When buyers have XOS valuations, for any BIC and IR mechanism $\cM$, $\rev(\cM)\leq 28\cdot \prev+4\cdot\optlp$.
\end{lemma}



\subsection{Proof of \Cref{lem:bound rev by opt} and \Cref{lem:bound rev by opt-XOS}}\label{subsec:proof_lem:bound rev by opt}

\begin{proof}
{The proof is stated for XOS buyers, whose LP contains a new set of variables $\pi$ compared to the LP for constrained-additive buyers. When the buyers have constrained-additive valuations, we can simply treat $\pi$ to be the same as $w$. Also, note that $V_{ij}(t_{ij})=t_{ij}$ for constrained-additive valuations.} 

Let tuple $(\hat{\sigma},\tilde{\vBeta},\vC,\vr)$ be the one stated in Lemma~\ref{lem:caiz17} for $\cM$. Consider the following choice of variables of the LP in \Cref{fig:bigLP} (or \Cref{fig:XOSLP}). For every $i,j,t_{ij}$, let 

$$w_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{iS}(t_{ij},t_{i,-j})$$
if the buyers' have constrained-additive valuations. Let
$$\pi_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{iS}(t_{ij},t_{i,-j})$$
$$w_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{iS}(t_{ij},t_{i,-j})\cdot\frac{\gamma_{ij}^{S}(t_i)}{V_{ij}(t_{ij})}.$$ 
%\argyrisnote{Should we say something about $\gamma_{ij}^S(\cdot)$? Like that they are $1$-supporting prices? fix: where $\gamma_{ij}^S(t_i)$ is equal to $\alpha_{ij}^{k(t_i,S)}(t_{ij})$, where $k(t_i,S)=\arg\max_{k\in[K]}\left(\sum_{j\in S}\alpha^k_{ij}(t_{ij}) \right)$.}
if the buyers' have XOS valuation.
For each $c_i$, we notice that by \Cref{lem:caiz17} and \Cref{thm:chms10}, $0\leq c_i\leq 8\cdot \prev\leq 55\cdot\estprev$ when $n\geq 110$. We round it up to the closest number in $\Delta$, and we denote it using $\hat{c}_i$. Clearly, $$\core(\sigma,\tilde{\vBeta},\vC,\vr)\leq \core(\sigma,\tilde{\vBeta},\hat{\vC},\vr).$$

 $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$ and $\hat\lambda_{ij}(\beta_{ij},\delta_{ij})$ can be set to non-zero only if $\beta_{ij}\in\{\tilde{\beta}_{ij}, \tilde{\beta}_{ij}^+\}$ and $\delta_{ij}=\hat{c}_i$.
More specifically, we choose the variables as follows.  \begin{itemize}
    \item $\lambda_{ij}(t_{ij},\tilde{\beta}_{ij},c_i):= r_{ij}\cdot w_{ij}(t_{ij})/f_{ij}(t_{ij})$, 
    \item $\lambda_{ij}(t_{ij},\tilde{\beta}_{ij}^+,c_i):= (1-r_{ij})\cdot w_{ij}(t_{ij})/f_{ij}(t_{ij})$,
    \item $\hat\lambda_{ij}(\tilde{\beta}_{ij},c_i)=r_{ij}$,
    \item $\hat\lambda_{ij}(\tilde{\beta}_{ij}^+,c_i)=1-r_{ij}$;
    \item $d_i=\hat{c}_i$.
\end{itemize}
%$\lambda_{ij}(t_{ij},\tilde{\beta}_{ij}^+,c_i):= (1-r)\cdot w_{ij}(t_{ij})/f_{ij}(t_{ij})$; $\hat\lambda_{ij}(\tilde{\beta}_{ij},c_i)=r$; $\hat\lambda_{ij}(\tilde{\beta}_{ij}^+,c_i)=1-r$; $d_i=c_i$.
%\argyrisnote{Shouldn't it be $\lambda_{ij}^{(r)}(t_{ij},\tilde{\beta}_{ij},c_i)=r\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}$ and; $\lambda_{ij}^{(n)}(t_{ij},\tilde{\beta}_{ij},c_i)=(1-r)\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}$ and 

%\argyrisnote{whether or not $d_i=c_i$ depends on the discretization we choose, right?}

We show that this is indeed a feasible solution of the LP in \Cref{fig:bigLP} by verifying each constraint. 
%(1) comes directly from the definition of the polytope $W_i$; 
We first prove that $(\pi_i,w_i)\in W_i$ for every $i$. This is clear for constrained-additive valuations. For XOS valuations,  consider the mapping $\sigma_{iS}^{(k)}(t_i)=\hat\sigma_{iS}(t_i)\cdot \ind[k=\argmax_{k'\in [K]}\sum_{j\in S}\alpha_{ij}^{(k')}(t_{ij})]$ for every $t_i$ (we break ties arbitrarily). Thus by the definition of $\gamma_{ij}^S$, we have $\hat\sigma_{iS}(t_i)\cdot \gamma_{ij}^S(t_i)=\sum_{k}\sigma_{iS}^{(k)}(t_i)\cdot \alpha_{ij}^{(k)}(t_i)$. Then clearly $(\pi_i,w_i)$ satisfies all of the conditions in~\Cref{def:W_i}. 

For Constraint~\LambdaMarginalConstraint, LHS equals to $f_{ij}(t_{ij})\cdot \left(\lambda_{ij}(t_{ij},\tilde{\beta}_{ij},c_i)+\lambda_{ij}(t_{ij},\tilde{\beta}^+_{ij},c_i)\right)=w_{ij}(t_{ij})$. Constraint~\PiConstraint~follows from the fact that $\hat{\sigma}$ is a feasible interim allocation rule, and each item $j$ can be allocated to at most one buyer for every type profile. Thus
$$\sum_i\sum_{t_{ij}}\pi_{ij}(t_{ij})=\sum_i\sum_{t_i}f_i(t_i)\sum_{S:j\in S}\hat\sigma_{iS}(t_i)\leq 1$$
%(4) comes from property 1 of \Cref{lem:caiz17}.
By property 1 of \Cref{lem:caiz17} and the choice of $\eps_r$, we have that for every $j$,
\begin{align*}
&\sum_{i\in[n]}\sum_{\beta_{ij} \in \cV_{ij}} \hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}] \\
=&\sum_{i\in[n]}\left(r_{ij}\cdot\Pr_{t_{ij}}[V_{ij}(t_{ij})\geq\tilde\beta_{ij}] + (1-r_{ij})\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq\tilde\beta_{ij}^+] \right)\\
=&\sum_{i\in[n]} \left(\Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde\beta_{ij}]+r_{ij}\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde\beta_{ij}]\right)\leq \frac{1}{2}
\end{align*}
Thus, Constraint~\ReduceDemandConstaint~is satisfied.
For Constraint~\MarginalToGlobalConstraint, we only need to verify the constraint for $\beta_{ij}=\tilde{\beta}_{ij}\in \cV_{ij}^0$.
LHS equals to $\frac{1}{2}\sum_{t_{ij}}w_{ij}(t_{ij})$. %\argyrisnote{Isn't it equal to $\frac{1}{2}\sum_{t_{ij}} w_{ij}(t_{ij})$}. 
We notice that $\gamma_{ij}^S(t_i)\leq V_{ij}(t_{ij})$ for all $i,j,S$ (for XOS valuations). Thus  
$$\sum_{t_{ij}\in \cT_{ij}}w_{ij}(t_{ij})\leq \sum_{t_{ij}\in \cT_{ij}}f_{ij}(t_{ij})\cdot\left( \sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{iS}(t_{ij},t_{i,-j})\right)=\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\hat\sigma_{iS}(t_i)$$

Since $r_{ij}\in [0,1]$ for all $i,j$, by property 2 of \Cref{lem:caiz17} and the choice of $\varepsilon_r$, we have

\begin{align*}
\text{LHS of Constraint~\MarginalToGlobalConstraint} \leq& \frac{1}{2}\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\hat\sigma_{iS}(t_i)=\Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde{\beta}_{ij}]+r_{ij}\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde{\beta}_{ij}] \\
=&\hat\lambda_{ij}(\beta_{ij}^+) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}^+] +\hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq\beta_{ij}]
\end{align*}

For Constraint~\CompareMarginalConstraint, since $\gamma_{ij}^S(t_i)\leq V_{ij}(t_{ij})$ for all $i,j,S$ and $\sum_{S\in [m]}\hat\sigma_{iS}(t_i)\leq 1$, we have $w_{ij}(t_{ij})\leq f_{ij}(t_{ij})$. Thus 
$$\lambda_{ij}(t_{ij},\tilde{\beta}_{ij},c_i)=r_{ij}\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}\leq r_{ij}= \hat\lambda_{ij}(\tilde{\beta}_{ij},c_i).$$ 
and
$$\lambda_{ij}(t_{ij},\tilde{\beta}_{ij}^+,c_i)=(1-r_{ij})\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}\leq 1-r_{ij}= \hat\lambda_{ij}(\tilde{\beta}_{ij}^+,c_i).$$ 
%\argyrisnote{Maybe change it to:
%For (6), since $w_{ij}(t_i)\leq f_{ij}(t_{ij})$ for all $i,j,S$, we have  
%$$\lambda_{ij}^{(r)}(t_{ij},\tilde{\beta}_{ij},c_i)=r\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}\leq r= \hat\lambda_{ij}^{(r)}(\tilde{\beta}_{ij},c_i).$$ }
%Similarly $\lambda_{ij}^{(n)}(t_{ij},\tilde{\beta}_{ij},c_i)\leq 1-r=\hat\lambda_{ij}^{(n)}(\tilde{\beta}_{ij},c_i)$.
Constraint~\BoundMeanDeltaConstraint~and ~\HatLambdaDistributionConstraint~are straightforward since $\hat\lambda_{ij}(\beta_{ij},\delta_i)=r_{ij}\cdot \ind[\beta_{ij}=\tilde{\beta}_{ij}\wedge \delta_{ij}=\hat{c}_i]$,  $\hat\lambda_{ij}(\beta_{ij},\delta_i)=(1-r_{ij})\cdot \ind[\beta_{ij}=\tilde{\beta}^+_{ij}\wedge \delta_{ij}=\hat{c}_i]$, and $d_i=\hat{c}_i$. 
%Lastly, Constraint~\BoundSumDeltaConstraint~follows from property 4 of \Cref{lem:caiz17}. 

Lastly, for Constraint~\BoundSumDeltaConstraint, we notice that for every $i\in [n]$, $\hat{c_i}\leq \max\{\frac{\estprev}{n},2c_i\}$. Thus by property 4 of \Cref{lem:caiz17}, when $n\geq 110$,
$$\sum_{i\in [n]}c_i\leq 2\cdot \sum_{i\in [n]}c_i+\estprev\leq 16\cdot\prev+\estprev\leq 111\cdot\estprev$$

Thus the solution is feasible. We are left to show that the objective of the above solution is at least $\core(\hat{\sigma},\tilde{\vBeta},\hat{\vC},\vr)$. In fact, by the definition of $w_{ij}(t_{ij})$,   

%$$\core(\cM,\tilde{\beta},\vec{c})=\sum_i\sum_j\sum_{t_{ij}}f_{ij}(t_{ij})\cdot w_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot \left(\ind[V_{ij}(t_{ij})< \tilde{\beta_{ij}}+c_i]+r\cdot \ind[V_{ij}(t_{ij})= \tilde{\beta_{ij}}+c_i] \right)$$ 
{
\begin{align*}
\core(\hat{\sigma},\tilde{\vBeta},\hat{\vC},\vr)=&\sum_{i\in[n]}\sum_{j\in[m]}\sum_{t_{ij}\in\cT_{ij}}%f_{ij}(t_{ij})\cdot 
w_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot \left(\ind[V_{ij}(t_{ij})< \tilde{\beta}_{ij}+\hat{c}_i]+r_{ij}\cdot \ind[V_{ij}(t_{ij})= \tilde{\beta}_{ij}+\hat{c}_i] \right)\\
\leq &\sum_i\sum_j\sum_{t_{ij}}%f_{ij}(t_{ij})\cdot
w_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot \ind[V_{ij}(t_{ij})\leq \tilde{\beta}_{ij}+\hat{c}_i].
\end{align*}
%\argyrisnote{I think also $c_i$ might have a rebate? In that case the definition of core might change? I think everything is fine if we double the value of $c_i$. I also think that this is not due to property 3 of \Cref{lem:caiz17}.}

This is exactly the objective of the LP in \Cref{fig:bigLP} 
%if $\varepsilon_r$ is sufficiently small
according to the choice of $\eps_r$, since \begin{align*}
    \lambda_{ij}(t_{ij},\tilde{\beta}_{ij},\delta_{ij})\cdot\ind[V_{ij}(t_{ij})\leq \tilde{\beta}_{ij}+\hat{c}_i]+\lambda_{ij}(t_{ij},\tilde{\beta}^+_{ij},\delta_{ij})\cdot&\ind[V_{ij}(t_{ij})\leq \tilde{\beta}^+_{ij}+\hat{c}_i]\\=&\frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}\cdot \ind[V_{ij}(t_{ij})\leq \tilde{\beta}_{ij}+\hat{c}_i]
\end{align*}
}
%and $\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})=r\cdot w_{ij}(t_{ij})\cdot \ind[\beta_{ij}=\tilde{\beta}_{ij}\wedge \delta_{ij}=c_i]$.
The proof is complete by invoking property 3 of \Cref{lem:caiz17}. 
\end{proof}






\subsection{Bounding the Difference between the Shifted~\core~and the Original~\core}\label{subsec:proof_lem:Q and Q-hat}

We first give the following definition as a generalization of \Cref{def:Q_j}.

\begin{definition}\label{def:Q_j-XOS}
%Given an optimal solution %$\{\lambda_{i,j}(\beta)\}_{\beta \in V_{i,j}(T_{i,j})}$,
%of the program above,
Let $(\pi, w,\lambda,\hat\lambda, \bd=(d_i)_{i\in [n]})$ be any feasible solution of the LP in \Cref{fig:XOSLP}. %For every $j\in [m]$, define 
For every $j\in [m]$, define 
%$$Q_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot %t_{ij}\cdot
%    \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot\ind[t_{ij}\leq \beta_{ij}+\delta_{ij}]
%$$

%For any $i,j,\beta_{ij}\in \cV_{ij},\delta_{ij}\in \Delta_i$, define

%$$g_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})<\beta_{ij} + \delta_{ij}]+\lambda_{ij}^{(r)}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})=\beta_{ij} + \delta_{ij}]$$

%We denote by $B_{i,j} \times \Delta_{i,j}$ a coupled distribution over $V_{i,j}(T_{i,j}) \times \Delta_{i}$ such that: $\Pr_{(\beta,\delta) \sim B_{i,j} \times \Delta_{i,j}}[\beta = a \land \delta = b]= \lambda'_{i,j}(\beta_{i,j}=a, \delta_{i,j} = b)$.


%For XOS buyers, let $(\pi, w,\lambda,\hat\lambda, \bd=(d_i)_{i\in [n]})$ be any feasible solution of the LP in \Cref{fig:XOSLP}. 

$$Q_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot\ind[V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}].
$$
\end{definition}



Recall that by Constraint \HatLambdaDistributionConstraint, for every $i,j$, $\hat\lambda_{ij}(\cdot,\cdot)$ can be viewed as a joint distribution $\cC_{ij}$ over $\cV_{ij}\times \Delta$, i.e. $\Pr_{(\beta_{ij},\delta_{ij}) \sim \cC_{ij}}[\beta_{ij} = a \land \delta_{ij} = b]= \hat\lambda_{ij}(\beta_{ij}=a, \delta_{ij} = b)$. Denote $\cB_{ij}$ the marginal distribution of $\beta_{ij}$ with respect to $\cC_{ij}$. Inspired by the ``shifted core'' technique by Cai and Zhao~\cite{CaiZ17}, we need further definitions to describe the welfare contribution by each item under a smaller threshold.  

\begin{definition}\label{def:hatQ_j}
For every $i\in [n]$, define\footnote{\label{fn:tau_i}If all $D_{ij}$s are continuous, then for every $i$ there exists $\tau_i$ that satisfies the following property:\\ $\sum_{j\in[m]} \Pr_{t_{ij}\sim D_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j + x)]\leq \frac{1}{2}$ and the inequality is achieved as equality for all $\tau_i>0$. However, this property might not be satisfied for discrete distributions. This is again a tie-breaking issue addressed in \Cref{remark:tie-breaking}. We refer the readers to Lemma 5 of \cite{CaiZ17} for a fix. For simplicity, in our proof we will assume that all $\tau_i$s satisfy the property mentioned above.  
%Instead of having a deterministic $\tau_i$, one can think of it as a randomization between $\tau_i$ and $\tau_i+\eps_i$ for some small $\eps_i>0$.  
} 
%$\tau_i\geq 0$ such that
$$\tau_i = \inf_{x\geq 0}\left\{ \sum_{j\in[m]} \Pr_{t_{ij}\sim D_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j + x)]\leq \frac{1}{2}\right\}$$
%$$\sum_{j\in[m]} \Pr_{t_{ij}\sim \cD_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j + \tau_i)]= \frac{1}{2}$$

%\argyrisnote{or maybe we could use the following definition since we are dealing with a discrete distribution (I don't think its nessessary though):}
%$$\tau_i = \inf_{x\in \cup_{j\in[m]} \{V_{i,j}(T_{i,j}\}} \sum_{j\in[m]} \Pr_{t_{i,j}\sim D_{i,j},\beta \sim B_{i,j}}[V_{i,j}(t_{i,j}) \geq \max(\beta, Q_j + x)]\leq \frac{1}{2}$$

Then for every $j\in [m]$, define
$$\hat Q_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot \ind[V_{ij}(t_{ij})\leq \min\{\beta_{ij}+\delta_{ij},Q_j+\tau_i\}]$$
\end{definition}
%\argyrisnote{Should't it be $\inf_{\tau\geq 0}\sum_{j\in[m]} \Pr_{t_{ij}\sim \cD_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j + \tau_i)] \leq \frac{1}{2}$? It could be the case that  that $\sum_{j\in[m]} \Pr_{t_{ij}\sim \cD_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j)]< \frac{1}{2}$}
%\mingfeinote{I changed the definition.}

We prove in \Cref{lem:Q and Q-hat_main body} that the difference between $\sum_{j\in[m]} Q_j$ and $\sum_{j\in[m]} \hat{Q}_j$ can be bounded using $\prev$. %The proof is postponed to \Cref{subsec:proof_lem:Q and Q-hat}.

\begin{lemma}\label{lem:Q and Q-hat_main body}
For every $j\in [m]$, $Q_j\geq \hat{Q}_j$. Moreover, there exists some absolute constant $c>0$ such that
$$\sum_{j\in [m]}Q_j\leq \sum_{j\in [m]}\hat{Q}_j+c\cdot \prev$$
\end{lemma}



To prove \Cref{lem:Q and Q-hat_main body}, we consider the following variant of the RPP mechanism, where the posted prices are allowed to be randomized. 

\paragraph{Rationed Randomized Posted Price Mechanism (RRPP).} Before the auction starts, the seller first draws a posted price $p_{ij}$ from some distribution $\cG_{ij}$, for every buyer $i$ and item $j$. All $\cG_{ij}$s are independent.
%There is a price $p_{ij}$ for bidder $i$ to purchase item $j$. 
The buyers then arrive in some arbitrary order, and each buyer $i$ can purchase \emph{at most one} item among the available ones at the realized posted price $p_{ij}$ for every item $j$.

Clearly any RRPP mechanism is also DSIC and IR. We notice that any RRPP mechanism can be viewed as a distribution of RPP mechanisms, as the seller can draw all the posted prices before the auction starts, and use the realized (and deterministic) set of posted prices to sell the items. Thus the highest revenue achievable among all RRPP mechanisms is the same as the optimum revenue among all RPP mechanisms, which is $\prev$. 

Before giving the proof of \Cref{lem:Q and Q-hat_main body}, we first prove a useful lemma that analyzes the revenue of RRPP. It's a generalization of Lemma 17 of \cite{CaiZ17}, which allows randomized posted prices.  

\begin{lemma}\label{lem:prev-useful}\cite{CaiZ17}
%For every $i,j$, let $\cG_{ij}$ be a joint distribution over $\cV_{ij}\times \mathbb{R}_+$, whose marginal distribution on $\beta_{ij}\in \cV_{ij}$ is $\cB_{ij}$. In other words, $\Pr_{(\beta_{ij},x_{ij})\sim \cG_{ij}}[\beta_{ij}=b]=\Pr_{\beta_{ij}\sim \cB_{ij}}[\beta_{ij}=b]$ for every $b\in \cV_{ij}$.
For every $i,j$, let $\cG_{ij}$ be any distribution over $\mathbb{R}_+$. All $\cG_{ij}$'s are independent from each other. Suppose both of the following inequalities hold, for some constant $a,b\in (0,1)$:
\begin{enumerate}
\item $\sum_{i\in [n]} \Pr_{t_{ij}\sim \cD_{ij},x_{ij}\sim \cG_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\leq a,\forall j\in [m]$.
\item
$\sum_{j\in [m]} \Pr_{t_{ij}\sim \cD_{ij},x_{ij}\sim \cG_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\leq b,\forall i\in [n]$.
\end{enumerate}
Then
\begin{equation*}
\sum_{i\in [n]}\sum_{j\in[m]} \E_{x_{ij}\sim \cG_{ij}}\left[x_{ij}\cdot \Pr_{t_{ij}\sim \cD_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\right]\leq \frac{1}{(1-a)(1-b)}\cdot \prev.
\end{equation*}
\end{lemma}

\begin{proof}
Consider an RRPP that sells item $j$ to buyer $i$ at price $x_{ij}\sim \cG_{ij}$. The mechanism
visits the buyers in some arbitrary order. For every $i,j$ and every realized $x_{ij}$, we will bound the probability of buyer $i$ purchasing item $j$, over the randomness of $\{\cD_{i'j'}\}_{i'\in[n],j'\in[m]}$ and $\{\cG_{i'j'}\}_{(i',j')\neq (i,j)}$. 
Notice that when it is buyer $i$'s turn, she purchases exactly item $j$ and pays $x_{ij}$ if all of the following three conditions hold: (i) $j$ is still available, (ii) $V_i(t_{ij})\geq x_{ij}$ and (iii) $\forall k\neq j, V_i(t_{ik})< x_{ik}$. The second condition means buyer $i$ can afford item $j$. The third condition means she cannot afford any other item $k\neq j$. Therefore, buyer $i$ purchases exactly item $j$.

Now let us compute the probability that all three conditions hold, when $t_{ij}\sim \cD_{ij}$ and $x_{ij}\sim \cG_{ij}$ for all $i,j$. Since every buyer's valuation is subadditive over the items, item $j$ is purchased by someone else only if there exists a buyer $k\neq i$ who has $V_k(t_{kj})\geq x_{kj}$. %Because $x_{kj}\geq 0$ for all $k$, 
By the union bound, the event described above happens with probability at most $\sum_{k\neq i} \Pr_{t_{kj},x_{kj}}\left[V_k(t_{kj})\geq x_{kj}\right]$, which is less than $a$ by Inequality 1 of the statement. Therefore, condition (i) holds with probability at least $1-a$. Clearly, condition (ii) holds with probability $\Pr_{t_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]$. Finally, condition (iii) holds with at least probability $1-b$, because the probability that there exists any item $k\neq j$ such that $V_i(t_{ik})\geq x_{ik}$ is no more than $\sum_{k\neq j}\Pr_{t_{ik},x_{ik}}[V_i(t_{ik})\geq x_{ik}]\leq b$ (Inequality 2 of the statement). Since the three conditions are independent, buyer $i$ purchases exactly item $j$ with probability at least $(1-a)(1-b)\cdot \Pr_{t_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]$. So the expected revenue of this mechanism is at least $(1-a)(1-b)\cdot \E_{x_{ij}\sim \cG_{ij}}\left[x_{ij}\cdot \Pr_{t_{ij}\sim \cD_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\right]$.
\end{proof}

A direct corollary of \Cref{lem:prev-useful} is that $\sum_i \tau_i$ can be bounded using $\prev$.

\begin{lemma}\label{lem:bounding tau_i}
$\sum_{i\in[n]} \tau_i\leq 8\cdot \prev$.
\end{lemma}
\begin{proof}
By Constraint \ReduceDemandConstaint~of the LP in \Cref{fig:bigLP} (or \Cref{fig:XOSLP}), for every item $j$,%\argyrisnote{(4) you mean?} 
\begin{align*}
    \sum_{i\in [n]}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)] &\leq \sum_{i\in [n]}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij})\geq \beta_{ij}]\\
    &=\sum_{i\in [n]}\sum_{\beta_{ij}\in \cV_{ij}}\hat\lambda_{ij}(\beta_{ij})\Pr_{t_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}]\leq \frac{1}{2}
\end{align*}
%\argyrisnote{I think there is one extra ]}


By the definition of $\tau_i$, for every $i$ we have
$$\sum_{j\in [m]}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]\leq\frac{1}{2}.$$
%\argyrisnote{I think it should be $\leq$? Either $\tau_i=0$ or $\sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]=\frac{1}{2}$, right? So the following statement still holds.}

Thus by \Cref{lem:prev-useful}, 
\begin{align*}
4\cdot \prev\geq& \sum_{i\in[n],j\in[m]} 
\E_{\beta_{ij}\sim\cB_{ij}}\left[\max(\beta_{ij}, Q_j+\tau_i)\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\right]\\
\geq & \sum_{i\in[n]}\tau_i\sum_{j\in[m]}\E_{\beta_{ij}\sim\cB_{ij}}\left[\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\right]\\
=&\frac{1}{2}\sum_{i\in[n]} \tau_i,
\end{align*}
{The last equality comes from the fact that by the definition of $\tau_i$, $\sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]=\frac{1}{2}$ for all $i$ such that $\tau_i>0$ (see \Cref{fn:tau_i}). We finish the proof.} %\yangnote{This is only true for continuous distribution.}
\end{proof}



\begin{lemma}\label{lem:Q and Q-hat}[(Restatement of \Cref{lem:Q and Q-hat_main body})]
%For sufficiently small $\varepsilon_r$ \todo{fix $\epsilon_r$} and 
For every $j\in [m]$, $Q_j\geq \hat{Q}_j$. 
%Moreover, there exists a \mingfeinote{restricted SPEM} $\cM$ such that
%$$\sum_{j\in [m]}Q_j\leq \sum_{j\in [m]}\hat{Q}_j+44\cdot \prev+8\cdot\rev(\cM) + \epsilon_r\cdot |\cV_{ij}^0|.$$
%$\cM$ can be computed in time \mingfeinote{Add time and query complexity}.
%\argyrisnote{Work In Progress}
Moreover,
$$\sum_{j\in [m]}Q_j\leq \sum_{j\in [m]}\hat{Q}_j+236.5\cdot \prev$$ %\varepsilon_r\cdot \sum_{i\in[n],j\in[m]}|\cV_{ij}^0|.$$
\end{lemma}

\begin{proof}

For every $j$, it's clear that $\hat{Q}_j\leq Q_j$ by the definition of $\hat{Q}_j$. It remains to bound $\sum_j(Q_j-\hat{Q}_j)$. In the proof, we abuse the notation and let $\hat\lambda_{ij}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta}\hat\lambda_{ij}(\beta_{ij},\delta_{ij})$. Also for every $i,j,t_{ij},\beta_{ij}\in \cV_{ij}$, let $\lambda_{ij}(t_{ij},\beta_{ij})=\sum_{\delta_{ij}\in \Delta}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$.

\begin{align*}
    &2\sum_{j\in [m]} \left(Q_j - \hat{Q}_j \right) \\
    \leq & \sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) V_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\
    \delta_{ij} \in \Delta}} \lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}] \\
    \leq & \sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\
    \delta_{ij} \in \Delta}} \left(\beta_{ij}+(V_{ij}(t_{ij})-\beta_{ij})^+\right)\cdot\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\\
    \leq & \sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\beta_{ij}\in \cV_{ij}} \beta_{ij}\cdot\lambda_{ij}(t_{ij},\beta_{ij})\\
    &+\sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\
    \delta_{ij} \in \Delta}} (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\\
\end{align*}

%\argyrisnote{In the continuous setting we don't use $g_{ij}(t_{ij},\beta_{ij},\delta_{ij})$, right?}
Here the first inequality uses the fact that $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot \ind[V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}]$ and\\ $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\ind[V_{ij}(t_{ij})\leq \min\{\beta_{ij}+\delta_{ij},Q_j+\tau_i\}]$ can differ only when $V_{ij}(t_{ij})>Q_j+\tau_i \wedge V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}$. In the last inequality, we drop the indicator $\ind[V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}]$ for the first term. %Here we abuse the notation and use $\lambda_{ij}(t_{ij},\beta_{ij})=\sum_{\delta_{ij}\in \Delta}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$ for all $t_{ij},\beta_{ij}$.


We bound the first term:
\notshow{
\begin{equation}\label{inequ:Q and Q_hat-term1}
\begin{aligned}
&\sum_{j} \sum_{i}  \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot \sum_{\beta_{ij}\in \cV_{ij}} \beta_{ij} \cdot \lambda_{ij}(t_{ij},\beta_{ij})\\
%=&\sum_{j\in[m]} \sum_{i\in[n]} 
%\sum_{\beta\in V_{i,j}(T_{i,j}) } %\beta
%\sum_{\substack{t_{i,j}\in T_{i,j}:\\V_{i,j}(t_{i,j}) \geq Q_j^*+\tau_i}}  f_i(t_{i,j})  \cdot \lambda_{i,j}(t_{i,j},\beta)\\
= & \sum_{i,j} \sum_{\beta_{ij}\leq Q_j+\tau_i} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})
+
\sum_{i,j}\sum_{\beta_{ij}> Q_j+\tau_i} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})\\
\leq &\sum_{i,j}
\sum_{\beta_{ij}\leq Q_j + \tau_i} \hat\lambda_{ij}(\beta_{ij}) \cdot \beta_{ij}
\sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})
+ 
\sum_{i,j}
\sum_{\beta_{ij} > Q_j + \tau_i} 
2\hat\lambda_{ij}(\beta_{ij})\cdot\beta_{ij}\cdot\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \beta_{ij}]\\
\leq & 2\sum_{i,j} 
\sum_{\beta_{ij}\in \cV_{ij}} \hat\lambda_{ij}(\beta_{ij}) \cdot \beta_{ij}\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\\
= & 2\sum_{i,j} 
\E_{\beta_{ij}\sim \cB_{ij}}\left[  \beta_{ij}\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\right]\\
\leq & 8\cdot\prev
\end{aligned}
\end{equation}
}

\begin{equation}\label{inequ:Q and Q_hat-term1}
\begin{aligned}
&\sum_{j} \sum_{i}  \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot \sum_{\beta_{ij}\in \cV_{ij}} \beta_{ij} \cdot \lambda_{ij}(t_{ij},\beta_{ij})\\
%=&\sum_{j\in[m]} \sum_{i\in[n]} 
%\sum_{\beta\in V_{i,j}(T_{i,j}) } %\beta
%\sum_{\substack{t_{i,j}\in T_{i,j}:\\V_{i,j}(t_{i,j}) \geq Q_j^*+\tau_i}}  f_i(t_{i,j})  \cdot \lambda_{i,j}(t_{i,j},\beta)\\
= & \sum_{i,j} \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\beta_{ij} < Q_j+\tau_i}} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})
+
\sum_{i,j}\sum_{\substack{\beta_{ij}\in \cV_{ij}\\\beta_{ij}\geq Q_j+\tau_i}} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})\\
%= & \sum_{i,j} \sum_{\substack{\beta_{ij}\in \cV_{ij}\cup\cV_{ij}^+\\\beta_{ij} < Q_j+\tau_i}} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})
%+
%\sum_{i,j}\sum_{\substack{\beta_{ij}\in \cV_{ij}\cup\cV_{ij}^+\\\beta_{ij}\geq Q_j+\tau_i}} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})\\
\leq & \sum_{i,j} \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\beta_{ij} < Q_j+\tau_i}} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})
\\
& \qquad\qquad\qquad\qquad + 
\sum_{i,j}\sum_{\substack{\beta_{ij}\in \cV_{ij}^0\\\beta_{ij}\geq Q_j+\tau_i}} \beta_{ij}^+ \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \left(\lambda_{ij}(t_{ij},\beta_{ij})+\lambda_{ij}(t_{ij},\beta_{ij}^+)\right)\\
\leq &\sum_{i,j}
\sum_{\substack{\beta_{ij}\in \cV_{ij}\\\beta_{ij} < Q_j + \tau_i} } \hat\lambda_{ij}(\beta_{ij}) \cdot \beta_{ij}
\sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})
+ 
\sum_{i,j}
\sum_{\substack{\beta_{ij}\in \cV_{ij}^0\\\beta_{ij} \geq Q_j + \tau_i} }
2\hat\lambda_{ij}(\beta_{ij})\cdot\beta_{ij}^+\cdot\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \beta_{ij}]\\
& \qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad + 
\sum_{i,j}
\sum_{\substack{\beta_{ij}\in \cV_{ij}^+\\\beta_{ij} \geq Q_j + \tau_i} }
2\hat\lambda_{ij}(\beta_{ij})\cdot\beta_{ij}\cdot\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \beta_{ij}] \\
\leq &\sum_{i,j}
\sum_{\substack{\beta_{ij}\in \cV_{ij}\\\beta_{ij} < Q_j + \tau_i} } \hat\lambda_{ij}(\beta_{ij}) \cdot \beta_{ij}
\sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})
+ 
\sum_{i,j}\left(
\sum_{\substack{\beta_{ij}\in \cV_{ij}\\\beta_{ij} \geq Q_j + \tau_i} }
2\hat\lambda_{ij}(\beta_{ij})\cdot\beta_{ij}\cdot\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \beta_{ij}] + \varepsilon_r |\cV_{ij}^0|\right)\\
\leq & 2\sum_{i,j} 
\sum_{\beta_{ij}\in \cV_{ij}} \hat\lambda_{ij}(\beta_{ij}) \cdot \beta_{ij}\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)] + \varepsilon_r\cdot \sum_{i,j}|\cV_{ij}^0|\\
= & 2\sum_{i,j} 
\E_{\beta_{ij}\sim \cB_{ij}}\left[  \beta_{ij}\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\right]+ \varepsilon_r\cdot \sum_{i,j}|\cV_{ij}^0|\\
\leq & 8\cdot\prev+ \varepsilon_r\cdot \sum_{i,j}|\cV_{ij}^0|\\
\leq & 9\cdot \prev
\end{aligned}
\end{equation}


The first inequality comes from the fact that for $\beta_{ij}\in \cV_{ij}^0$,
then $\beta_{ij} < \beta_{ij}^+$ and from the fact that for sufficiently small $\varepsilon_r>0$,
then $Q_j + \tau_i\leq\beta_{ij}$ iff $Q_j + \tau_i\leq\beta_{ij}^+$. The second inequality comes from Constraint~\CompareMarginalConstraint~and  \MarginalToGlobalConstraint~of the LP in \Cref{fig:bigLP} (or \Cref{fig:XOSLP}).\footnote{\label{fn:constraint 7}Note that this is the only place that Constraint~\MarginalToGlobalConstraint~is used in our proof.}
For the second last inequality, notice that by Constraint \ReduceDemandConstaint~of the LP in \Cref{fig:bigLP} (or \Cref{fig:XOSLP}), for every item $j$, 
\begin{align*}
    \sum_{i}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]&\leq \sum_{i}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij})\geq \beta_{ij}]\\
    &=\sum_{i}\sum_{\beta_{ij}\in\cV_{ij}}\hat\lambda_{ij}(\beta_{ij})\Pr_{t_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}]\leq \frac{1}{2}
\end{align*}

By the definition of $\tau_i$, for every buyer $i$ we have
$$\sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]\leq\frac{1}{2}$$

The second last inequality then follows from \Cref{lem:prev-useful}. The last inequality follows from the fact that $\eps_r\leq \frac{\prev}{\sum_{i,j}|\cV_{ij}^0|}$.
For the second term, we have

\begin{align*}
&\sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\\
\leq & \sum_{j} \sum_{i} \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} \hat\lambda_{ij}(\beta_{ij}, \delta_{ij})\cdot\sum_{t_{ij}} f_{ij}(t_{ij})  (V_{ij}(t_{ij})-\beta_{ij})\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij} \wedge V_{ij}(t_{ij})\geq \max(\beta_{ij}, Q_j + \tau_i)]\\
= & \sum_{i,j}\E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}}\left[\sum_{t_{ij}}f_{ij}(t_{ij})u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right],
\end{align*}

where
$$u_{ij}(t_{ij},\beta_{ij},\delta_{ij})=(V_{ij}(t_{ij})-\beta_{ij})\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij} \wedge V_{ij}(t_{ij})\geq \max(\beta_{ij}, Q_j + \tau_i)]$$

We notice that by the definition of $\tau_i$, the following inequality holds for every buyer $i$.

\begin{equation}\label{inequ:Q and Q_hat-1} 
\sum_j\Pr_{t_{ij}\sim D_{ij},(\beta_{ij},\delta_{ij})\sim \cC_{ij}}[u_{ij}(t_{ij},\beta_{ij},\delta_{ij})>0]\leq \sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]\leq\frac{1}{2}    
\end{equation}

Denote $\cC_i=\times_{j=1}^m \cC_{ij}$ and $\beta_{i}=(\beta_{ij})_{j\in [m]}, \delta_{i}=(\delta_{ij})_{j\in [m]}$, we have  
\begin{align*}
    &\sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_{t_i}f_i(t_i)\cdot\max_j u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]\\
\geq & \sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_j\sum_{t_{ij}}f_{ij}(t_{ij})\cdot u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot \prod_{k\not=j}\Pr_{t_{ik}\sim D_{ik}}[u_{ik}(t_{ik},\beta_{ik},\delta_{ik})=0]\right]\\
=&\sum_{i}\sum_j\E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}}\left[\sum_{t_{ij}}f_{ij}(t_{ij})\cdot u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot \prod_{k\not=j}\Pr_{t_{ik}\sim D_{ik},(\beta_{ik},\delta_{ik})\sim \cC_{ik}}[u_{ik}(t_{ik},\beta_{ik},\delta_{ik})=0]\right]\\
\geq & \frac{1}{2}\cdot \sum_{i,j}\E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}}\left[\sum_{t_{ij}}f_{ij}(t_{ij})u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]
\end{align*}

Here the equality uses the fact that all $\cC_{ij}$'s are independent. The last inequality comes from Inequality~\eqref{inequ:Q and Q_hat-1} and the union bound. Now the second term is bounded by \begin{align*}
& 2\cdot \sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_{t_i}f_i(t_i)\cdot\max_j u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]\\
\leq & 2\cdot \sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_{t_i}f_i(t_i)\cdot\max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]
\end{align*}

\begin{definition}
For every $i,j,t_i\in \cT_i, S\subseteq [m]$, let 
$$\eta_i(t_i,S)=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]$$

\notshow{For every $i,j,t_i\in \cT_i,\beta_i\in \times_j\cV_{ij}, S\subseteq [m]$, let 
$$\eta_i(t_i,\beta_i,S)=\E_{\delta_i}\left[\max_{j\in S}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]$$
}

\end{definition}


\noindent Therefore, we can rewrite $2\cdot \sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_{t_i}f_i(t_i)\cdot\max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]$ as $\sum_i\sum_{t_i} f_i(t_i)\cdot \eta(t_i,[m])$.


\begin{definition}\label{def:Lipschitz}
A function $v(\cdot,\cdot)$ is \textbf{$a$-Lipschitz} if for any type $t,t'\in T$, and set $X,Y\subseteq [m]$,
$$\left|v(t,X)-v(t',Y)\right|\leq a\cdot \left(\left|X\Delta Y\right|+\left|\{j\in X\cap Y:t_j\not=t_j'\}\right|\right),$$ where $X\Delta Y=\left(X\setminus Y\right)\cup \left(Y\setminus X\right)$ is the symmetric difference between $X$ and $Y$.
\end{definition}


\begin{lemma}\label{lem:eta-lipschitz}
For every $i$, $\eta_i(\cdot, \cdot)$ is subadditive over independent items and $d_i$-Lipschitz. Note that $d_i$ is the variable in the LP in \Cref{fig:bigLP}.
%\mingfeinote{For every $i,t_i,\beta_i,\delta_i$, $\eta_i(t_i,\beta_i,\delta_i,\cdot)$ is monotone, subadditive, has no externalities, and it's $\delta_i$-Lipschitz.}
\end{lemma}

\begin{proof}

For every $i,j,t_{ij},\beta_{ij},\delta_{ij}$, denote $h_{ij}(t_{ij},\beta_{ij},\delta_{ij})=(V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]$.

We will first verify that for each $t_i\in T_i$, $\eta_i(t_i,\cdot)$ is monotone, subadditive and has no externalities.

Monotonicity: Let $S_1\subseteq S_2 \subseteq [m]$.
Then:
\begin{align*}
\eta_i(t_i,S_1)=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_1}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right] 
\leq  \E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_2}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right]
=  \eta_i(t_i,S_2)
\end{align*}

Subadditivity: For any set $S_1,S_2,S_3\subseteq [m]$ such that $S_1 \cup S_2 = S_3$,
it holds that:
\begin{align*}
\eta_i(t_i,S_3)&=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_3}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right] \\
&\leq\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\bigg[\max_{j\in S_1}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} + \max_{j\in S_2}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\bigg] \\
&=\eta_i(t_i,S_1) + \eta_i(t_i,S_2)
\end{align*}
The first inequality follows because $S_1\cup S_2=S_3$.

No externalities: for every $S\subseteq [m]$ and $t_i,t_i'\in \cT_i$ such that $t_{ij}=t_{ij}'$ for every $j\in S$, we have
$$\eta_i(t_i,S)=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right]=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S}\left\{ h_{ij}(t_{ij}',\beta_{ij},\delta_{ij})\right\}\right]=\eta_i(t_i',S)$$

Now we are going to prove that $\eta_i(\cdot,\cdot)$ is $d_i$-Lipschitz.
For $t_i,t_i'\in \cT_i$ and $X,Y \subseteq[m]$,
let $Z = \{j \in X\cap Y \land t_{ij}=t_{ij}'\}$.
It is enough to show that:
\begin{align*}
\eta_i(t_i,X) - \eta_i(t_i',Y) \leq {\left(|X\setminus Y|+(|X\cap Y|-|Z|)\right)\cdot d_i}= {(|X|-|Z|)\cdot d_i}\\ %(m-|Z|)\cdot d_i \\
\eta_i(t'_i,Y) - \eta_i(t_i,X) \leq {\left(|Y\setminus X|+(|X\cap Y|-|Z|)\right)\cdot d_i}={(|Y|-|Z|)\cdot d_i}%(m-|Z|)\cdot d_i
\end{align*}

We are only going to show $\eta_i(t_i,X) - \eta_i(t_i',Y) \leq  {(|X|-|Z|)\cdot d_i} %(m-|Z|)\cdot d_i 
$,
since the other case is similar.
Because $\eta_i(t_i,\cdot)$ is monotone, it suffices to prove that:
$$
\eta_i(t_i,X) - \eta_i(t_i',Y) \leq \eta_i(t_i,X) - \eta_i(t_i',Z) \leq  {(|X|-|Z|)\cdot d_i } %(m-|Z|)\cdot d_i 
$$
For each $j \in Z$, $t_{ij} =t_{ij}'$, which implies that $\eta_i(t_i',Z) = \eta_i(t_i,Z)$.
Note that:
\begin{align*}
&\eta_i(t_i,X) - \eta_i(t_i',Z)\\ 
= & \eta_i(t_i,X) - \eta_i(t_i,Z)\\
= & \E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\big[\max_{j\in X}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} - \max_{j\in Z}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} \big] \\
\leq & \E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\big[\max_{j\in Z}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} +\sum_{j\in X \backslash Z} h_{ij}(t_{ij},\beta_{ij},\delta_{ij}) - \max_{j\in Z}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} \big] \\
= &  \E_{(\beta_{i},\delta_{i})\sim \cC_{i}} \left[\sum_{j\in X \backslash Z} h_{ij}(t_{ij},\beta_{ij},\delta_{ij}) \right]\\
= &  \sum_{j\in X \backslash Z} \E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}} \left[ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]\\
\leq &  \sum_{j\in X \backslash Z} \E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}} \left[ \delta_{ij} \right]\\
\leq & (|X|-|Z|)d_i %\leq (m-|Z|)d_i
\end{align*}
Here the second last inequality follows by Constraint \BoundMeanDeltaConstraint~of the LP in \Cref{fig:bigLP} (or \Cref{fig:XOSLP}).
\end{proof}

\begin{lemma}\label{lemma:concentrate}\cite{CaiZ17}
Let $g(t,\cdot)$ with $t\sim D=\prod_j D_j$ be a function drawn from a distribution that is  subadditive over independent items of ground set $I$. If $g(\cdot,\cdot)$ is $c$-Lipschitz, then if we let $a$ be the median of the value of the grand bundle $g(t,I)$, i.e. $a=\inf\left\{x\geq 0: \Pr_t[g(t,I)\leq x]\geq \frac{1}{2}\right\}$,
$$\mathds{E}_t[g(t,I)]\leq 2a+\frac{5c}{2}.$$
\end{lemma}

%\todo{Add definition of subadditive over independent items. Also, define $c$-Lipschitz.}

To finish the proof of \Cref{lem:Q and Q-hat}, we will bound $\sum_i\sum_{t_i}f_i(t_i)\cdot \eta_i(t_i,[m])$ using a modified two-part tariff mechanism. 
%by the revenue of some restricted SPEM. 
Consider the following variant of two-part tariff $\cM$, with a randomized posted price $\beta_{ij}\sim \cB_{ij}$ for buyer $i$ and item $j$, and restricting the buyer to purchase at most one item. The procedure of the mechanism is shown in Mechanism~\ref{mech:variant-tpt}~\footnote{The result holds for any buyers' order, we choose the lexicographical order to keep the notation light.}.

\begin{algorithm}[ht]
\floatname{algorithm}{Mechanism}
%\setstretch{1.35}
%\vspace{.1in}
\begin{algorithmic}[1]
\setcounter{ALG@line}{-1}
\State Before the mechanism starts, the seller determines a \textbf{distribution} of posted price $\cB_{ij}$ for every buyer $i$ and item $j$. Recall that $\cB_{ij}$ is the marginal distribution of $\beta_{ij}$. 
\State Bidders arrive sequentially in the lexicographical order.
\State When every buyer $i$ arrives, the seller shows her the set of available items $S_i(t_{<i},\beta_{<i})\subseteq [m]$ (see the remark below), as well as the \emph{distribution} of the posted prices $\{\cB_{ij}\}_{j\in [m]}$. %Note that $S_i(t_{<i})$ is the set of items that are not purchased by the first $i-1$ buyers, which depends on $t_{<i}$. Let $S_1(t_{<1})=[m]$.
\State Buyer $i$ is asked to pay an \emph{entry fee} defined as follows:

\centerline{$\xi_i(S_i(t_{<i},\beta_{<i}))=\Med_{t_i\sim D_i}\{\eta_i(t_i,S_i(t_{<i},\beta_{<i}))\}$.} \noindent Here $\Med_x[h(x)]$ denotes the median of a non-negative function $h(x)$ on random variable $x$, i.e.
$\Med_x[h(x)]=\inf\{a\geq 0:\Pr_{x}[h(x)\leq a]\geq\frac{1}{2}\}$.
\State If buyer $i$ (with type $t_i$) agrees to pay the entry fee, then the seller will sample a realized posted price $\beta_{ij}\sim \cB_{ij}$ for every available item $j\in S_i(t_{<i},\beta_{<i})$. The buyer is restricted to purchase \textbf{at most one} item. The buyer then either chooses her favorite item $j^*=\argmax_{j\in S_i(t_{<i},\beta_{<i})}\left(V_{ij}(t_{ij})-\beta_{ij}\right)$, and pays $\beta_{ij^*}$, or leaves with nothing if $V_{ij}(t_{ij})<\beta_{ij},\forall j\in S_i(t_{<i},\beta_{<i})$. If the buyer refuses to pay the entry fee, she gets nothing and pays 0. 
\end{algorithmic}
\caption{{\sf \quad The Rationed Two-part Tariff with Randomized Posted Price $\cM$}}\label{mech:variant-tpt}
\end{algorithm}

\begin{remark}
We notice that in Mechanism~\ref{mech:variant-tpt}, the set of available items when each buyer $i$ comes to the auction, depends on both $t_{<i}$ and the realized prices for the first $i-1$ buyers (denoted by $\beta_{<i}$). Let $S_i(t_{<i},\beta_{<i})$ be the random set of available items when buyer $i$ comes to the auction. Let $S_1(t_{<1},\beta_{<1})=[m]$.
\end{remark} 

It's not hard to see that $\cM$ stated in Mechanism~\ref{mech:variant-tpt} is BIC and IR: When every buyer sees the set of available items and the distribution of posted prices, she can calculate her expected surplus of this set, over the randomness of the posted prices. Then she will accept the entry fee if and only if the expected surplus is at least the entry fee. 


In Mechanism~\ref{mech:variant-tpt}, by union bound, for every item $j$,

$$\Pr[j\in S_i(t_{<i},\beta_{<i})]\geq 1-\sum_{k<i}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}]\geq \frac{1}{2}\quad{\text{ (Due to Constraint~\ReduceDemandConstaint)}}$$
%\argyrisnote{Maybe we should mention that $\Pr_{\beta_{ij}\sim \Beta_{ij}}[t_{ij}\geq \beta_{ij}]$ that }

%Consider the following entry fee function in $\cM$: 
We notice that for every realization of $t_{<i},\beta_{<i}$, after seeing the remaining item set $S_i(t_{<i},\beta_{<i})$, buyer $i$'s expected surplus if she enters the mechanism is:
$$\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_i(t_{<i},\beta_{<i})}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\right\}\right]\geq \eta_i(t_i,S_i(t_{<i},\beta_{<i})).$$

Thus the buyer will accepts the entry fee with probability at least $1/2$. Hence

\begin{equation}\label{inequ:Q and Q_hat-term2}
\begin{aligned}
\rev(\cM) & \geq  \frac{1}{2}\sum_i\E_{t_{<i},\beta_{<i}}[\xi_i(S_i(t_{<i},\beta_{<i}))]\geq \frac{1}{2}\cdot \sum_i(\frac{1}{2}\E_{t_i,t_{<i},\beta_{<i}}[\eta_i(t_i,S_i(t_{<i},\beta_{<i}))]-\frac{5}{4}d_i)\\
 & \geq \frac{1}{2}\cdot \sum_i(\frac{1}{4}\E_{t_i}[\eta_i(t_i,[m])]-\frac{5}{4}d_i) \geq\frac{1}{8}\cdot \sum_i \E_{t_i}[\eta_i(t_i,[m])]-5\cdot \prev 
\end{aligned}
\end{equation}

%\argyrisnote{Is it $\delta$ instead of $\theta$?We lose a factor of $2$ in the second inequality because each item is available with probability at least $\frac{1}{2}$?}
%\mingfeinote{Changed the proof a little. See if you agree now.}

%\argyrisnote{Should we also take expectation over $t_i\sim D_i$ in the first term above?}
%\mingfeinote{In the first term, $\xi_i$ is the $\Med_{t_i}$, the median over $t_i\sim D_i$.}

Here the second inequality is obtained by applying \Cref{lemma:concentrate} to function $\eta_i(t_i,\cdot)$ and ground set $I=S_i(t_{<i},\beta_{<i})$ for every $t_{<i},\beta_{<i}$. The last inequality comes from constraint \BoundSumDeltaConstraint~of the LP in \Cref{fig:bigLP}. The third inequality comes from the following:  

%For every $i,j,t_{ij},\beta_{ij},\delta_{ij}$, denote $h_{ij}(t_{ij},\beta_{ij},\delta_{ij})=(V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]$. Then for every $t_i,\beta_i,\delta_i$,

Fix any $t_i,\beta_i,\delta_i$. Let $j^*=\argmax_{j\in [m]}(V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]$. Then 

%\argyrisnote{You cannot fix $\beta_i,\delta_i$ right? $\eta$ takes expectation over them?} \mingfeinote{$t_i,\beta_i,\delta_i$ are fixed only for the following inequality.}
\begin{align*}
&\E_{t_{<i},\beta_{<i}}\left[\max_{j\in S_i(t_{<i},\beta_{<i})}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]\\
\geq & \E_{t_{<i},\beta_{<i}}\left[\max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\cdot \ind[j^*\in S_i(t_{<i},\beta_{<i})]\right]\\
= & \max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\cdot \Pr_{t_{<i},\beta_{<i}}[j^*\in S_i(t_{<i},\beta_{<i})]\\
\geq & \frac{1}{2}\cdot \max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}
\end{align*}

Taking expectation over $t_i$ and $(\beta_i,\delta_i)\sim \cC_i$ on both sides, we have 
$$\E_{t_i,t_{<i},\beta_{<i}}[\eta_i(t_i,S_i(t_{<i},\beta_{<i}))]\geq \frac{1}{2}\E_{t_i}[\eta_i(t_i,[m])],$$

%By \Cref{lem:eta-lipschitz}, for every $i,t_i$, $\eta_i(t_i,\cdot)$ is an XOS function. Denote $\{a_j\}_{j\in [m]}$ the supporting price of $\eta_i(t_i,\cdot)$ for set $[m]$. Then

%$$\E_{t_{<i},\beta_{<i}}[\eta_i(S_i(t_{<i},\beta_{<i}))]\geq\E_{t_{<i},\beta_{<i}}\left[\sum_{j\in S_i(t_{<i})}a_j\right]=\sum_j a_j\cdot \Pr_{t_{<i},\beta_{<i}}[j\in S_i(t_{<i},\beta_{<i})]\geq \frac{1}{2}\sum_j\theta_j=\frac{1}{2}\eta(t_i,[m])$$
 
which is exactly the third inequality of \eqref{inequ:Q and Q_hat-term2}. By combining Inequalities \eqref{inequ:Q and Q_hat-term1} and \eqref{inequ:Q and Q_hat-term2}, we have
$$2\sum_j(Q_j - \hat{Q}_j) \leq 89\cdot\prev + 16\cdot\rev(\cM)$$

Finally, since in $\cM$, each buyer is restricted to purchase at most one item, it can be treated as a BIC and IR mechanism in the unit-demand setting. By \cite{ChawlaHMS10,KleinbergW12,CaiDW16}, $\rev(\cM)\leq 24\cdot \prev$. We complete our proof for Lemma~\ref{lem:Q and Q-hat}.

%\todo{Say that the entry fee can be computed efficiently.}
%\argyrisnote{I don't think it is necessary? as mentioned in the comment after the statement of the theorem.}
%\argyrisnote{
%Also by Combining the mentioned inequalities don't we get that $2\sum_j(Q_j - \hat{Q}_j) \leq 48 \prev + 16 \aperev$?
%Isn't restricted SPEM with entry fee just \prev, where we shift the price of each item by the same number? So the previous bound just becomes $64\prev$?} \mingfeinote{Thanks for pointing it out! I divided the constant by 2. Also, I don't think the restricted SPEM is equivalent to $\prev$ when the posted price are randomized. In $\prev$ the posted price are drawn and given to the buyer before the buyer makes any decision. In restricted SPEM, the buyer has to decide whether to pay this fixed entry fee before seeing the exact posted price.}
%\argyrisnote{Why don't we use a mechanism that shows the items to the buyer and sets entry fee to the $i$-th buyer equal to $\delta_i=\Med_{t_i\sim D_i}\{\eta_i(t_i,S_i(U)\}$?
%The buyer accepts the entry fee with probability at least $\frac{1}{4}$, the probability to accept the entry fee, if all the items are available $\frac{1}{2}$ times the probability that her favourite item is available $\frac{1}{2}$. That way we can covnert the mechanism into a real SPEM that does not depend on which items have been sold, right?}



\notshow{
\begin{align*}
& \sum_{j\in[m]}\sum_{i\in[n]} \sum_{\substack{t_{i,j}\in T_{i,j}\\V_{i,j}(t_{i,j}) \geq Q_j^* + \tau_i}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
\sum_{\delta \in \Delta V_{i}} (V_{i,j}(t_{i,j})-\beta)\cdot
\lambda_{i,j}(t_{i,j},\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \beta ] \\
= & \sum_{j\in[m]}\sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
\sum_{\delta \in \Delta V_{i}} (V_{i,j}(t_{i,j})-\beta)\cdot
\lambda_{i,j}(t_{i,j},\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] \\
\leq & \sum_{j\in[m]} \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] 
\end{align*}


Observe that the quantity above is the sum of the truncated utilities if we pretend that the buyers are additive,
when the price is set to 
%$\max(Q_j + \tau_i, \beta_{i,j})$
$\beta_{i,j}$
of the $i$-th agent for the $j$-th item,
where $\beta_{i,j}$ and the truncation $\delta_{i,j}$ is sampled (independently from the other items and agents, but the distribution between $\beta_{i,j}$ and $\delta_{i,j}$ is coupled) from $B_{i,j} \times \Delta_{i,j}$.
By the constraint of the program,
the expected truncated utility of the $i$-th agent is at most $\delta_i$.
Let

$$u_{ADD} = \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] 
$$

Let $u_{UD}$ be the expected truncated utility if the buyer was unit-demand,
notice that a lower bound of $u_{UD}$ is:
\begin{align*}
u_{UD} \geq & \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) > \max( \beta, Q_j^* + \tau_i) ] \\
& \quad \cdot \prod_{k\neq i}\Pr_{\substack{\beta \sim B_{i,k}\\t_{i,k}\sim D_{i,k}}}[V_{i,k}(t_{i,k}) \leq \max( \beta, Q_k^* + \tau_i) ] \\
\geq & \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) > \max( \beta, Q_j^* + \tau_i) ] \frac{1}{2} \\
%= & \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
% (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
%\lambda_{i,j}'(\beta, \delta)
%\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] \frac{1}{2} \\
= & \frac{u_{ADD}}{2}
\end{align*}

Now we are going to show that there exists a simple mechanism that generates revenue close to $u_{UD}$.
Let $B\times \Delta$ be the coupled distribution of $B_i \times \Delta_i$.
Let 
$$u^T_i(t, X) = \E_{(\beta, \delta) \sim B \times \Delta} [ \max_{j \in X} (V_{i,j}(t_{i,j})- \beta_j)\mathds{1}[\delta_{i,j} + \beta_j \geq V_{i,j}(t_{i,j}) \geq \beta_j ]$$

Note that $\sum_{i\in[n]}\E_{t_i \sim \DD_i}[u^T_i(t, [m])] \geq u_{UD}$.



\begin{lemma}
The function $u^T_i(\cdot, \cdot)$ is $\delta_i$-Lipschitz and subadditive over the items.
\end{lemma}

}

%\todo{Since values $\beta$ have been choosen so that each item is sold with probability $\frac{1}{2}$, we can still bound the objective by a simple mechanism.}
%Thus the median and mean of the utility are close,
%so we can find a proper entry fee to get the truncated utility (minus $O(1)Srev$) as revenue.
%Observe that Unit-Demand prices + entry fee is bounded \srev.


\notshow{

\todo{Let $t_i \in T_i$.
We denote by $W_{t_i}$ the the polytope of feasible welfares normalised to $[0,1]$  when the $i$-th agent has type $t_i$ (note that this can be achieved by dividing the supporting price that the agent has for the allocation by $V_{i,j}(t_{i,j})$).
Let $W_i$ be a mixture of polytopes $\{W_{t}\}_{ t \in T}$ with distribution $\{f(t)\}_{t \in T}$.
%Note that the bit complexity of each vertex of each polytope is $O(m)$.
%The bit complexity of each node in the polytope depends on $\max_{i\in[n], t_i \in T_i, j\in[m], S \in 2^{[m]}}b(v_j^S(t_{i,j}))$.
The bit complexity of the polytope depends on the supporting prices, which (I believe) its reasonable to assume that are bounded.

Note that for $t_i \in T_i$,
we can optimize any objective over $W_{t_i}$ by using a demand oracle. 
By sampling we can get a sampling an empirical polytope close to the polytope of $W_i$. Thus we can calculate the value of the LP in \Cref{fig:bigLP} with respect to the sampled polytope.

Observe that the way $W_i$ is defined here,
is the scaled by $f_i(t_i)$ version of the $W_i$ that was defined in the program

%Thus we lose $\epsilon \cdot n \cdot m \cdot H$ in the objective by sampling in order to get a feasible solution, where $\epsilon$ depends on the number of samples we used to form the empirical polytope and $H$ is the highest value for an item and we can get a feasible solution.
%Since each element is within $\epsilon$ of a feasible, and by reducing the value of $w_{i,j}(t_{i,j})$ by $\epsilon$ we can still get a feasible solution of the original problem, I think we are fine.
}

}

\end{proof}

\subsection{Analyzing the Revenue of $\Mtpt$ and the Proof of Theorem~\ref{thm:bounding-lp-simple-mech-XOS}}\label{sec:proof of bounding LP with simple mech}

In this section, we will show that $\sum_{j\in[m]} Q_j$ can be bounded using the revenue of the two-part tariff $\Mtpt$ defined in Mechanism~\ref{def:constructed-SPEM}. To analyze the revenue of $\Mtpt$, we require the following definition.

%how to bound $\sum_j\hat{Q}_j$ using simple mechanisms that can be computed efficiently. 
%Then \Cref{thm:bounding-lp-simple-mech} follows directly from \Cref{lem:Q and Q-hat} and \Cref{lem:bounding Q-hat}, since the objective of any feasible solution of the LP in \Cref{fig:bigLP} is represented as $\sum_{j\in [m]}Q_j$.


%\begin{lemma}\label{lem:Meff-computation}
%The mechanism $\Meff$ in \Cref{def:constructed-SPEM} can be computed efficiently. Formally, for every $i,j$ and $S\subseteq [m]$, both the posted price $\theta_{ij}$ and entry fee $\xi_i(S)$ can be computed in time \mingfeinote{Add time complexity and query complexity to the adjusted demand oracle}.
%\end{lemma


%\begin{lemma}\label{lem:bounding Q-hat}
%Let $\cM$ and $\Meff$ be the mechanism stated in \Cref{lem:Q and Q-hat} and \Cref{def:constructed-SPEM} accordingly. Then $\sum_j \hat{Q}_j\leq O(1)\cdot \prev+O(1)\cdot \rev(\cM) + O(1)\cdot \rev(\Meff)$.
%\end{lemma}

%To prove \Cref{lem:bounding Q-hat}, 

\begin{definition}\label{def:mu}
%For any $i,t_i,\beta_i=(\beta_{ij})_j,\delta_i=(\delta_{ij})_j$, let

%$$C_i(t_i,\beta_i,\delta_i)=\{j\in [m]\mid V_{ij}(t_{ij})\leq \min\{\beta_{ij}+\delta_{ij},Q_j+\tau_i\}\}$$

For any buyer $i$ and type $t_i$, let $C_i(t_i)=\{j\in [m]\mid V_{ij}(t_{ij})\leq Q_j+\tau_i\}$. For any $t_i\in \cT_i$ and set $S\subseteq [m]$, let
%$$\mu_i(t_i,S)=\E_{(\beta_i,\delta_i)\sim \cC_i}\left[\max_{S'\subseteq S}\left(v_i(t_i,S'\cap C_i(t_i,\beta_i,\delta_i))-\sum_{j\in S'}Q_j\right)\right]$$ 

$$\mu_i(t_i,S)=\max_{S'\subseteq S}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)$$ 
\end{definition}

\begin{lemma}\label{lem:mu_i lipschitz}
For every $i$, {if $v_i(\cdot,\cdot)$ is subadditive over  independent itmes}, then $\mu_i(\cdot, \cdot)$ is subadditive over independent items and $\tau_i$-Lipschitz.
\end{lemma}

\begin{proof}
First we are going to show that $\mu_i(t,\cdot)$ is monotone.
Note that for sets $S_1 \subseteq S_2$ the following holds:
\begin{align*}
    \mu_i(t_i,S_1)=& \max_{S'\subseteq S_1}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    \leq &\max_{S'\subseteq S_2}\left(  v_i(t_i, S'\cap C_i(t_i)) -\sum_{j\in S'}Q_j\right)\\
    = & \mu_i(t_i,S_2)
\end{align*}

Now we are going to show that $\mu_i(t,\cdot)$ is subadditive.
Let $S_1,S_2,S_3\subseteq[m]$ such that $S_1 \cup S_2 = S_3$ and $S_1 \cap S_2 = S_c$.
Let $S_a = S_1 \backslash S_c$ and $S_b=S_2$,
then for any $t_i\in T_i$ we have the following:
\begin{align*}
    \mu_i(t_i,S_3)=& \max_{S'\subseteq S_3}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    \leq &\max_{S'\subseteq S_3}\left(  v_i(t_i,\left(S_a\cap S'\right)\cap C_i(t_i)) + v_i(t_i,\left(S_b\cap S'\right)\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    = & \max_{S'\subseteq S_3}\left(  \left(v_i(t_i,\left(S_a\cap S'\right)\cap C_i(t_i))- \sum_{j\in S_a\cap S'}Q_j \right)+ \left(v_i(t_i,\left(S_b\cap S'\right)\cap C_i(t_i))-\sum_{j\in S_b\cap S'}Q_j\right)\right)\\
    \leq & \max_{S'\subseteq S_a}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right) + \max_{S'\subseteq S_b}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    = & \mu_i(t_i,S_a) + \mu_i(t_i,S_b) \\
    \leq & \mu_i(t_i,S_1) + \mu_i(t_i,S_2)
\end{align*}

The first inequality follows because $v_i(t_i,\cdot)$ is a subadditive function and $S_a\cup S_b=S_3$. The second inequality follows because {$\max$ is subadditive.}
%$S_a \cap S_b = \emptyset$ and $S_a \cup S_b = S_3$. 
The final inequality follows from the fact that $S_b =S_2$, $S_1 \supseteq S_a$ and that $\mu_i(t_i,\cdot)$ is monotone.

We now prove that $\mu_i(\cdot,\cdot)$ has no externalities. Fix any $S\subseteq [m]$ and $t_i,t_i'\in \cT_i$ such that $t_{ij}=t_{ij}'$ {for all $j\in S$}. We notice that by the definition of $C_i$, $S'\cap C_i(t_i)=S'\cap C_i(t_i')$ for all $S'\subseteq S$. Since $v_i(\cdot,\cdot)$ has no externalities, $v_i(t_i,S'\cap C_i(t_i))=v_i(t_i',S'\cap C_i(t_i'))$ for every $S'\subseteq S$. Thus $\mu_i(t_i,S)=\mu_i(t_i',S)$.

Now we are going to show that $\mu_i(\cdot,\cdot)$ is $\tau_i$-Lipschitz.
Let $t_i,t_i' \in \cT_i$ and $X,Y \subseteq[m]$ and $c= |\{j \in [m]: j \in X \Delta Y \text{ or }t_{ij} \neq t_{ij}'\}|$,~\footnote{$\Delta$ stands for the symmetric difference between two sets.} we need to show that:
$$
|\mu_i(t_i,X) - \mu_i(t_i',Y)| \leq c\cdot \tau_i
$$
Let $Z = \{j :j \in X\cap Y \text{ and } t_{ij}=t_{ij}'\}$.
Since $\mu_i(t_i,\cdot)$ is monotone, in order to show that $\mu_i(\cdot,\cdot)$ is $\tau_i$-Lipschitz,
it is enough to show that
\begin{align*}
\mu_i(t_i,X) - \mu_i(t_i',Y) \leq \mu_i(t_i,X) - \mu_i(t_i',Z) \leq c\cdot \tau_i \\
\mu_i(t'_i,Y) - \mu_i(t_i,X) \leq \mu_i(t'_i,Y) - \mu_i(t_i,Z) \leq c\cdot \tau_i
\end{align*}
We are only going to prove that $\mu_i(t_i,X) - \mu_i(t_i',Z) \leq c\cdot \tau_i$ since the other case is similar.
Because for each $j\in Z$, $t_{i,j}'=t_{i,j}$, then $\mu_i(t_i',Z)= \mu_i(t_i,Z)$.
%Observe that $|Z|+c = m$. Thus it is enough to show:
%$$\mu_i(t_i,X) - \mu_i(t_i,Z) \leq (m-|Z|)\cdot \tau_i \Leftrightarrow \mu_i(t_i,X)  \leq (m-|Z|)\cdot \tau_i +  \mu_i(t_i,Z)$$
We have
\begin{align*}
    \mu_i(t_i,X)=& \max_{S'\subseteq X}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    \leq &\max_{S'\subseteq X}\left(\sum_{j\in S'\backslash Z}\left(v_i(t_i,\{j\}\cap C_i(t_i)) - Q_j \right) +  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right)\right)\\
    \leq &\max_{S'\subseteq X}\left(\sum_{j\in S'\backslash Z}\left(V_{ij}(t_{ij}) - Q_j \right)^+\ind[V_{ij}(t_{ij}) \leq Q_j + \tau_i] +  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right)\right)\\
    =& \max_{S'\subseteq Z}  \left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in  S'}Q_j\right) + \sum_{j\in X\backslash Z}\left(V_{ij}(t_{ij}) - Q_j \right)^+\ind[V_{ij}(t_{ij}) \leq Q_j + \tau_i]\\
    %= & \max_{S'\subseteq Z}  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right) + \sum_{j\in X\backslash Z}\left(V_{ij}(t_{ij}) - Q_j \right)^+\ind[V_{ij}(t_{ij}) \leq Q_j + \tau_i]\\
    \leq & \max_{S'\subseteq Z}  \left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right) + (|X| - |Z|)\tau_i\\
    %\leq & \max_{S'\subseteq Z}  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right) + (|X| - |Z|)\tau_i\\
    %\leq &\mu_i(t_i,Z) +  (m-|Z|)\cdot \tau_i
    \leq &\mu_i(t_i,Z) +  c\cdot \tau_i
\end{align*}
The first inequality follows because $v_i(t_i,\cdot)$ is subadditive.
The second inequality follows because $v_i(t_i,\{j\}\cap C_i(t_i)) - Q_j \leq (V_{ij}(t_{ij}) - Q_j)^+\ind[V_{ij}(t_{ij})\leq Q_j + \tau_i]$.
\end{proof}

\begin{lemma}\label{lem:lower bounding mu}
	%Let $\cM$ be the restricted SPEM stated in \Cref{lem:Q and Q-hat}.
	For every type profile $t\in \cT$, let $\textsc{SOLD}(t)$ be the set of items sold in mechanism $\Mtpt$. Then
\begin{align*}
\E_{t}\left[\sum_{i\in[n]} \mu_i\left(t_i,S_i(t_{< i})\right) \right]&\geq \sum_j \Pr_{t}[j\notin \sold(t)]\cdot(2\hat{Q}_j-Q_j)\\
&\geq \sum_{j} \Pr_t\left[j\notin \sold(t)\right]\cdot Q_j - 473\cdot \prev %- 16\cdot \rev(\cM)
\end{align*}
\end{lemma}

\begin{proof}
By the definition of polytope $W_i$, for every buyer $i$ and $t_i\in \cT_i$, there exists an vector of non-negative numbers $\{\sigma_{iS}^{(k)}(t_i)\}_{S\subseteq [m],k\in [K]}$, such that $\sum_{S,k} \sigma_{iS}^{(k)}(t_i)\leq 1$ and
\begin{equation}
\pi_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_{iS}^{(k)}(t_{ij},t_{i,-j})
\end{equation}

\begin{equation}\label{equ:w and gamma}
w_{ij}(t_{ij})\cdot V_{ij}(t_{ij}) \leq f_{ij}(t_{ij})\cdot \sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_{ij},t_{i,-j})\cdot\alpha_{ij}^{(k)}(t_{ij})
\end{equation}

%For every $t_i$, define
%$$\hat\gamma_{ij}^S(t_i)=\gamma_{ij}^S(t_i)\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]$$

%Then clearly for every $t_i$ and $S$, $\{\hat\gamma_{ij}^S(t_i)\}_j$ is the supporting price for $v_i(t_i,S\cap C_i(t_i))$. 
We have
\begin{align*}
&\E_{t}\left[\sum_i \mu_i\left(t_i,S_i(t_{< i})\right) \right]\\
\geq & \sum_i \E_{t_i, t_{-i}}\left[\sum_{S\subseteq [m]}\sum_k\sigma_{iS}^{(k)}(t_i)\cdot\mu_i\left(t_i,S_i(t_{<i})\cap S\right)\right]\\
\geq & \sum_i \E_{t_i, t_{-i}}\left[\sum_{S,k}\sigma_{iS}^{(k)}(t_i)\cdot\sum_{j\in S} \ind\left[j\in S_i(t_{<i})\right]\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)^+ \right]\\
=& \sum_i \E_{t_i}\left[\sum_{j\in [m]}\Pr_{t_{-i}}[j\in S_i(t_{<i})]\cdot\sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_i)\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)^+ \right]\\
\geq & \sum_i\sum_j \Pr_{t}[j\notin \sold(t)]\cdot \E_{t_i}\left[\sum_{S: j\in S}\sum_k \sigma_{iS}^{(k)}(t_i)\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)^+\right]\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_i} f_i(t_i)\cdot \sum_{S: j\in S}\sum_k \sigma_{iS}^{(k)}(t_i)\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)\\
= & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot\sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_i)\cdot(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j)\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} w_{ij}(t_{ij}) V_{ij}(t_{ij})\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-\sum_j\Pr_t[j\not\in \sold(t)]\cdot Q_j
\end{align*}

%\argyrisnote{I don't see why:
%$\sum_i \sum_{t_{ij}} f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{,%-j}(t_{i,-j})\cdot\sum_{S:j\in S}\sigma_{iS}(t_i)Q_j =Q_j$? We could overallocate the item since we have constraints only on $w_{i,j}$?}

The first inequality is because $\mu_i(t_i,S)$ is monotone in set $S$ for any $i,t_i$ and $\sum_{S,k}\sigma_{iS}^{(k)}(t_i)\leq 1$. For any fixed $i,t_i$ and set $S$, if we let $S'$ be the set of items that are in $S\cap S_i(t_{<i})$ and satisfy that $\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\geq 0$. Clearly $S'\subseteq C_i(t_i)$. Then 
\begin{align*}
\mu_i\left(t_i,S_i(t_{<i})\cap S\right)&\geq v_i(t_i,S')-\sum_{j\in S'}Q_j\\
&= \max_{k'\in [K]}\sum_{j\in S'}\alpha_{ij}^{(k')}(t_{ij})-\sum_{j\in S'}Q_j\geq \sum_{j\in S'} \left(\alpha_{ij}^{(k)}(t_{ij})-Q_j\right)\\
&=\sum_{j\in S'} \left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)~~~~~(S'\subseteq C_i(t_i))
\end{align*} 

This inequality is exactly the second inequality above. The third inequality is because $\Pr_{t_{<i}}[j\in S_i(t_{<i})]\geq \Pr_{t}[j\notin \sold(t)]$ for all $j$ and $i$, as the LHS is the probability that the item is not sold after the seller has visited the first $i-1$ buyers and the RHS is the probability that the item remains unsold till the end of the mechanism $\Mtpt$. 
%The second last inequality follows from the definition of $\hat\gamma_{ij}^S(t_i)$ and the fact that
The last inequality follows from Inequality~\eqref{equ:w and gamma} and Constraint \PiConstraint~of the LP in \Cref{fig:bigLP} (or in \Cref{fig:XOSLP}):

$$\sum_i\sum_{t_{ij}}f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_i)=\sum_i\sum_{t_{ij}}\pi_{ij}(t_{ij})\leq 1$$

Notice that by \Cref{def:Q_j} and Constraint \LambdaMarginalConstraint~of the LP in \Cref{fig:bigLP} (or in \Cref{fig:XOSLP}), for every $i,j,t_{ij}$, 

$$%\sum_{\beta_{ij},\delta_{ij}}g_{ij}(t_{ij},\beta_{ij},\delta_{ij})\leq
\sum_{\beta_{ij},\delta_{ij}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=w_{ij}(t_{ij})/f_{ij}(t_{ij})$$
%\argyrisnote{In the continuous version, we do not use $g_{ij}$, right?}
Thus we have

\begin{align*}
&\sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} w_{ij}(t_{ij}) V_{ij}(t_{ij})\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-\sum_j\Pr_t[j\not\in \sold(t)]\cdot Q_j\\
= & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} f_{ij}(t_{ij})V_{ij}(t_{ij})\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i] \sum_{\beta_{ij},\delta_{ij}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\\
&\quad\quad-\sum_j\Pr_t[j\not\in \sold(t)]\cdot Q_j\\
\geq &\sum_j \Pr_{t}[j\notin \sold(t)]\cdot (2\hat{Q}_j-Q_j)~~~~~\text{(\Cref{def:hatQ_j})}\\
= &  \sum_j \Pr_{t}[j\notin \sold(t)]\cdot Q_j-  \sum_j\Pr_{t}[j\notin \sold(t)]\cdot2(Q_j-\hat{Q}_j)\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot Q_j - \sum_j 2(Q_j-\hat{Q}_j )~~~~~{\text{(\Cref{lem:Q and Q-hat}, $Q_j-\hat{Q}_j\geq 0$ for all $j$)}}\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot Q_j- 473\cdot\prev%-16\cdot\rev(\cM)
~~~~~\text{(\Cref{lem:Q and Q-hat})}
\end{align*}
\end{proof}

Now we give the proof of \Cref{thm:bounding-lp-simple-mech-XOS}. Note that this is also the proof of \Cref{thm:bounding-lp-simple-mech}.

\begin{prevproof}{Theorem}{thm:bounding-lp-simple-mech-XOS}

For every $i,t_{<i}$, we apply \Cref{lemma:concentrate} to function $\mu_i(t_i,\cdot)$ and ground set $S_i(t_{<i})$. By \Cref{def:mu}, we have
\begin{equation}\label{equ:bounding-mu_i}
\E_{t_i}[\mu_i(t_i,S_i(t_{<i}))]\leq 2\cdot \Med_{t_i}(\mu_i(t_i,S_i(t_{<i})))+\frac{5}{2}\cdot \tau_i
\end{equation}

We now bound the revenue of $\Mtpt$. For every $i\in [n]$, $t_i\in \cT_i$ and $S\subseteq [m]$, let $\mu'_i(t_i,S)=\max_{S'\subseteq S}(v_i(t_i,S')-\sum_{j\in S'}Q_j)$ which is at least as large as $\mu_i(t_i,S)$. Then the %utility 
surplus of buyer $i$ with true type $\hat{t}_i$, for the set $S_i(t_{<i})$ is $\mu'_i(\hat{t}_i,S_i(t_{<i}))$. By Mechanism~\ref{def:constructed-SPEM}, the entry fee $\xi_i(S_i(t_{<i}),t_i')=\mu'_i(t_i',S_i(t_{<i}))$ for every sampled type $t_i'$. Thus for every $t_{<i}$, we have
$$\Pr_{\hat{t}_i,t_i'\sim D_i}\left[\mu'_i(\hat{t}_i,S_i(t_{<i}))\geq \xi_i(S_i(t_{<i}),t_i')\geq \Med_{t_i}(\mu_i(t_i,S_i(t_{<i})))\right]\geq \frac{1}{8}$$

In other words, for every $t_{<i}$, with probability at least $1/8$, the buyer accepts the entry fee, and the entry fee is at least $\Med_{t_i}(\mu_i(t_i,S_i(t_{<i})))$. Thus the revenue of $\Mtpt$ from the entry fee is at least
\begin{align*}
%\frac{1}{8}\sum_i\E_{t_{<i}}[\xi_i(S_i(t_{<i}))]\geq & 
&\frac{1}{8}\sum_i\E_{t_{<i}}\left[\Med_{t_i}(\mu_i(t_i,S_i(t_{<i})))\right]\\
\geq & \frac{1}{16}\sum_i\E_{t_i,t_{<i}}[\mu_i(t_i,S_i(t_{<i}))]-\frac{5}{32}\cdot \sum_i\tau_i~~~~~~\text{(Inequality~\eqref{equ:bounding-mu_i})}\\
\geq & \frac{1}{16}\sum_{j} \Pr_t\left[j\notin \sold(t)\right]\cdot Q_j - \frac{493}{16}\cdot\prev ~~~~~~\text{(\Cref{lem:lower bounding mu} and \Cref{lem:bounding tau_i})}%- 4\cdot \rev(\cM)
\end{align*}
%The first inequality comes from the fact that $\mu_i(t_i,S)\leq \max_{S'\subseteq S}(v_i(t_i,S')-\sum_{j\in S'}Q_j)$ for all $i,t_{i}$ and $S\subseteq [m]$. The second inequality follows from \Cref{equ:bounding-mu_i}.
%The third inequality follows from \Cref{lem:lower bounding mu} and \Cref{lem:bounding tau_i}. 
We notice that for $\Mtpt$, the revenue from the posted prices are $\sum_j \Pr[j\in \sold(t)]\cdot Q_j$. Thus
\begin{align*}
\rev(\Mtpt)\geq & \frac{1}{16}\sum_{j} \Pr_t\left[j\notin \sold(t)\right]\cdot Q_j - \frac{493}{16}\cdot \prev +\sum_j \Pr[j\in \sold(t)]\cdot Q_j\\
\geq & \frac{1}{16}\cdot \sum_{j\in [m]}Q_j-\frac{493}{16}\cdot \prev
%27\cdot \prev - 4\cdot \rev(\cM)
\end{align*}

Thus
%$$2\cdot \sum_jQ_j\leq 216\cdot \prev+32\cdot \rev(\cM)+8\cdot\rev(\Meff)$$

$$2\cdot \sum_jQ_j\leq 986\cdot \prev+32\cdot\rev(\Mtpt)$$

We then show that $\Mtpt$ can be computed in polynomial time: By \Cref{def:Q_j}, the posted price $Q_j$ can be computed in time $\poly(n,m,\sum_{i,j}|\cT_{ij}|)$, given the feasible solution of the LP in \Cref{fig:bigLP} (or in \Cref{fig:XOSLP}). Given the set of available items $S_i(t_{<i})$, for every sampled type $t_i'$, calculating the entry fee requires a single query from the demand oracle. For every buyer $i$ with reported type $t_i$, the mechanism requires a single query from the demand oracle to obtain her favorite bundle among the set of available items, under prices $\{Q_j\}_{j\in [m]}$, and to determine whether the buyer will accept the entry fee.  

Lastly, by \Cref{thm:chms10}, we can compute an RPP $\Mpp$ with the desired running time and query complexity, such that $\Mpp\geq \frac{1}{6.75}(1-\frac{2}{n})\cdot\prev$. We finish our proof.
\end{prevproof}



==> arXiv/appx_sample_access.tex <==
\section{Missing Details from \Cref{sec:sample access}}\label{appx:sample access}

\begin{definition}\label{def:kolmogorov}
The Kolmogorov distance between two distributions $\cD$ and $\widehat{\cD}$ supported on $\mathbb{R}$ is defined as
$$
d_K(\cD,\widehat{\cD}) = \sup_{z\in \mathbb{R}}\left| \Pr_{t\sim \cD}[t\leq z] -\Pr_{\widehat{t}\sim \widehat{\cD}}[\widehat{t}\leq z]\right|
$$
\end{definition}

We need the following robustness result from Cai and Daskalakis~\cite{CaiD17}.
\begin{theorem}[Theorem~3 in \cite{CaiD17}]\label{thm:robust mechanism}
Suppose all bidders' valuations are constrained additive. Let $\cM$ be a Sequential Posted Price with Entry Fee Mechanism (as defined in Mechanism~\ref{def:general SPEM}~\footnote{Indeed the result holds for any buyers' order, we choose the lexicographical order to keep the notation light.}) whose prices are $\{p_{ij}\}_{i\in[n], j\in[m]}$ and its entry fee function for the $i$-th bidder is $\xi_i:2^{[m]}\rightarrow\mathbb{R}_+$.
%Let $\cM(\cD)$  ($\cM(\widehat{\cD})$ resp.) be the expected revenue of mechanism $\cM$ when the agent are samples from $\cD$ ($\widehat{\cD}$ resp).
If for each $i\in[n]$ and $j\in[m]$ we have $d_K(\cD_{ij},\widehat{\cD}_{ij})\leq \eps$, and $\cD_{i,j}$ and $\widehat{\cD}_{i,j}$ are both supported on  $[0,1]$ (that is when each bidder's value for a single item is at most $1$), then
$$
|\rev(\cM,\cD) - \rev(\cM,\widehat{\cD})| \leq 4 n m^2 \eps,
$$ where $\rev(\cM,\cD)$ and $\rev(\cM,\widehat{\cD})$ are the revenues of $\cM$ under $\cD=\bigtimes_{i,j} \cD_{ij}$ and  $\widehat{\cD}=\bigtimes_{i,j} \widehat{\cD}_{ij}$  respectively.
\end{theorem}


\begin{algorithm}[H]
\floatname{algorithm}{Mechanism}
%\setstretch{1.35}
%\vspace{.1in}
\begin{algorithmic}[1]
\setcounter{ALG@line}{-1}
\State Before the mechanism starts, the seller decides on a collection of $\{p_{ij}\}_{i\in[n],j\in[m]}$ and a collection of  entry fee functions $\{\xi_i(\cdot)\}_{i\in [n]}$, where $\xi_i:2^{[m]}\rightarrow\mathbb{R}_+$ is buyer $i$'s entry fee.  
\State Bidders arrive sequentially in the lexicographical order.
\State When buyer $i$ arrive, the seller shows her the set of available items $S\subseteq [m]$, as well as their prices $\{p_{ij}\}_{j\in S}$ and asks buyer $i$ to pay an \emph{entry fee} of $\xi_i(S)$. Note that $S$ is the set of items that are not purchased by the first $i-1$ buyers.
\If{Bidder $i$ pays the entry fee ${\delta_i}(S)$}
        \State $i$ receives her favorite bundle $S_i^{*}$ and pays $\sum_{j\in S_i^{*}}p_{ij}$.
        \State $S\gets S\backslash S_i^{*}$.
    \Else
        \State $i$ gets nothing and pays $0$.
    \EndIf
\end{algorithmic}
\caption{{\sf \quad Sequential Posted Price with Entry Fee Mechanism (SPEM)}}\label{def:general SPEM}
\end{algorithm}

\begin{lemma}\label{lem:revenue close kolmogorov}
Suppose all bidders' valuations are constrained additive. If for each $i\in[n]$ and $j\in[m]$ we have $d_K(\cD_{ij},\widehat{\cD}_{ij})\leq \eps$, and $\cD_{i,j}$ and $\widehat{\cD}_{i,j}$ are both supported on  $[0,1]$ (that is when each bidder's value for a single item is at most $1$), then 
$$ c_1\cdot \opt(\widehat{\cD})- O(nm^2\eps)\leq \opt(\cD)\leq \frac{\opt(\widehat{\cD})}{c_2}+ O(nm^2\eps)$$ for some absolute constant $c_1, c_2>0$, where 
$\opt({\cD})$ (or $\opt(\widehat{\cD})$) is the optimal revenue for distribution $\cD=\bigtimes_{i,j} \cD_{ij}$ (or $\widehat{\cD}=\bigtimes_{i,j} \widehat{\cD}_{ij}$).
\end{lemma}

\begin{proof}
%\argyrisnote{Since any TPT is a SPEM and any RPP is a SPEM if we treat the buyers' valuation as Unit-Demand, the optimal SPEM achieves at least a constant fraction of the optimal revenue.}Since any RPP or TPT is also a SPEM, the optimal SPEM achieves at least a constant fraction of the optimal revenue. Let $M_1$ be the optimal SPEM for $\cD$, and we denote its revenue as $\rev(M_1)$.  Let $M_2$ be the optimal SPEM for $\widehat{\cD}$, and we denote its revenue as $\rev(M_2)$. By Theorem~\ref{thm:robust mechanism}, we know that $|\rev(M_1)-\rev(M_2)|\leq 4nm^2\varepsilon$. Hence, $\opt(\widehat{\cD})\geq \rev(M_2)\geq \rev(M_1)-4nm^2\varepsilon\geq  \Omega(\opt(\cD))-4nm^2\varepsilon$ and  $\opt({\cD})\geq \rev(M_1)\geq  \rev(M_2)-4nm^2\varepsilon \geq \Omega(\opt(\widehat{\cD}))-4nm^2\varepsilon$.

Let $M_1$, $M_2$ be the optimal RPP and TPT for $\cD$, and we denote their revenue as $\rev(M_1)$, $\rev(M_2)$ respectively. Let $M_3$, $M_4$ be the optimal RPP and TPT for $\widehat{\cD}$, and we denote their revenue as $\rev(M_3)$, $\rev(M_4)$ respectively. Since any TPT is a SPEM, by Theorem~\ref{thm:robust mechanism}, we know that $|\rev(M_2)-\rev(M_4)|\leq 4nm^2\varepsilon$, as $$\rev(M_4)\geq \rev(M_2,\widehat{\cD})\geq \rev(M_2,\cD)-4nm^2\varepsilon=\rev(M_2)-4nm^2\varepsilon,$$ and $$\rev(M_2)\geq \rev(M_4,{\cD})\geq \rev(M_4,\widehat{\cD})-4nm^2\varepsilon=\rev(M_4)-4nm^2\varepsilon.$$
Similarly, since any RPP is also a SPEM if we treat the buyers' valuation as Unit-Demand, we have $|\rev(M_1)-\rev(M_3)|\leq 4nm^2\varepsilon$. By \Cref{lem:caiz17-constrained-additive}, $\max\{\rev(M_1),\rev(M_2)\}\geq \Omega(\opt(\cD))$. Hence, $\opt(\widehat{\cD})\geq \max\{\rev(M_3),\rev(M_4)\}\geq \max\{\rev(M_1),\rev(M_2)\}-4nm^2\varepsilon\geq  \Omega(\opt(\cD))-4nm^2\varepsilon$. Similarly, $\opt({\cD})\geq \Omega(\opt(\widehat{\cD}))-4nm^2\varepsilon$.

\end{proof}



\begin{prevproof}{Theorem}{thm:sample access}
For each $D_{ij}$, we first take $O\left(\frac{\log(nm/\delta)}{\varepsilon^2}\right)$ samples. Let $\widehat{D}_{ij}$ be the uniform distribution over the samples. By the union bound and the DKW inequality~\cite{DvoretzkyKW56}, $d_K(D_{ij},\widehat{D}_{ij})\leq \eps$ for all $i\in[n]$ and $j\in[m]$ with probability at least $1-\delta$. Now we run the algorithm from \Cref{thm:main XOS-main body} on $\bigtimes_{i,j}\widehat{D}_{ij}$ and let $\cM$ be the computed mechanism. Note that $\rev(\cM,\widehat{D})$, the revenue of $\cM$ under $\widehat{D}=\bigtimes_{i,j} \widehat{D}_{ij}$, is $\Omega(\opt(\widehat{D}))$ -- the optimal revenue for distribution $\widehat{D}$. By Theorem~\ref{thm:robust mechanism}, $\rev(\cM,{D})\geq \rev(\cM,\widehat{D})-O(nm^2\eps)$. By Lemma~\ref{lem:revenue close kolmogorov}, $\opt(\widehat{D})\geq\Omega(\opt({D}))-O(nm^2\eps)$. Chaining the ineuqalities together, we have that $\rev(\cM,{D})\geq \Omega(\opt({D}))-O(nm^2\eps)$.
\end{prevproof}

==> arXiv/exante.tex <==
\section{Some Examples}\label{sec:example}
\subsection{Non-Concavity of~\core}\label{sec:core non-concavity}

In this section, we show that the~$\core(\sigma,\theta(\sigma))$ function is non-concave in the interim allocation rule $\sigma$. We first provide the formal definition of $\theta(\sigma)$ for a single-bidder two-item instance, and we use $\icore(\sigma)$ to denote $\core(\sigma,\theta(\sigma))$.
\begin{definition}[Core for a single additive bidder over two items with continuous distributions - \cite{CaiZ17}]\label{def:core-single interim}
Consider a single bidder interested in two items, whose value is sampled from continuous distribution $D$ with support $T=\supp(D)$ and density function $f(t)$ for $t\in T$.
Consider a feasible interim allocation $\sigma=\{\sigma_1(t),\sigma_2(t)\}_{t\in \supp(D)}$,
that is $\sigma_1(t)$ ($\sigma_2(t)$ resp.) is the probability that the allocation rule awards item $1$ (item $2$ resp.) to a bidder with type $t$.
Define 
$$\beta_1(\sigma) = \argmin_{\beta\geq 0}\left[ \Pr_{t_1\sim D_1} \left[t_1\geq \beta\right]=\E_{t\sim D}\left[\sigma_1(t) \right]\right] \quad \quad \quad \beta_2(\sigma) = \argmin_{\beta\geq 0}\left[ \Pr_{t_2\sim D_2} \left[t_2\geq \beta\right]=\E_{t\sim D}\left[\sigma_2(t) \right] \right] $$
and
$$c(\sigma)= \argmin_{a\geq 0}\left\{\Pr_{t\sim D}\left[t_1\leq \beta_1(\sigma)+a\right]+\Pr_{t\sim D}\left[t_2\leq \beta_2(\sigma)+a\right]\geq\frac{1}{2}\right\}$$
The term $\icore$ for interim allocation $\sigma$ is defined as follows:
%$$\icore(\sigma)=\int_{t\in T}f(t)\cdot \sigma_{1}(t)t_{1}\cdot \ind[t_{1}\leq \beta_{1}+c]
%+ \int_{t\in T}f(t)\cdot \sigma_{2}(t)t_{2}\cdot \ind[t_{2}\leq \beta_{2}+c]$$
%
$$\icore(\sigma)=
\E_{t\sim D}\left[\sigma_{1}(t)t_{1}\cdot \ind[t_{1}\leq \beta_{1}(\sigma)+c(\sigma)]\right]
+
\E_{t\sim D}\left[\sigma_{2}(t)t_{2}\cdot \ind[t_{2}\leq \beta_{2}(\sigma)+c(\sigma)]\right]$$

\end{definition}

In Example~\ref{ex:non-concave interim} we show that 
%even in the single-bidder and two-items setting, 
$\icore(\sigma)$ is a non-concave function even in the setting with a single bidder and two items. The reason for the $\icore$ being non-concave lies in the fact that the interval which we truncate depends on the interim allocation $\sigma$.
%A naive solution would be to compute the concave hull of $\core(q)$,
%but that requires exponential in the number of items.
Computing the concave hull of $\icore(\sigma)$ in the worst case requires exponential time in the dimension of the space, which is $m$ is our case. 
%These facts make the ex-ante relaxation approach not applicable to solve our problem.
%\argyrisnote{Argyris: Is the previous sentence left by accident? I don't think we mention something about ex-ante until now?}

\begin{example}\label{ex:non-concave interim}
Consider a single additive bidder interested in two items whose values are both drawn from the uniform distribution $U[0,1]$. %We are going to show that $\core(q)$ is a non-concave function by an example.
Consider two interim allocation rules $\sigma$ and $\sigma'$:
\begin{itemize}
    \item $\sigma$: Award the first item to the buyer if her value for it lies in the interval $[0,1/2]$ and never award the second item to the buyer.
    \item $\sigma'$: Always award the first item to the buyer and never award the second item to the buyer.
\end{itemize}

\noindent According to Definition~\ref{def:core-single},
for allocation rule $\sigma$, the dual parameters are $\beta_1(\sigma)=1/2$, $\beta_2(\sigma)=1$ and $c(\sigma)=0$,
which implies $\icore(\sigma)=1/8$.
Similarly for allocation rule $\sigma'$ we have $\beta_1(\sigma')=0$, $\beta_2(\sigma')=1$ and $c(\sigma')=0$,
which implies that $\icore(\sigma')=0$.

Consider the interim allocation $\sigma''$ that uses  allocation rule $\sigma$ with probability $50\%$ and $\sigma'$ with $50\%$.
Note that $\sigma''$ is in the convex combination of $\sigma$ and $\sigma'$ 
and more specifically $\sigma''=\frac{\sigma+\sigma'}{2}$.
For interim allocation $\sigma''$ we have that $\beta_1(\sigma'')=1/4$, $\beta_2(\sigma'')=1$ and $c(\sigma'')=0$,
which implies that $\icore(\sigma'')=\frac{1}{32}$.
%, that is $\sigma_1(t)=1$
%and $\sigma_2(t)=0$ for any $t \in [0,1]^2$. 
%Consider the values $q=(1/2,0)$ and $q'=(1,0)$.
%According to Definition~\ref{def:core-single},
%for $q$ we have 
%that $\beta^{(q)}_1 = 1/2,\beta^{(q)}_2 = 1$ and $c^{(q)}=0$ 
%and for $q'$ we have $\beta^{(q')}_1= 0,\beta^{(q')}_2=1$ and $c^{(q')}=0$.
We notice that the second item contributes nothing to the $\icore$,
but it ensures that $c=0$ regardless of the allocation of the first item.
%Observe that $\icore(q) = 1/8 $ and
%$\maxcore(q') =  0$. Let $q'' = (q+q')/2=(3/4,0)$.
%For $q''$, observe that $\beta_1^{(q'')} = 1/4,\beta_2^{(q'')}=1$ and $c^{(q'')}=0$. We have $\maxcore(q'') = 1/32$. 
Thus $\icore\left(\sigma''\right) < \frac{1}{2}(\icore(\sigma)+\icore(\sigma'))$, which implies that $\icore(\cdot)$ is not a concave function.
\end{example}

\subsection{Why can't we use the Ex-Ante Relaxation?}\label{sec:exante}
%\todo[inline, size=\small]{Why not Ex-ante relaxation? We have cross bidder dual parameter constraints, and Non-Convex single-agent Objective: the core of the average of two allocation rules is not the same as the average of the two core values. Give an example for one item. Mention computing convex hull takes time exponential in the dimension. Chawla-Miller fails because their single agent objective is not poly-time computable.}

An influential framework known as the ex-ante relaxation has been widely used in Mechanism Design, but is insufficient for our problem. Informally speaking,
ex-ante relaxation reduces a multi-bidder objective to the sum of  single-bidder objectives subject to some global supply constraints over ex-ante allocation probabilities. 
To solve the ex-ante relaxation program efficiently, the single-bidder objective has to be concave and efficiently computable given the ex-ante probabilities~\cite{Alaei11}. 

In revenue maximization, the single-bidder objective -- the optimal revenue subject to ex-ante probabilities -- is indeed a concave function. However, we do not have a polynomial time algorithm to even compute the single-bidder objective given a set of fixed ex-ante probabilities.~\footnote{The closest thing we know is a QPTAS for a unit-demand bidder. See \Cref{sec:related work}.} To fix this issue, one can try to find a concave function that is always a good approximation to the single-bidder objective for any ex-ante probabilities. To the best of our knowledge, such a concave function only exists for unit-demand bidders via the copies setting technique~\cite{ChawlaHMS10}. Alternatively, one can replace the global objective -- optimal revenue by the upper bound of revenue proposed in~\cite{CaiZ17}. Yet the corresponding single-bidder objective for one term $\core$ in the upper bound is highly non-concave, which makes the ex-ante relaxation not applicable.

%while the objective can be (approximately) computed via copies setting \cite{ChawlaHMS10}, it is unclear how to compute or approximate the single-bidder revenue efficiently for more general valuations (see the examples in \cite{Alaei11}). 

%For revenue maximization, the ex-ante relaxation relaxes the revenue optimization problem to maximizing the sum of each bidder's revenue subject to some global supply constraints over ex-ante allocation probabilities.

%Under item-independence, for special bidders' valuations such as unit-demand or additive, special kind of item pricing mechanisms that approximate the optimal revenue are known to be efficiently computable via a nice approach called Ex-Ante Relaxation~\cite{Alaei11, ChawlaM16} %(Argyris: Is this a more accurate statement?).
%A popular approach for designing revenue maximizing mechanisms is the ex-ante approach \cite{Alaei11}.
%Informally speaking,ex-ante relaxation reduces a multi-bidder objective to (the sum of) concave single-bidder objectives subject to some global supply constraints over ex-ante allocation probabilities.
%,in settings where bidders are sampled independently.
%In revenue maximization, the single-bidder objective -- the optimal revenue subject to ex-ante probabilities -- is indeed a concave function. However, while the objective can be (approximately) computed via copies setting \cite{ChawlaHMS10}, it is unclear how to compute or approximate the single-bidder revenue efficiently for more general valuations (see the examples in \cite{Alaei11}). 

 %We refer the readers to \Cref{sec:tour to LP} for the example and more discussions about ex-ante relaxation. Our main contribution in this paper is to provide a new relaxation of the revenue optimization problem that is poly-time solvable and used to construct approximately-optimal mechanisms for up to XOS valuations. 


%To solve the ex-ante relaxation program efficiently, the single-bidder objective has to be concave and efficiently computable given the ex-ante probabilities~\cite{Alaei11}. However, as discussed in \Cref{subsec:technique}, the single-bidder objective in revenue maximization, which is defined as the optimal revenue for a single bidder $i$ subject to ex-ante allocation probabilities $\{q_{ij}\}_{j\in [m]}$, does not seem to be efficiently computable for XOS valuations.   

%Optimizing the single-bidder revenue subject to supply constraints is a concave function, but it is not clear how to evaluate it or approximate it with a simpler concave function apart from basic cases where the bidders' valuations are Additive or Unit-Demand (See the examples in \cite{Alaei11}). 
%A paper by Chawla and Miller \cite{ChawlaM16} circumvents this obstacle, by using the ex-ante approach, and substitutes the revenue per bidder, with the corresponding Core-Tail Decomposition \cite{LiY13,BabaioffILW14,RubinsteinW15,CaiDW16,CaiZ17} and bound each term with simple mechanisms for bidder's valuation up to matroid rank.
%This idea is also our main computational inspiration by \cite{ChawlaM16}.
%One caveat of their approach, is that the term that corresponds to $\core$ in their decomposition is highly non-concave as we show formally later.
%To illustrate why ex-ante relaxation is not applicable for the alternative global objective $\core$, we formally define the $\core$ function for a single additive bidder and two items, but its restrictions extend to the general multi-bidder setting and the $\core$ function as defined in $\cite{CaiZ17}$.



Although the term $\core$ was originally defined for interim allocation rules (as in \Cref{def:core-single interim}), it can also be defined for ex-ante probabilities. We only define it for the single-bidder two-item case. Let $q=\{q_1,q_2\}\in[0,1]^2$,
and $\maxcore=\max_{\sigma\in \Sigma(q)} \icore(\sigma)$,
where $\Sigma(q)$ is the set of feasible interim allocations that awards the first item with probability at most $q_1$ and the second item with probability at most $q_2$.
Example~\ref{ex:non convex core} also shows that $\maxcore(\cdot)$ is a non-concave function by observing that $\sigma \in \Sigma(1/2,0)$,$\sigma' \in \Sigma(1,0)$ and $\sigma'' \in \Sigma(3/4,0)$.




\begin{definition}[Core for a single additive bidder over two items - \cite{CaiZ17}]\label{def:core-single}
Consider a single bidder interested in two items, whose value is sampled from $D_1\times D_2$.
Consider a supply constraints $q_1,q_2 \in [0,1]$. Note that $q_1$ (or $q_2$) is the probability that a mechanism awards the first item (or the second item) to the bidder.
Define 
$$\beta_1 = \argmin_{\beta\geq 0}\left[ \Pr_{t_1\sim D_1} \left[t_1\geq \beta\right]=q_1 \right] \quad \quad \quad \beta_2 = \argmin_{\beta\geq 0}\left[ \Pr_{t_2\sim D_2} \left[t_2\geq \beta\right]=q_2 \right] $$
and

$$c= \argmin_{a\geq 0}\left\{\Pr_{t_1\sim D_1}\left[t_1\leq \beta_1+a\right]+\Pr_{t_2\sim D_2}\left[t_2\leq \beta_2+a\right]\geq\frac{1}{2}\right\}$$
The term $\maxcore$ is defined as follows:
$$
\maxcore\left(q\right) = \max_{\substack{x_1:\cT_1 \rightarrow [0,1]\\ \sum_{t_1\in \cT_1}f_1(t_1) x_1(t_1)= q_1}}\sum_{\substack{t_1\in \cT_1 \\ t_1 \leq \beta_1 + c}} f_1(t_1)\cdot t_1 \cdot x_1(t_1) + 
\max_{\substack{x_2:\cT_2 \rightarrow [0,1]\\ \sum_{t_2\in \cT_2}f_2(t_2) x_2(t_2)=q_2}}
\sum_{\substack{t_2\in \cT_2 \\ t_2 \leq \beta_2 + c}} f_2(t_2)\cdot t_2 \cdot x_2(t_2)
$$
\end{definition}
\notshow{
\begin{definition}[Core for an additive bidder - \cite{ChawlaM16}]
Consider a single additive bidder sampled from $D$ with supply constraints $\{q_{j}\}_{j\in[m]}\in [0,1]^{m}$ (Note that $q_{j}$ is the probability that a mechanism awards item $j$ to bidder $i$).
For item $j\in[m]$, define 
$$\beta_{j} = \argmin_{\beta\geq 0}\left[ \Pr_{t_j\sim D_j} \left[t_j\geq \beta_j\right]=q_j \right] $$
$$c= \argmin_{c\geq 0}\left[ \Pr_{t\sim D}\left[\forall_{j\in[m]}t_j\leq \beta_j+c \right]\geq\frac{1}{2}\right]$$
The term $\core$ is defined as follows:
$$
\core\left(\{q_j\}_{j\in[m]}\right) =
$$
\end{definition}


}
%\mingfeinote{Mingfei: It's not clear from Lemma 1 that the term CORE depends on q. Also maybe we should use a different notation since here the term is the maximum core over allocations.}

In Example~\ref{ex:non convex core} we show that 
%even in the single-bidder and two-items setting, 
$\maxcore(q)$ is a non-concave function even in the setting with a single bidder and two items. The reason for the $\maxcore$ being non-concave lies in the fact that the interval which we truncate depends on the supply constraints $q$.
%A naive solution would be to compute the concave hull of $\core(q)$,
%but that requires exponential in the number of items.
Computing the concave hull of $\maxcore(q)$ in the worst case requires exponential time in the dimension of the space, which is $m$ is our case. These facts make the ex-ante relaxation approach not applicable to solve our problem.

\begin{example}\label{ex:non convex core}
Consider a single additive bidder interested in two items whose values are both drawn from the uniform distribution $U[0,1]$. %We are going to show that $\core(q)$ is a non-concave function by an example.
Consider the values $q=(1/2,0)$ and $q'=(1,0)$.
According to Definition~\ref{def:core-single},
for $q$ we have 
that $\beta^{(q)}_1 = 1/2,\beta^{(q)}_2 = 1$ and $c^{(q)}=0$ 
and for $q'$ we have $\beta^{(q')}_1= 0,\beta^{(q')}_2=1$ and $c^{(q')}=0$.
We notice that the second item contributes nothing to the $\maxcore$,
but it ensures that $c=0$ regardless of the supply demand for the first item.
Observe that $\maxcore(q) = 1/8 $ and
$\maxcore(q') =  0$. Let $q'' = (q+q')/2=(3/4,0)$.
For $q''$, observe that $\beta_1^{(q'')} = 1/4,\beta_2^{(q'')}=1$ and $c^{(q'')}=0$. We have $\maxcore(q'') = 1/32$. Thus $\maxcore\left(q''\right) < \frac{1}{2}(\maxcore(q)+\maxcore(q'))$, which implies that $\maxcore(\cdot)$ is not a concave function.
\end{example}

%One of our main technical contributions is to show how to relax $\maxcore$ with a simpler concave function that we can efficiently compute and at the same time still be able to bound the relaxed $\maxcore$ with simple mechanisms for XOS valuations. The \cite{CaiZ17} approach also introduces additional global constraints across bidders (Constraint (4) in \Cref{lem:caiz17-constrained-additive}), making the ex-ante relaxation more inappropriate for us.


%\vspace{-.1in}

==> arXiv/marginal_reduced_xos.tex <==

\section{Accessing Single-Bidder Marginal Reduced Form Polytopes for XOS Valuations}\label{sec:mrf for xos}

Our goal in this section is to prove \Cref{thm:main XOS-main body} for XOS valuations. 

%extend \Cref{thm:main} to the case where buyers have XOS valuations. We summarize our result for XOS valuations in Theorem~\ref{thm:main XOS}.

%\argyrisnote{Argyris: I marked with my color the difference between Theorem~\ref{thm:main} and Theorem~\ref{thm:main XOS}.
%We also need to adjust Theorem~\ref{thm:bounding-lp-simple-mech} to include XOS buyers.

%Moreover, we need to update \Cref{def:bit complexity}.}


\begin{theorem}\label{thm:main XOS}
(Restatement of \Cref{thm:main XOS-main body} for XOS valuations) Let $T=\sum_{i,j}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance (\Cref{def:bit complexity}). %~\footnote{For any instance of our problem, define \emph{the bit complexity of the problem instance}, as the maximum bit complexity of $n$,$m$,$f_{ij}(t_{ij})$ \argyrisnote{and $\alpha_{ij}^{(k)}(t_{ij})$ for XOS buyers
%over all $i,j,t_{ij}\in \cT_{ij}$}.
%See \Cref{def:bit complexity} for more details.} For XOS buyers, 
For XOS buyers, for any $\delta>0$, there exists an algorithm that computes a rationed posted price mechanism or a two-part tariff mechanism, such that the revenue of the mechanism is at least $c\cdot \opt$ for some absolute constant $c>0$ with probability $1-\delta-\frac{2}{n}$.
Our algorithm assumes query access to a value oracle and an adjustable demand oracle (see \Cref{sec:prelim}) of buyers' valuations, and has running time $\poly(n,m,T,b,\log (1/\delta))$.
\end{theorem}




%Inspired by our construction of a marginal reduced form polytope for constraint additive valuation as described in Section~\ref{sec:mrf for constraint additive},
%we show how to extend the results to cover the case where the valuation of the buyer is XOS.
%In this section,
%our goal is to approximate the marginal reduced form polytope of an agent $W_i$ with XOS valuation,
%where her support is $\cT_i$ and her support for the $j$-th item is $\cT_{ij}$ and be able to construct an efficient separation oracle for the constructed polytope.
%We denote as $M_i=\sum_{j\in[m]}|\cT_{ij}|$.



%\mingfeinote{Formal Definiton of the polytope $W_i$. Move it before stating the LP.

%Mingfei: We need a name for the polytope.

%}



%\vspace{.3in}

%Similar to Section~\ref{sec:multi-approx-polytope},
%we need to construct a "truncated" and a "box" polytope in order to mix them and be able to approximate the marginal reduced form polytope $W_i$.
%However polytope $W_i$ is no longer down-monotone and we cannot use the framework from Section~\ref{sec:multi-approx-polytope}.


%In Definition~\ref{def:welfare frequent} we state the polytope that can be thought of as the truncated polytope that was in Definition~\ref{def:truncated polytope} and in Definition~\ref{def:welfare rare} we describe the polytope that corresponds to the box polytope that was described Definition~\ref{def:box polytope}.


%Recall that in \Cref{sec:mrf-XOS}, we give a generalized 
We remind the readers the definition of the single-bidder marginal reduced form polytope $W_i$ for XOS valuations:

\begin{definition}[Restatement of \Cref{def:W_i}]\label{def:W_i-restate}
For every $i\in [n]$, the single-bidder marginal reduced form polytope $W_i\subseteq [0,1]^{2\cdot \sum_j|\cT_{ij}|}$ is defined as follows. Let $\pi_i=(\pi_{ij}(t_{ij}))_{j,t_{ij}\in \cT_{ij}}$ and $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}\in \cT_{ij}}$. Then $(\pi_i,w_i)\in W_i$ if and only if there exist a number $\sigma_S^{(k)}(t_i)\in [0,1]$ for every $t_i\in \cT_i, S\subseteq [m],k\in [K]$, such that
\begin{enumerate}
    \item $\sum_{S,k}\sigma_S^{(k)}(t_i)\leq 1 $, $\forall t_i\in \cT_i$.
    \item $%f_{ij}(t_{ij})\geq\pi_{ij}(t_{ij})\geq 
    {\pi_{ij}(t_{ij})=}f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})$, for all $i,j,t_{ij}\in \cT_{ij}$.
    \item ${w_{ij}(t_{ij})\leq} f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}$, for all $i,j,t_{ij}\in \cT_{ij}$. {If $V_{ij}(t_{ij})=0$, we slightly abuse notation and treat $\frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}$ as $0$ for all $k$.}
\end{enumerate}
\end{definition}

The following observation follows directly from \Cref{def:W_i}.

\begin{observation}\label{obs:W_i-upper-bound}
For any $(\pi_i,w_i)\in W_i$ and any $j\in [m], t_{ij}\in \cT_{ij}$, $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})\leq f_{ij}(t_{ij})$.
\end{observation}
\begin{proof}
The first inequality follows directly from the fact that $\alpha_{ij}^{(k)}(t_{ij})\leq V_{ij}(t_{ij})=\max_{k'}\alpha_{ij}^{(k')}(t_{ij})$. The second inequality follows from $\sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\leq \sum_{S}\sum_{k}\sigma_S^{(k)}(t_{ij},t_{i,-j})\leq 1$.
\end{proof}

In \Cref{sec:program-XOS}, we provide an LP (\Cref{fig:XOSLP}) that helps us to compute the simple mechanisms efficiently. In \Cref{thm:bounding-lp-simple-mech-XOS}, we have proved that given any optimal solution to the LP in \Cref{fig:XOSLP}, we can compute a simple mechanism in polynomial time, whose revenue is a constant factor of the optimal revenue. However, constraint {\Wconstraint} is implicit and thus it's unclear if we can solve the LP in polynomial time. Similar to the idea in \Cref{sec:multi-approx-polytope}, we fix this issue by constructing another polytope $\widehat{W}_i$. Unfortunately, for XOS valuations, $W_i$ is not a down-monotone polytope anymore. To see this, we simply notice that by \Cref{obs:W_i-upper-bound}, $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})$ for every coordinate $(j,t_{ij})$. Thus given any $(\pi_i,w_i)\in W_i$ where $w_{ij}(t_{ij})>0$ for some $j,t_{ij}$, the vector $(\textbf{0},w_i)$ is clearly not in $W_i$. Thus the argument in \Cref{sec:multi-approx-polytope} does not apply here.




\subsection{Basic Properties of the Single-Bidder Marginal Reduced Form for XOS Valuations}

In this section we present some basic definitions and properties of the single-bidder Marginal Reduced Form polytope $W_i$ (\Cref{def:W_i}). We fixed any buyer $i$ throughout this section unless otherwise specified. 

\begin{definition}\label{def:welfare frequent}
For any $\eps>0$,
we denote as $W_i^{tr(\eps)}\subseteq [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$ the \emph{$\eps$-truncated polytope} of $W_i$.
An element $(\widehat{\pi}_i,\widehat{w}_i)\in W_i^{tr(\eps)}$
if there exists $(\pi_i,w_i)\in W_i$ such that for all $j\in[m]$ and $t_{ij}\in \cT_{ij}$:
\begin{align*}
    \widehat{w}_{ij}(t_{ij}) &=
w_{ij}(t_{ij})\cdot\ind[ f_{ij}(t_{ij})\geq \eps]\\ \widehat{\pi}_{ij}(t_{ij}) &=
\pi_{ij}(t_{ij})\cdot\ind[ f_{ij}(t_{ij})\geq \eps]
\end{align*}

\end{definition}

Similar to Section~\ref{sec:multi-approx-polytope}, we show that $W^{tr(\eps)}_i$ is a mixture (\Cref{def:mixture}) of a set of polytopes $\{W^{tr(\eps)}_{t_i}\}_{t_i\in \cT_i}$ defined in \Cref{def:welfare frequent-t_i} over $\cD$.
%Definition~\ref{def:welfare frequent-t_i} describes the set of polytopes that we take a mixture on.



\begin{definition}\label{def:welfare frequent-t_i}
For any $i, t_i \in \cT_i$ and $\eps>0$, we define the polytopes $W_{t_i},W^{tr(\eps)}_{t_i} \subseteq [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$ as follows: An element{ $\left(x=\left\{x(t'_{ij})\right\}_{t'_{ij}\in \cT_{ij}},y=\left\{y(t'_{ij})\right\}_{t'_{ij}\in \cT_{ij}}\right)\in W_{t_i}$} if there exists a collection of non-negative numbers $\{\sigma_S^{(k)}\}_{S\subseteq [m], k\in [K]}$, such that $\sum_{S \subseteq [m]}\sum_{k \in [K]} \sigma_S^{(k)} \leq 1$,  and for any $j,t_{ij}'\in \cT_{ij}$,
{
\begin{align*}
%&{\pi}_{ij}(t_{ij}')=\sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^{(k)}\cdot \ind[t_{ij}'=t_{ij}]\\
%&{w}_{ij}(t_{ij}')\leq \sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^{(k)}\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}\cdot\ind[t_{ij}'=t_{ij}].
&x(t_{ij}')=\sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^{(k)}\cdot \ind[t_{ij}'=t_{ij}]\\
&y(t_{ij}')\leq \sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^{(k)}\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}\cdot\ind[t_{ij}'=t_{ij}].
\end{align*}
}

%Moreover, an element $(\widehat{\pi}_i,\widehat{w}_i)\in W^{tr(\eps)}_{t_i}$ if there exists $({\pi}_i,{w}_i)\in W^{tr(\eps)}_{t_i}$ such that for any $j,t_{ij}'$,

{Moreover, an element $\left(\hat{x}=\left\{\hat{x}(t'_{ij})\right\}_{t'_{ij}\in \cT_{ij}}, \hat{y}=\left\{\hat{y}(t'_{ij})\right\}_{t'_{ij}\in \cT_{ij}}\right)\in W^{tr(\eps)}_{t_i}$ if there exists $(x,y)\in W_{t_i}$ such that for any $j,t_{ij}'$,
\begin{align*}
\hat{x}(t_{ij}')&=
x(t_{ij}')\cdot\ind[ f_{ij}(t_{ij})\geq \eps]\\
\hat{y}(t_{ij}')&= y(t_{ij}')\cdot\ind[ f_{ij}(t_{ij})\geq \eps]
\end{align*}}
\end{definition}

The following observation directly follows from \Cref{def:W_i} and \Cref{def:welfare frequent-t_i}.

\begin{observation}\label{obs:mix}
$W_{i}$ is a mixture of $\{W_{t_i}\}_{t_i\in \cT_i}$ over distribution $D_i$. For any $\eps>0$, $W_{i}^{tr(\eps)}$ is a mixture of $\{W^{tr(\eps)}_{t_i}\}_{t_i\in \cT_i}$ over distribution $D_i$.
\end{observation}

The following observation is useful in later proofs.

\notshow{
\begin{observation}\label{obs:bound xos mrf}
Let $\widetilde{W}_i$ be a mixture of $\{W_{t_i}\}_{t_i\in \cT_i}$ over distribution $\widetilde{D}_i$.
Then for any $a'\geq a>0$,  $a\widetilde{W}_i\subseteq a' \widetilde{W}_i$
\end{observation}
}
\begin{observation}\label{obs:bound xos mrf}
For any $\eps>0$ and $a'\geq a>0$, $a\cdot W_i\subseteq a'\cdot W_i$ and $a\cdot W^{tr(\eps)}_i\subseteq a'\cdot W^{tr(\eps)}_i$.
\end{observation}

\begin{proof}
Let $c=\frac{a}{a'}\leq 1$. For the first statement, it suffices to prove that $(c\pi_i,cw_i)\in W_i$, for all $(\pi_i,w_i)\in W_i$. Let $\{\sigma_S^{(k)}(t_i)\}_{t_i,S,k}$ be the collection of numbers that satisfy all properties of \Cref{def:W_i}. Then since $c\leq 1$, by considering the collection of numbers $\{c\cdot \sigma_S^{(k)}(t_i)\}_{t_i,S,k}$, we immediately have that $(c\pi_i,cw_i)\in W_i$. For the second statement, let $(\pi_i',w_i')$ be the vector achieved by zeroing out all coordinates $(j,t_{ij})$ where $f_{ij}(t_{ij})<\eps$ for the vector $(\pi_i,w_i)$. By the definition of $W^{tr(\eps)}_i$, we immediately have $(\pi_i',w_i')\in W^{tr(\eps)}_i$ and $(c\pi_i',cw_i')\in W^{tr(\eps)}_i$.
\end{proof}

{We next present several desirable properties of the polytopes we consider here.}
\notshow{
\begin{proof}
For any $(\pi_i,w_i)\in aW^{tr(\eps)}_i$,
there exists for each $t_i\in \cT_i$, $\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)\in W^{tr(\eps)}_{t_i}$ such that
$$
(\pi_i,w_i) = \sum_{t_i\in \cT_i} a \cdot f_i(t_i)\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)
$$
If we show that for each $t_i\in \cT_i$, $\frac{a}{a'} \cdot \left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)\in W^{tr(\eps)}_{t_i}$,
then we have that $(\pi_i,w_i)=\sum_{t_i\in \cT_i} a' \cdot
f_i(t_i)\frac{a}{a'}\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)$,
which implies that $(\pi_i,w_i)\in a'W^{tr(\eps)}_i$.
Fix some $t_i\in \cT_i$ and   consider the numbers $\sigma_S^{(k)}$ for $S\subseteq [m]$, $k\in [K]$ associated with $\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)$ according to Definition~\ref{def:welfare frequent-t_i}. 


Observe that $\frac{a}{a'}\leq 1$ and for each $S\subseteq[m]$ and $k\in [K]$,
we consider the number $\widehat{\sigma}_S^{(k)}=\frac{a}{a'}\sigma_S^k$.
Using Definition~\ref{def:welfare frequent-t_i} with numbers $\{\widehat{\sigma}_S^{(k)}\}_{S,k}$ is enough to show that $\frac{a}{a'} \cdot \left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)\in W^{tr(\eps)}_{t_i}$ which concludes the proof.
\end{proof}
}



%Unfortunately,
%for $t_i\in \cT_i$,
%polytope $W_{t_i}$ is not down-monotone.
%Fortunately enough,
%$W_{t_i}$ has special structure that still enable us to get results similar to that in Section~\ref{sec:multi-approx-polytope}.
%We summarize the important properties of polytope $W_{t_i}$ in Lemma~\ref{lem:W_t_i modify}.


\begin{lemma}\label{lem:W_t_i modify}
For any $t_i\in \cT_i$, any subset of items $B\subseteq[m]$, % and $(\pi_i,w_i)\in W_{t_i}$,
and any {$(x,y)\in W_{t_i}$},
%$(\pi_i,w_i)\in W_{t_i}$ (or for $\eps>0$, $(\pi_i,w_i)\in W^{tr(\eps)}_{t_i}$),
consider any %$(\widehat{\pi}_i,\widehat{w}_i)\in [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$ such that for each $j\in[m]$ and $t_{ij}'\in \cT_{ij}$
{$(\hat{x},\hat{y})\in [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$ }such that for each $j\in[m]$ and $t_{ij}'\in \cT_{ij}$,

{
\begin{align*}
\hat{x}(t_{ij}')= & x(t_{ij}') \ind[j\in B]\quad\text{ and } \quad \hat{y}(t_{ij}')\leq  y(t_{ij}') \ind[j\in B].
%\widehat{w}_{ij}(t_{ij}')\leq w_{ij}(t_{ij}') \ind[j\in B], \quad
%\widehat{\pi}_{ij}(t_{ij}')= & \pi_{ij}(t_{ij}') \ind[j\in B]
\end{align*}}
%then $(\widehat{\pi}_i,\widehat{w}_i)\in W_{t_i}$ (or 
Then $(\widehat{x},\widehat{y})\in W_{t_i}$. {Moreover,  if $(x,y)\in W_{t_i}^{tr(\eps)}$, then $(\hat{x},\hat{y})$ is also in $W_{t_i}^{tr(\eps)}$. Finally, $W_{t_i}^{tr(\eps)}\subseteq W_{t_i}$.}
\end{lemma}

\begin{proof}
%It suffices to prove the case where $\widehat{w}_{ij}(t_{ij}')=w_{ij}(t_{ij}') \ind[j\in B], \forall j, t_{ij}'$, since by \Cref{def:welfare frequent-t_i}, we can decrease any $\widehat{w}_{ij}(t_{ij}')$ while maintaining the vector to be in $W_{t_i}$. 
%We are only going to prove the case where $(\pi_i,w_i)\in W_{t_i}$ over distribution $\widetilde{D}_i$,
%since the other case is similar.

It suffices to prove the case where $\hat{y}(t_{ij}')=y(t_{ij}') \ind[j\in B], \forall j, t_{ij}'$, since by \Cref{def:welfare frequent-t_i}, we can decrease any $\hat{y}(t_{ij}')$ while maintaining the vector $(\hat{x},\hat{y})$ to be in $W_{t_i}$. 

%Since $(\pi_i,w_i)\in W_{t_i}$, let $\{\sigma_S^{(k)}\}_{S\subseteq [m], k\in [K]}$ be the collection of numbers from \Cref{def:welfare frequent-t_i}. Each $\sigma_S^{(k)}$ can be viewed as the probability of the buyer receiving bundle $S$, and enabling the $k$-th additive function. Consider another collection of numbers $\{\widehat{\sigma}_S^{(k)}\}_{S\subseteq [m], k\in [K]}$ by simply discarding items in $[m]\backslash B$. Formally,$\widehat{\sigma}_S^{(k)}=\sum_{T\subseteq [m]\backslash B}\sigma_{S\cup T}^{(k)}, \forall S\subseteq B,k\in [K]$, and $\widehat{\sigma}_S^{(k)}=0$ otherwise. Notice that for every $j\in B$ and $k\in [K]$, $\sum_{S:j\in S} \sigma_S^{(k)}=\sum_{S:j\in S}\widehat{\sigma}_S^{(k)}$. It's not hard to verify that $(\widehat{\pi}_i,\widehat{w}_i)$ and $\{\widehat{\sigma}_S^{(k)}\}_{S,k}$ satisfy all inequalities in \Cref{def:welfare frequent-t_i}. Thus $(\widehat{\pi}_i,\widehat{w}_i)\in W_{t_i}$.

Since $(x,y)\in W_{t_i}$, let $\{\sigma_S^{(k)}\}_{S\subseteq [m], k\in [K]}$ be the collection of numbers from \Cref{def:welfare frequent-t_i}. Each $\sigma_S^{(k)}$ can be viewed as the probability of the buyer receiving bundle $S$, and enabling the $k$-th additive function. Consider another collection of numbers $\{\widehat{\sigma}_S^{(k)}\}_{S\subseteq [m], k\in [K]}$ by simply discarding items in $[m]\backslash B$. Formally, $\widehat{\sigma}_S^{(k)}=\sum_{T\subseteq [m]\backslash B}\sigma_{S\cup T}^{(k)}, \forall S\subseteq B,k\in [K]$, and $\widehat{\sigma}_S^{(k)}=0$ otherwise. Notice that for every $j\in B$ and $k\in [K]$, $\sum_{S:j\in S} \sigma_S^{(k)}=\sum_{S:j\in S}\widehat{\sigma}_S^{(k)}$. It is not hard to verify that $(\hat{x},\hat{y})$ and $\{\widehat{\sigma}_S^{(k)}\}_{S,k}$ satisfy all inequalities in \Cref{def:welfare frequent-t_i}. Thus $(\hat{x},\hat{y})\in W_{t_i}$.

{Now $W_{t_i}^{tr(\eps)}\subseteq W_{t_i}$ follows from choosing $B$ to be $\{j: f_{ij}(t_{ij})\geq \eps \}$. For any $(x,y)\in W_{t_i}^{tr(\eps)}$ and any choice set $B\subseteq [m]$, $(\hat{x},\hat{y})\in W_{t_i}$. Since $\hat{x}(t_{ij}')=
\hat{x}(t_{ij}')\cdot\ind[ f_{ij}(t_{ij})\geq \eps]$
 and $\hat{y}(t_{ij}')= \hat{y}(t_{ij}')\cdot\ind[ f_{ij}(t_{ij})\geq \eps]$. By \Cref{def:welfare frequent-t_i}, $(\hat{x},\hat{y})$ also lies in $W_{t_i}^{tr(\eps)}$.}
\notshow{
Let $\widetilde{\sigma}_S^{(k)}$ be the numbers associated with an arbitrary element $(\widetilde{\pi}_i,\widetilde{w}_i)\in W_{t_i}$ according to Definition~\ref{def:W_i-t_i}.
Notice that $\widetilde{\sigma}_S^{(k)}$ can be viewed as a joint distribution $\widetilde{\cJ}$ over $2^{[m]} \times [K]$,
where for $S\subseteq [m]$ and $k\in[K]$,
we sample element $(S,k)$ with probability $\sigma_S^{(k)}$.
Under this lens, $\widetilde{\pi}_{ij}(t_{ij}')$ is the probability that we allocate the item to the agent $$\widetilde{\pi}_{ij}(t_{ij}')=\ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widetilde{\cJ}}[\ind[j\in S]]=\ind[t_{ij}'=t_{ij}]\Pr_{(S,k)\sim \widetilde{\cJ}}[j\in S]$$
and $\widetilde{w_{ij}}(t_{ij}')$ is a lower bound on the expected contribution to the welfare of the agent when we are able to choose which additive function to activate
$$\widetilde{w_{ij}}(t_{ij}')\leq \ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widetilde{\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right]$$

Let $\cJ$ be the associated joint distribution over $2^{[m]}\times [K]$ of the element $(\pi_i,w_i)$.
We are going to show how to construct distribution $\widehat{\cJ}$ that certifies that $(\widehat{\pi}_i,\widehat{w}_i)\in W_i$.
We consider the distribution $\widehat{\cJ}$ that takes a sample from $2^{[m]}\times [K]$ in the following way:
\begin{enumerate}
    \item First, take a sample $(S,k)\sim \cJ$ and consider the set $\widehat{S}= S \backslash B$.
    %\item For each $j\notin (S \cup B)$, take a sample $p_j$ from a Bernoulli distribution with probability of success $\frac{\widehat{\pi}_{ij}(t_{ij})-\Pr_{(S,k)\sim {\cJ}}[j\in S]}{1-\Pr_{(S,k)\sim {\cJ}}[j\in S]}$. If $p_j=1$, then $\widehat{S}=\widehat{S}\cup \{j\}$. Notice that since $\Pr_{(S,k)\sim {\cJ}}[j\in S]=\pi_{ij}(t_{ij})$, $0 \leq \frac{\widehat{\pi}_{ij}(t_{ij})-\pi_{ij}(t_{ij})}{1-\pi_{ij}(t_{ij})}\leq 1$.
    \item Return $(\widehat{S},k)$.
\end{enumerate}

Now we are going to show that $\widehat{\cJ}$ certifies, that $(\widehat{\pi}_i,\widehat{w}_i)\in W_i$.
Observe that for each $j\in B$,
$$
\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]=0
$$
which implies that for each $j\in B$ and $t_{ij}'\in \cT_{ij}$
$$\ind[t_{ij}'=t_{ij}]\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]= \ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widehat{\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right]=0$$



For each $j\notin B$,
notice that when we take a sample $(\widehat{S},\widehat{k})\sim \widehat{\cJ}$,
the probability that $j\in \widehat{S}$ is equal to the probability that when we take a sample $(S,k)\sim \cJ$, $j\in S$
$$
\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]= \Pr_{(S,k)\sim \cJ}[j\in S] $$
which implies that for each $j\notin B$ and $t_{ij}'\in \cT_{ij}$
$$\ind[t_{ij}'=t_{ij}]\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]=\ind[t_{ij}'=t_{ij}] \widehat{\pi}_{ij}(t_{ij})$$


Moreover, by the construction of $\widehat{\cJ}$ for any $k^*\in[K]$ and $j\notin B$,
notice that
$$
\Pr_{(\widehat{S},\widehat{k})\sim \widehat{\cJ}} \left[\ind[j\in \widehat{S} \land k^*=\widehat{k}]\right] = \Pr_{({S},{k})\sim {\cJ}} \left[\ind[j\in S \land k^*=k]\right]
$$
which implies that for each $j\notin B$ and $t_{ij}'\in \cT_{ij}$
\begin{align*}
\ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widehat{\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right]= &
\ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim {\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right] \\
\geq & \ind[t_{ij}'=t_{ij}]{w_{ij}}(t_{ij}') \\
\geq & \ind[t_{ij}'=t_{ij}]\widehat{w_{ij}}(t_{ij}')    
\end{align*}
which certifies that $(\widehat{\pi}_i,\widehat{w}_i)\in W_{t_i}$.
}
\end{proof}




\notshow{
\begin{proof}
Let $\widetilde{\sigma}_S^{(k)}$ be the numbers associated with an arbitrary element $(\widetilde{\pi}_i,\widetilde{w}_i)\in W_{t_i}$ according to Definition~\ref{def:W_i-t_i}.
Notice that $\widetilde{\sigma}_S^{(k)}$ can be viewed as a joint distribution $\widetilde{\cJ}$ over $2^{[m]} \times [K]$,
where for $S\subseteq [m]$ and $k\in[K]$,
we sample element $(S,k)$ with probability $\sigma_S^{(k)}$.
Under this lens, $\widetilde{\pi}_{ij}(t_{ij}')$ is the probability that we allocate the item to the agent $$\widetilde{\pi}_{ij}(t_{ij}')=\ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widetilde{\cJ}}[\ind[j\in S]]=\ind[t_{ij}'=t_{ij}]\Pr_{(S,k)\sim \widetilde{\cJ}}[j\in S]$$
and $\widetilde{w_{ij}}(t_{ij}')$ is a lower bound on the expected contribution to the welfare of the agent when we are able to choose which additive function to activate
$$\widetilde{w_{ij}}(t_{ij}')\leq \ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widetilde{\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right]$$.

Let $\cJ$ be the associated joint distribution over $2^{[m]}\times [K]$ of the element $(\pi_i,w_i)$.
We are going to show how to construct distribution $\widehat{\cJ}$ that certifies that $(\widehat{\pi}_i,\widehat{w}_i)\in W_i$.
We consider the distribution $\widehat{\cJ}$ that takes a sample from $2^{[m]}\times [K]$ in the following way:
\begin{enumerate}
    \item First, take a sample $(S,k)\sim \cJ$ and consider the set $\widehat{S}= S \backslash B$.
    \item For each $j\notin (S \cup B)$, take a sample $p_j$ from a Bernoulli distribution with probability of success $\frac{\widehat{\pi}_{ij}(t_{ij})-\Pr_{(S,k)\sim {\cJ}}[j\in S]}{1-\Pr_{(S,k)\sim {\cJ}}[j\in S]}$. If $p_j=1$, then $\widehat{S}=\widehat{S}\cup \{j\}$. Notice that since $\Pr_{(S,k)\sim {\cJ}}[j\in S]=\pi_{ij}(t_{ij})$, $0 \leq \frac{\widehat{\pi}_{ij}(t_{ij})-\pi_{ij}(t_{ij})}{1-\pi_{ij}(t_{ij})}\leq 1$.
    \item Return $(\widehat{S},k)$.
\end{enumerate}

Now we are going to show that $\widehat{\cJ}$ certifies, that $(\widehat{\pi}_i,\widehat{w}_i)\in W_i$.
Observe that for each $j\in B$,
$$
\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]=0
$$
which implies that for each $j\in B$ and $t_{ij}'\in \cT_{ij}$
$$\ind[t_{ij}'=t_{ij}]\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]= \ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widehat{\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right]=0$$



For each $j\notin B$,
notice that when we take a sample $(\widehat{S},\widehat{k})\sim \widehat{\cJ}$,
the probability that $j\in \widehat{S}$ is equal to
$$
\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]= \Pr_{(S,k)\sim \cJ}[j\in S] + (1-\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S])\frac{\widehat{\pi}_{ij}(t_{ij})-\Pr_{(S,k)\sim \cJ}[j\in S]}{1-\Pr_{(S,k)\sim {\cJ}}[j\in S]}
= \widehat{\pi}_{ij}(t_{ij})$$
The first term is the probability that when we take a sample $(S,k)\sim \cJ$,
then $j \in S$ and the second term is the probability that $j\notin S$ times $\frac{\widehat{\pi}_{ij}(t_{ij})-\Pr_{(S,k)\sim \cJ}[j\in S]}{1-\Pr_{(S,k)\sim {\cJ}}[j\in S]}$.
Thus if
$j\notin B$,
and for any $t_{ij}'\in \cT_{ij}$
$$\ind[t_{ij}'=t_{ij}]\Pr_{(S,k)\sim \widehat{\cJ}}[j\in S]=\ind[t_{ij}'=t_{ij}] \widehat{\pi}_{ij}(t_{ij})$$


Moreover, by the construction of $\widehat{\cJ}$ for any $k^*\in[K]$ and $j\notin B$,
notice that
$$
\Pr_{(\widehat{S},\widehat{k})\sim \widehat{\cJ}} \left[\ind[j\in \widehat{S} \land k^*=\widehat{k}]\right] \geq \Pr_{({S},{k})\sim {\cJ}} \left[\ind[j\in S \land k^*=k]\right]
$$
which implies that for each $j\notin B$ and $t_{ij}'\in \cT_{ij}$
\begin{align*}
\ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim \widehat{\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right]\geq &
\ind[t_{ij}'=t_{ij}]\E_{(S,k)\sim {\cJ}}\left[\alpha_{ij}^{(k)}(t_{ij})\cdot \ind[j\in S]\right] \\
\geq & \ind[t_{ij}'=t_{ij}]{w_{ij}}(t_{ij}') \\
\geq & \ind[t_{ij}'=t_{ij}]\widehat{w_{ij}}(t_{ij}')    
\end{align*}

\end{proof}
}


\begin{lemma}\label{lem:contain subtypes}
Given any $\eps>0$ and any distribution $\widetilde{D}_i$ over $\cT_i$. Let $\widetilde{W}_i^{tr(\eps)}$ be a mixture of %$\{W_{t_i}\}_{t_i\in \cT_i}$ 
$\left\{W^{tr(\eps)}_{t_i}\right\}_{t_i\in \cT_i}$ over $\widetilde{D}_i$, {that is, $\widetilde{W}_i^{tr(\eps)}:=\sum_{t_i\in\cT_i} \Pr_{s\sim \widetilde{D}_i}[s=t_i] \cdot W^{tr(\eps)}_{t_i}$.} For each $j\in [m]$, let $S_j \subseteq \cT_{ij}$ be any set. For any $(\pi_i,w_i)\in \widetilde{W}_i^{tr(\eps)}$ and any $(\widehat{\pi}_i,\widehat{w}_i)\in [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$ such that for each $j\in[m]$ and $t_{ij}'\in \cT_{ij}$,
\begin{align*}
\widehat{\pi}_{ij}(t_{ij}')=  \pi_{ij}(t_{ij}') \ind[t_{ij}'\in S_j]\quad \text{and} \quad \widehat{w}_{ij}(t_{ij}')\leq  w_{ij}(t_{ij}') \ind[t_{ij}'\in S_j].
\end{align*}
then $(\widehat{\pi}_i,\widehat{w}_i)\in \widetilde{W}_i^{tr(\eps)}$.
\end{lemma}

\begin{proof}
%We are going to prove the case where $\widetilde{W}_i$ is a mixture of $\{W_{t_i}\}_{t_i\in \cT_i}$, because the other case is similar.

It suffices to prove the case where $\widehat{w}_{ij}(t_{ij}')= w_{ij}(t_{ij}') \ind[t_{ij}'\in S_j], \forall j, t_{ij}'$. This is because $\widetilde{W}_i^{tr(\eps)}$ is a mixture of $\{W^{tr(\eps)}_{t_i}\}_{t_i\in \cT_i}$. By \Cref{def:welfare frequent-t_i}, for every $t_i$ and any vector $(x,y)\in W^{tr(\eps)}_{t_i}$, we can decrease any $y(t_{ij}')$ while maintaining the vector $(x,y)$ to be in $W^{tr(\eps)}_{t_i}$. Thus, for any $(\widehat{\pi}_i,\widehat{w}_i)\in \widetilde{W}_i^{tr(\eps)}$, it remains in $\widetilde{W}_i^{tr(\eps)}$ after decreasing any $\widehat{w}_{ij}(t_{ij}')$.  

For each $t_i\in \cT_i$, let $\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)\in W_{t_i}^{tr(\eps)}$ such that $\left(\pi_i,w_i\right) = \sum_{t_i\in \cT_i}\Pr_{s\sim \widetilde{D}_i}\left[s=t_i\right]\cdot\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)$. Consider vector $\left(\widehat{\pi}^{(t_i)}_i,\widehat{w}^{(t_i)}_i\right)$ such that for every $j\in [m]$ and $t_{ij}'\in\cT_{ij}$
$$
\widehat{\pi}^{(t_i)}_{ij}(t_{ij}')=  \pi_{ij}^{(t_i)}(t_{ij}') \ind[t_{ij}\in S_j]\quad \text{and} \quad \widehat{w}_{ij}^{(t_i)}(t_{ij}')=  w_{ij}^{(t_i)}(t_{ij}') \ind[t_{ij}\in S_j].
$$

%Consider the set $B_{t_i}=\{j: t_{ij} \in S_j\}$ and $\{\widehat{w}^{(t_i)}_i\in[0,1]^{\sum_j|\cT_{ij}|}\}_{t_i\in \cT_i}$ such that %for all $t_i \in \cT_i$, $j\in [m]$ and  $t_{ij}\in \cT_{ij}$
%\begin{align*}
%    \widehat{w}^{(t_i)}_{ij}(t_{ij}') \leq& w^{(t_i)}_{ij}(t_{ij}') \qquad \qquad &\forall t_i \in \cT_i, j\in[m],t_{ij}'\in \cT_{ij}\\
%    \sum_{t_i'\in \cT_i:t_{ij}'=t_{ij}}\Pr_{t_i''\sim \widetilde{D}_i}\left[t_i''=t_i'\right] \widehat{w}^{(t_i')}_{ij}(t_{ij}) = &\widehat{w}_{ij}(t_{ij}) &\forall j\in[m], t_{ij}\in \cT_{ij}
%\end{align*}

{For each $t_i \in \cT_i$, define set $B(t_i):=\{j: t_{ij} \in S_j\}$,
by applying Lemma~\ref{lem:W_t_i modify} to  $\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)$ and set $B(t_i)$},
we have that $\left(\widehat{\pi}^{(t_i)}_i,\widehat{w}^{(t_i)}_i \right)\in W_{t_i}^{tr(\eps)}$.

We notice that by \Cref{def:welfare frequent-t_i}, $w_{ij}^{(t_i)}(t_{ij}')=\pi_{ij}^{(t_i)}(t_{ij}')=0$ if $t'_{ij}\not=t_{ij}$. Thus, for every $j\in [m]$ and $t'_{ij}\in \cT_{ij}$, 
$$
\widehat{\pi}^{(t_i)}_{ij}(t_{ij}')=  \pi_{ij}^{(t_i)}(t_{ij}') \ind[t_{ij}'\in S_j] \quad \text{and} \quad \widehat{w}_{ij}^{(t_i)}(t_{ij}')=  w_{ij}^{(t_i)}(t_{ij}') \ind[t_{ij}'\in S_j].
$$
The proof concludes by noticing that $\left(\widehat{\pi}_i,\widehat{w}_i\right) = \sum_{t_i\in \cT_i}\Pr_{s\sim \widetilde{D}_i}\left[s=t_i\right]\cdot\left(\widehat{\pi}^{(t_i)}_i,\widehat{w}^{(t_i)}_i\right)\in \widetilde{W}_i^{tr(\eps)}$.
%The proof follows by applying Lemma~\ref{lem:W_t_i modify} to each $\left(\widehat{\pi}^{(t_i)},\widehat{w}^{(t_i)} \right)$ with set $B=B_{t_i}$ and for each $j\in[m]$ and $t_{ij}\in \cT_{ij}$
\end{proof}

The following corollary follows from Observation~\ref{obs:mix} and Lemma~\ref{lem:W_t_i modify}.
\begin{corollary}\label{obs:contained trauncated xos}
For any $\eps>0$, $W_i^{tr(\eps)}\subseteq W_i$.
\end{corollary}

\begin{proof}
This follows easily from the claim that $W_{t_i}^{tr(\eps)}\subseteq W_{t_i}$ (\Cref{lem:W_t_i modify}).
\end{proof}

\notshow{
\begin{proof}
Let $(\pi_i,w_i)\in W_i^{tr(\eps)}$,
by Observation~\ref{obs:mix} for each $t_i\in \cT_i$, there exists $\left(\pi^{(t_i)}_i,w^{(t_i)}_i\right)\in W_{t_i}^{tr(\eps)}$ such that $(\pi_i,w_i)= \sum_{t_i\in \cT_i}f_i(t_i)\cdot(\pi^{(t_i)}_i,w^{(t_i)}_i)$.
In order to prove the claim,
it suffices to show that $\left( \pi^{(t_i)}_i,w^{(t_i)}_i\right)\in W_{t_i}$. Then $(\pi_i,w_i)\in W_i$ due to Observation~\ref{obs:mix}.


For each $t_i\in \cT_i$,
by Definition~\ref{def:welfare frequent-t_i},
there exists a $\left(\widehat{\pi}^{(t_i)}_i,\widehat{w}^{(t_i)}_i \right)\in W_{t_i}$ such that for each $j\in[m], t_{ij}\in \cT_{ij}$,
\begin{align*}
{\pi}_{ij}^{(t_i)}(t_{ij}) = \widehat{\pi}_{ij}^{(t_i)}(t_{ij})\ind[f_{ij}(t_{ij})\geq \eps],\quad
{w}_{ij}^{(t_i)}(t_{ij}) = \widehat{w}_{ij}^{(t_i)}(t_{ij})\ind[f_{ij}(t_{ij})\geq \eps]
\end{align*}

By applying Lemma~\ref{lem:W_t_i modify} to each $\left(\widehat{\pi}^{(t_i)}_i,\widehat{w}^{(t_i)}_i \right)$ with set $B=\{j\in [m]: f_{ij}(t_{ij})\geq\eps\}$,
we conclude that $\left({\pi}^{(t_i)}_i,{w}^{(t_i)}_i \right)\in W_{t_i}$. Thus $(\pi_i,w_i)\in W_i$. 
\end{proof}
}


Similar to the constrained-additive case, we define the $\eps$-box polytope of $W_i$ for XOS valuations in Definition~\ref{def:welfare rare}. %In Lemma~\ref{lem:welfare rare} we show that a scaled $\eps$-box polytope of $W_i$ is contained in $W_i$.

%We also consider the following polytope:
\begin{definition}\label{def:welfare rare}
%Let $T_i = \sum_{j\in[m]}|\cT_{ij}|$. \mingfeinote{Replace it by $T = \sum_{i,j}|\cT_{ij}|$.}
For $\eps>0$,
we denote as $W_i^{box(\eps)}\subseteq [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$ the $\eps$-box polytope of $W_i$: $(\pi_i,w_i)\in W_i^{box(\eps)}$ if and only if for every $j\in[m]$ and  $t_{ij}\in \cT_{ij}$ it holds that
\begin{align*}
    0 \leq w_{ij}(t_{ij}) \leq \pi_{ij}(t_{ij}) \leq \min(\eps,f_{ij}(t_{ij}))
\end{align*}
\end{definition}

\notshow{
I don't think they are no longer needed

\begin{observation}\label{obs:W_i(t_i) null}
Let $\textbf{0}$ be the vector with 0 in all entries. For any $t_i$ and $\pi_i\in [0,1]^{M_i}$such that $\pi_{ij}(t_{ij}')\leq \ind[t_{ij}'=t_{ij}]$, $(\pi_i,\textbf{0})\in W_{t_i}$. 
\end{observation}

\begin{proof}
We are going to choose numbers $\{\sigma_S^k\}_{S\subseteq[m],k\in[K]}$ and use Definition~\ref{def:welfare frequent-t_i} to prove the statement.

We are going to choose numbers $\{\sigma_S^k(t_i)\}_{t_i\in \cT_i,S\subseteq[m],k\in[K]}$ and use Definition~\ref{def:welfare frequent-t_i} to prove the statement.
Fix a $k^*\in [K]$ (the choice of $k^*$ is not going to matter in our proof).
For each $S\subseteq [m]$ and $k\in[K]$
$$
\sigma_S^{k} = \prod_{j\in S}\pi_{ij}(t_{ij}) \prod_{j\notin S}(1-\pi_{ij}(t_{ij}))
\ind[k=k^*]$$
Now we are going to prove the first property in Definition~\ref{def:welfare frequent-t_i}.
Notice that
$$
\sum_{S\subseteq[m]}\sum_{k\in[K]}\sigma_S^{k} =
\sum_{S\subseteq[m]}\sigma_S^{k^*} =\sum_{S\subseteq[m]} \prod_{j\in S}\pi_{ij}(t_{ij})\prod_{j\notin S}(1-\pi_{ij}(t_{ij}))
$$
Consider a random variables $C_j$ that is sampled from a Bernoulli Distribution, with probability of success $0\leq \pi_{ij}(t_{ij})\leq 1$.
Then $\prod_{j\in S}\pi_{ij}(t_{ij})\prod_{j\notin S}(1-\pi_{ij}(t_{ij}))$ 
is equal to the probability that for each $j\in S$, $C_j=1$ and for $j\notin S$, $C_j=0$,
which implies that $\sum_{S\subseteq[m]} \prod_{j\in S}\pi_{ij}(t_{ij})\prod_{j\notin S}(1-\pi_{ij}(t_{ij}))= 1$.

Now we prove that $\sigma$ satisfied the second property of Definition ~\ref{def:welfare frequent-t_i}.
For each $j\in[m]$,
observe that 
\begin{align*}
\sum_{ S: k \in S}\sum_{k\in[K]}\sigma_S^{k} =&
\sum_{S:j\in S}\sigma_S^{k^*} \\ =& \pi_{ij}(t_{ij})\sum_{S: j \in S} \prod_{j'\in S \land j'\neq j}\pi_{ij'}(t_{ij'})
\prod_{j'\notin S}(1-\pi_{ij'}(t_{ij'})) \\
=& \pi_{ij}(t_{ij})
\end{align*}

where the last equality follows by considering random variable $C_j$ as described above.
Then for $S:j \in S$, $\prod_{j'\in S\land j'\neq j}\pi_{ij'}(t_{ij'})\prod_{j'\notin S}(1-\pi_{ij'}(t_{ij'}))$ 
is equal to the probability that for each $j\in S\backslash\{j\}$, $C_j=1$ and for $j\notin S$, $C_j=0$,
which implies that $\sum_{S: j \in S} \prod_{j'\in S \land j'\neq j}\pi_{ij'}(t_{ij'})
\prod_{j'\notin S}(1-\pi_{ij'}(t_{ij'}))= 1$.


The third property of Definition~\ref{def:welfare frequent-t_i} follow trivially since the LHS is $0$.
\end{proof}

A corollary of Observation~\ref{obs:W_i(t_i) null} is the following.
\begin{corollary}\label{obs:W_i(t_i)-1}
Let $\textbf{0}$ be the vector with 0 in all entries. For any $t_i$ and $\pi_i\in [0,1]^{M_i}$such that $\pi_{ij}(t_{ij}')\leq \ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij})\geq \eps]$, $(\pi_i,\textbf{0})\in W_{t_i}^{tr(\eps)}$. 
\end{corollary}

\begin{proof}
We Choosing $\sigma_{S}^k=0$ for all $S,k$ finishes the proof.
\end{proof}


%We also consider the following polytope:
\begin{definition}\label{def:welfare rare}
%Let $T_i = \sum_{j\in[m]}|\cT_{ij}|$. \mingfeinote{Replace it by $T = \sum_{i,j}|\cT_{ij}|$.}
For $\eps>0$,
we denote as $W_i^{box(\eps)}\subseteq [0,1]^{2M_i}$ the $\eps$-box polytope of $W_i$,
such that $(\widehat{\pi}_i,\widehat{w}_i)\in W_i^{box(\eps)}$ if and only if for every $j\in[m]$ and  $t_{ij}$ it holds that
\begin{align*}
    0 \leq w_{ij}(t_{ij}) \leq \pi_{ij}(t_{ij}) \leq \cdot\min(\eps,f_{ij}(t_{ij}))
\end{align*}
\end{definition}


%where we denote by $\pi_S$ the probability that we award exactly bundle $S$ to the agent.




Clearly the first polytope $W_i^{tr(\eps)}\subseteq W_i$. 
We prove in the following lemma that the second polytope $\left(1-\eps \cdot M_i \right) W_i^{box(\eps)} \subseteq W_i, \forall \eps<\nicefrac{1}{M_i}$. 

}
\notshow{
\begin{observation}\label{obs:box within a box}
For any $\eps>0$ and $a'\geq a >0$,
$a W_i^{box(\eps)}\subseteq a' W_i^{box(\eps)}$
\end{observation}
}

The following lemma is similar to \Cref{lem:box polytope constraint additive}. 

\begin{lemma}\label{lem:welfare rare}
Let $T =\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$, then $\left(1-\eps \cdot T \right) W_i^{box(\eps)} \subseteq  W_i$, for all $\eps < \nicefrac{1}{T}$.
\end{lemma}
\begin{proof}

For any $(\pi_i,w_i)\in W_i^{box(\eps)}$, we will prove that $(\pi_i,\pi_i)\in W_i$. Then $(\pi_i,w_i)\in W_i$ since $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})$ for any $j,t_{ij}$.

To prove $(\pi_i,\pi_i)\in W_i$, we consider the following set of numbers $\{\sigma_{S}^{(k)}(t_i)\}_{t_i,S,k}$ (see \Cref{def:W_i}): For each $j\in [m], t_{ij}\in \cT_{ij}$, let $c_j(t_{ij})=\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right)$ and
$$p_j(t_{ij})=\frac{\pi_{ij}(t_{ij})}{f_{ij}(t_{ij})\cdot \sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))}.$$ 

{Note that for every $j'\in[m]$, there exists a  $t_{ij'}\in\cT_{ij'}$ such that $f_{ij'}(t_{ij'})\geq 1/|\cT_{ij'}|$. Due to our choice of $\eps$, the corresponding $c_{j'}(t_{ij'})<1$. Hence, $\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))>0$, and $p_j(t_{ij})$  is well-defined.}

For every $t_i$, define~\footnote{When there are two indices $k,k'\in [K]$ such that $k,k^*\in \argmax_{k'}\alpha_{ij}^{(k')}(t_{ij})$, we break ties in lexicographic order.}
\begin{align*}
\sigma_{S}^{(k)}(t_i)=
\begin{cases}
p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'})), &\text{if } S=\{j\} \text{ and } k=\argmax_{k'}\alpha_{ij}^{(k')}(t_{ij})\\
0, &\text{o.w.}
\end{cases}
\end{align*}

For every $j$, let $C_j(t_{ij})$ be the independent Bernoulli random variable that activates with probability $c_j(t_{ij})$. Then for every $j$, 
$$
\Pr_{C_j(t_{ij}), t_{ij}\sim D_{ij}}\left[C_j(t_{ij})=1\right] \leq \sum_{t_{ij}\in \cT_{ij}} f_{ij}(t_{ij})\cdot\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right) \leq \eps \cdot |\cT_{ij}|
$$
By the union bound,
$$\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))=\Pr_{\substack{t_{i,-j}\sim\cD_{i-j}\\ \forall j' \neq j, C_{j'}(t_{ij'})}}[C_{j'}(t_{ij'}) =0,\forall j'\not=j]\geq 1-\sum_j\Pr[C_j(t_{ij})=1]\geq 1-\eps\cdot T$$

Now we prove that $(\pi_i,\pi_i)\in W_i$ by verifying all three conditions in \Cref{def:W_i}. For the first condition, since $(\pi_i,w_i)\in (1-\eps T)W_i^{box(\eps)}$, $0 \leq w_{ij}(t_{ij}) \leq \pi_{ij}(t_{ij}) \leq \left(1-\eps \cdot T \right)\cdot f_{ij}(t_{ij})\cdot c_j(t_{ij})$. Thus $p_j(t_{ij})\leq 1$ for every $j,t_{ij}$. We have that $\sum_{S,k}\sigma_S^{(k)}(t_i)=\sum_jp_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))\leq \sum_j c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))$. We notice that $\sum_j c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))$ is exactly the probability that there exists a unique $C_j(t_{ij})=1$. Thus $\sum_{S,k}\sigma_S^{(k)}(t_i)\leq 1$ for all $t_i\in \cT_i$.

The second condition: 
\begin{align*}
&f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\\
=&f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))=\pi_{ij}(t_{ij})
\end{align*}

The third condition:
\begin{align*}
&f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}\\
=&f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))\cdot \frac{\max_k\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}=\pi_{ij}(t_{ij})
\end{align*}

By \Cref{def:W_i}, $(\pi_i,\pi_i)\in W_i$. Thus, $(\pi_i,w_i)\in W_i$.
\end{proof}

\vspace{.2in}

Similar to \Cref{lem:boxable polytope contained}, we prove in the following lemma that
%for $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$ we try to approximate polytope $\frac{1}{2}W_i^{tr(\eps)} + \frac{1-\eps T}{2}W_i^{box(\eps)}$.
%We prove in the following lemma that the mentioned polytope,
%contains a multiplicative factor of $W_i$.
$W_i$ can be approximated by the polytope $\frac{1}{2}W_i^{tr(\eps)} + \frac{1-\eps T}{2}W_i^{box(\eps)}$ within a multiplicative factor.

\begin{lemma}\label{lem:xos mrf contain}
Let $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$ and any $0\leq \eps<\frac{1}{T}$, then $$\frac{1-\eps T}{2}W_i \subseteq \frac{1}{2}W_i^{tr(\eps)} + \frac{1-\eps T}{2}W_i^{box(\eps)} \subseteq  W_i.$$
\end{lemma}
\begin{proof}
Let $W'=\frac{1}{2}W_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W_{i}^{box(\epsilon)}$. Then $W'\subseteq  W_i$ directly follows from Corollary~\ref{obs:contained trauncated xos} and Lemma~\ref{lem:welfare rare}. We are going to show that for each $(\pi_i,w_i) \in \frac{1-\eps \cdot T}{2}\cdot W_i$, $(\pi_i,w_i) \in W'$. We consider the following vector $(\pi_{i}^{tr}, w_{i}^{tr})$ such that for every $j\in [m], t_{ij}\in \cT_{ij}$,
\begin{align*}
\pi_{ij}^{tr}(t_{ij})=
\pi_{ij}(t_{ij})\ind[f_{ij}(t_{ij})\geq \eps], \qquad
w_{ij}^{tr}(t_{ij})=
w_{ij}(t_{ij})\ind[f_{ij}(t_{ij})\geq \eps]
\end{align*}
Then by \Cref{def:welfare frequent} and Observation~\ref{obs:bound xos mrf}, $(\pi_{i}^{tr}, w_{i}^{tr})\in \frac{1-\eps\cdot T}{2}W_{i}^{tr(\eps)}\subseteq \frac{1}{2}W_{i}^{tr(\eps)}$. Consider the vector $(\pi_{i}^{box}, w_{i}^{box})$ such that
\begin{align*}
\pi_{ij}^{box}(t_{ij})=
\pi_{ij}(t_{ij})\ind[f_{ij}(t_{ij})< \eps] , \qquad
w_{ij}^{box}(t_{ij})=
w_{ij}(t_{ij})\ind[f_{ij}(t_{ij}) < \eps]
\end{align*}
For every $j\in [m], t_{ij}\in \cT_{ij}$, since $(\pi_i,w_i)\in \frac{1-\eps \cdot T}{2}\cdot W_i$, by \Cref{obs:W_i-upper-bound} we have $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})\leq \frac{1-\eps \cdot T}{2}\cdot f_{ij}(t_{ij})$. Thus $w_{ij}^{box}(t_{ij})\leq \pi_{ij}^{box}(t_{ij})\leq \frac{1-\eps \cdot T}{2}\cdot f_{ij}(t_{ij})\cdot \ind[f_{ij}(t_{ij})<\eps]\leq \frac{1-\eps \cdot T}{2}\cdot \min(f_{ij}(t_{ij}),\eps)$. Thus $(\pi_{i}^{box}, w_{i}^{box})\in \frac{1-\eps T}{2}W_{i}^{box(\eps)}$. Now observe that $(\pi_i,w_i) = (\pi^{tr}_i + \pi^{box}_i,w^{tr}_i + w^{box}_i)\in \frac{1}{2}W_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W_{i}^{box(\eps)}$,
which concludes the proof.
\end{proof}


\subsection{Approximating the Single-Bidder Marginal Reduced Form Polytope}

In this section we provide the important step that allows us to prove \Cref{thm:main XOS}. In the constrained-additive case (\Cref{thm:multiplicative approx for constraint additive-main body}), we construct (with high probability) another polytope $\widehat{W}_i$ such that (i) $c\cdot W_i\subseteq \widehat{W}_i\subseteq W_i$ for some absolute constant $c>0$, and (ii) we have an efficient separation oracle for $\widehat{W}_i$. The proof heavily relies on the fact that $W_i$ is down-monotone and thus cannot be easily extended  to the single-bidder marginal reduced form polytope $W_i$ in the XOS case. Here we prove a similar statement with a weaker version of property (i): For every vector $x$ in $W_i$, there exists another vector $x'$ in $\widehat{W}_i$ such that for every coordinate $j$, $x_j/x_j'\in [a,b]$ for some absolute constant $0<a<b$, and vice versa. It's not hard to see that the original property (i) directly implies this weaker version. A formal statement is shown in \Cref{cor:rfs for xos mult}.


\begin{theorem}\label{cor:rfs for xos mult}
Let $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance (\Cref{def:bit complexity}). For any $i\in [n]$ and $\delta>0$, there is an algorithm that constructs a convex polytope $\widehat{W}_i\in [0,1]^{2\cdot\sum_{j\in [m]}|\cT_{ij}|}$ using $\poly(n,m,T,\log(1/\delta))$ samples from $D_i$, such that with probability at least $1-\delta$ all of the following are satisfied:
%Consider parameters $0 < \eps < 1/T$, $\delta\in (\eps T,1)$ and
%Consider integer $k\geq \Omega\left( T^4\left( Tb+\log\left(T\right)\right) \right)$.
%If we have access to 
%$\Omega(kT^3)$ independent samples from $\cD$,
%then with probability at least $1-2T\exp(-2T k)$,
%we can construct a polytope $\widehat{W}_i$


\begin{enumerate}
    \item For each $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$,
there exists a $(\pi_i,w_i) \in W_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:

$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{3}{2}\right],\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$$


\item For each $(\pi_i,w_i) \in W_{i}$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:


$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{16},\frac{3}{8}\right],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{16},\frac{5}{16}\right]$$


\item The vertex-complexity (\Cref{def:vertex-complexity}) of $\widehat{W}_i$ is $\poly(n,m,T,b,\log(1/\delta))$. 

\item There exists a separation oracle $SO$ for $\widehat{W}_i$, given access to the value oracle and an adjustable demand oracle (\Cref{def:adjustable demand oracle}) of buyer $i$'s valuation. The running time of $SO$ on any input with bit complexity $b'$ is $\poly(n,m,T,b,b',\log(1/\delta))$ and makes $\poly(n,m,T,b,b',\log(1/\delta))$ queries to both oracles.
%Given access to an adjustable demand oracle $\dem_i(\cdot,\cdot,\cdot)$ and a value oracle $\val_i(\cdot,\cdot)$,
%we can construct a separation oracle $SO$ for $\widehat{W}_i$.
%The running time of $SO$ on any input with bit complexity $b'$ is $\poly\left(b,b',T,\log(1/\delta)\right)$ and perform $\poly\left(b,b',T,\log(1/\delta)\right)$ queries to $\dem_i,\val_i$ with input of bit complexity at most $\poly\left(b,b',T,\log(1/\delta)\right)$.
\end{enumerate}

The algorithm constructs the polytope and the separation orcle $SO$ in time %$\poly(n,m,T,\log(1/\delta))$ 
$\poly(n,m,T,b,\log(1/\delta))$.
\end{theorem}



\subsubsection{Efficiently Optimizing over the Polytope}
%Our final objective is not only to construct a polytope that is in a multiplicative sense close to $W_i$,
%but to also be able to have an efficient separation oracle for it.
%Similar to Section~\ref{sec:multi-approx-polytope},
%we are going to show how to optimize over the constructed polytope.
%As in the proof of Theorem~\ref{thm:special case of multiplicative approx},
%one important requirement is to be able to efficiently optimize over the set of polytopes that $W_i$ is a mixture of.
%In Observation~\ref{obs:mix} we show how we can write polytope $W_i$ as a mixture of polytopes.
%In Observation~\ref{obs:bit complexity mrf xos} and 
%Lemma~\ref{lem:optimize} describe the bit complexity of corners and the optimal solutions over polytopes in $\{W_{t_i}\}_{t_i\in \cT_i}$ and how we can use the adjustable demand oracle in a creative way to optimize over them.

Both \Cref{obs:bit complexity mrf xos} and \Cref{lem:optimize} are useful to show that there exists an efficient separation oracle for our constructed polytope.

In \Cref{lem:optimize}, we show that given access to the adjustable demand oracle and the value oracle, we can optimize any linear objective over the polytope $W_{t_i}^{tr(\eps)}$ (\Cref{def:welfare frequent-t_i}).

\begin{lemma}\label{lem:optimize}
Let $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$,
and $b$ be the bit complexity of the instance.
%let $b$ be the bit complexity of any element in $\{\alpha^{(k)}_j(t_{ij})\}_{j\in[m],k\in[K]}$.
For any $t_i\in \cT_i$ and any $\eps>0$, given access to the adjustable demand oracle $\adem_i(\cdot,\cdot,\cdot)$ and the value oracle for buyer $i$'s valuation $v_i(\cdot,\cdot)$, there exists an algorithm that takes arbitrary $\bm{x},\bm{y}\in \mathbb{R}^{\sum_j|\cT_{ij}|}$ as input and finds $$(\pi_i^*,w_i^*)\in \text{argmax}_{(\pi_i,w_i)\in W_{t_i}^{tr(\eps)}}\bm{x}\cdot \pi_i+ \bm{y}\cdot w_i.$$ The algorithm runs in time $poly(n,m,T,b,b',1/\eps)$ and makes $O(m)$ queries to both oracles, where $b'$ is the bit complexity of $(\bm{x},\bm{y})$. Moreover the bit complexity of $(\pi_i^*,w_i^*)$ is at most $O(b T)$.
%Similarly for any $\eps>0$,
%we can find an element $(\widehat{\pi}^{tr}_i,\widehat{w}^{tr}_i)\in W_{t_i}^{tr(\eps)}$ such that  $(\widehat{\pi}^{tr}_i,\widehat{w}^{tr}_i)\in \text{argmax}\{\textbf{a}'\cdot w_i:w_i\in W_{t_i}^{tr(\eps)}\}$ and the bit complexity of $(\widehat{\pi}^{tr},\widehat{w}^{tr})$ is at most $O(b T)$.
\end{lemma}

\begin{proof}
%By equivalence of separation and optimization,
%it is enough to design an optimization algorithm over linear objectives for polytope $\mathcal{P}'_k$.
%Since $\mathcal{P}'_k$ is the Minkowski addition of at most $k$ polytopes in $\{W_t\}_{t\in T}$,
%it is enough to design an optimization algorithm for linear objectives for each polytope $W_t$, where $t \in T$.
We are going to solve the problem:
\begin{align*}
    \max&\quad \bm{x}\cdot \pi_i + \bm{y}\cdot w_i \\
    s.t.&\quad (\pi_i,w_i) \in W_{t_i}^{tr(\eps)}
\end{align*}
By \Cref{def:welfare frequent-t_i}, $\pi_{ij}(t_{ij}')=w_{ij}(t_{ij}')=0$ if $t_{ij}'\not=t_{ij}$ or $f_{ij}(t_{ij})<\eps$. Let $Q=\{j\in[m]: f_{ij}(t_{ij})\geq \eps\}$. Then according to \Cref{def:welfare frequent-t_i}, the problem is equivalent to
\begin{align*}
  (O_1)\quad   \max &\sum_{j\in Q}\left( x_j(t_{ij})\cdot \pi_{ij}(t_{ij}) + y_j(t_{ij})\cdot w_{ij}(t_{ij})  \right)\\
    s.t.& \sum_{S\subseteq [m]}\sum_{k\in[K]}\sigma_S^{(k)} \leq 1 \\
    & \pi_{ij}(t_{ij}) = \sum_{S:j\in S}\sum_{k\in[K]}\sigma_S^{(k)} \quad &\forall j\in[m] \\
    &0\leq w_{ij}(t_{ij}) \leq \sum_{S:j\in S}\sum_{k\in[K]}\sigma_S^{(k)} \frac{\alpha^{(k)}_{ij}(t_{ij})}{V_{ij}(t_{ij})} &\forall j\in[m] \\
    &\sigma_S^{(k)}\geq 0  &\forall S\subseteq [m], k\in[K]
\end{align*}

We notice that at the maximum, $w_{ij}(t_{ij})$ must be equal to $\sum_{S:j\in S}\sum_{k\in[K]}\sigma_S^{(k)} \frac{\alpha^{(k)}_{ij}(t_{ij})}{V_{ij}(t_{ij})}$ if $y_j(t_{ij})>0$, and $0$ otherwise. $(O_1)$ is equivalent to (denote $y_j(t_{ij})^+=\max\{y_j(t_{ij}),0\}$):
\begin{align*}
    (O_2)\quad\max &\sum_{j\in Q}\left( x_j(t_{ij})\cdot \pi_{ij}(t_{ij}) + y_j(t_{ij})^+\cdot w_{ij}(t_{ij})  \right)\\
    s.t.& \sum_{S\subseteq [m]}\sum_{k\in[K]}\sigma_S^{(k)} \leq 1 \\
    & \pi_{ij}(t_{ij}) = \sum_{S:j\in S}\sum_{k\in[K]}\sigma_S^{(k)} \quad &\forall j\in[m] \\
    &w_{ij}(t_{ij}) = \sum_{S:j\in S}\sum_{k\in[K]}\sigma_S^{(k)} \frac{\alpha^{(k)}_{ij}(t_{ij})}{V_{ij}(t_{ij})} &\forall j\in[m]\\
    &\sigma_S^{(k)}\geq 0  &\forall S\subseteq [m], k\in[K]
\end{align*}
%which is equivalent to a solution of
%Notice that in order to find an optimal solution of program $(O_1)$, it is enough to find a solution to program $(O_2)$

%\begin{align*}
%    (O_2)\quad \max &\sum_{j\in[m]}\left( x_j(t_{ij})\cdot \sum_{S:j\in S}\sum_{k\in[K]}\sigma_S^k + y_j(t_{ij})^+\sum_{S:j\in S}\sum_{k\in[K]}\sigma_S^k \frac{\alpha^{(k)}_{ij}(t_{ij})}{V_{ij}(t_{ij})}  \right)\\
%    s.t.& \sum_{S\subseteq [m]}\sum_{k\in[K]}\sigma_S^k \leq1 \\
%    &\sigma_S^k\geq 0  \qquad \qquad \qquad \qquad \qquad S\subseteq [m], k\in[K]
%\end{align*}
or equivalently
%Thus in order to identify a solution of $(O_1)$,
%it is enough to identify parameters $\{\widehat{\sigma}_S^k\}_{S,k}$ of Program $(O_2)$
\begin{align*}
   (O_3)\quad \max &\sum_{S\subseteq [m]} \sum_{k\in[K]}  \sigma_S^{(k)}\left(\sum_{j\in S\cap Q}\left( y_j(t_{ij})^+\frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})} + x_j(t_{ij})\right) \right)\\
    s.t.& \sum_{S\subseteq [m]}\sum_{k\in[K]}\sigma_S^{(k)} \leq 1 \\
    &\sigma_S^{(k)}\geq 0  \qquad \qquad \qquad \qquad \qquad S\subseteq [m], k\in[K]
\end{align*}

%Note that in order to identify the values of $\{\widehat{\sigma}_S^k\}_{S,k}$ of the program above,
%it is enough to identify the value of $S^*\subseteq [m]$ and $k^*\in [K]$ such that
%that maximize $\sum_{j\in S}\left( c_{w}(t_{ij})^+\frac{\alpha_j^{(k)}(t_j)}{V_j(t_j)} + c_{\pi}(t_{ij})\right)$.
%Consider the Program $(O)$. 

Clearly, to solve $(O_3)$, it suffices to find $S^*\subseteq Q$ and $k^*\in [K]$ that lies in $$\argmax_{S\subseteq Q, k\in[K]}\sum_{j\in S}\left(y_j(t_{ij})^+\cdot\frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})} + x_j(t_{ij})\right).$$
%\begin{align*}
%    (O_3)\quad (S^*,k^*)=\argmax_{S\subseteq [m], k\in [K]} &\sum_{j\in S}\left( c_{w}(t_{ij})^+\frac{\alpha_j^{(k)}(t_j)}{V_j(t_j)} + c_{\pi}(t_{ij})\right) 
%\end{align*}
We notice that since $y_j(t_{ij})^+\cdot\frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}\geq 0$ for every $j,k$, thus $j\in S^*$ for every $j$ such that $x_j(t_{ij})\geq 0$. Consider the vector $\textbf{b}\in \mathbb{R}^m_+$ and $\textbf{p}\in \mathbb{R}^m_+$ such that for each $j\in[m]$,
\begin{align*}
b_j=\frac{y_j(t_{ij})^+}{V_{ij}(t_{ij})},\quad
p_j =
\begin{cases}
-x_j(t_{ij})\ind[x_j(t_{ij})<0], & j\in Q\\
\infty, & j\not\in Q
\end{cases}
\end{align*}

Then $(S^*,k^*)\in \argmax\sum_{j\in S}\left( b_j\alpha_{ij}^{(k)}(t_{ij}) - p_j \right)$%\todo{Yang: If $x_j>0$ but $y_j^+=0$, the adjustable demand oracle may or may not include $j$. An easy fix is to allow negative prices and set $p_j$ to be $-x_j$.}
, which can be achieved by a single query to the adjustable demand oracle with input $(t_i,\textbf{b},\textbf{p})$. Now the corresponding vector $(\pi_i^*,w_i^*)$ can be computed according to $(O_2)$, with $\sigma_S^{(k)}=\ind[S=S^*\cup S_{+} \land k=k^*]$, where $S_{+}:=\{j\in[m]: x_{j}(t_{ij})>0\}$. ~\footnote{Both $\alpha^{(k^*)}_{ij}(t_{ij})$ and $V_{ij}(t_{ij})=\max_{k}\alpha^{(k)}_{ij}(t_{ij})$ can be computed with $O(1)$ queries to the adjustable demand oracle.}
%\argyrisnote{Argyris: I think this is one way to fix. I was thinking about considering $S_+=\{j\in[m]: x_j>0 \wedge y_j^+=0\}$ and $\sigma_S^{(k)}=\ind[S=S^*\cup S_+ \wedge k=k^*]$. What do you think? With this way, we de not have to change the definition} \yangnote{Yang: We need to define $S_+$ as $\{\}$}

\notshow{

Let $(S^*,k^*)$ be the optimal solution of $(O_3)$.
Note that the solution $\widehat{\sigma}_{S}^{k}=\ind[S=S^*\land k=k^*]$ is an optimal solution of $(O_2)$.
%Thus it is enough to identify the value of $S^*\subseteq [m]$ and $k^*\in[K]$ of 
%Let $S^*,k^*= {\arg\max}_{S\subseteq [m], k\in [K]} \sum_{j\in S}\left( c_{w}(t_{ij})^+\frac{\alpha_j^k(t_j)}{V_j(t_j)} + c_{\pi}(t_{ij})\right)$ and $S_\pi= \{j\in[m]: c_\pi(t_{ij}) > 0\}$.
Consider the set $S_\pi=\{j\in [m]: c_\pi(t_{ij})>0\}$ and the following program
\begin{align*}
(O_4)  \quad  {\arg\max}_{S\subseteq [m], k\in [K]} &\sum_{j\in S}\left( \frac{c_{w}(t_{ij})^+}{V_j(t_j)}\alpha_j^{(k)}(t_j) + c_{\pi}(t_{ij})\ind[c_{\pi}(t_{ij}) \leq 0]\right)
\end{align*}


Let $(S^*,k^*)$ be the optimal solution of $(O_4)$.
Observe that $(S^*\cup S_\pi,k^*)$ is an optimal solution of $(O_3)$.
Consider the vector $\textbf{b}\in \mathbb{R}^m_+$ and $\textbf{p}\in \mathbb{R}^m_+$ such that for each $j\in[m]$.
\begin{align*}
\textbf{b}_j =& \frac{c_w(t_{ij})^+}{V_{ij}(t_{ij})}\\
\textbf{p}_j =& -c_{\pi}(t_{ij})\ind[c_{\pi}(t_{ij})\leq 0]
\end{align*}

Observe we can rewrite Program $(O_4)$

\begin{align*}
(O_5)  \quad  {\arg\max}_{S\subseteq [m], k\in [K]} &\sum_{j\in S}\left( \textbf{b}_j\alpha_j^{(k)}(t_j) - \textbf{p}_j \right)
\end{align*}



Also observe that we can find $(S^*,k^*)$ by a querying a scalable demand oracle with input $\dem(t_i,\textbf{b},\textbf{p})$.
Given our reasoning above,
having values $(S^*,k^*)$ that optimize Program $(O_5)$,
we can find $(\pi^*_i,w_i^*)\in W_i$ that maximizes Program $(O_1)$,
where
\begin{align*}
\pi_{ij}^*(t_{ij}') =& \ind[t_{ij}'=t_{ij}\land j\in S_\pi \cup S^*] \\
w_{ij}^*(t_{ij}') =& \frac{\alpha_{ij}^{(k^*)}(t_{ij}')}{V_{ij}(t_{ij}')}\ind[t_{ij}'=t_{ij}\land j\in S^*]
\end{align*}
where we can calculate the values of $\alpha^{(k^*)}_{ij}(t_{ij})$ and $V_{ij}(t_{ij})=\max_{k}\alpha^{(k)}_{ij}(t_{ij})$ by one more call to the adjastuble demand oracle and two accesses to value oracles.
The bit complexity of each coordinate of $(\pi_i^*,w_i^*)$ is at most $O(b)$,
which implies that the bit complexity of $(\pi_i^*,w_i^*)$ is at most $O(b T)$.

We can similarly calculate 
\begin{align*}
    \arg\max_{(\pi,w)} c_\pi^T\pi^{tr} + c_w^T w^{tr} \\
    s.t.: (\pi^{tr},w^{tr}) \in W^{tr(\eps)}_{t_i}
\end{align*}

}


Finally, the bit complexity of each coordinate of $(\pi_i^*,w_i^*)$ is at most $O(b)$,
which implies that the bit complexity of $(\pi_i^*,w_i^*)$ is at most $O(b T)$.
\end{proof}

\begin{corollary}\label{obs:bit complexity mrf xos}
Let $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$ and $b$ be the bit complexity of the instance.
For any $t_i\in \cT_i$, %both $W_{t_i}$ and
$W_{t_i}^{tr(\eps)}$ has vertex-complexity $O(bT)$. 

%the bit complexity of corners in $W_{t_i}^{tr(\eps)}$ is at most the bit complexity of the corners in $W_{t_i}$.
%Let $b$ be the bit complexity of any element in $\{a^k_j(t_{ij})\}_{j\in[m],k\in[K]}$.
%Moreover the bit complexity of corners in $W_{t_i}$ is $O(b T)$.
\end{corollary}



\subsubsection{Proof of \Cref{cor:rfs for xos mult}}


\notshow{
\begin{theorem}\label{thm:multi-approx-mixture}
Let $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance (\Cref{def:bit complexity}).
%Let $b$ be an upper bound on the bit complexity of any element in $\{\alpha^k_j(t_{ij})\}_{j\in[m],t_{ij}\in \cT_{ij},k\in[K]}$.
Consider parameters $0 < \eps \leq 1/T$, $\eta\in (\eps T,1)$ \argyrisnote{Argyris: I think we only need that $\eta \in [0,1]$ now    } and
integer $k\geq \Omega\left( T^4\left( Tb+\log\left(\frac{1}{\eta \eps}\right)\right) \right)$.
If we have access to $n=\left\lceil\frac{8kT}{(\eta\eps)^2}\right\rceil$ independent samples from $\cD$,
then with probability at least $1-2T\exp(-2T k)$,
we can construct a polytope $\widehat{W}_i$ such that

\begin{enumerate}
    \item For each $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$,
there exists a $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:

$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{2}-\frac{\max\left(\eps\cdot  T,\eta\right)}{2}, \frac{3}{2}+\frac{\eta}{2}\right],\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{2}-\frac{\max\left(\eps\cdot  T,\eta\right)}{2} ,1+\frac{\eta}{2}\right]$$


\item For each $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:


$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{2}-\frac{\max\left(\eps\cdot  T,\eta\right)}{2}, \frac{3}{2}+\frac{\eta}{2}\right],
\quad 
\frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{2}-\frac{\max\left(\eps\cdot  T,\eta\right)}{2} ,1+\frac{\eta}{2}\right]$$


\item Given access to a scalable demand oracle $\dem_i(\cdot,\cdot,\cdot)$ and a value oracle $\val_i(\cdot,\cdot)$,
we can construct a separation oracle $SO$ for $\widehat{W}_i$. The running time of $SO$ on any input with bit complexity $b'$ is $\poly\left(b,b',k,T,\frac{1}{\eps},\frac{1}{\eta}\right)$ and perform $\poly\left(b,b',k,T,\frac{1}{\eps},\frac{1}{\eta}\right)$ queries to $\dem_i,\val_i$ with input of bit complexity at most $\poly\left(b,b',T\right)$.
\end{enumerate}
\end{theorem}
}


%%%% Proof starts here %%%%%%%%
Choose parameter $\eps=\frac{1}{2T}$ and any $k=\Omega\left( T^4\left( Tb+\log\left(1/\eps\right)+n\log(1/\delta)\right) \right)$ %\argyrisnote{$k=\Omega\left( T^4\left( Tb+\log\left(1/\eps\right)+\log(1/\delta)\right) \right)$ instead?}. 
Hence, in this proof, $1-\eps T=1/2$. Let $\widehat{D}_i$ be the empirical distribution induced by $N=\left\lceil\frac{32kT}{\eps^2}\right\rceil$ independent samples from $D_i$.
Let $\widehat{W}_{i}^{tr(\eps)}$ be the mixture of $\{W_{t_i}^{tr(\eps)}\}_{t_i\in T_i}$ over the empirical distribution $\widehat{D}_i$. By~\Cref{obs:bit complexity mrf xos}, the bit complexity of each corner of polytopes in $\{W_{t_i}^{tr(\eps)}\}_{t_i\in\cT_i}$ is at most $O(T b)$.
By Theorem~\ref{thm:approx mixture}, with probability at least $1-2Te^{-2Tk}\geq 1-\delta$, %\argyrisnote{($1-2Te^{-2Tk}\geq 1-\delta$ instead?)}, 
both of the following properties hold:
\begin{enumerate}[label=(\roman*)]
    \item For each $(\widehat{\pi}_i,\widehat{w}_i)\in \widehat{W}_i^{tr(\eps)}$,
    there exists a $(\pi_i,w_i)\in {W}_i^{tr(\eps)}$ such that $||(\widehat{\pi}_i,\widehat{w}_i)-(\pi_i,w_i)||_\infty \leq \frac{\eps}{2}$
    \item For each $(\pi_i,w_i)\in {W}_i^{tr(\eps)}$,
    there exists a $(\widehat{\pi}_i,\widehat{w}_i)\in \widehat{W}_i^{tr(\eps)}$ such that $||(\widehat{\pi}_i,\widehat{w}_i)-(\pi_i,w_i)||_\infty \leq \frac{\eps}{2}$
\end{enumerate}

For the rest of the proof, we condition on the event where both properties above hold. Let $W_i'=\frac{1}{2}W_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}$. Consider the polytope $\widehat{W}_i = \frac{1}{2}\widehat{W}_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}$.
%Then with probability $1-2M_i\exp(-2M_ik)$, both of the following properties are satisfied : 
We are going to show that for each $(\pi_i,w_i) \in W_i'$, there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j,t_{ij}$, 

$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{4}, \frac{3}{2}\right]\quad \text{and} \quad
\frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right].$$
It is not hard to see that this implies Property 2 in the statement of \Cref{cor:rfs for xos mult}, as $W_i'=\frac{1}{2}W_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}\supseteq \frac{1}{4}W_i$(due to \Cref{lem:xos mrf contain} and our choice of $\eps$). %$W_i'=\frac{1}{2}W_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}\supseteq \frac{1}{4}W_i$, so Property 2 in the statement of \Cref{cor:rfs for xos mult} follows from Property 1.

%The other direction is similar.




%Back to the proof of \Cref{thm:multi-approx-mixture}. 
For any $(\pi_i,w_i) \in W_i'$,
we rewrite $(\pi_i,w_i)$ as  $\frac{1}{2}(\pi_i^{tr},w_i^{tr}) + \frac{1}{2}(\pi_i^{box},w_i^{box})$ where  $(\pi_i^{tr},w_i^{tr}) \in W^{tr(\eps)}_{i}$ and $(\pi_i^{box},w_i^{box}) \in \frac{1}{2} W_i^{box(\eps)}$.
For every $j\in [m]$, we partition $\cT_{ij}$ into four disjoint sets: 
\begin{align*}
S_{j}^{(1)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land \eps < w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})  \} \\
S_j^{(2)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land w_{ij}(t_{ij})\leq \eps < \pi_{ij}(t_{ij})  \} \\
S_j^{(3)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij}) \leq \eps \}\\
S_j^{(4)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) <\eps\}
\end{align*}





By property (ii), there exists a $(\widehat{\pi}^{tr}_{i},\widehat{w}^{tr}_i)\in \widehat{W}^{tr(\eps)}_{i}$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:
\begin{align*}
\pi^{tr}_{ij}(t_{ij}) - \eps/2\leq \widehat{\pi}^{tr}_{ij}(t_{ij}) \leq \pi^{tr}_{ij}(t_{ij}) + \eps/2 \\
w^{tr}_{ij}(t_{ij}) - \eps/2\leq \widehat{w}^{tr}_{ij}(t_{ij}) \leq w^{tr}_{ij}(t_{ij}) + \eps/2
\end{align*}

Now consider the following vector $(\widetilde{\pi}^{tr}_i,\widetilde{w}^{tr}_i) \in [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$:
\begin{align*}
\widetilde{\pi}^{tr}_{ij}(t_{ij}) =&
\begin{cases}
\widehat{\pi}_{ij}^{tr}(t_{ij}) \quad & \text{ if $t_{ij}\in S_j^{(1)}\cup S_j^{(2)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\widetilde{w}^{tr}_{ij}(t_{ij}) =&
\begin{cases}
\widehat{w}_{ij}^{tr}(t_{ij}) \quad & \text{ if $t_{ij}\in S_j^{(1)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\end{align*}

{In other words, $$(\widetilde{\pi}^{tr}_{ij}(t_{ij}),\widetilde{w}^{tr}_{ij}(t_{ij}))=(\widehat{\pi}^{tr}_{ij}(t_{ij})\cdot \ind[{\pi}_{ij}(t_{ij})> \eps],\widehat{w}^{tr}_{ij}(t_{ij})\cdot\ind[{w}_{ij}(t_{ij})> \eps]),$$}
%\todo{Isn't his shorter definition of $(\widetilde{\pi}^{tr}_{ij},\widetilde{w}^{tr}_{ij})$ is equivalent?}\todo{Argyris: I agree.} By Lemma~\ref{lem:contain subtypes}
and %$(\widetilde{\pi}_i,\widetilde{w}_i)\in \widehat{W}_i^{tr(\eps)}$.
%\argyrisnote{I think we mean: 
$(\widetilde{\pi}^{tr}_i,\widetilde{w}^{tr}_i)\in \widehat{W}_i^{tr(\eps)}$.
\notshow{
\begin{lemma}
$(\widetilde{\pi}^{tr}_i,\widetilde{w}^{tr}_i) \in \widehat{W}_{i}^{tr(\eps)}$.
\end{lemma}
%We will prove that  
%Let $\eta_i\in [0,1]^{\sum_{j\in [m]}|\cT_{ij}|}$ be the vector such that 
\begin{proof}
Since $(\widehat{\pi}^{tr}_{i},\widehat{w}^{tr}_i)\in \widehat{W}_{i}^{tr(\eps)}$, for every $t_i$, there exists $(\widehat{\pi}^{(t_i)},\widehat{w}^{(t_i)})\in {W}_{t_i}^{tr(\eps)}$, such that $(\widehat{\pi}^{tr}_{i},\widehat{w}^{tr}_i)=\sum_{t_i\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\widehat{\pi}^{(t_i)},\widehat{w}^{(t_i)})$. Define $(\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})$ as follows:

\begin{align*}
\widetilde{\pi}^{(t_i)}_j(t_{ij}') =&
\begin{cases}
\widehat{\pi}^{(t_i)}_j(t_{ij}) \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(1)}$} \\
\min\left(1 ,a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))/\widehat{f}_{ij}(t_{ij})\right)  \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(2)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\widetilde{w}^{(t_i)}_{j}(t_{ij}') =&
\begin{cases}
\widehat{w}_{j}^{(t_i)}(t_{ij}) \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(1)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\end{align*}

%By \Cref{obs:W_i(t_i)-1} and \Cref{obs:W_i(t_i)-2} 
By \Cref{cor:W_t_i truncate} we have $(\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})\in {W}_{t_i}^{tr(\eps)}$. Since $\widehat{W}_{i}^{tr(\eps)}$ is a mixture of ${W}_{t_i}^{tr(\eps)}$ over distribution $\widehat{D}_i$, we have that $(\widetilde{\pi}^{tr}_{i},\widetilde{w}^{tr}_i)=\sum_{t_i\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})$ is in $\widehat{W}_{i}^{tr(\eps)}$. 
\end{proof}
}




%Let $a=1-\eps\cdot T>0$. 
Consider another vector $(\widetilde{\pi}^{box}_i,\widetilde{w}^{box}_i) \in [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$: 
\begin{align*}
(\widetilde{\pi}^{box}_{ij}(t_{ij}),\widetilde{w}^{box}_{ij}(t_{ij})) =&
\begin{cases}
({\pi}_{ij}^{box}(t_{ij}),w^{box}_{ij}(t_{ij})) \quad & \text{ if $t_{ij}\in S_{j}^{(1)}\cup S_{j}^{(4)}$} \\ 
(w_{ij}(t_{ij})/2, w_{ij}(t_{ij})/2)  \quad & \text{ if $t_{ij}\in S_{j}^{(2)}$} \\
({\pi}_{ij}(t_{ij})/2, w_{ij}(t_{ij})/2) \quad & \text{ if $t_{ij}\in S_{j}^{(3)}$} \\
\end{cases}
\end{align*}

For every $j\in[m]$ and $t_{ij}\in \cT_{ij}$, clearly $\widetilde{\pi}_{ij}^{box}(t_{ij})\geq \widetilde{w}_{ij}^{box}(t_{ij})$ since $\pi_{ij}^{box}(t_{ij})\geq w_{ij}^{box}(t_{ij})$ and $\pi_{ij}(t_{ij})\geq w_{ij}(t_{ij})$. Moreover, if $t_{ij}\in S_j^{(1)}\cup S_j^{(4)}$, $\widetilde{\pi}_{ij}^{box}(t_{ij})=\pi_{ij}^{box}(t_{ij})\leq \frac{1}{2}\cdot \min\{\eps,f_{ij}(t_{ij})\}$, since $(\pi_i^{box},w_i^{box}) \in \frac{1}{2}W_i^{box(\eps)}$.
If $t_{ij}\in S_j^{(2)}\cup S_j^{(3)}$, by the definitions of $S_j^{(2)}$ and $S_j^{(3)}$, we have that $\widetilde\pi_{ij}^{box}(t_{ij})\leq \eps/2=\frac{1}{2}\cdot \min\{\eps,f_{ij}(t_{ij})\}$.
Thus $(\widetilde{\pi}^{box}_i,\widetilde{w}^{box}_i)\in \frac{1}{2} {W}_{i}^{box(\eps)}$.
Now define $(\widetilde{\pi}_i,\widetilde{w}_i)=\frac{1}{2}(\widetilde{\pi}^{tr}_i,\widetilde{w}^{tr}_i) + \frac{1}{2}(\widetilde{\pi}^{box}_i,\widetilde{w}^{box}_i)$.
Then $(\widetilde{\pi}_i,\widetilde{w}_i)\in \widehat{W}_i$.
It remains to prove that $(\widetilde{\pi}_i,\widetilde{w}_i)$ satisfies: for all $j, t_{ij}$

$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{4}, \frac{3}{2}\right]\quad \text{and} \quad
\frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right].$$


%$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{2}-\frac{\max\left(\eps\cdot  T,\eta\right)}{2}, \frac{3}{2}+\frac{\eta}{2}\right],
%\quad 
%\frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{2}-\frac{\max\left(\eps\cdot  T,\eta\right)}{2} ,1+\frac{\eta}{2}\right]$$

We verify all cases based on which set $t_{ij}$ is in. 
\paragraph{Case 1: $t_{ij}\in S_j^{(1)}$.} 
Recall that for $t_{ij}\in S_j^{(1)}$, $\eps<w_{ij}(t_{ij}) \leq \pi_{ij}(t_{ij})$. We have that $$\widetilde\pi_{ij}(t_{ij})-\pi_{ij}(t_{ij})=\frac{1}{2}(\hat\pi_{ij}^{tr}(t_{ij})-\pi_{ij}^{tr}(t_{ij})).$$ According to property (ii), $\frac{1}{2}(\hat\pi_{ij}^{tr}(t_{ij})-\pi_{ij}^{tr}(t_{ij}))\in [-\frac{\eps}{4},\frac{\eps}{4}]$, so $\frac{1}{2}(\hat\pi_{ij}^{tr}(t_{ij})-\pi_{ij}^{tr}(t_{ij}))$ also lies in $[-\frac{\pi_{ij}(t_{ij})}{4},\frac{\pi_{ij}(t_{ij})}{4}]$. %$$-\frac{1}{4}\cdot \pi_{ij}(t_{ij})\leq-\frac{\eps }{4}\leq\frac{1}{2}(\hat\pi_{ij}^{tr}(t_{ij})-\pi_{ij}^{tr}(t_{ij}))\leq\frac{\eps}{4}\leq \frac{1}{4}\cdot \pi_{ij}(t_{ij})$$
Similarly, 
$$\widetilde {w}_{ij}(t_{ij})-w_{ij}(t_{ij})=\frac{1}{2}(\hat{w}_{ij}^{tr}(t_{ij})-w_{ij}^{tr}(t_{ij}))\in [-\frac{\eps }{4},\frac{\eps }{4}] \subseteq [-\frac{w_{ij}(t_{ij})}{4}, \frac{w_{ij}(t_{ij})}{4}].$$
Hence, $$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{3}{4}, \frac{5}{4}\right]\quad \text{and} \quad
\frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{3}{4},\frac{5}{4}\right].$$


\paragraph{Case 2: $t_{ij}\in S_j^{(2)}$.}
Recall that
$
\widetilde{w}_{ij}(t_{ij}) = \frac{1}{4}\cdot {w}_{ij}(t_{ij})
$ and $\widetilde{\pi}_{ij}(t_{ij}) = \frac{1}{4}\cdot {w}_{ij}(t_{ij}) + \frac{1}{2}\cdot\widehat{\pi}^{tr}_{ij}(t_{ij})$. We have that
$$
\widetilde{\pi}_{ij}(t_{ij}) \leq \frac{1}{4}\cdot {w}_{ij}(t_{ij}) + \frac{{\pi}^{tr}_{ij}(t_{ij})}{2}  + \frac{\eps}{4} \leq \frac{3}{2}\cdot{\pi}_{ij}(t_{ij}).
$$
The first inequality follows from property (ii), and the second inequality follows from $\pi_{ij}(t_{ij}) =\frac{\pi^{tr}_{ij}(t_{ij})}{2} + \frac{\pi^{box}_{ij}(t_{ij})}{2}\geq \frac{\pi^{tr}_{ij}(t_{ij})}{2}$ and $w_{ij}(t_{ij})\leq \eps < \pi_{ij}(t_{ij})$ when $t_{ij}\in S_j^{(2)}$. We also have that
$$
\widetilde{\pi}_{ij}(t_{ij})\geq \frac{\widetilde{\pi}^{tr}_{ij}(t_{ij})}{2} \geq \frac{{\pi}^{tr}_{ij}(t_{ij})}{2}  - \frac{\eps}{4} = \pi_{ij}(t_{ij}) - \frac{\pi_{ij}^{box}(t_{ij})}{2} - \frac{ \eps}{4}\geq \pi_{ij}(t_{ij})- \frac{\eps}{2} \geq \frac{1}{2}{\pi}_{ij}(t_{ij}) 
$$
The first inequality follows from the non-negativity of $\widetilde{\pi}^{box}_{ij}(t_{ij})$; the second inequality follows from property (ii); the third inequality is due to the fact that $\pi^{box}_{ij}(t_{ij})\leq \eps/2$; the last inequality is because $\eps<\pi_{ij}(t_{ij})$.

Hence, $$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{2}, \frac{3}{2}\right]\quad \text{and} \quad
\frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}= \frac{1}{4}.$$

%where again we used that $\pi_{ij}(t_{ij}) =\frac{\pi^{tr}_{ij}(t_{ij})}{2} + \frac{\pi^{box}_{ij}(t_{ij})}{2}$, 
%$\pi^{box}_{ij}(t_{ij})\leq a \eps \leq \eps$,
%for $j,t_{ij}\in S_j^{(2)}$ $\frac{w^{box}_{ij}(t_{ij})}{2}\leq w_{ij}(t_{ij}) \leq \eps < \pi_{ij}(t_{ij})$
%for $j,t_{ij}\in S_j^{(2)}$ $\eps < \pi_{ij}(t_{ij})$


\paragraph{Case 3: $t_{ij}\in S_j^{(3)}\cup S_j^{(4)}$.}
Recall that when $t_{ij}\in S_j^{(3)}$, $\widetilde{\pi}_{ij}(t_{ij}) = \frac{1}{4}\cdot {\pi}_{ij}(t_{ij})$ and $\widetilde{w}_{ij}(t_{ij}) = \frac{1}{4}\cdot {w}_{ij}(t_{ij})$. 
%\begin{align*}
%\widetilde{\pi}_{ij}(t_{ij}) = \frac{1}{2} {\pi}_{ij}(t_{ij}) \\
%\widetilde{w}_{ij}(t_{ij}) = \frac{1}{2} {w}_{ij}(t_{ij})
%\end{align*}
When $t_{ij}\in S_j^{(4)}$, as $f_{ij}(t_{ij})<\eps$, $w_{ij}^{tr}(t_{ij})=\pi_{ij}^{tr}(t_{ij})=0$. Thus $\widetilde{\pi}_{ij}(t_{ij})=\frac{1}{2}\pi_{ij}^{box}(t_{ij})=\pi_{ij}(t_{ij})$, and $w_{ij}(t_{ij})=\frac{1}{2}w_{ij}^{box}(t_{ij})=w_{ij}(t_{ij})$. 

To sum up, we have argued that for each $(\pi_i,w_i) \in W_i'$, there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j,t_{ij}$, 

$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{4}, \frac{3}{2}\right]\quad \text{and} \quad
\frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right].$$

With a similar analysis,
~{\footnote{{We only need to switch the role of $(\widetilde{\pi}_i,\widetilde{w}_i)$ and $(\pi_i,w_i)$. We provide a brief sketch here. First, rewrite $(\widetilde{\pi}_i,\widetilde{w}_i)$ as $\frac{1}{2}(\widehat{\pi}^{tr}_i,\widehat{w}^{tr}_i)+\frac{1}{2}(\widetilde{\pi}^{box}_i,\widetilde{w}^{box}_i)$, where $(\widehat{\pi}^{tr}_i,\widehat{w}^{tr}_i)\in \widehat{W}^{tr(\eps)}_i$ and $(\widetilde{\pi}^{box}_i,\widetilde{w}^{box}_i)\in \frac{1}{2}W_i^{box(\eps)}$. Also, redefine $S_j^{(i)}$ in the same fashion but according to $(\widetilde{\pi}_i,\widetilde{w}_i)$. Take $({\pi}^{tr}_i,{w}^{tr}_i)\in W_i^{tr(\eps)}$ to be the point guaranteed to exist by property (i), and define $(\bar{\pi}^{tr}_{ij}(t_{ij}),\bar{w}^{tr}_{ij}(t_{ij})):= ({\pi}^{tr}_{ij}(t_{ij})\cdot \ind[\widetilde{\pi}_{ij}(t_{ij})>\eps],w^{tr}_{ij}(t_{ij})\cdot \ind[\widetilde{w}_{ij}(t_{ij})>\eps])$. Also, define $(\pi_{ij}^{box}(t_{ij}),w_{ij}^{box}(t_{ij}))$ according to which set $t_{ij}$ belongs to in a fashion similar to the proof above. Now define $(\pi_i,w_i)=\frac{1}{2}(\bar{\pi}^{tr}_{i},\bar{w}^{tr}_{i})+\frac{1}{2}({\pi}^{box}_{i},{w}^{box}_{i})$. Using a similar case analysis, we can prove the claim that $\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{3}{2}\right]$ and  $\frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$ for all $j\in[m]$ and $t_{ij}\in \cT_{ij}$.}}}
we can also show that for each $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$, there exists a $({\pi}_i,{w}_i) \in W_i'$ such that for all $j,t_{ij}$, 

$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{3}{2}\right]\quad\text{and}\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right].$$

Thus Property 1 in the statement of \Cref{cor:rfs for xos mult} follows from the fact that $W_i'=\frac{1}{2}W_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}\subseteq W_i$ (\Cref{lem:xos mrf contain}). 

Let $\{t_i^{(1)},...,t_i^{(N)}\}$
be the $N$ samples from $D_i$. Then 
$$
\widehat{W}_i = \sum_{\ell\in[N]}\frac{1}{2N}\cdot W_{t_i^{(\ell)}}^{tr(\eps)} 
+ \frac{1}{4}W^{box(\eps)}_{i} 
$$
is the Minkowski addition of $N+1$ polytopes. For Property 3 of the statement,
since the vertex-complexity of $W_{t_i}^{tr(\eps)}$ is $O(bT)$ for each $t_i$ (\Cref{obs:bit complexity mrf xos}), and the vertex-complexity of $W_i^{box(\eps)}$ is no more than $\poly(b,T)$, the vertex-complexity of $\widehat{W}_i$ is no more than $poly(n,m,T,b,\log(1/\delta))$. 

At last, we show the existence of an efficient separation oracle $SO$ for $\widehat{W}_i$, by efficiently optimizing any linear objective over $\widehat{W}_i$. Since $\widehat{W}_i$ is the Minkowski addition of polytopes $\{W_{t_i^{(\ell)}}^{tr(\eps)}\}_{\ell\in [N]}$ and $W^{box(\eps)}_{i}$, in order to maximize over $\widehat{W}_i$, it's sufficient to maximize over each polytope. By \Cref{lem:optimize}, we can efficiently optimize any linear objective over $W_{t_i}^{tr(\eps)}$ for every $t_i$, given the adjustable demand oracle and value oracle. Thus it is sufficient to solve
$\max\{\bm{x}\cdot \pi_i+\bm{y}\cdot w_i: (\pi_i,w_i)\in W^{box(\eps)}_{i}\}$ for any vector $\bm{x},\bm{y}$. Since in $W^{box(\eps)}_{i}$, the constraint for each coordinate $(j,t_{ij})$ is separate: $0\leq w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})\leq \min(\eps,f_{ij}(t_{ij}))$. Thus the optimum can be achieved by solving the following LP for every coordinate:
\begin{align*}
    \max&\quad x_j(t_{ij})\cdot \pi_{ij}(t_{ij}) + y_j(t_{ij})\cdot w_{ij}(t_{ij}) \\
    s.t.&\quad 0\leq w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})\leq \min(\eps,f_{ij}(t_{ij}))
\end{align*}
Note that the bit complexity of the output of our optimization algorithm is $poly(n,m,T,b,\log(1/\delta))$.
Thus by \Cref{thm:equivalence of opt and sep}, there exists a separation oracle $SO$ of $\widehat{W}_i$, that satisfies Property 4 in the statement of \Cref{cor:rfs for xos mult}.


















%Now we are left to prove that we can have access to an efficient separation oracle for $\widehat{W}_i$.
%Similar to the proof of Theorem~\ref{thm:special case of multiplicative approx},
%$\widehat{W}_i$ is the Minkowski sum of $N$ polytopes in $\{W_{t_i}^{tr(\eps)}\}_{t_i\in \cT_i}$.
%With the help of Lemma~\ref{lem:optimize} and Observation~\ref{obs:bit complexity mrf xos}, we can use arguments similar to the proof of Theorem~\ref{thm:special case of multiplicative approx},
%and argue that we can construct an efficient seperation oracle for $\widehat{W}_i$ as stated.





\notshow{

\begin{proof}
By applying Theorem~\ref{thm:multi-approx-mixture} with $\eps=\frac{1}{2T}$, $\eta=\frac{1}{2}$, integer $k=\Omega\left(\frac{1}{2T}\log\left(\frac{n2T}{\delta} \right),T^4\left(Tb +\log\left( \frac{1}{\eta\eps}\right) \right)\right)$  and
having access to $\left\lceil\frac{8kT}{(\eta \eps )^2} \right\rceil=\poly\left(b,T, \log\left(\frac{1}{\delta}\right) \right)$ samples,
we can construct a polytope $\widehat{W}_i$ such that with probability at least $1-2T\exp(-2Tk)\geq 1-\frac{\delta}{n}$    
\begin{enumerate}
    \item For each $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$,
there exists a $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:


$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{7}{4}\right],\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$$


\item For each $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:


$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{7}{4}\right],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$$


\item  Given access to a scalable demand oracle $\dem_i(\cdot,\cdot,\cdot)$ and a value oracle $\val_i(\cdot,\cdot)$,
we can construct a separation oracle $SO_i$ for $\widehat{W}_i$. The running time of $SO_i$ on any input with bit complexity $b'$ is $\poly\left(b,b',T,\log\left(\frac{1}{\delta}\right)\right)$ and perform $\poly\left(b,b',T,\log\left(\frac{1}{\delta}\right)\right)$ queries to $\dem_i,\val_i$ with input of bit complexity $\poly\left(b,b',T,\log\left(\frac{1}{\delta}\right)\right)$. 
\end{enumerate}
By Lemma~\ref{lem:xos mrf contain},
we know that $\frac{1}{4}W_i\subseteq\frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i}\subseteq W_i$.


Thus for each $(\widetilde{\pi}_i,\widetilde{w}_i)\in \widehat{W}_i$ there exists a $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1}{4}W^{box(\eps)}_{i} \subseteq W_i$ such that
$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{7}{4}\right],\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$$


And for 
$(\pi_i,w_i)\in 
\frac{1}{2}W_i^{tr(\eps)} + \frac{1}{4}W_i^{box} \subseteq \frac{1}{4}W_i$
%$(\pi_i,w_i)\in \frac{2}{5}W_i\subseteq\frac{1}{4}W_i$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:


$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{7}{4}\right],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$$


\end{proof}

}










%\subsection{Putting Everything Together}

%The following is the main theorem of the section.

































\notshow{

\begin{lemma}\label{lem:W_t_i modify}
%Let $\textbf{0}$ be the vector with 0 in all entries. 
For any $t_i$ and $(\pi_i,w_i)\in W_{t_i}$ and set of items $B\subseteq [m]$.
Consider $\widehat{\pi}_i,\widehat{w}_i\in [0,1]^{\sum_{j\in[m]}|\cT_{ij}|}$ such that for $j\in S$:
\begin{align*}
\widehat{w}_{ij}(t_{ij}) = w_{ij}(t_{ij}) \\
\widehat{\pi}_{ij}(t_{ij}) = \pi_{ij}(t_{ij})    
\end{align*}
and for $j\notin S$:
\begin{align*}
\widehat{w}_{ij}(t_{ij}) = 0 \\
0 \leq \widehat{\pi}_{ij}(t_{ij}) \leq 1   
\end{align*}
For $j\in [m]$ and $t_{ij}'\neq t_{ij}$
\begin{align*}
\widehat{w}_{ij}(t_{ij}) = 0 \\
\widehat{\pi}_{ij}(t_{ij}) = 0
\end{align*}
then $(\pi,w)\in W_{t_i}$.
\end{lemma}


\begin{proof}
%Moreover, given a type $t_i\in \cT_i$,
%we denote the subset of bad items $b(t_i)\subseteq [m]$ such that
%$$
%j \in b(t_i) \text{ iff }t_{ij} \notin S_j
%$$
Note that for each $j\in[m]$ and $t_{ij}'\neq t_{ij}$,
then $\widehat{w}_{ij}(t_{ij}')=\widehat{\pi}_{ij}(t_{ij}')={w}_{ij}(t_{ij}')={\pi}_{ij}(t_{ij}')=0$.
Let $\{\sigma_{S}^k\}_{S,k}$ be the set of numbers associated with $(\pi,w)\in W_{t_i}$ according to Definition~\ref{def:welfare frequent-t_i}.
We consider the set of numbers $\{\widehat{\sigma}_{S}^k\}_{S,k}$,
and we are going to prove that the element in $W_{t_i}$ associated with $\{\widehat{\sigma}_{S}^k\}_{S,k}$, is $(\widehat{w}_i,\widehat{\pi}_i)$.
For each $k\in [K]$ and $S\subseteq [m]$,
where $S=S_b\cup S_g$, where $S_B\subseteq B$ and $S_G\subseteq [m] \backslash B$:
$$
\widehat{\sigma}_{S}^k = 
\left(\prod_{j\in S_B} \widehat{\pi}_{ij}(t_{ij})\prod_{j \in B\backslash S_B} (1-\widehat{\pi}_{ij}(t_{ij})) \right) \left(\sum_{\substack{S_G \subseteq T \subseteq S_G \cup B}} {\sigma}_{T}^k\right)
$$
First observe that each set for $T\subseteq [m]$,
there exists a unique set $U\subseteq [m]\backslash B$, such that $U\subseteq T\subseteq U\cup B$ (in that case $U=T \backslash B$).
Thus
%for fixed $S_B\subseteq B$, we have that:

\begin{align*}
\sum_{S_B\subseteq B}\sum_{k\in [K]}\sum_{S_G\subseteq[m]\backslash B} \widehat{\sigma}_{S_B\cup S_G}^k = &\sum_{S_B\subseteq B}
\left(\prod_{j\in S_B} \widehat{\pi}_{ij}(t_{ij})\prod_{j \in B\backslash S_B} (1-\widehat{\pi}_{ij}(t_{ij})) \right) \sum_{k\in [K]}\sum_{S_G\subseteq[m]\backslash B}\left(\sum_{\substack{S_G \subseteq T \subseteq S_G \cup B}} {\sigma}_{T}^k\right) \\
=&\sum_{S_B\subseteq B}\left(\prod_{j\in S_B} \widehat{\pi}_{ij}(t_{ij})\prod_{j \in B\backslash S_B} (1-\widehat{\pi}_{ij}(t_{ij})) \right) \sum_{k\in [K]}\sum_{T\subseteq[m]}{\sigma}_{T}^k \\
=&\sum_{S_B\subseteq B}\prod_{j\in S_B} \widehat{\pi}_{ij}(t_{ij})\prod_{j \in B\backslash S_B} (1-\widehat{\pi}_{ij}(t_{ij})) 
\end{align*}

Consider $|B|$ random variables,
such that for each $j\in B$, random variables $C_j$ is sampled from a Bernoulli distribution with probability of success $\widehat{\pi}_{ij}(t_{ij})$.
Observe that $\prod_{j\in S_B} \widehat{\pi}_{ij}(t_{ij})\prod_{j \in B\backslash S_B} (1-\widehat{\pi}_{ij}(t_{ij}))$,
is the probability that once we take a sample from the $|B|$ random variables,
$C_j=1$ only if $j\in S_B$ and $C_j=0$ if $j\notin S_B$.
Thus
\begin{align*}
\sum_{S_B\subseteq B}\sum_{k\in [K]}\sum_{S_G\subseteq[m]\backslash B} \widehat{\sigma}_{S_B\cup S_G}^k 
=&\sum_{S_B\subseteq B}\prod_{j\in S_B} \widehat{\pi}_{ij}(t_{ij})\prod_{j \in B\backslash S_B} (1-\widehat{\pi}_{ij}(t_{ij})) \\
=& 1
\end{align*}

which proves that $\{\widehat{\sigma}_{S}^k\}_{S,k}$ first property of Definition~\ref{def:welfare frequent-t_i}.
Now we are going to prove the second property.
For $j\in B$:

\begin{align*}
\sum_{S_B\subseteq B:j\in S_B}\sum_{k\in [K]}\sum_{S_G\subseteq[m]\backslash B} \widehat{\sigma}_{S_B\cup S_G}^k 
=& \widehat{\pi}_{ij}(t_{ij}) \sum_{\substack{S_B\subseteq B\\j\in B}}\prod_{\substack{j'\in S_B \\ \land j'\neq j}} \widehat{\pi}_{ij'}(t_{ij'})\prod_{j' \in B\backslash S_B} (1-\widehat{\pi}_{ij'}(t_{ij'})) \\
=& \widehat{\pi}_{ij}(t_{ij})
\end{align*}

The last equation follows by a similar way of thinking as above,
by interpreting $\prod_{\substack{j'\in S_B \\\land j'\neq j}} \widehat{\pi}_{ij'}(t_{ij'})\prod_{j' \in B\backslash S_B} (1-\widehat{\pi}_{ij'}(t_{ij'}))$,
as the event where we have $|B|$ random variables $C_j$,
where $C_j$ is sampled from a Bernoulli distribution with probability of success $\widehat{\pi}_{ij}(t_{ij})$.
Notice that for $j\in B$, setting $\widehat{w}_{ij}(t_{ij})$ trivially satisfy the third requirement.

For $j\notin B$,
observe that

\begin{align*}
\sum_{\substack{S_G\subseteq[m]\backslash B\\j \in S_G}}\sum_{S_B\subseteq B}\sum_{k\in [K]} \widehat{\sigma}_{S_B\cup S_G}^k = 
&\sum_{S_B\subseteq B}
\left(\prod_{j\in S_B} \widehat{\pi}_{ij}(t_{ij})\prod_{j \in B\backslash S_B} (1-\widehat{\pi}_{ij}(t_{ij})) \right) \sum_{k\in [K]}\sum_{\substack{S_G\subseteq[m]\backslash B\\j \in S_G}}\left(\sum_{\substack{S_G \subseteq T \subseteq S_G \cup B}} {\sigma}_{T}^k\right) \\
=&\sum_{k\in [K]}\sum_{\substack{S_G\subseteq[m]\backslash B\\j \in S_G}}\left(\sum_{\substack{S_G \subseteq T \subseteq S_G \cup B}} {\sigma}_{T}^k\right)\\
=&\sum_{k\in [K]}\sum_{\substack{S\subseteq[m]\\j \in S}} {\sigma}_{S}^k=\pi_{ij}(t_{ij})
\end{align*}

We can similarly prove that 
\begin{align*}
\sum_{\substack{S_G\subseteq[m]\backslash B\\j \in S_G}}\sum_{S_B\subseteq B}\sum_{k\in [K]} \widehat{\sigma}_{S_B\cup S_G}^k \frac{\alpha_j^{(k)}}{V_{ij}(t_{ij})}= 
w_{ij}(t_{ij})
\end{align*}

which concludes the proof.
\end{proof}

A corollary of Lemma~\ref{lem:W_t_i modify} is the following.

\begin{corollary}\label{cor:W_t_i truncate}
%Let $\textbf{0}$ be the vector with 0 in all entries. 
For any $t_i$ and $(\pi^{tr}_i,w^{tr}_i)\in W_{t_i}^{tr(\eps)}$ and set of items $B\subseteq [m]$.
Consider $\widehat{\pi}^{tr}_i,\widehat{w}^{tr}_i\in [0,1]^{\sum_{j\in[m]}|\cT_{ij}|}$ such that for $j\in S$:
\begin{align*}
\widehat{w}^{tr}_{ij}(t_{ij}) = w_{ij}^{tr}(t_{ij}) \\
\widehat{\pi}^{tr}_{ij}(t_{ij}) = \pi^{tr}_{ij}(t_{ij})    
\end{align*}
and for $j\notin S$:
\begin{align*}
\widehat{w}^{tr}_{ij}(t_{ij}) = 0 \\
0 \leq \widehat{\pi}^{tr}_{ij}(t_{ij}) \leq 1   
\end{align*}
For $j\in [m]$ and $t_{ij}'\neq t_{ij}$
\begin{align*}
\widehat{w}_{ij}^{tr}(t_{ij}) = 0 \\
\widehat{\pi}_{ij}^{tr}(t_{ij}) = 0
\end{align*}
then $(\pi^{tr},w^{tr})\in W_{t_i}^{tr(\eps)}$.
\end{corollary}








A corollary of Lemma~\ref{lem:W_t_i modify} is the following.
\begin{observation}\label{obs:W_i(t_i)-2}
Fix any $t_i$. For any $j$, $S_j\subseteq \cT_{ij}$, $(\pi,w)\in W_{t_i}$, define $(\pi',w')\in [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$ as: 
$$\pi_{j}'(t_{ij}')=\pi_j(t_{ij}')\cdot\ind[t_{ij}'\in S_j],\quad w_{j}'(t_{ij}')=w_j(t_{ij}')\cdot\ind[t_{ij}'\in S_j].$$ 
Then $(\pi',w')\in W_{t_i}$. 
\end{observation}















We conclude with the main theorem of this sections.
We show how to construct a polytope $\widehat{W}_i$,
such that each element in $\widehat{W}_i$ is within a multiplicative factor of an element in $\frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$ and vice versa and we have access to an efficient seperation oracle for $\widehat{W}_i$.
\argyrisnote{Unfortunately we cannot show that our polytope is contained in $W_i$ and contains a constant factor of $W_i$ as we did in Section~\ref{sec:multi-approx-polytope},
but we have the necessary properties to be able to ``round" our solution to one that can give us meaningful guarantees.}


\begin{theorem}\label{thm:multi-approx-mixture}
Let $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance (\Cref{def:bit complexity}).
%Let $b$ be an upper bound on the bit complexity of any element in $\{\alpha^k_j(t_{ij})\}_{j\in[m],t_{ij}\in \cT_{ij},k\in[K]}$.
Consider parameters $0 < \eps < 1/T$, $\delta\in (\eps T,1)$ and
integer $k\geq \Omega\left( T^4\left( Tb+\log\left(\frac{1}{\delta \eps}\right)\right) \right)$.
If we have access to $n=\left\lceil\frac{8kT}{(\delta\eps)^2}\right\rceil$ independent samples from $\cD$,
then with probability at least $1-2T\exp(-2T k)$,
we can construct a polytope $\widehat{W}_i$ such that there exists a constant $c\geq 1$

\begin{enumerate}
    \item For each $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$,
there exists a $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:

$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{2}-c\cdot(\delta+\eps \cdot T),1+c\cdot\delta\right],\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{2}-c\cdot(\delta+\eps \cdot T),1+c\cdot\delta\right]$$


\item For each $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:


$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{2}-c\cdot(\delta+\eps \cdot T),1+c\cdot\delta\right],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{2}-c\cdot(\delta+\eps \cdot T),1+c\cdot\delta\right]$$

\item Given access to a scalable demand oracle and an value oracle for the $i$-th buyer, we can construct an efficient separation oracle for $\widehat{W}_i$.

\item \argyrisnote{Write instead:} Given access to a scalable demand oracle $\dem_i(\cdot,\cdot,\cdot)$ and a value oracle $\val_i(\cdot,\cdot)$,
we can construct a separation oracle $SO$ for $\widehat{W}_i$. The running time of $SO$ on any input with bit complexity $b'$ is $\poly(d,b,b',\frac{1}{\eps},\log(1/\delta),\mathcal{A}(\poly(d,b,b',\frac{1}{\eps},\log(1/\delta))))$.
\end{enumerate}
\end{theorem}

\mingfeinote{
1.$\alpha_{ij}^k(t_{ij})$ not $a_j$.

2. The notation is inconsistent for XOS and c-a. Here you use $M_i=\sum_j|\cT_{ij}|$. Also there is a `T' in the statement.

3. Figure out the exact constant for $\delta$. I suggest you pick a specific constant for $\delta$ at the end of the proof.  

4. Argue for $W_i$ instead of $\frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps M_i}{2}W^{box(\eps)}_{i}$. Put Lemma 22 inside in the proof.

}

\begin{proof}
Let $\widehat{D}_i$ be the empirical distribution induced by $n$ independent samples from $D_i$.
Let $\widehat{W}_{i}^{tr(\eps)}$ be the mixture of $\{W_{t_i}^{tr(\eps)}\}_{t_i\in T_i}$ over the empirical distribution $\widehat{D}_i$.
By Observation~\ref{obs:bit complexity mrf xos},
the bit complexity of corners of polytopes in $\{W_{t_i}^{tr(\eps)}\}_{t_i\in\cT_i}$ is at most $O(T b)$.
By Theorem~\ref{thm:approx mixture} we have that with probability at least $1-2T\exp(-2Tk)$ the two following properties hold:
\begin{enumerate}
    \item Property (1): for each $(\widehat{\pi},\widehat{w})\in \widehat{W}_i^{tr(\eps)}$,
    there exists a $({\pi},{w})\in {W}_i^{tr(\eps)}$ such that $||(\widehat{pi},\widehat{w})-({pi},{w})||_\infty \leq \eps \delta$
    \item Property (2): for each $({\pi},{w})\in {W}_i^{tr(\eps)}$,
    there exists a $(\widehat{\pi},\widehat{w})\in \widehat{W}_i^{tr(\eps)}$ such that $||(\widehat{pi},\widehat{w})-({pi},{w})||_\infty \leq \eps \delta$
\end{enumerate}
For the rest of the proof, we condition that both of the events we described above happens.
Consider the polytope $\widehat{W}_i = \frac{1}{2}\widehat{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$.
%Then with probability $1-2M_i\exp(-2M_ik)$, both of the following properties are satisfied : 
We are going to show that for each $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ and constant $c\geq $, such that


$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{2}-c\cdot(\delta+\eps \cdot T),1+c\cdot\delta\right],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{2}-c\cdot(\delta+\eps \cdot T),1+c\cdot\delta\right]$$
The other direction is similar.

For every $j,t_{ij}$, let $\widehat{f}_{ij}(t_{ij})=\Pr_{t_i'\sim \widehat{D}_i}[t_{ij}'=t_{ij}]$ be the marginal probability of $t_{ij}$ when $t_i\sim \widehat{D}_i$. We first prove the following lemma using Property (1) and Property (2). 

\begin{lemma}\label{lem:f_hat and f} %\yangnote{Why does this require Theorem~\ref{thm:approx mixture}? This follows from Chernoff+union bound directly.} \argyrisnote{Argyris: I think we could, but we need to take a union-bound that we can avoid with this approach.}
For every $t_{ij}$ such that $f_{ij}(t_{ij})\geq \eps$, we have $\frac{\widehat{f}_{ij}(t_{ij})}{f_{ij}(t_{ij})}\in [1-\delta,1+\delta]$.
\end{lemma}
\begin{proof}

For any $t_i$, consider the following vector $(\pi_{i}^{(t_i)},w_i^{(t_i)})$ such that $\pi_{ij}^{(t_i)}(t_{ij}')=\ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij})\geq \eps], w_{ij}^{(t_i)}(t_{ij}')=0$. By \Cref{def:welfare frequent-t_i}, we have $(\pi_{i}^{(t_i)},w_i^{(t_i)})\in W_{t_i}^{tr(\eps)}$ by considering the set of numbers $\{\sigma_S^{(k)}\}_{S,k}$ such that %$\sigma_S^{(k)}=\ind[S=[m]\wedge k=\argmax_{k'}\alpha_{ij}^{(k')}(t_{ij})]$ 
\argyrisnote{$\sigma_S^{(k)}=\ind[S=[j]\wedge k=\argmax_{k'}\alpha_{ij}^{(k')}(t_{ij})]$}. Now let $(\pi_{i},w_i)=\sum_{t_{i}\in \cT_i}f_i(t_i)\cdot (\pi_{i}^{(t_i)},w_i^{(t_i)})$. 
Since $W_{i}^{tr(\eps)}$ is a mixture of $W_{t_i}^{tr(\eps)}$ over $t_i\sim D_i$,
then $(\pi_{i},w_i)\in W_{i}^{tr(\eps)}$. Moreover, $w_{ij}(t_{ij})=0$ and $$\pi_{ij}(t_{ij})=\sum_{t_i'\in \cT_i}f_i(t_i')\cdot \ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij}')\geq \eps]=f_{ij}(t_{ij})\cdot \ind[f_{ij}(t_{ij})\geq \eps]$$  

Similarly, let $(\widehat\pi_{i},\widehat w_i)=\sum_{t_{i}\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\pi_{i}^{(t_i)},w_i^{(t_i)})$.
Then $(\widehat\pi_{i},\widehat w_i)\in \widehat{W}_{i}^{tr(\eps)}$. Moreover, $\widehat w_{ij}(t_{ij})=0$ and $$\widehat\pi_{ij}(t_{ij})=\sum_{t_i'\in \cT_i}\Pr_{x\sim \widehat{D}_i}[x=t_i']\cdot \ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij}')\geq \eps]=\widehat f_{ij}(t_{ij})\cdot \ind[f_{ij}(t_{ij})\geq \eps]$$   

Now by Property (2), there exists $(\pi_{i}',w_i')\in  \widehat{W}_{i}^{tr(\eps)}$, such that $||\pi_i-\pi_i'||_{\infty}\leq \delta \eps$. Thus for $t_{ij}$ such that $f_{ij}(t_{ij})\geq \eps$, we have 
$$(1-\delta)f_{ij}(t_{ij})\leq f_{ij}(t_{ij})-\delta \eps =\pi_{ij}(t_{ij})-\delta \eps \leq  \pi_{ij}'(t_{ij}) \leq \widehat{f}_{ij}(t_{ij})$$

the last inequality is because $\widehat{W}_{i}^{tr(\eps)}$ is a mixture of $W_{t_i}^{tr(\eps)}$ over $t_i\sim \widehat D_i$,
which implies  
$$\pi_{ij}'(t_{ij})\leq \sum_{t_{i'}\in \cT_i}\Pr_{x\sim \widehat{D}_i}[x=t_i']\cdot \ind[t_{ij}=t_{ij}']=\widehat{f}_{ij}(t_{ij}).$$

On the other hand, again by Property (1), there exists $(\pi_{i}'',w_i'')\in W_{i}^{tr(\eps)}$, such that $||\widehat\pi_i-\pi_i''||_{\infty}<\delta \eps$. Thus for $t_{ij}$ such that $f_{ij}(t_{ij})\geq \eps$, we have 
$$\widehat f_{ij}(t_{ij})=\widehat\pi_{ij}(t_{ij})\leq \pi_{ij}''(t_{ij})+\delta \eps\leq (1+\delta)\cdot f_{ij}(t_{ij})$$
the last inequality uses the fact that $\pi_{ij}''(t_{ij})\leq f_{ij}(t_{ij})$ and $f_{ij}(t_{ij})\geq \eps$.


\end{proof}


%is close to $(\pi,w_i)$ in a multiplicative sense, since the other directions is similar.


Back to the proof of \Cref{thm:multi-approx-mixture}. Since $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}$,
we can decompose $(\pi_i,w_i) = \frac{1}{2}(\pi_i^{tr},w_i^{tr}) + \frac{1}{2}(\pi_i^{box},w_i^{box})$ such that $(\pi_i^{tr},w_i^{tr}) \in W^{tr(\eps)}_{i}$ and $(\pi_i^{box},w_i^{box}) \in (1-\eps T)W_i^{box(\eps)}$.
For every $j\in [m]$, we partition $\cT_{ij}$ into four disjoint sets: 
\begin{align*}
S_{j}^{(1)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land \eps < w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})  \} \\
S_j^{(2)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land w_{ij}(t_{ij})\leq \eps < \pi_{ij}(t_{ij})  \} \\
S_j^{(3)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij}) \leq \eps \}\\
S_j^{(4)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) <\eps\}
\end{align*}




By Property (2), there exists a $(\widehat{\pi}^{tr}_{i},\widehat{w}^{tr}_i)\in \widehat{W}^{tr(\eps)}_{i}$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:
\begin{align*}
\pi^{tr}_{ij}(t_{ij}) - \delta\eps\leq \widehat{\pi}^{tr}_{ij}(t_{ij}) \leq \pi^{tr}_{ij}(t_{ij}) + \delta\eps \\
w^{tr}_{ij}(t_{ij}) - \delta\eps\leq \widehat{w}^{tr}_{ij}(t_{ij}) \leq w^{tr}_{ij}(t_{ij}) + \delta\eps
\end{align*}

Let $a=1-\eps\cdot T>0$. Now consider the following vector $(\widetilde{\pi}^{tr}_i,\widetilde{w}^{tr}_i) \in [0,1]^{2M_i}$:
\begin{align*}
\widetilde{\pi}^{tr}_{ij}(t_{ij}) =&
\begin{cases}
\widehat{\pi}_{ij}^{tr}(t_{ij}) \quad & \text{ if $t_{ij}\in S_j^{(1)}$} \\
\min\left( \widehat{f}_{ij}(t_{ij}) ,a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))\right)  \quad & \text{ if $t_{ij}\in S_j^{(2)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\widetilde{w}^{tr}_{ij}(t_{ij}) =&
\begin{cases}
\widehat{w}_{ij}^{tr}(t_{ij}) \quad & \text{ if $t_{ij}\in S_j^{(1)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\end{align*}


\begin{lemma}
$(\widetilde{\pi}^{tr}_i,\widetilde{w}^{tr}_i) \in \widehat{W}_{i}^{tr(\eps)}$.
\end{lemma}
%We will prove that  
%Let $\eta_i\in [0,1]^{\sum_{j\in [m]}|\cT_{ij}|}$ be the vector such that 
\begin{proof}
Since $(\widehat{\pi}^{tr}_{i},\widehat{w}^{tr}_i)\in \widehat{W}_{i}^{tr(\eps)}$, for every $t_i$, there exists $(\widehat{\pi}^{(t_i)},\widehat{w}^{(t_i)})\in {W}_{t_i}^{tr(\eps)}$, such that $(\widehat{\pi}^{tr}_{i},\widehat{w}^{tr}_i)=\sum_{t_i\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\widehat{\pi}^{(t_i)},\widehat{w}^{(t_i)})$. Define $(\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})$ as follows:

\begin{align*}
\widetilde{\pi}^{(t_i)}_j(t_{ij}') =&
\begin{cases}
\widehat{\pi}^{(t_i)}_j(t_{ij}) \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(1)}$} \\
\min\left(1 ,a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))/\widehat{f}_{ij}(t_{ij})\right)  \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(2)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\widetilde{w}^{(t_i)}_{j}(t_{ij}') =&
\begin{cases}
\widehat{w}_{j}^{(t_i)}(t_{ij}) \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(1)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\end{align*}

%By \Cref{obs:W_i(t_i)-1} and \Cref{obs:W_i(t_i)-2} 
By \Cref{cor:W_t_i truncate} we have $(\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})\in {W}_{t_i}^{tr(\eps)}$. Since $\widehat{W}_{i}^{tr(\eps)}$ is a mixture of ${W}_{t_i}^{tr(\eps)}$ over distribution $\widehat{D}_i$, we have that $(\widetilde{\pi}^{tr}_{i},\widetilde{w}^{tr}_i)=\sum_{t_i\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})$ is in $\widehat{W}_{i}^{tr(\eps)}$. 
\end{proof}




Now we consider another vector $(\widetilde{\pi}^{box}_i,\widetilde{w}^{box}_i)$: 
\begin{align*}
(\widetilde{\pi}^{box}_{ij}(t_{ij}),\widetilde{w}^{box}_{ij}(t_{ij})) =&
\begin{cases}
({\pi}_{ij}^{box}(t_{ij}),w^{box}_{ij}(t_{ij})) \quad & \text{ if $t_{ij}\in S_{j}^{(1)}\cup S_{j}^{(4)}$} \\ 
(a\cdot w_{ij}(t_{ij}),a\cdot w_{ij}(t_{ij}))  \quad & \text{ if $t_{ij}\in S_{j}^{(2)}$} \\
(a\cdot{\pi}_{ij}(t_{ij}),a\cdot w_{ij}(t_{ij})) \quad & \text{ if $t_{ij}\in S_{j}^{(3)}$} \\
\end{cases}
\end{align*}

For every $j,t_{ij}$, clearly $\widetilde{\pi}_{ij}^{box}(t_{ij})\geq \widetilde{w}_{ij}^{box}(t_{ij})$ since $\pi_{ij}^{box}(t_{ij})\geq w_{ij}^{box}(t_{ij})$ and $\pi_{ij}(t_{ij})\geq w_{ij}(t_{ij})$. Moreover, if $t_{ij}\in S_j^{(1)}\cup S_j^{(4)}$, $\widetilde{\pi}_{ij}^{box}(t_{ij})=\pi_{ij}^{box}(t_{ij})\leq a\cdot \min\{\eps,f_{ij}(t_{ij})\}$.
If $t_{ij}\in S_j^{(2)}\cup S_j^{(3)}$, by definition of $S_j^{(2)}$ and $S_j^{(3)}$, we have that $\widetilde\pi_{ij}^{box}(t_{ij})\leq a\cdot\eps=a\cdot \min\{\eps,f_{ij}(t_{ij})\}$.
Thus $(\widetilde{\pi}^{box}_i,\widetilde{w}^{box}_i)\in a {W}_{i}^{box(\eps)}$.
Now define $(\widetilde{\pi},\widetilde{w})=\frac{1}{2}(\widetilde{\pi}^{tr}_i,\widetilde{w}^f_i) + \frac{1}{2}(\widetilde{\pi}^{box}_i,\widetilde{w}^r_i)$.
Then $(\widetilde{\pi}_i,\widetilde{w}_i)\in \widehat{W}_i$.
We remain to prove that $(\widetilde{\pi}_i,\widetilde{w}_i)$ satisfies:


$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}]$$

We will verify all cases depending on which set $t_{ij}$ is in. First observe that for $t_{ij}\in S_j^{(1)}$, $\eps<w_{ij}(t_{ij}) \leq \pi_{ij}(t_{ij})$. We have $$-\frac{\delta}{2}\cdot \pi_{ij}(t_{ij})\leq-\frac{\eps \delta}{2}\leq\widetilde\pi_{ij}(t_{ij})-\pi_{ij}(t_{ij})=\frac{1}{2}(\hat\pi_{ij}^{tr}(t_{ij})-\pi_{ij}^{tr}(t_{ij}))\leq\frac{\eps\delta}{2}\leq \frac{\delta}{2}\cdot \pi_{ij}(t_{ij})$$
Similarly, 
$$-\frac{\delta}{2}\cdot w_{ij}(t_{ij})\leq-\frac{\eps \delta}{2}\leq\widetilde {w}_{ij}(t_{ij})-w_{ij}(t_{ij})=\frac{1}{2}(\hat{w}_{ij}^f(t_{ij})-w_{ij}^f(t_{ij}))\leq\frac{\eps \delta}{2}\leq \frac{\delta}{2}\cdot w_{ij}(t_{ij})$$



For $t_{ij}\in S_j^{(2)}$,
we have
$
\widetilde{w}_{ij}(t_{ij}) = \frac{a}{2}\cdot {w}_{ij}(t_{ij})
$.
For $\widetilde{\pi}_{ij}(t_{ij})$, when $\widehat{f}_{ij}(t_{ij}) \geq a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))$,
$
\widetilde{\pi}_{ij}(t_{ij}) = \frac{a}{2}\cdot {\pi}_{ij}(t_{ij})
$.

Now we deal with the case where $\widehat{f}_{ij}(t_{ij}) < a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))$.
By Lemma~\ref{lem:xos mrf contain}, since $(\pi_i,w_i) \in \frac{1}{2}{W}_{i}^{tr(\eps)} + \frac{1-\eps T}{2}W^{box(\eps)}_{i}\subseteq W_i$, we have $\pi_{ij}(t_{ij})-w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij}) \leq f_{ij}(t_{ij})$. Also by \Cref{lem:f_hat and f}, $\widehat{f}_{ij}(t_{ij}) \geq (1-\delta)f_{ij}(t_{ij})$. Thus if $\widehat{f}_{ij}(t_{ij}) < a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))$,
then
$$
\left(1-\delta\right)\left(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}) \right)\leq \left(1-\delta \right)f_{ij}(t_{ij})\leq \widehat{f}_{ij}(t_{ij})
$$


%If $\Pr_{t_{ij}'\sim \widehat{D}_j} \left[ t_{ij}'=t_{ij} \right] < \pi_{ij}(t_{ij}) - w_{ij}(t_{ij})$,
%then 
%by combining the fact that $f_{ij}(t_{ij})\geq \epsilon $ and $f_{ij}(t_{ij}) - \epsilon' \leq \Pr_{t_{ij}'\sim \widehat{D}_{j}}\left[t_{ij}'=t_{ij} \right]\leq f_{ij}(t_{ij}) + \epsilon'$ we can infer that
%$$
%f_{ij}(t_{ij}) - \frac{\epsilon'}{\epsilon}f_{ij}(t_{ij}) \leq f_{ij}(t_{ij}) - \epsilon' \leq \Pr_{t_{ij}'\sim \widehat{D}_{j}}\left[t_{ij}'=t_{ij} \right]\leq f_{ij}(t_{ij}) + \epsilon' \leq f_{ij}(t_{ij}) + \frac{\epsilon'}{\epsilon}f_{ij}(t_{ij})
%$$

%Moreover we have that $\pi_{ij}(t_{ij}) - w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij}) \leq f_{ij}(t_{ij})$.
Thus
\begin{align*}
    \widetilde{\pi}_{ij}(t_{ij}) = \frac{1}{2} \left(\widehat{f}_{ij}(t_{ij}) + a\cdot w_{ij}(t_{ij})\right) \geq \frac{1}{2} \left(1-\delta\right)(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij})) + \frac{a}{2}w_{ij}(t_{ij}) \geq \frac{1-\delta}{2} \pi_{ij}(t_{ij}),
\end{align*}
where the last inequality uses the fact that $a\geq 1-\delta$. On the other hand,
\begin{align*}
    \widetilde{\pi}_{ij}(t_{ij})<\frac{a}{2} (\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}) + w_{ij}(t_{ij})) \leq \frac{a}{2} \pi_{ij}(t_{ij})
\end{align*}

For $t_{ij}\in S_j^{(3)}$, we have $\widetilde{\pi}_{ij}(t_{ij}) = \frac{a}{2}\cdot {\pi}_{ij}(t_{ij})$ and $\widetilde{w}_{ij}(t_{ij}) = \frac{a}{2}\cdot {w}_{ij}(t_{ij})$. 
%\begin{align*}
%\widetilde{\pi}_{ij}(t_{ij}) = \frac{1}{2} {\pi}_{ij}(t_{ij}) \\
%\widetilde{w}_{ij}(t_{ij}) = \frac{1}{2} {w}_{ij}(t_{ij})
%\end{align*}
For $t_{ij}\in S_j^{(4)}$, since $f_{ij}(t_{ij})<\eps$, $w_{ij}^f(t_{ij})=\pi_{ij}^f(t_{ij})=0$. Thus $\widetilde{\pi}_{ij}(t_{ij})=\frac{1}{2}\pi_{ij}^r(t_{ij})=\pi_{ij}(t_{ij})$, and $w_{ij}(t_{ij})=\frac{1}{2}w_{ij}^r(t_{ij})=w_{ij}(t_{ij})$. 
%\begin{align*}
%\widetilde{\pi}_{ij}(t_{ij}) =  {\pi}_{ij}(t_{ij}) \\
%\widetilde{w}_{ij}(t_{ij}) = {w}_{ij}(t_{ij})
%\end{align*}


Now we are left to prove that we can have access to an efficient separation oracle for $\widehat{W}_i$.
Similar to the proof of Theorem~\ref{thm:special case of multiplicative approx},
$\widehat{W}_i$ is the Minkowski sum of polytope $W_i^{tr(\eps)}$ and $n$ polytopes in $\{W_{t_i}^{tr(\eps)}\}_{t_i\in \cT_i}$.
With Lemma~\ref{lem:optimize} and using arguments similar to the proof of Theorem~\ref{thm:special case of multiplicative approx},
we can argue that we can construct an efficient seperation oracle for $\widehat{W}_i$.
\end{proof}
}

















%A corollary of Theorem~\ref{thm:multi-approx-mixture} is the following.











\subsection{Putting Everything Together}

%Ideally we would like to solve the LP in Figure~\ref{fig:XOSLP},
%however we do not have access to the Marginal Reduced Form polytope $W_i$ for the buyers.
%A way to get around this issue is to use the proxy polytope described in Corollary~\ref{cor:rfs for xos mult} instead of the real one.
%Unfortunately for each $i$,
%the proxy polytope $\widehat{W}_i$ is not contained $W_i$.
%However we are still able to round a solution from an element of $\widehat{W}_i$ to get an element of $W_i$ using a different LP.
%We are going to describe this rounding procedure now.

In this section, we put all pieces together and provide a complete proof of \Cref{thm:main XOS}.
Denote $(P)$ the LP in \Cref{fig:XOSLP} and $\optlp$ the optimal objective of $(P)$. We consider another LP denoted as $(P')$. In $(P')$, in addition to all variables in $(P)$, we introduce new variables $\widehat{\pi}_i=\{\widehat{\pi}_{ij}(t_{ij})\}_{j\in[m],t_{ij}\in\cT_{ij}}$ and $\widehat{w}_i=\{\widehat{w}_{ij}(t_{ij})\}_{j\in[m],t_{ij}\in\cT_{ij}}$ for every $i\in [n]$. Both $(P)$ and $(P')$ have the same objective function. The only difference between $(P)$ and $(P')$ is that in $(P')$, we replace Constraint {\Wconstraint} with the following constraints:
$$\text{Constraint {\WconstraintNew}}: \quad (\widehat{\pi}_i,\widehat{w}_i) \in \widehat{W}_i, \pi_i \geq \frac{3}{2}\widehat{\pi}_i\geq \bm{0}, w_i \leq \frac{1}{4}\widehat{w}_i,\quad\forall i\in [n].$$ Here $\widehat{W}_i$ is the proxy polytope from \Cref{cor:rfs for xos mult} for each $i\in [n]$. Both inequalities hold coordinate-wisely. Denote $\optlp'$ the optimal objective of $(P')$.     
%Since for each bidder $i\in[n]$,
%we have access to a scalable demand oracle $\dem_i(\cdot,\cdot,\cdot)$ and a value oracle $\val_i(\cdot,\cdot)$,
By Property 4 of \Cref{cor:rfs for xos mult}, there exists an efficient separation oracle for each $\widehat{W}_i$. Thus we can solve $(P')$ in polynomial time using the Ellipsoid algorithm (\Cref{thm:ellipsoid}). The following lemma shows the relationship between $(P)$ and $(P')$. 
%Furthermore,
%since the rest of the constraints are linear, we can construct an efficient separation oracle for them too.
%Thus we have an efficient separation oracle for LP in Figure~\ref{fig:computable XOS}.


\notshow{
\begin{figure}[H]
\colorbox{MyGray}{
\begin{minipage}{.98\textwidth}
$$\quad\textbf{max  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}} 
 f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot \sum_{\substack{\beta_{ij}\in \cV_{ij}\\
 \delta_{ij} \in \Delta}} \lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})\leq \beta_{ij} + \delta_{ij}]$$
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
\vspace{-.3in}
  \begin{align*}
 & s.t.\\
 &\quad\textbf{Allocation Feasibility Constraints:}\\
 &\quad\Wconstraint \quad (\widehat{\pi}_i,\widehat{w}_i) \in \widehat{W}_i ,\quad \pi_i \geq \frac{3}{2}\widehat{\pi}_i,w_i \leq \frac{1}{4}\widehat{w}_i & \forall i \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
&\quad \PiConstraint \quad \sum_i \sum_{t_{ij}\in \cT_{ij}} \pi_{ij}(t_{ij})\leq 1 %\fr
& \forall j \\  
 &\quad\textbf{Natural Feasibility Constraints:}\\
    &\quad\LambdaMarginalConstraint\quad f_{ij}(t_{ij})\cdot\sum_{\beta_{ij}\in \cV_{ij}}\sum_{\delta_{ij}\in \Delta} \lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij}) = w_{ij}(t_{ij}) & \forall i,j,t_{ij}\in \cT_{ij}\\
    &\quad\CompareMarginalConstraint\quad\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}(\beta_{ij}, \delta_{ij}) & \forall i,j, t_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}\\
    &\quad\HatLambdaDistributionConstraint\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\ \delta_{ij} \in \Delta}} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) = 1 & \forall i,j\\
    &\quad\textbf{Problem Specific Constraints:}\\
    &\quad\ReduceDemandConstaint \quad \sum_{i\in[n]}\sum_{\beta_{ij} \in \cV_{ij}}\sum_{\delta_{ij}\in \Delta} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}] \leq \frac{1}{2}& \forall j\\
    %& (5)\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \lambda_{ij}(t_{ij},\beta_{ij}) \leq  \hat\lambda_{ij}(\beta_{ij}^+) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})> \beta_{ij}] & \forall i,j,\beta_{ij}\in \cV_{ij}\\
    %&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad+\hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq\beta_{ij}]\\
    & \quad\MarginalToGlobalConstraint\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \left(\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})+ \lambda_{ij}(t_{ij},\beta_{ij}^+,\delta_{ij})\right) \leq \\
    &\qquad\qquad\qquad\hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \cdot \Pr_{t_{ij}}[t_{ij}\geq \beta_{ij}]+\hat\lambda_{ij}(\beta_{ij}^+,\delta_{ij}) \cdot \Pr_{t_{ij}}[t_{ij}\geq\beta_{ij}^+] & \forall i,j,\beta_{ij}\in \cV_{ij}^0,\delta_{ij}\in \Delta\\
    %& \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) &\forall i\in[n], j \in[m] \\
    &\quad\BoundMeanDeltaConstraint\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\ \delta_{ij} \in \Delta}} \delta_{ij}\cdot \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \leq d_i  & \forall i,j\\
    &\quad\BoundSumDeltaConstraint\quad\sum_{i\in[n]} d_i \leq %\yangnote{16}\cdot \prev \\
    {111\cdot \estprev}\\
     & \lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}(\beta_{ij},\delta_{ij})\geq 0,\pi_{ij}(t_{ij})\geq 0, w_{ij}(t_{ij})\geq 0, d_i\geq 0 & \forall i,j,t_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}
\end{align*}
\end{minipage}}
\caption{Efficiently Computable LP for XOS Valuations}~\label{fig:computable XOS}.

\end{figure}

}



\notshow{
\begin{theorem}\label{thm:XOS mrf}
Let $T=\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance.
Consider the LP in Figure~\ref{fig:computable XOS},
where for each $i\in[n]$, polytope $\widehat{W}_i$ is defined in \Cref{cor:rfs for xos mult}. 
%using $\poly\left(b,T,\log\left( \frac{n}{\eta}\right)\right)$ samples from $D_i$. 
We condition on the event that each proxy polytope $\widehat{W}_i$ satisfies the properties in \Cref{cor:rfs for xos mult}. Then
\begin{enumerate}
\item For any $(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda, \bd)$  feasible solution of the LP in \Cref{fig:computable XOS},
there exists $\widetilde{\pi}\in [0,1]^{\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|}$ such that $(\widetilde{\pi},w,\lambda,\hat\lambda, \bd)$ is a feasible solution of the LP in Figure~\ref{fig:XOSLP}.
\item Let $\opt$ be the value of the optimal solution of the LP in Figure~\ref{fig:XOSLP} and $\widehat{\opt}$ be the value of the optimal solution of the LP in Figure~\ref{fig:computable XOS}. Then $\widehat{\opt}\geq \frac{\opt}{64}$
%For any feasible solution $(\pi,w,\lambda,\hat\lambda, \bd)$  of the LP in Figure~\ref{fig:XOSLP},
%there exists $\hat{\pi},\hat{w}$ such that $(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda, \bd)$ is feasible solution of the LP in \Cref{fig:computable XOS},
%there exists $\widetilde{\pi}\in [0,1]^{\sum_{i\in[n]}\sum_{j\in[m]}|\cT_{ij}|}$ such that .
\end{enumerate}
\end{theorem}
}


\begin{lemma}\label{lem:XOS-P to P'}
Suppose for every $i\in [n]$, $\widehat{W}_i$ satisfies the properties in \Cref{cor:rfs for xos mult}. Then
\begin{itemize}
\item For any feasible solution $(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda, \bd)$ to $(P')$,
there exists $\widetilde{\pi}\in [0,1]^{\sum_{i,j}|\cT_{ij}|}$ such that $(\widetilde{\pi},w,\lambda,\hat\lambda, \bd)$ is a feasible solution to $(P)$.
\item $\optlp\leq 64\cdot \optlp'$.
\end{itemize}
\end{lemma}

\begin{proof}
%For each $i\in [n]$, proxy polytope $\widehat{W}_i$ satisfies the properties mentioned in \Cref{cor:rfs for xos mult}
%We condition on the event that for each $i\in[n]$,
%for the proxy marginal reduced form $\widehat{W}_i$ that was constructed from Corollary~\ref{cor:rfs for xos mult} satisfies the following properties

%\begin{itemize}
%    \item Property (1): For each $i\in[n]$ and $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$,
%there exists a $(\pi_i,w_i) \in W_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:

%$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{7}{4}\right],\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$$


%\item Property (2): For each $i\in[n]$ and $(\pi_i,w_i) \in \frac{1}{4}{W}_{i}$,
%there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:


%$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{7}{4}\right],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in \left[\frac{1}{4},\frac{5}{4}\right]$$

%\end{itemize}

%By Corollary~\ref{cor:rfs for xos mult}, for each $i\in[n]$,
%this events happens with probability at least $1-\frac{\eta}{n}$.
%By Union-Bound all these events happen with probability at least $1-\eta$.

We prove the first part of the statement. Let $(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda, \bd)$ be any feasible solution to $(P')$. Then for every $i\in[n]$, $(\widehat{\pi}_i,\widehat{w}_i)\in \widehat{W}_i$. By Property 1 of \Cref{cor:rfs for xos mult}, there exists a $(\widetilde{\pi}_i,\widetilde{w}_i)\in W_i$ such that for each $j\in[m]$ and $t_{ij}\in \cT_{ij}$,
$$\widetilde{\pi}_{ij}(t_{ij}) \leq \frac{3}{2} \widehat{\pi}_{ij}(t_{ij})\leq{\pi}_{ij}(t_{ij}) \quad \widetilde{w}_{ij}(t_{ij}) \geq \frac{1}{4} \widehat{w}_{ij}(t_{ij}) \geq{w}_{ij}(t_{ij}) $$

Let $\widetilde{\pi}=\{\widetilde{\pi}_i\}_{i\in [n]}$. We are going to show that $(\widetilde\pi,w,\lambda,\hat\lambda, \bd)$ is a feasible solution to $(P)$ by verifying all constraints. 
%for the LP in Figure~\ref{fig:XOSLP}.
%By Definition~\ref{def:W_i}, we can easily observe that since $(\widetilde{\pi}_i,\widetilde{w_i})\in W_i$ and for each $j\in[m]$ and $t_{ij}\in \cT_{ij}$, $\widetilde{w}_{ij}(t_{ij})\geq w_{ij}(t_{ij})$,
%then $(\widetilde{\pi}_i,w_i)\in W_i$, which implies that the proposed solution satisfies 
For Constraint~$\Wconstraint$, since $(\widetilde{\pi}_i,\widetilde{w}_i)\in W_i$ and $w_{ij}(t_{ij})\leq \widetilde{w}_{ij}(t_{ij}),\forall j,t_{ij}$, thus by \Cref{def:W_i} $(\widetilde{\pi}_i,w_i)\in W_i$.

%Now all we are left to do is to show that $(\widetilde{\pi},w,\lambda,\hat\lambda, \bd)$ is a feasible solution of the LP in Figure~\ref{fig:XOSLP}.
%Notice that the only difference between the LP in Figure~\ref{fig:XOSLP} and the LP in Figure~\ref{fig:computable XOS} is Constraint $\Wconstraint$.

%Since for each $i\in[n]$,$j\in[m]$ and $t_{ij}\in \cT_{ij}$,$\widetilde{\pi}_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})$ and $(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda, \bd)$ is a feasible solution of the LP in Figure ~\ref{fig:computable XOS},
%then solution $(\widetilde\pi,w,\lambda,\hat\lambda, \bd)$ satisfies Constraint~$\PiConstraint$ of LP in Figure~\ref{fig:XOSLP}.

For Constraint {\PiConstraint}, since $(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda, \bd)$ is a feasible solution to $(P')$, for every $j\in [m]$,  $$\sum_i\sum_{t_{ij}\in \cT_{ij}}\widetilde{\pi}_{ij}(t_{ij})\leq \sum_i\sum_{t_{ij}\in \cT_{ij}}\pi_{ij}(t_{ij})\leq 1.$$ Furthermore, Constraints~$\LambdaMarginalConstraint-\BoundSumDeltaConstraint$ are clearly satisfied since $(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda, \bd)$ is a feasible solution to $(P')$.
Thus $(\widetilde{\pi},w,\lambda,\hat\lambda, \bd)$ is a feasible solution to $(P)$.

Now we prove the second part of the statement.
Let $(\pi^*,w^*,\lambda^*,\hat\lambda^*, \bd^*)$ be any optimal feasible solution to $(P)$. %We notice that $\left(\frac{1}{4}\pi_i^*,\frac{1}{4}w_i^*\right)\in \frac{1}{4}W_i$ and by Property (2), we know that 
For every buyer $i$, $(\pi_i^*,w_i^*)\in W_i$. By Property 2 of \Cref{cor:rfs for xos mult}, there exists a $(\widehat{\pi}_i,\widehat{w}_i)\in \widehat{W}_i$ such that for every $j,t_{ij}$, 
$$\widehat{\pi}_{ij}(t_{ij})\leq \frac{3}{8}\pi_{ij}^*(t_{ij}),\quad \widehat{w}_{ij}(t_{ij})\geq \frac{1}{16}w_{ij}^*(t_{ij})$$
We are going to show that $\left(\pi=\frac{3}{2}\widehat{\pi},w=\frac{1}{64}w^*,\hat\pi,\hat w,\lambda=\frac{1}{64}\lambda^*,\hat\lambda=\hat\lambda^*,\bd= \bd^*\right)$ is a feasible solution to $(P')$, which implies that $\optlp'\geq \optlp/64$. Firstly, for each $i\in[n]$, $(\widehat{\pi}_i,\widehat{w}_i)\in \widehat{W}_i$ and 
$$
\pi_i = \frac{3}{2}\widehat{\pi}_i, \qquad w_i = \frac{1}{64}w_i^* \leq \frac{1}{4}\widehat{w}_i 
$$
Thus Constraint {\WconstraintNew} is satisfied. For Constraint~$\PiConstraint$, since $(\pi^*,w^*,\lambda^*,\hat\lambda^*, \bd^*)$ is a feasible solution to $(P)$, we have that for every $j$, 
$$
\sum_{i\in[n]} \sum_{t_{ij}\in \cT_{ij}}\pi_{ij}(t_{ij})=\sum_{i\in[n]} \sum_{t_{ij}\in \cT_{ij}}\frac{3}{2}\hat\pi_{ij}(t_{ij}) \leq \sum_{i\in[n]} \sum_{t_{ij}\in \cT_{ij}}\frac{9}{16}\pi^*_{ij}(t_{ij}) \leq \frac{9}{16}<1
$$
%which implies that Constraint~$\PiConstraint$ is satisfied.

One can easily verify that when $(\pi^*,w^*,\lambda^*,\hat\lambda^*, \bd^*)$ is a feasible solution to $(P)$, 
%and Constraints~$\LambdaMarginalConstraint-\BoundSumDeltaConstraint$, 
$\left(\frac{1}{64}\pi^*,\frac{1}{64}w^*,\frac{1}{64}\lambda^*,\hat\lambda^*, \bd^*\right)$ is also a feasible solution to $(P)$, 
%Because Constraints~$\LambdaMarginalConstraint-\BoundSumDeltaConstraint$ depend on the variables that the solution $\left(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda,\bd \right)$ of the LP in Figure~\ref{fig:computable XOS} and the feasible solution  $\left(\frac{1}{64}\pi^*,w=\frac{1}{64}w^*,\lambda=\frac{1}{64}\lambda^*,\hat\lambda=\hat\lambda^*, \bd=\bd^*\right)$ of the LP in Figure~\ref{fig:XOSLP} have in common,
which implies that $\left(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda,\bd\right)$ satisfies Constraints~$\LambdaMarginalConstraint-\BoundSumDeltaConstraint$. Thus $\left(\pi,w,\hat\pi,\hat w,\lambda,\hat\lambda,\bd \right)$ is a feasible solution to $(P')$. The objective of the solution is a $\frac{1}{64}$-fraction of the objective of $(\pi^*,w^*,\lambda^*,\hat\lambda^*, \bd^*)$ since $\lambda=\frac{1}{64}\lambda^*$, which concludes the proof.  
%Moreover we can easily observe that the value of the objective with this solution is $\frac{\opt}{64}$ which concludes the proof.





%depend on the variables that the LP in Figure~\ref{fig:computable XOS} and in Figure~\ref{fig:XOSLP} have in common,
%then Constraints~$\LambdaMarginalConstraint-\BoundSumDeltaConstraint$ are satisfied for the LP in Figure~\ref{fig:computable XOS}.
\end{proof}



Now we are ready to give the proof of \Cref{thm:main XOS}.


\begin{prevproof}{Theorem}{thm:main XOS}

{We consider a fixed $\delta \in(0,1)$.
For each $i\in[n]$,
%$\widetilde{W}_i$ 
let $\widehat{W}_i$ be the proxy polytope for the single-bidder marginal reduced form polytope $W_i$ that is constructed in \Cref{cor:rfs for xos mult} with parameter $\delta'=\frac{\delta}{n}$.
Let $\cE_1$ be the event that the RPP mechanism  computed in \Cref{thm:chms10} has revenue $\estprev=\Omega(\prev)$, and let $\cE_2$  be the event that for each $i\in[n]$,
the proxy polytope $\widehat{W}_i$, satisfies the properties in \Cref{cor:rfs for xos mult}.
By the union bound combined with \Cref{thm:chms10} and \Cref{cor:rfs for xos mult}, with probability at least $1-\delta-\frac{2}{n}$, both events happen.
}

%Since for each bidder $i\in[n]$ we have access to a scalable demand oracle $\dem_i(\cdot,\cdot,\cdot)$ and a value oracle $\val_i(\cdot,\cdot)$,
%by Property (3) of Corollary~\ref{cor:rfs for xos mult} we can construct a separation oracle $SO_i$ for each $\widehat{W}_i$.
%Thus we can solve the LP in Figure~\ref{fig:computable XOS} in time $\poly\left(b,T,\frac{1}{\delta}\right)$.

We condition on the event that both $\cE_1$ and $\cE_2$ happens. By \Cref{thm:ellipsoid} and Property 3 and 4 of \Cref{cor:rfs for xos mult}, there exists an algorithm that solves the LP $(P')$ in time $\poly(n,m,T,b,\log (1/\delta))$, given access to the adjustable demand oracle and value oracle for all buyers' valuations. Let $(\pi^*,w^*,\hat\pi^*,\hat w^*,\lambda^*,\hat\lambda^*, \bd^*)$ be an optimal solution to $(P')$. %with value equal to $\widehat{\opt}_{LP}$ and let $\opt_{LP}$ be the value of LP in Figure~\ref{fig:XOSLP}.
By \Cref{thm:chms10}, \Cref{lem:XOS-P to P'} and \Cref{lem:bound rev by opt-XOS}, $\opt \leq 28 \prev + 4 \opt_{LP}\leq \frac{n}{n-2}189\cdot \estprev + 256\cdot\opt_{LP}'$.


\Cref{lem:XOS-P to P'} also guarantees the existence of $\widetilde{\pi}\in [0,1]^{\sum_{i,j}|\cT_{ij}|}$ such that $(\widetilde{\pi},w^*,\lambda^*,\hat\lambda^*, \bd^*)$ is a feasible solution to $(P)$. Although we do not know the value $\widetilde{\pi}$, it turns out sufficient to know $\lambda^*$ to compute a simple and approximately optimal mechanism. We compute the prices $\{Q^*_j\}_{j\in[m]}$ using $\lambda^*$ according to \Cref{def:Q_j-XOS}. In particular,
$$Q^*_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta}}\lambda^*_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot\ind[V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}],
$$

and $$2\sum_{j\in[m]} Q^*_j=\opt_{LP}'.$$ According to \Cref{thm:bounding-lp-simple-mech-XOS}, we can construct a two-part tariff mechanism $\Mtpt$ with prices $\{Q^*_j\}_{j\in[m]}$ and a rationed posted price mechanism $\Mpp$ (computed in \Cref{thm:chms10}) in time $\poly(n,m,T)$, such that $$\opt_{LP}'=2\sum_{j\in[m]} Q^*_j= O(\rev(\Mtpt))+O(\estprev).$$

To sum up, we can compute in time $\poly(n,m,T,b,\log (1/\delta))$ a two-part tariff mechanism $\Mtpt$ and a rationed posted price mechanism $\Mpp$, such that $\opt\leq c_1\cdot\rev(\Mpp) + c_2\cdot \rev(\Mtpt)$ for some absolute constants $c_1,c_2>0$ with probability at least $1-\delta-\frac{2}{n}$.
\end{prevproof}




















==> arXiv/sampling.tex <==
\section{Sample Access to the Distribution}\label{sec:sample access}

%\argyrisnote{Argyris: It would be helpful if we also included in Lemma~\ref{lem:caiz17} that core can be bounded by $\Mtpt$.}

In this section, we focus on the case where we have only access to the bidders' distribution. %We consider constrained-additive bidders, and 
Our goal is again to compute an approximately optimal mechanism. Our plan is as follows: (i) for each $i\in[n]$ and $j\in[m]$, take $O(\log(1/\delta)/\varepsilon^2)$ samples from $D_{ij}$, and let $\widehat{D}$ be the uniform distribution over the samples. By the DKW inequality~\cite{DvoretzkyKW56}, $\widehat{D}_{ij}$ and $D_{ij}$ have Kolmogorov distance (\Cref{def:kolmogorov}) no more than $\varepsilon$ with probability at least $1-\delta$. (ii) We then apply our algorithm in \Cref{thm:main XOS-main body}
%\Cref{thm:main}
to compute an RPP or TPT that is approximately optimal w.r.t. distributions $\{\widehat{D}_{ij}\}_{i\in[n],j\in[m]}$. We show that the computed simple mechanism is approximately optimal for the true distributions as well. The proof of Theorem~\ref{thm:sample access} is postponed to \Cref{appx:sample access}.%learn an approximate distribution $\widehat{D}_{ij}$ for each $i$ and $j$ so that  $\hat{D}_{ij}$ and the true distribution $D_{ij}$ are close in Kolmogorov distance. We then apply our algorithm to the approximate distributions $\{\widehat{D}_{ij}\}_{i\in[n],j\in[m]}$.
%Unfortunately we cannot apply Theorem~\ref{thm:bounding-lp-simple-mech} to $\cD$ since we only have sample access to $\cD$. By the existential results of Cai and Zhao \cite{CaiZ17} summarized in Lemma~\ref{lem:caiz17},the revenue of any BIC mechanism $\cM$, can be bounded by a constant time the revenue achieved by a RPSM mechanism and and a TPT mechanism. Note that we can still apply Theorem~\ref{thm:chms10} to efficiently compute a constant factor approximation of the optimal RPSM mechanism, so we are going to turn our attention to efficiently compute mechanisms that guarantee a constant factor approximation of the optimal revenue of a general TPT Mechanism. See Theorem~\ref{thm:sample tpt} for a formal mechanism.

\notshow{
Unfortunately we cannot apply Theorem~\ref{thm:bounding-lp-simple-mech} to $\cD$ to compute an approximately optimal TPT mechanism,
since we only have sample access to $\cD$. 
In order to deal with this issue,
for each agent and each item,
we construct an empirical distribution over values that the agent has.
We measure the distance the distance between our empirical and real distribution in Kolmogorov distance as described in Definition~\ref{def:kolmogorov}.
}

\begin{theorem}\label{thm:sample access}
Suppose all bidders' valuations are constrained additive. If for each $i\in[n]$ and $j\in[m]$,  $D_{ij}$ is supported on {numbers in $[0,1]$ with bit complexity no more than $b$}, %(that is when each bidder's value for a single item is at most $1$),
then for any $\eps>0$ and $\delta>0$, with probability $1-\delta$, we can compute in time {$\poly(n,m,1/\varepsilon,\log (1/\delta),b)$} a rationed posted price mechanism or a two-part tariff mechanism, whose revenue is  at least $c\cdot \opt-O(nm^2\eps)$ for some absolute constant $c$. The algorithm takes $O\left(\frac{\log(nm/\delta)}{\varepsilon^2}\right)$ samples from each $D_{ij}$ and assumes query access to a demand oracle for each bidder.
\end{theorem}





\notshow{
We need another theorem from Brustle et al.~\cite{BrustleCD20} that states that the optimal revenue is Lipschitz with respect to the Kolmogorov distance between the type distributions.


\begin{theorem}[Lipschitz Continuity of the Optimal Revenue, adapted from Theorem 6 in~\cite{BrustleCD20}]\label{thm:continuous of OPT under Prokhorov}
For any distributions $\cD=\bigtimes_{i\in[n], j\in[m]} D_{ij}$ and $\widehat{\cD}=\bigtimes_{i\in[n], j\in[m]} \widehat{D}_{ij}$, where $D_{ij}$ and $D_{ij}$ are supported on $[0,1]$ for every $i\in[n]$ and $j\in [m]$

if $d_K(D_{ij},\widehat{D}_{ij})\leq \varepsilon$ for all $i\in[n]$ and $j\in [m]$, then $$\left \lvert\opt(\DD)-\opt(\hDD)\right\rvert\leq O\left(n\kappa+n\sqrt{m\LL H\kappa}\right),$$
		where $\kappa=O\left(n m \LL H \varepsilon+  m \LL \sqrt{nH\varepsilon}\right)$.
	\end{theorem}
}


\notshow{For this section,
we are going to consider general TPT mechanisms,
whose format is described in Mechanism~\ref{def:general SPEM}.
Notice that Mechanism~\ref{def:general SPEM} is a generalization of Mechanism~\ref{def:constructed-SPEM},
since now the seller can decide the entry fee to by any arbitrary (but deterministic) function that depends on the set of items left.
We prove formally that claim in Observation~\ref{obs:restricted to general tpt}.
We prove in Theorem~\ref{thm:sample tpt} that we can calculate a TPT mechanism $\widehat{\Mtpt}$ and a RPSM $\widehat{\Mpp}$,
whose revenue is within a constant multiplicative and additive factor of the optimal revenue induced by any TPT mechanism.

\argyrisnote{Maybe we should emphasize in Theorem~\ref{thm:bounding-lp-simple-mech} that the types samples to set the entry fee are collected before the mechanism starts and do not change.}
\begin{observation}\label{obs:restricted to general tpt}
For any TPT mechanism (as described in Mechanism~\ref{def:constructed-SPEM}),
When the $i$-th agent arrives at the mechanism,
then the entry fee that the buyer has to pay depends only on the set of items that remain and is chosen deterministic.
That is,
there exists a function $\xi_i:2^{[m]}\rightarrow\mathbb{R}_+$ such that the entry fee imposed to the $i$-th agent when the the set of items that remains is $S$, is $\xi_i(S)$.
\end{observation}

\begin{proof}
Consider an instance of Mechanism~\ref{def:constructed-SPEM} $\Mtpt$,
where $\{p_j\}_{j\in[m]}$ are the posted prices and $t_i$ is the sampled type used to determine the entry fee for the $i$-th agent.
Consider the function $\xi_i:2^{[m]}\rightarrow\mathbb{R}_+$ and define $\xi_i(S)=\max_{S'\subseteq S}\left(v_i(t_i',S')-\sum_{j\in S'}Q_j\right)$.
Then observe that the entry fee imposed at the $i$-th agent when the set of items that remain is exactly $S$ is equal to $\xi_i(S)$.
\end{proof}
}



%We denote by $\Mopt$ the optimal two-part tariff mechanism with anonymous prices $\{p_j\}_{j\in[m]}$ and entry fee functions $\{\xi_i: 2^{[m]}\rightarrow\mathbb{R}_+\}_{i\in[n]}$.
%In the general two-part tariff mechanism,
%when the $i$-th agent arrives,
%the set of items that are still available is $S$.
%The price for an item $j\in S$ is $p_j$ and in order to participate in the mechanism she has to pay an entry fee of $\xi_i(S)$.
%We denote by $\Mopt(\cD)$ the expected revenue from $\Mopt$ when the agents are drawn from $\cD$.


\notshow{

\begin{theorem}\label{thm:sample tpt}
Assume that the agent's valuation is constraint additive and her type is sampled from the distribution $\cD$,
where we only have sample access to it.
Let $\Mtpt$ be the optimal general two part tariff mechanism (as described in Mechanism~\ref{def:general SPEM}).
We can compute in time $\poly\left(n,m,\frac{1}{\eps}\right)$ a RPSM mechanism $\widehat{\Mpp}$ and a general two part tariff mechanism $\widehat{\Mtpt}$  such that there exists constants $c_1,c_2,c_3>0$:
$$
\rev(\Mtpt,\cD) \leq c_1 \rev(\widehat{\Mpp},\cD) + c_2  \rev(\widehat{\Mtpt},\cD) + c_3 n m^2 H \eps
$$

\end{theorem}
\begin{proof}
For each agent $i\in[n]$ and item $j\in[m]$,
we denote by $\widehat{\cD}_{ij}$ the empirical distribution induced by \argyrisnote{$k(\eps)$ samples so that Kolmogorov distance is $\eps$} from $\cD_{ij}$. 
With probability at least $\argyrisnote{smth}$,
for each $i$ and $j$ we have that $||D_{ij}-\widehat{D}_{ij}||_K \leq \eps$.
For the rest of the proof we condition on the event that for each $i\in[n]$ and $j\in[m]$,
$||D_{ij}-\widehat{D}_{ij}||_K \leq \eps$.
For each agent $i\in[n]$ we denote by $\widehat{\cD}_i=\times_{j\in[m]}\widehat{\cD}_{ij}$ and $\widehat{\cD}=\prod_{i\in[n]}\widehat{\cD}_i$.


%We denote by $\Mopt(\widehat{\cD})$ the expected revenue of $\Mopt$ when the agents distribution are sampled from $\widehat{\cD}$.
First we want to relate the expected revenue of $\Mopt$ when we sample the agents type from $\widehat{\cD}$.
We make use of a theorem proved in \cite{CaiD17}.







A corollary of Theorem~\ref{thm:robust mechanism} is the following

$${\Mtpt}({\cD}) \leq \Mtpt(\widehat{\cD}) + 4nm^2H\eps$$


\argyrisnote{I think we should slightly modify the statement of theorem~\ref{thm:bounding-lp-simple-mech}.}
Applying Theorem~\ref{thm:bounding-lp-simple-mech} on the constructed empirical distribution $\widehat{\cD}$ and we get we can compute in time $\poly(n,m,k(\eps))$ a RSPM mechanism $\Mpp$ and a TPT mechanism $\Mtpt$ such that there exists constants $c_1,c_2 \geq 0$ and \argyrisnote{with probability smth} 
%,We can compute in time $\poly(n,m,k)$ a RSPM mechanism $\Mpp$ and a two-part tariff mechanism $\Mtpt$ such that there exists constants $c_1,c_2 \geq 0$:
\begin{align}
\Mtpt(\widehat{\cD}) \leq c_1 \widehat{\Mpp}(\widehat{\cD}) + c_2 \widehat{\Mtpt}(\widehat{\cD})\label{eq:real tpt}
\end{align}
%\end{lemma}

%\begin{corollary}\label{col:opt empirical to opt}[Applyinh Theorem~\ref{thm:bounding-lp-simple-mech} on $\widehat{\Mtpt}$ and $\widehat{\Mpp}$]
Moreover we have that
\begin{align}
\widehat{\Mtpt}(\widehat{\cD}) \leq& \widehat{\Mtpt}({\cD}) +  4nm^2H\eps\label{eq:tpt}\\
\widehat{\Mpp}(\widehat{\cD}) \leq& \widehat{\Mpp}({\cD})+ 4nm^2H\eps \label{eq:pp}
\end{align}
%\end{corollary}
Observe that the first inequality is a direct application of Theorem~\ref{thm:robust mechanism} on $\Mtpt$.

In order to prove the second inequality,
it is enough to observe that if we assume that the agents are unit demand, then the set of RPSM is the same as the set of TPT mechanisms without entry fee.
Thus we can directly apply Theorem~\ref{thm:robust mechanism} and assume that the agents valuation are Unit-demand.

By combining Equation~\ref{eq:real tpt}, Equation~\ref{eq:tpt} and Equation~\ref{eq:pp} we prove the statement.

\end{proof}

We conclude with the main theorem of this section.

\begin{theorem}\label{thm:sample opt}
Assume that the agent's valuation is constraint additive and her type is sampled from the distribution $\cD$,
where we only have sample access to it.
Let $\Mopt$ be the optimal BIC mechanism.
We can compute in time $\poly\left(n,m,\frac{1}{\eps}\right)$ a RPSM mechanism $\widehat{\Mpp}$ and a general two part tariff mechanism $\widehat{\Mtpt}$ such that $\argyrisnote{with probability smth}$ there exists constants $c_1,c_2,c_3>0$:
$$
\rev(\Mopt,\cD) \leq c_1 \rev(\widehat{\Mpp},\cD) + c_2  \rev(\widehat{\Mtpt},\cD) + c_3 n m^2 H \eps
$$
\end{theorem}

\begin{proof}
The proof follows by combining Lemma~\ref{lem:caiz17}, Theorem~\ref{thm:chms10} and Theorem~\ref{thm:sample tpt}.
\end{proof}

}

==> caiz_result.tex <==
\begin{definition}\label{def:core}
For any $i\in [n],j\in [m]$, let $\cV_{ij}^0 = \{ V_{ij}(t_{ij}): t_{ij} \in \cT_{ij}\}$. For any feasible interim allocation $\sigma$, and non-negative numbers {$\tilde{\vBeta}=\{\tilde{\beta}_{ij}\in \cV_{ij}^0\}_{i\in[n],j\in[m]}$, $\vC=\{c_i\}_{i\in[n]}$} and $\vr=\{r_{ij}\}_{i\in [n],j\in [m]}\in [0,1]^{nm}$ (which we refer to as the dual parameters), %~\footnote{$\tilde{\vBeta}$, $\vC$, and $r$ are the dual parameters that we refer to in the introduction.}
define $\core(\sigma,\tilde{\vBeta},\vC,\vr)$ as the welfare under allocation $\sigma$ truncated at $\tilde{\beta}_{ij}+c_i$ for every $i,j$.
%, with rebate ratio $r$ (see the remark below). 
Formally, $$\core(\sigma,\tilde{\vBeta},\vC,\vr)=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \left(\ind[t_{ij}< \tilde{\beta}_{ij}+c_i]+r_{ij}\cdot \ind[t_{ij}= \tilde{\beta}_{ij}+c_i] \right)$$
if the buyers have constrained-additive valuations, and
$$\core(\sigma,\tilde{\vBeta},\vC,\vr)=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}\gamma_{ij}^S(t_i)\cdot \left(\ind[V_{ij}(t_{ij})< \tilde{\beta}_{ij}+c_i]+r_{ij}\ind[V_{ij}(t_{ij})= \tilde{\beta}_{ij}+c_i] \right)$$ if the buyers have XOS valuations.
Here $\gamma_{ij}^S(t_i)=\alpha_{ij}^{k^*(t_i,S)}(t_{ij})$, where $\displaystyle k^*(t_i,S)=\arg\max_{k\in[K]}\big(\sum_{j\in S}\alpha^k_{ij}(t_{ij})\big)$.
\end{definition}

\begin{lemma}\cite{CaiZ17}\label{lem:caiz17}
Given any BIC and IR mechanism $\cM$, there exists \textbf{(i)} a feasible interim allocation $\sigma$,\footnote{Note that when buyers have constrained-additive valuations, it suffice to take $\sigma$ to be the interim allocation rule of $\cM$. For XOS valuations, $\sigma$ will be the interim allocation of a modified version of $\cM$. See Section~5 in~\cite{CaiZ16a} for details.} where $\sigma_{iS}(t_i)$ is the interim probability for buyer $i$ to receive exactly bundle $S$ when her type is $t_i$, \textbf{(ii)} non-negative numbers {$\tilde{\vBeta}^{(\sigma)}=\{\tilde{\beta}_{ij}^{(\sigma)}\in \cV_{ij}^0\}_{i\in[n],j\in[m]}$, $\vC^{(\sigma)}=\{c_i^{(\sigma)}\}_{i\in[n]}$} %\argyrisnote{can we say instead $\{\tilde{\beta}_{ij}\in \cV_{ij}^0\}_{i,j}, \{c_i\}_{i\in[n]}$?}
 and $\vr^{(\sigma)}\in [0,1]^{nm}$ that depend on $\sigma$, and \textbf{(iii)} a two-part tariff mechanism $\cM_1^{(\sigma)}$ such that %\yangnote{Yang: We need to make sure all the $\tilde{\beta}_{ij}$ are in $\cV_{ij}$ and all $c_i$ are in $\Delta_i$. I think it's fine to say $\tilde{\beta}_{ij}\in \cV^0_{ij}$, and we only choose $c_i$'s such that for at least one item $j$, $\tilde{\beta}_{ij}+c_i \in \cV^0_{ij}$.}
\begin{enumerate}
    \item $\sum_{i\in[n]} \left(\Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde\beta_{ij}^{(\sigma)}]+r_{ij}^{(\sigma)}\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde\beta_{ij}^{(\sigma)}]\right)\leq \frac{1}{2}$.
    \item $\frac{1}{2}\cdot\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\sigma_{iS}(t_i)\leq \Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde\beta_{ij}^{(\sigma)}]+r_{ij}^{(\sigma)}\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde\beta_{ij}^{(\sigma)}],\forall i,j$.
    \item $\rev(\cM)\leq 28\cdot \prev+4\cdot\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$.
    \item $\sum_{i\in [n]} c_i^{(\sigma)}\leq 8\cdot \prev$.
    \item $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})\leq 64\cdot \prev + 8\cdot \rev(\cM_1^{(\sigma)})$.
\end{enumerate}
\end{lemma}

==> generalized_sampling_polytope.tex <==
\section{Multiplicative Approximation of Down-Monotone and Boxable Polytopes}\label{sec:multi-approx-polytope}


In this section, we prove a result that works for more general polytopes. Throughout this section, we assume that the polytope we consider is convex and \emph{down-monotone}. Formally, a polytope $\cP\subseteq [0,1]^d$ is down-monotone if and only if for every $\bx\in \cP$ and $\textbf{0}\leq \bx'\leq \bx$, we have $\bx'\in \cP$.
To state our result for more general polytopes, we need the following definitions.

\begin{definition}
For any two sets $A,B \subseteq \mathbb{R}^d$,
we denote by $A+B$ the \emph{Minkowski addition} of set $A$ and set $B$ where:
$$A+B = \{a + b : a \in A\land b \in B\}
$$

Note that if both $A$ and $B$ are convex, then $A+B$ is also convex.
\end{definition}

\begin{definition}
Let $\ell$ be a finite integer. For any set of convex sets $\{\cP_i\}_{i\in [\ell]}$ and a distribution $\cD=\{q_i\}_{i\in[\ell]}$ %over the elements in $[N]$.
, the set $\cP = \sum_{i\in[\ell]}q_i \cP_i$
is called the mixture of $\{\cP_i\}_{i\in [\ell]}$ over distribution $\cD$.
\end{definition}


\begin{definition}\label{def:truncated polytope}
%\argyrisnote{Argyris: I don't think downward closed refer to polytopes? I named it lower-closed instead}
Let $\cP,\cQ\subseteq [0,1]^d$ be down-monotone polytopes. For each coordinate $j\in[d]$,
we define the width of $\cP$ at coordinate $j$ as %$l_j(\cP)=\max_{\bx\in \cP}x_j$.
{$l_j(\cP)=\sup_{\bx\in \cP}x_j$.}
%We say that $\cP$ is lower-closed if for each $p \in \cP$,
%then for $p'\in [0,1]^d$ such that
%$$
%0\leq p'(j)\leq p(j) \quad \forall j \in[d]
%$$
%we have that $p' \in \cP$.
%Moreover w
For any $\eps>0$, we define the {($\eps,\cQ$)-truncated polytope of $\cP$ (denoted as $\cP^{tr(\eps,\cQ)}$)} in the following way: $\bx\in \cP^{tr(\eps,\cQ)}$ if and only if there exists $\bx'\in \cP$ such that $x_j=x_j'\cdot \ind[l_j(\cQ)\geq \eps],\forall j\in [d]$.
%For each $\bx\in \cP$, then for the element $p'\in [0,1]^d$ such that
%$$
%p'(i)=
%\begin{cases}
%p(i) \quad &\text{if $\eps \leq l_i(\cP)$} \\
%0 & \text{o.w.}
%\end{cases}\quad \forall i\in[d]
%$$
%Note that if $\cP$ is lower-closed,
%then for each $\eps>0$, $\cP_\eps^t \subseteq \cP$.
We notice that since $\cP$ is down-monotone, $\cP^{tr(\eps,\cQ)}\subseteq \cP$. Moreover, $\cP^{tr(\eps,\cQ)}$ is convex if $\cP$ is convex.
We also denote as $\cP^{tr(\eps)}= \cP^{tr(\eps,\cP)}$.
\end{definition}


\begin{definition}\label{def:box polytope}
Let $\cP\subseteq [0,1]^d$.
%First we are going to describe a way to partition the coordinates of $\cP$.
%For each $i\in[d]$,
%we say that the $i$-th coordinate of $\cP$ is $\eps$-good if $l_j(\cP) \geq \eps$. 
%We say that the $i$-th coordinate of $\cP$ is $\eps$-bad if it is not $\eps$-good.
For any $\eps>0$, define the $\eps$-box polytope $\pbox$ of $\cP$ as follows: 
{$\pbox=\{\bx\subseteq [0,1]^d: x_j\leq \min\left( \eps,l_j(\cP)\right),\forall j\in [d]\}$.} Clearly, $\pbox$ is convex.
%For any element $p\in [0,\eps]^d$ such that:
%$$
%p(i) \leq
%\min\left( \eps,l_i(\cP)\right) \quad \forall i \in[d]
%$$
%then $p\in \cP^b_\eps$.
%Under some natural polytopes $\cP$,
%we can prove that for sufficiently small $\eps$,
%then $\cP_\eps^b \subseteq \cP$.
%This property is going to be very usefull.
%\mingfeinote{Mingfei: What does this sentence mean?}
\end{definition}


\Cref{thm:special case of multiplicative approx-main body} is the main theorem of this section. We prove that if $\cP$ is a mixture of a set of down-monotone, convex polytope, and $\cP$ contains the polytope $c\cdot\pbox$ for some {$c\leq1$}, then there exists another down-monotone, convex polytope $\widehat{\cP}$ sandwiched between $c/6\cdot \cP$ and $\cP$. And more importantly, we have an efficient separation oracle for $\widehat{\cP}$. 

\begin{theorem}\label{thm:special case of multiplicative approx-main body}
Let $\ell$ be a positive integer. Let $\cP \subseteq [0,1]^d$ be a mixture of $\{\cP_i\}_{i\in[\ell]}$ over distribution $\cD=\{q_i\}_{i\in [\ell]}$,
where for each $i\in[\ell]$, $\cP_i\subseteq [0,1]^d$ is a down-monotone, convex polytope. 
Assume for all $i$,
the bit complexity of each corner of $\cP_i$ is at most $b$. Suppose for every $i\in [\ell]$, there is an algorithm $\mathcal{A}$ that can maximize any linear objective over $\cP_i$, i.e. solve $\max\{\textbf{a}\cdot \bx:\bx\in \cP_i\}$ for any $\textbf{a}\in \mathbb{R}^d$ with bit complexity $y$, in time $\mathcal{A}(y)$.
Suppose $c\cdot\pbox\subseteq \cP$ for some $\eps>0$ and absolute constant $c\in (0,1]$, then for any $\delta\in (0,1)$ there is an algorithm (with running time $\poly(d,\frac{1}{\eps},\log(1/\delta))$) that with probability at least $1-\delta$, constructs a down-monotone, convex polytope $\widehat{\cP}\in [0,1]^{d}$ using $\poly(d,\frac{1}{\eps},\log(1/\delta))$ samples from $\cD$, such that
\begin{enumerate}
\item $\frac{c}{6}\cdot\cP\subseteq \widehat{\cP}\subseteq \cP$. 
\item There exists a separation oracle $SO$ for $\widehat{\cP}$. The running time of $SO$ on any input with bit complexity $b'$ is $\poly(d,b,b',\frac{1}{\eps},\log(1/\delta),\mathcal{A}(\poly(d,b,b',\frac{1}{\eps},\log(1/\delta))))$.
\end{enumerate}
\end{theorem}


%\mingfeinote{Mingfei: Maybe it's a good idea to first verify that $W_i$ satisfies all the constraints and apply it to solve our problem, before giving the proof.}
%\argyrisnote{Argyris: I agree, maybe we can create a subsection for the proof of the theorem and devote the rest of this section for its application to contraint additive.}


The complete proof of \Cref{thm:special case of multiplicative approx-main body} is postponed to \Cref{subsec:proof_general_polytope}. Here we will only give a sketch of the proof. We first prove that if a down-monotone, convex polytope $\cP$ contains $c$ times the $\eps$-box polytope, then the convex set $\frac{c}{2}(\ptruncated + \pbox)$ is sandwiched between $\frac{c}{2}\cP$ and $\cP$ (\Cref{lem:boxable polytope contained} in \Cref{subsec:proof_general_polytope}). Now it's sufficient to design the polytope $\widehat{\cP}$ that is close to $\frac{c}{2}(\ptruncated + \pbox)$. For $\eps>0$ and every $i\in [\ell]$, let $\ptruncatedI$ be the $(\eps,\cP)$-truncated polytope of $\cP_i$. It's clearly that $\ptruncated$ is a mixture of $\{\ptruncatedI\}_{i\in [\ell]}$ over distribution $\cD$. We will construct our polytope $\widehat{\cP}$ using $\ptruncatedEmp$, the mixture of $\{\ptruncatedI\}_{i\in [\ell]}$ over the empirical distribution $\widehat{\cD}$. Cai et al.~\cite{CaiDW12b,CaiDW13a} proved that with polynomially many samples from $\cD$, $\ptruncatedEmp$ and $\ptruncated$ are close within an additive error $\eps$ in the $\ell_\infty$-norm (\Cref{thm:approx mixture} in \Cref{subsec:proof_general_polytope}). Then we choose $\widehat{\cP}=\frac{c}{3}(\ptruncatedEmp + \pbox)$ and prove that $\widehat{\cP}$ is a multiplicative approximation of $\cP$.
%$\frac{c}{2}(\ptruncated +\pbox)$. %\mingfeinote{pin down the constant here when reading the proof.}
%within a multiplicative factor, in any direction.     

To apply \Cref{thm:special case of multiplicative approx-main body} to the marginal reduced form polytope $W_i$, we first show that $W_i$ is a mixture of a set of polytopes $\{W_{i,t_i}\}_{t_i\in \cT_i}$ over $D_i$, where each $W_{i,t_i}$ contains the marginal reduced form of all feasible allocations for a specific type $t_i$ (\Cref{def:W_i-t_i} in \Cref{subsec:proof_general_polytope}).
%since the marginal reduced form $\widehat{w}_i$ is implemented by a feasible allocation $\{\sigma_S(t_i)\}_S$ where $t_i\sim D_i$.  
For every $t_i$, we can maximize any linear objective over $W_{i,t_i}$ via a query to the demand oracle (or a scalable demand oracle for XOS buyers). Finally, we prove that $W_i$ contains ($c$ times) the $\eps$-box polytope of itself, for some $c\in (0,1)$ and $\eps>0$. 





==> intro.tex <==
\section{Introduction}\label{sec:intro}
Revenue-maximization in multi-item auctions has been recognized as a central problem in Economics and more recently in Computer Science. %In the problem, a seller is selling $m$ heterogeneous items to $n$ bidders, where the $i$-th bidder's type is drawn independently from their own distribution $D_i$. The goal is to design a mechanism to maximize the seller's expected revenue. 
While Myerson's celebrated work showed that a simple mechanism is optimal in single-item settings~\cite{Myerson81}, the optimal multi-item mechanism is known to be prohibitively complex and notoriously difficult to characterize even in basic settings. Facing the challenge, a major research effort has been dedicated to understanding the computational complexity for finding an approximately revenue-optimal  mechanism in multi-item settings. Despite significant progress%both in terms of efficient algorithms and intractability results
, there is still a substantial gap in our understanding of the problem, % even in the natural item-independent setting.
for example, in the natural and extensively studied \emph{item-independent} setting, first introduced in the influential paper by Chawla, Hartline, and Kleinberg~\cite{ChawlaHK07}. 


Formally, the item-independent setting is defined as follows: A seller is selling $m$ heterogeneous items to $n$ bidders, where the $i$-th bidder's type is drawn independently from an $m$-dimensional product distribution $D_i=\bigtimes_{j\in[m]} D_{ij}$.\footnote{$[m]$ denotes $\{1,2,...,m\}$.  $D_{ij}$ is the distribution of bidder $i$'s value for item $j$. The definition is extended to XOS in \Cref{sec:prelim}.} We only understand the computational complexity of finding the revenue-optimal mechanism in the item-independent setting for the two most basic valuations: unit-demand and additive valuations. First, we know that finding an exactly optimal mechanism is computationally intractable even for a single bidder with either unit-demand~\cite{chen2015complexity} or additive valuation~\cite{DaskalakisDT14}. Second, there exists a polynomial time algorithm that computes a mechanism whose revenue is at least a constant fraction of the optimal revenue when bidders have unit-demand~\cite{ChawlaHMS10,ChawlaMS15} or additive valuations~\cite{Yao15}. However, unit-demand and additive valuations are only two extremes within a broader class of value functions known as the constrained additive valuations, where the bidder's value is additive subject to a downward-closed feasibility constraint.\footnote{A bidder has constrained-additive valuation if the bidder's value for a bundle $S$ is defined as $\max_{V\in 2^S\cap \mathcal{I}}\sum_{j\in V} t_j$, where $t_j$ is the bidder's value for item $j$, and $\mathcal{I}$ is a downward-closed set system over the items specifying the feasible bundles. Note that constrained-additive valuations contain familiar valuations such as additive,  %($\mathcal{I}=[m]$),
unit-demand, %($\mathcal{I}$ is the collection of all singletons of $[m]$),
or matroid-rank valuations. %($\mathcal{I}$ is a matroid).
} Furthermore, all constrained additive valuations are contained in an even more general class known as the XOS valuations. Beyond unit-demand and additive valuations, our understanding was limited, and we only knew how to compute an approximately optimal mechanism when bidders are symmetric, i.e., all $D_i$'s are identical~\cite{ChawlaM16,CaiZ17}. Finding a polynomial time algorithm for asymmetric bidders was thus raised as a major open problem in both~\cite{ChawlaM16,CaiZ17}. In this paper, we resolve this~open~problem.

\medskip \noindent \hspace{0.7cm}\begin{minipage}{0.92\columnwidth}
\begin{enumerate}
\item[{\bf Result I:}] For the item-independent setting with (asymmetric) XOS bidders, %~\footnote{The item-independence setting is extended to XOS valuations in~\cite{RubinsteinW15}.}
there exists an algorithm that computes a Dominant Strategy Incentive Compatible (DSIC) and Individually Rational (IR) mechanism whose revenue is at least $c\cdot\opt$ for some absolute constant $c>0$, where $\opt$ is the optimal revenue achievable by any Bayesian Incentive Compatible (BIC) and IR mechanism. Our algorithm has running time polynomial in %$n$, $m$, and 
$\sum_{i\in[n],j\in[m]}|\cT_{ij}|$, where $\cT_{ij}$ is the support~of~$D_{ij}$. See \Cref{thm:main XOS-main body} for the formal statement.
\end{enumerate}
\end{minipage}

\noindent %Our algorithm assumes query access to a demand oracle when the bidders' valuations are constrained additive. When the bidders' valuations are XOS, our algorithm requires a more powerful oracle, which we refer to as the adjustable demand oracle (\Cref{def:adjustable demand oracle}). In~\Cref{lem:example_adjustable_oracle}, we show that the stronger oracle is necessary for our approach. 

%Substantial progress has been made on this problem. For example, a line of works~\cite{AlaeiFHHM12,CaiDW12a,CaiDW12b,CaiDW13a,CaiDW13b,cai2021efficient} provide algorithms for finding almost revenue-optimal mechanisms in multi-item settings in time polynomial in the total number of types, i.e., $\sum_{i\in [n]}|\supp(D_i)|$ ($\supp(D_i)$ denotes the support of $D_i$). However, the number of types for any bidder could easily be exponential in the number of items making these algorithms prohibitively slow. For unstructured type distributions, such dependence is unavoidable as even describing the distributions requires time $\Omega(\sum_{i\in [n]}|\supp(D_i)|)$, but what if $D_i$ is a distribution with structure and permits a more succinct description, e.g., a product distribution? Indeed one of the biggest challenges in Bayesian Algorithmic Mechanism Design is designing algorithms to compute (approximately) optimal mechanisms that are not brute-force in the size of the bidder type space.

%In this paper, we study the central problem in a classical setting, where each bidder's values for the $m$ items are sampled independently.

%In particular, if bidders' type distributions are arbitrary, even representing an approximately optimal mechanism for a single bidder requires description size that is exponential in the number of items~\cite{dughmiLN14}. 

%Despite the challenge, we have witnessed significant progress in computing the optimal mechanism. We now have algorithms for finding almost revenue-optimal mechanisms in multi-item settings in time polynomial in the total number of types, i.e., $\sum_{i\in [n]}|\supp(D_i)|$ ($\supp(D_i)$ denotes the support of $D_i$)~\cite{AlaeiFHHM12,CaiDW12a,CaiDW12b,CaiDW13a,CaiDW13b,cai2021efficient}. However, the number of types for any bidder could easily be exponential in the number of items.  

%These algorithms target settings where bidders are independent and run in time polynomial in the sum of the number of types for each bidder. However, the number of types for a bidder could easily be exponential in the number of items. , which is $\sum_{i\in[n]}\left(\prod_{j\in[m]} |\cT_{ij}|\right)$ in our setting. Comparing to these algorithms, our algorithm achieves an exponential speed-up in the item-independence setting. 


%Removed vspace here\vspace{-.1in}
\paragraph{Computing Approximately Optimal Mechanisms under Structured Distributions.} When the bidders' types are drawn from arbitrary distributions, a line of works provide algorithms for finding almost revenue-optimal mechanisms in multi-item settings in time polynomial in the total number of types, i.e., $\sum_{i\in [n]}|\supp(D_i)|$ ($\supp(D_i)$ denotes the support of $D_i$)
~\cite{AlaeiFHHM12,CaiDW12a,CaiDW12b,CaiDW13a,CaiDW13b,cai2021efficient}. 

However, the total number of types could be exponential in the number of items, e.g., there are $\sum_{i\in [n]}\left(\prod_{j\in[m]} |\cT_{ij}|\right)$ types in the item-independent case, making these algorithms unsuitable. For unstructured type distributions, such dependence is unavoidable as even describing the distributions requires time $\Omega\left(\sum_{i\in [n]}|\supp(D_i)|\right)$. What if the type distributions are \emph{structured and permit a more succinct description}, e.g., product measures? Arguably, high-dimensional distributions  that arise in practice (such as bidders' type distributions in multi-item auctions) are rarely arbitrary, as arbitrary high-dimensional distributions cannot be represented or learned efficiently; see e.g.~\cite{Daskalakis18} for a discussion. Indeed, one of the biggest challenges in Bayesian Algorithmic Mechanism Design is designing algorithms to compute (approximately) optimal mechanisms that are not brute-force in the size of the bidder type space when the type distributions are structured. In this paper, we develop computational tools to exploit the item-independence to obtain an exponential speed-up in running time. 

%When the type distributions can be represented as other structured distributions such as Bayesian networks, Markov Random Fields, or Topic Models, recent results show how to utilize the structure to improve the learnability, approximability, and communication complexity of multi-item auctions~\cite{BrustleCD20,CaiO21,cai2021recommender}.  We believe that tools developed in this work would be useful to obtain similar improvement in terms of the computational complexity for computing approximately optimal mechanisms for structured distributions beyond product measures. 

%There is a line of works dedicated to designing algorithms for finding almost revenue-optimal mechanisms~\cite{AlaeiFHHM12,CaiDW12a,CaiDW12b,CaiDW13a,CaiDW13b,cai2021efficient}. These algorithms target settings where bidders are independent but items may be correlated, and they all run in time polynomial in the total number of types, which is $\sum_{i\in[n]}\left(\prod_{j\in[m]} |\cT_{ij}|\right)$ in our setting. Comparing to these algorithms, our algorithm achieves an exponential speed-up in the item-independent setting. 



%Removed vspace here\vspace{-.15in}
\paragraph{Simple vs. Optimal.} An additional feature of our algorithm is that the mechanisms computed have a simple structure. It is either a \emph{posted price mechanism} or a \emph{two-part tariff mechanism}. Given the description of the two mechanisms, it is clear that both of them are~DSIC~and~IR. %and guarantees that the better of the two achieves at least a constant fraction of the optimal revenue.

%Removed vspace here\vspace{-.15in}
\paragraph{Rationed Posted Price Mechanism (RPP)} There is a price $p_{ij}$ for bidder $i$ to purchase item $j$. The bidders arrive in some arbitrary order, and each bidder can purchase \emph{at most one} item among the available ones at the given price.\footnote{Usually, posted price mechanisms do not restrict the maximum number of items a bidder can buy. We consider a rationed version of posted price mechanism to make the computational task easy.} 

%Removed vspace here\vspace{-.15in}
\paragraph{Two-part Tariff Mechanism (TPT)}  All bidders face the same set of prices $\{p_j\}_{j\in[m]}$. Bidders arrive in some arbitrary order. For each bidder, we show her the available items and the associated price for each item, then ask her to pay an entry fee depending on the bidder's identity and the available items. If the bidder accepts the entry fee, she proceeds to purchase any of the available items at the given prices; if she rejects the entry fee, then she pays nothing and receives nothing.

A recent line of works focus on designing simple and approximately optimal mechanisms% approximately revenue-optimal and have achieved great success
~\cite{ChawlaHK07,ChawlaHMS10,Alaei11,HartN12,KleinbergW12,CaiH13,BILW14,Yao15,RubinsteinW15,CaiDW16,ChawlaM16,CaiZ17}. The main takeaway of these results is that in the item-independent setting, there exists a simple mechanism that achieves a constant fraction of the optimal revenue. The most general setting where such a simple $O(1)$-approximation is known is exactly the setting in \textbf{Result I}, where bidders have XOS valuations~\cite{CaiZ17}. More specifically, \cite{CaiZ17} show that there is a RPP or TPT that achieves a constant fraction of the optimal revenue, however their result is purely existential and does not suggest how to compute these simple mechanisms. Our result makes their existential result constructive.

%Despite being structurally appealing, these results are largely non-constructive in multi-bidder settings except for basic cases, either when bidders are symmetric~\cite{ChawlaM16, CaiZ17} or when they have additive or unit-demand valuations~\cite{ChawlaHMS10, Yao15, CaiDW16}. Making these simple vs. optimal results constructive in the constrained-additive setting is posed as an open problem in~\cite{ChawlaM16, CaiZ17}.

%We resolve this open problem by providing a polynomial time algorithm to compute simple mechanisms that achieve a constant fraction of the optimal revenue in multi-item auctions when bidders have XOS valuations, matching the most general existential (but non-constructive) result by Cai and Zhao~\cite{CaiZ17}.~\footnote{This was called the \emph{anonymous sequential posted price with entry fee mechanism (ASPE)} in Cai and Zhao~\cite{CaiZ17}.}   

%To state our result, we first specify the setting and how the input is provided. We use the following setting as the running example: selling $m$ items to $n$ bidders with constrained-additive valuations in the item-independent setting.

%A seller is selling $m$ items to $n$ bidders with constrained-additive valuations in the item-independent setting.~\footnote{A bidder has constrained additive valuation if the bidder's value for a bundle $S$ is defined as $\max_{V\in 2^S\cap \mathcal{I}}\sum_{j\in V} t_j$, where $t_j$ is the bidder's value for item $j$, and $\mathcal{I}$ is a downward-closed set system over the items specifying the feasible bundles. Note that constrained-additive valuations contain familiar valuations such as additive, unit-demand, or matroid-rank valuations.}
%Since constrained-additive valuations are already rich and present all the obstacles we need to overcome, we use them as the running example in the introduction. 
%Item-independence means that each bidder $i$'s value for each item $j$ is drawn independently from a known distribution $D_{ij}$. The input to our problem is simply the~product~distribution~$\bigtimes_{i\in[n],j\in[m]} D_{ij}$. 



Finally, combining our result with the learnability result for multi-item auctions in~\cite{CaiD17}, we can extend our algorithm to the case when we only have sample access to the distributions.

\medskip \noindent \hspace{0.7cm}\begin{minipage}{0.92\columnwidth}
\begin{enumerate}
\item[{\bf Result II:}] For constrained-additive bidders, there exists an algorithm that computes a simple, DSIC, and IR mechanism whose revenue is at least $c\cdot\opt-O(\varepsilon \cdot \poly(n,m))$ for some absolute constant $c>0$ in time polynomial in $n$, $m$, and $1/\varepsilon$, given sample access to bidders' type distributions, and assuming each bidder's value for each item lies in $[0,1]$. See \Cref{thm:sample access} for the formal~statement.
\end{enumerate}
\end{minipage}

\vspace{0.07in}
Due to space limit, we only include the formal statements of our results and proof sketches. All details can be found in the full version of the paper on arXiv~\url{https://arxiv.org/abs/2111.03962}.
%Removed vspace here\vspace{-.1in}

%\medskip
%\noindent An important implication of \textbf{Result II} is that our algorithm can be used to handle continuous distributions with a small additional additive error.

%Given the entry fee and item prices, the decision making for the buyer is straightforward, as she only accepts the entry fee when the surplus for winning her favorite bundle is larger than the entry fee. T

\subsection{Our Approach and Techniques}\label{subsec:technique}
Our main technical contribution is \emph{a novel relaxation of the revenue optimization problem that can be solved approximately in polynomial time} and \emph{an accompanying rounding scheme that converts the solution to a simple and approximately optimal mechanism}.\footnote{An influential framework known as the ex-ante relaxation has been widely used in Mechanism Design, but is insufficient for our problem. See \Cref{sec:exante} for a detailed discussion.} Our first step is to replace the objective of revenue with a duality-based benchmark of the revenue proposed in~\cite{CaiZ17}. One can view the new objective as maximizing the virtual welfare, similar to Myerson's elegant solution for the single-item case. The main difference is that, while one can use \emph{a fixed set of virtual valuations for any allocation} in the single-item case, due to the multi-dimensionality of our problem, \emph{the virtual valuations must depend on the allocation, causing the virtual welfare to be a non-concave function in the allocation}. In this paper, we develop algorithmic tools to concavify and approximately optimize the virtual welfare maximization problem. We believe our techniques will be useful to address other similar challenges in Multi-Dimensional Mechanism Design.


More specifically, for every BIC and IR mechanism $\cM$ with allocation rule $\sigma$ and payment rule $p$, one can choose a set of \emph{dual parameters}  $\theta(\sigma)$ based on $\sigma$ to construct an upper bound $U(\sigma,\theta(\sigma))$ for the revenue of $\cM$. We refer to $\theta$ as the dual parameters because $\theta$ corresponds to a set of ``canonical'' dual variables, which can be used to derive the virtual valuations via the Cai-Devanur-Weinberg duality framework~\cite{CaiDW16}. The upper bound  $U(\sigma,\theta(\sigma))$ is then simply the corresponding virtual welfare. The computational problem is to find an allocation $\sigma$ that (approximately) maximizes $U(\sigma,\theta(\sigma))$. With such a $\sigma$, we could use the result in~\cite{CaiZ17} to convert it to a simple and approximately optimal mechanism. Unfortunately, the function $U(\sigma,\theta(\sigma))$ is highly non-concave in $\sigma$,\footnote{See \Cref{sec:core non-concavity} for an example of the non-concavity of the function. } and thus hard to maximize efficiently. See~\Cref{sec:tour to LP} for a detailed~discussion.



%The starting point of our algorithm is the existential result by Cai and Zhao~\cite{CaiZ17}, in which they show that there exists a \emph{rationed posted price mechanism} or a \emph{two-part tariff mechanism} that achieves at least a constant fraction of the optimal revenue when bidders have XOS valuations.%~\footnote{All constrained-additive valuations are XOS valuations as well.} 
%Using the result from~\cite{ChawlaHMS10}, we can compute in polynomial time a RPP that is a constant factor approximation to the optimal RPP (Theorem~\ref{thm:chms10}), so the remaining challenge is how to compute the TPT that is guaranteed to generate high revenue by Cai and Zhao~\cite{CaiZ17}. It is unclear how one can directly find an approximately optimal TPT among all TPTs, as (i) there are exponentially many parameters associated with a TPT (the entry fees depend on the set of available items), and (ii) the revenue of a TPT relies on the parameters in a highly complex and non-concave way, so the natural idea is to make the non-constructive proof by Cai and Zhao~\cite{CaiZ17} constructive.

%We first provide a 10,000-foot view of the analysis by Cai and Zhao~\cite{CaiZ17}. \textbf{Step (i):} They show that for any BIC and IR mechanism $M$, one can choose a set of ``canonical'' dual variables and construct an upper bound of the revenue of $M$ via the Cai-Devanur-Weinberg duality framework~\cite{CaiDW16}. In particular, any set of canonical dual variables is indexed by a set of parameters which we refer to as the \emph{dual parameters}, and they argue that for any mechanism $M$, and any set of dual parameters $\theta$, the revenue of $M$ is upper bounded by $\core(M,\theta)$.~\footnote{Intuitively, $\core(M,\theta)$ corresponds to the welfare of $M$ under truncated valuations, where the truncation depends on $\theta$. Strictly speaking, the revenue of $M$ is upper bounded by a constant times $\core(M,\theta)$ plus a constant times $\prev$, where $\prev$ is the highest revenue achievable by any RPP. Since we know how to approximate $\prev$, we omit it in our discussion.} \textbf{Step  (ii):} They show that there is a mapping $f$ that maps a mechanism $M$ to a set of dual parameters $\theta=f(M)$, such that $\core(M,f(M))$ can be approximated by a TPT. Additionally, this TPT can be efficiently constructed given $M$ and $f(M)$. To make their result constructive, one only needs to find a mechanism $M$ that approximately maximizes the upper bound $\core(M,f(M))$ over all mechanisms. Unfortunately, the function $\core(M,f(M))$ is highly non-concave in $M$, and the only setting that Cai and Zhao~\cite{CaiZ17} manage to approximate optimize $\core(M,f(M))$ is when the bidders have identical distributions, as the function $\core(M,f(M))$ can be greatly simplified due to the symmetry among~bidders. \todo[inline]{Shrink the above two paragraphs and move the rest to appendix.}
%Removed vspace here\vspace{-.15in}
\paragraph{LP Relaxation via Lifting.} We further relax our objective, i.e., $U(\sigma,\theta(\sigma))$, to obtain a computationally tractable problem. One specific difficulty in optimizing $U(\sigma,\theta(\sigma))$ comes from the fact that $\theta(\sigma)$ is highly non-linear in $\sigma$. We address this difficulty in two steps. In the first step of our relaxation, we flip the dependence of $\sigma$ and $\theta$ by relaxing the problem to the following two-stage optimization problem (\Cref{fig:LP-fixed-parameter}): 

\vspace{.05in}
\textbf{- Stage I:} Maximize $H(\theta)$ subject to some constraints. $H(\theta)$ is the optimal value of the Stage II~problem.

\vspace{.05in}

\textbf{- Stage II:} Maximize an LP over $\sigma$ with $\theta$-dependent constraints.

\vspace{.05in}


%we disentangle $\sigma$ and $\theta$ in the objective $U(\cdot,\cdot)$, and represent their dependence using joint constraints. 
\noindent This makes the problem much more structured and significantly disentangles the complex dependence between $\sigma$ and $\theta$. Yet we still do not know how to solve it efficiently. In the second step of our relaxation, we merge the two-stage optimization into a single LP. In particular, we \emph{lift the problem to a higher dimensional space and optimize over joint distributions of the allocation $\sigma$ and the dual parameters $\theta$ via an LP (\Cref{fig:bigLP}).}  Since the number of dual parameters is already exponential in the number of bidders and the number of items, it is too expensive to represent such a joint distribution explicitly. We show it is unnecessary to search over all joint distributions. By leveraging the independence across bidders and items, it suffices for us to consider a set of succinctly representable distributions -- the ones whose marginals over the dual parameters are product measures. See \Cref{sec:tour to LP} for a more detailed discussion on the development of our relaxation. 


%Removed vspace here\vspace{-.15in}
\paragraph{``Rounding'' any Feasible Solution to a Simple Mechanism.}Can we still approximate the optimal solution of the LP relaxation using a simple mechanism? Unfortunately, the result from~\cite{CaiZ17} no longer applies. %Obviously, the optimum solution of the LP is an upper bound of $\core(M,f(M))$ for any mechanism $M$,~\footnote{Recall that $\core(M,f(M))$ is an upper bound of the revenue of $M$, so it suffices to produce a simple mechanism to approximate the optimum of the LP relaxation.} as $(M,f(M))$ is a feasible solution of our LP. However, as the optimum solution may correspond to a joint distribution of mechanisms and dual parameters, it is not clear that it can still be approximated by a simple mechanism. 
We provide a \emph{generalization of~\cite{CaiZ17}}, that is, given any feasible solution of our LP relaxation, we can construct in polynomial time a simple mechanism whose revenue is at least a constant fraction of the objective value of the feasible solution (\Cref{thm:bounding-lp-simple-mech}). Our proof 
%\argyrisnote{Argyris: removed reference to appendix}
%(in \Cref{sec:proof of bounding LP with simple mech})
provides several novel ideas to handle the new challenges due to the relaxation, which may be of independent~interest.
%Removed vspace here\vspace{-.15in}


\paragraph{Marginal Reduced Forms.} We deliberately postpone the discussion on  how we represent the allocation of a mechanism until now. A widely used succinct representation a mechanism $\cM$ is known as the reduced form or the interim allocation rule:
$\{r_{ij}(t_i)\}_{i\in[n],j\in[m], t_{i}\in\bigtimes_{j\in[m]}\cT_{ij}}$ where $r_{ij}(t_i)$ is the probability for bidder $i$ to receive item $j$ when \emph{her type is $t_i=(t_{i1},\ldots, t_{im})$}~\cite{CaiDW12a}. Despite being more succinct than the ex-post allocation rule, the reduced form is still too expensive to store in our setting, as its size is exponential in $m$. %Ex-ante probabilities are succinct but do not have sufficient information. 
A key innovation in our relaxation is the introduction of an even more succinct representation -- the \emph{marginal reduced forms} and a \emph{multiplicative approximation} to the polytope of all feasible marginal reduced forms. Although this is a natural concept, to the best of our knowledge, we are the first to introduce and make use of it. 
The marginal reduced form is represented as : $\left\{w_{ij}(t_{ij})\right\}_{i\in[n],j\in[m], t_{ij}\in\cT_{ij}}$, where $w_{ij}(t_{ij})$ is the probability for bidder $i$ to receive item $j$ in $\cM$ and \emph{her value for item $j$ is $t_{ij}$}.\footnote{We refer to $\{w_{ij}(t_{ij})\}_{i\in[n],j\in[m], t_{ij}\in\cT_{ij}}$ as the marginal reduced forms as they are the marginals of the reduced forms multiplied by the probability that $t_{ij}$ is bidder $i$'s value for item $j$, i.e., $\frac{w_{ij}(t_{ij})}{\Pr_{D_{ij}}[t_{ij}]}=\E_{t_{i,-j}\sim \bigtimes_{\ell\neq j}D_{i\ell}}\left[r_{ij}\left(t_{ij},t_{i,-j}\right)\right]$.} Importantly, the size of a marginal reduced form is polynomial in the input size of our problem. As our LP relaxation uses marginal reduced forms as decision variables, it is crucial for us to be able to optimize over the polytope $P$ that contains all \emph{feasible marginal reduced forms}. To the best of our knowledge, $P$ does not have a succinct explicit description or an efficient separation oracle. To overcome the obstacle, we provide \emph{an efficient separation oracle for a different polytope $Q$ that is a multiplicative approximation to $P$, i.e., $c\cdot P\subseteq Q\subseteq P$ for some absolute constant $c\in(0,1)$} (\Cref{thm:multiplicative approx for constraint additive-main body}). Using the separation oracle for $Q$, we can find a $c$-approximation to the optimum of the LP relaxation efficiently. Note that a sampling technique
was developed in~\cite{CaiDW12b} to approximate the polytope of feasible reduced forms. However, their technique only provides an ``additive approximation to the polytope'', which is insufficient for our purpose. Indeed, our multiplicative approximation holds for a wide class of polytopes that frequently appear in Mechanism Design.
%\argyrisnote{Argyris: Removed reference to a theorem in Appendix}
%(\Cref{thm:special case of multiplicative approx}). 
We believe our technique has further applications, for example, to convert the additive FPRAS of Cai-Daskalakis-Weinberg~\cite{CaiDW12a,CaiDW12b,CaiDW13a,CaiDW13b} to a multiplicative FPRAS.
%Removed vspace here\vspace{-.1in}



%Our technique strengthens theirs and obtains a multiplicative approximation to the polytope and might be of independent interest.
%\argyrisnote{Argyris: Maybe we should mention that this work for a class of polytopes (down-monotone polytopes)?}
%\todo[inline]{Mention that to obtain this result, it is important to treat the rare types and frequent types separately, and only use the additive approximation on the frequent types.}

%\vspace{-.1in}
%\paragraph{Generalize\mingfeinote{Generalizing} the Cai-Zhao \core~Analysis} Finally, how do we construct a simple mechanism after solving the LP relaxation? Obviously, the optimum solution of the LP is an upper bound of $\core(M,f(M))$ for any mechanism $M$, but since the optimum solution may correspond to a joint distribution of mechanisms and dual parameters, it is not clear that it can be approximated by a simple mechanism. We prove a generalization of the analysis for the $\core$ by Cai and Zhao~\cite{CaiZ17}, that is, given any feasible solution of the LP, we can construct in polynomial time a TPT whose revenue is at least a constant fraction of the objective value of the feasible solution (\Cref{thm:bounding-lp-simple-mech}). The proof follows a similar strategy as in~\cite{CaiZ17}, but requires several new ideas in a few key steps, for example, when proving the ``shifted \core'' is close to the original \core~(Lemma~\ref{lem:Q and Q-hat}).


%We optimize the mechanism and the dual parameters jointly. In particular, we \emph{concaveify} the objective -- $\core(M,\theta)$ -- by optimizing over joint distributions of mechanisms and dual parameters.
%\paragraph{}We take a different approach. Our first key insight is the following, other than  \textbf{search over the dual parameters rather than the mechanism.} More specifically, for every dual parameter $\theta$%\paragraph{Innovation 1: Search over the Dual Parameters}
%This is indeed the approach taken by Cai and Zhao. However, As the function $\core(M,f(M))$ is highly non-concave in $M$, and the only setting where they manage to find an approxiamtely optimal $\core$ is when the bidders are symmetric.

%can be approximated by a specific TPT that depends on both $M$ and the chosen dual parameters. To facilitate our discussion, we introduce some notation. For any mechanism $M$, there is a set $R(M)$ of dual parameters, such that for any dual parameter $\theta \in R(M)$, the revenue of $M$ is upper bounded by a function $\core(M,\theta)$, which we denote as $\rev(M)\lesssim \core(M,\theta)$.~\footnote{We write $a\lesssim b$ if $a=O(b+\prev)$, where $\prev$ is the highest revenue achievable by any RPP.} Next, they show that for every $\theta\in R(M)$, $\core(M,\theta)\lesssim $, then argue that this upper bound can be approximated by a specific TPT that depends on both $M$ and the chosen dual variables

\subsection{Related Work}\label{sec:related work}
\paragraph{Simple vs. Optimal.} 
We provide an algorithm for the most general setting where an $O(1)$-approximation to the optimal revenue is known using simple mechanisms. It is worth mentioning that a recent result by D\"{u}tting et al.~\cite{DuttingKL20} shows that simple mechanisms can be used to obtain a $O(\log\log m)$-approximation to the optimal revenue even when the bidders have subadditive valuations. We leave it as an interesting open problem to extend our algorithm to bidders with subadditive valuations.

%Removed vspace here\vspace{-.15in}
\paragraph{$(1-\varepsilon)$-Approximation in Item-Independent Settings.} We focus on constant factor approximations for general valuations. For more specialized valuations, e.g., unit-demand/additive, there are several interesting results for finding $(1-\varepsilon)$-approximation to the ``optimal mechanism''. For example, PTASes are known if we restrict our attention to finding the optimal simple mechanism for a single bidder, e.g., item-pricing~\cite{CaiD11b} or partition mechanisms~\cite{rubinstein2016computational}. For multiple bidders, PTASes are known for bidders with additive valuations under extra assumptions on  distributions (such as i.i.d., MHR,\footnote{That is, $f_{ij}(v)/1-F_{ij}(v)$ is monotone non-decreasing (MHR) for each $i,j$, where $f_{ij}$ is the pdf and $F_{ij}$ is the cdf.} etc.)~\cite{DaskalakisW12,CaiH13}.  The only result that does not require simplicity of the mechanism or extra assumptions on the distribution is \cite{kothari2019approximation}, but their algorithm is only a quasi-polynomial time approximation scheme (QPTAS) and computes a $(1-\varepsilon)$-approximation to the optimal revenue for a single unit-demand bidder.
%Removed vspace here\vspace{-.15in}

\paragraph{Structured Distributions beyond Item-Independence.} When the type distributions can be represented as other structured distributions such as Bayesian networks, Markov Random Fields, or Topic Models, recent results show how to utilize the structure to improve the learnability, approximability, and communication complexity of multi-item auctions~\cite{BrustleCD20,CaiO21,cai2021recommender}.  We believe that tools developed in this work would be useful to obtain similar improvement in terms of the computational complexity for computing approximately optimal mechanisms for structured distributions beyond item-independence. 

%Removed vspace here\vspace{-.15in}

%Under item-independence, it is known that finding an exactly optimal mechanism is computationally intractable even for a single bidder with either additive~\cite{DaskalakisDT14} or unit-demand valuation~\cite{chen2015complexity}. \cite{kothari2019approximation} provides a quasi-polynomial time approximation scheme (QPTAS) for computing a $(1-\varepsilon)$-approximation to the optimal revenue for a single unit-demand bidder. PTASes are known if we restrict our attention to finding the optimal simple mechanism, e.g., item-pricing~\cite{CaiD11b} or partition mechanisms~\cite{Rubinstein16}. For multiple bidders, PTASes are known for bidders with additive valuations under extra assumptions on the item distributions (such as i.i.d., MHR,~\footnote{That is, $f_{ij}(v)/(1-F_{ij}(v)$ is monotone non-decreasing (MHR) for each  $i,j$, where $f_{ij}$ is the pdf and $F_{ij}$ is the cdf.} etc.)~\cite{DaskalakisW12,CaiH13}. Assuming only item-independence, constant factor approximations are known for limited cases, either when bidders are symmetric~\cite{ChawlaM16, CaiZ17} or when they have additive or unit-demand valuations~\cite{ChawlaHMS10, Yao15, CaiDW16}. Our result greatly extends the state of the art by showing an efficient algorithm for computing a constant factor approximation for \emph{asymmetric bidders with constrained-additive valuations}.


%For example,~\cite{CaiD11b} develops a PTAS for finding the optimal item-pricing mechanism for a unit-demand buyer over independent MHR items,~\footnote{That is, $f_j(v)/(1-F_j(v)$ is monotone non-decreasing (MHR) for each item $j$, where $f_j$ is the pdf and $F_j$ is the cdf.} and~\cite{Rubinstein16} develops a PTAS for the optimal ``partitioning mechanism'' for an additive buyer over independent items. 

%For the general setting (when items may be correlated), a line of works  ~\cite{AlaeiFHHM12,CaiDW12a,CaiDW12b,CaiDW13a,CaiDW13b,cai2021efficient} develop FPTASes for computing nearly revenue-optimal mechanisms in general settings. These works achieve polynomial dependence in the number of bidders, and the size of each bidder's support (which makes it exponential  in $m$ for independent items). Our result complements these results by showing that the running time can be significantly improved when items are independent.%When items are independent, %These results leave an interesting open problem -- can the dependence on $m$ be improved for more structural distributions? Our result provides an affirmative answer when 
%\paragraph{Learning from Samples?}

==> notes.tex <==
%\argyrisnote{Important Note: I think we should abandon supporting prices for Polytope $W_i$ and use that XOS is the maximum over different additive functions. When we are using the $W_i$ in that way, I think that the supporting prices are in $W_i$.}

%\argyrisnote{Crazy Suggestion: Why don't we write the LP for continuous distributions and argue that when the distribution is discrete, we can do the rebate trick to make it continuous, but we also have access to the separation oracles required to solve the systems? In first sight, it is not obvious why this shouldn't work?}

%\argyrisnote{Question: Do we have something to gain by constructing mechanism that we can calculate entirely offline and does not depend on the order that buyers arrive? For example we do not depend the entry fee on the items that have been sold? Similarly to \cite{ChawlaHMS09}, we could possible call them robust?}


\mingfeinote{

Our selling point:

We are trying to maximize the CORE, which is the truncated welfare.

Insight 1: Having the marginal $w_{ij}(t_{ij})$ instead of the original reduced form.

Insight 2: The ``coupling''

The route to our program:

\begin{enumerate}
\item The original approach: Variables are $w_{ij}(t_{ij})$, the cutoff $\beta$ and $\delta$ depend on w. The ex-ante relaxation: variables are ex-ante probabilities. 

Issue: we can't optimize over the ex-ante prob.

\item Fix any $\beta$ and $\delta$ (dual parameter), maximize the CORE over all $w$ that subject to some constraint between $w$ and $\beta,\delta$. The reason why we need the constraints is that we want the optimum of the LP can be bounded using simple mechanism. %\todo{Write a program for fixed $\beta$ and $\delta$.} 

Observation: 1. We can solve the LP for every fixed $\beta$ and $\delta$; 

2. Lemma 1 implies that the best CORE is no more than the maximum of the LP optimum over all $\beta$ and $\delta$. %\todo{Remove property 4 in Lemma 1.}

Issue: It's too expensive to check all possible $\beta$ and $\delta$.

\item We allow a joint distribution over all possible $\beta$ and $\delta$. It's exponential size. So we can't have a explicit distribution over it. So we put a product measure on it. 
\end{enumerate}

}

\todo{
\vspace{.1in}
For the program:

%1. Make labels for the program. 

2. %A program for constrained-additive, replace $\pi$ by $w$. 
In the XOS proof, point out the place where we use $\pi$, say ``trade $\pi$ as $w$ for c-a''.

%3. Group and reorder the constraints.

%4. Do the discretization of $\delta_{ij}$ (the definition of $\Delta$) before stating the program.

%\vspace{.1in}
%For the proof:

%4. The statement for Theorem 1.

%5. Construction of SPEM: Replace the median by the entry fee of a sampled buyer type.

%\vspace{.1in}
%For the polytope:

%6. Write a general statement for constrained-additive: $Q$ is a mixture of the set of polytopes $Q_t$. $Q$ is downward-closed. If $Q$ contains a $L_{\infty}$-box, and we can optimize over $Q_t$ for any $t$, then there exists a polytope $Q'$ that satisfies $a\cdot Q\subseteq Q'\subseteq b\cdot Q$, and there exists an efficient separation oracle for $Q'$. 
}


%\argyrisnote{General suggestion: Maybe we shouldn't consider a continuous distribution, but a tailor-made "slighly" modified discrete distribution. It is weird to talk about continious distribution and use sum over types}

==> polytope_sampling.tex <==
\section{Sampling from Polytope}
\notshow{
\vspace{.5in}
\mingfeinote{The original multiplicative approximation. Don't look at it.}


First we are going to show how we can have access to a multiplicative approximation of the polytope $W_i$,
when the buyer's valuation is additive under downward-closed set of feasibility constraints $\mathcal{F}$, for several interesting classes of $\mathcal{F}$. %We require the following definitions.

We first introduce the concept on downward-closed constraints called $(b,c)$-balance, which is proposed by Chekuri et al.~\cite{ChekuriVZ14}.  

\begin{definition}[Definition~1.2   \cite{ChekuriVZ14}]\label{def:crs}
Let $\cF \subseteq 2^{I}$ be a downward-closed feasibility constraint over ground set $I$ and $P_{\cF}$ be the convex hull of characteristic vectors in $\cF$: $P_{\cF}=conv(\ind_S\mid S\in \cF)$. For every $q=(q_j)_{j\in I} \in P_{\cF}$, we denote by $A(q)$ the random set obtained by including each element $j\in I$ independently with probability $q_j$. We say an element $j\in I$ is active if $j\in A(q)$.
%the distribution over active sets induced by the vector of activation probabilities $q$.
%Each item $j\in[m]$ can be active or inactive independent of each other,
%where the $j$-th item is activated with probability $q_j$.
Our goal is to collect a subset of active elements that is feasible w.r.t. $\mathcal{F}$. 

%We assume that the buyer's valuation is additive over $m$ heterogeneous items with feasibility constraints.
A Contention Resolution Scheme (CRS) $\pi$,
takes as input the vector of activation probabilities $q \in P_{\cF}$ and a subset of items $A \subseteq 2^{[m]}$, and outputs a random set $\pi_q(A)\subseteq A$ such that for each $O \in \supp(\pi_q(A))$ we have $O\in \cF$.
%\begin{enumerate}
%    \item $O \subseteq A$
%    \item $O \in \mathcal{F}$
%\end{enumerate}%$\pi_q(A) \in  2^A \cap\mathcal{F}$.
%a subset of active items such that the outputted set of active items are in $\mathcal{F}$.

Let $b,c\in [0,1]$. A CRS $\pi$ is called $(b,c)$-balanced,
if for every $q \in b \cdot P_{\cF}$\footnote{For every $a\in \mathbb{R}_+$ and set $S\subseteq \mathbb{R}^n$, $a\cdot S=\{a\cdot x\mid x\in S\}$. } and for all $j\in[m]$ such that $q_j >0$:
$$
\Pr_{\substack{A \sim A(q)\\O \sim \pi_q(A)}}\left[j \in O \mid j \in A \right] \geq c
$$

%If $\pi$ is CRS for $\mathcal{F}$,
%then for any $q\in P$, $A \subseteq 2^{[m]}$, $O \in \supp(\pi_q(A))$ then $O \in \mathcal{F}$.

{The constraint $\cF$ is called $(b,c)$-balanced if there exists a CRS $\pi$ (not necessarily efficient) for $\cF$ that is $(b,c)$-balanced.}
\end{definition}



%For this section, we only require the existence of a CRS that is $(b,c)$-balanced and we do not care if it is efficiently implementable.


Now for every $i\in [n]$, we will construct another convex set $\widehat{W}_i$ that approximates $W_i$. Formally, $c\cdot \widehat{W}_i\subseteq W_i\subseteq \widehat{W}_i$ for some $c<1$. Moreover, we can construct a separation oracle for $\widehat{W}_i$ efficiently, with access to the demand oracle. 


\begin{lemma}
%Let $v(\cdot, \cdot):T\times2^{[m]}\rightarrow \mathbb{R}_+$ be an additive valuation of a buyer under downward-closed feasibility constraints $\mathcal{F}$.
Fixed any buyer $i$. Let $b,c\in [0,1]$. Suppose her valuation $v_i(\cdot,\cdot)$ is constrained-additive and the feasibility constraint $\cF_i$ is $(b,c)$-balanced. Let $\cP$ be the convex hull of characteristic vectors of $\cF_i$. 
Let $W_i$ be the polytope defined in \mingfeinote{Add reference}. Consider the convex set $\widehat{W}_i$,
where an element $(\pi_i=(\pi_{ij}(t_{ij}))_{j,t_{ij}},w_i=(w_{ij}(t_{ij}))_{j,t_{ij}}) \in \widehat{W}_i$ if and only if all of the following conditions are satisfied: 

\begin{enumerate}
    \item $w_{ij}(t_{ij})\leq c\cdot f_{ij}(t_{ij}),\forall j\in [m],t_{ij}\in \cT_{ij}$.
    \item $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})\leq f_{ij}(t_{ij}),\forall j\in [m],t_{ij}\in \cT_{ij}$.
    \item $q\in b\cdot \cP$, where $q=(q_j)_{j\in [m]}$ satisfies that $q_j=\frac{1}{c}\cdot \sum_{t_{ij}\in \cT_{ij}}w_{ij}(t_{ij})$.
\end{enumerate}

%\begin{align*}
% q &\in  b \cdot\cP \\
% c\cdot q_j &=  \sum_{t_{ij} \in \cT_{ij}} w_i(t_{ij})  \quad  &\forall j \in[m] \\
% w(t_j) &\leq  c\cdot f(t_j) & \forall j\in[m], t_j \in T_j\\
% w(t_j) &\leq  \pi(t_j) \leq f(t_j) &\forall j\in[m], t_j \in T_j\\
%\end{align*}
%If there exists a $(b,c)$-balanced CRS $\pi$ for $\mathcal{F}$,
Then we have $b c \cdot W_i \subseteq \widehat{W}_i \subseteq W_i$.
Moreover, there exists a separation oracle for $\widehat{W}_i$ such that for every input, it runs in time $poly(n,m,\sum_{i,j}|\cT_{ij}|)$ and requires $O(1)$ queries from the demand oracle for $v_i(\cdot, \cdot)$.
\end{lemma}

\mingfeinote{Change the proof based on the statement above. I think it's better to keep the subscript $i$. }

\begin{proof}
First, one can easily verify that $\widehat{W}_i$ is indeed a convex set, since $\cP$ is convex. Now we are going to prove that $b c \cdot W_i \subseteq \widehat{W}_i$.

Remember that when the valuation $v(\cdot,\cdot)$ is constraint additive,
then $(\pi,w) \in W$ if
for each type $t \in T$,
there exists a joint distribution over allocation rules and activated additive function
%$\sigma_t(\cdot, \cdot):  2^{[m]} \times \mathcal{F} \rightarrow \Delta^{}$ \todo{need to make it more formal} such that:
$\sigma_t \in \Delta^{2^{m}\cdot |\mathcal{F}|}$ such that: \todo{maybe we should add to notation how we index vectors.}
\begin{align*}
\pi(t_j) =& \sum_{\substack{t' \in T:\\t_j'=t_j}} \sum_{[j] \subseteq S} f(t')\sigma_{t'}(S)\\
w(t_j) =& \sum_{\substack{t' \in T:\\t_j'=t_j}} \sum_{[j] \subseteq S} f(t')\sum_{F \in \mathcal{F}}
\sigma_{t'}(S, F) \frac{V(t_j)\mathds{1}[j \in F]}{V(t_j)}
\end{align*}
Note that because $v$ is additive over constraints $\mathcal{F}$,
for each type $t \in T$
we can restrict  our attention to joint distribution over sets in $\mathcal{F}$ only,
$\sigma'_t\in \Delta^{ |\mathcal{F}|}$.
%$\sigma'(\cdot,\cdot):T \times \mathcal{F}\rightarrow [0,1]$ in $\mathcal{F}$.
%Let $\Sigma'$ be the the set of all jointallocation described above.
We relax the allocation constraint and we introduce additional variable $\{q_j\}_{j\in[m]}$ to:
\begin{align*}
w(t_j) =& \sum_{\substack{t' \in T:\\t_j'=t_j}}  f(t')\sum_{\substack{[j] \subseteq S \\S \in \mathcal{F}}} \sigma'_{t'}( S)\\
\sigma'_{t'} \in& \Delta^{|\mathcal{F}|} &\forall t' \in T \\ 
q_j = &\sum_{t_j \in T_j} w(t_j)  \quad & \forall j \in [m]\\
 w(t_j) \leq & \pi(t_j) \leq f(t_j) \\
\end{align*}


Note that $q_j$ is just the probability that we award item $j$ and $j$ is included in the activated additive function,
when using joint distribution $\sigma'$ \todo{need to make it a bit more formal}.
Since for each $t\in T$, $\sigma'_t$ only allocates items that are in $\mathcal{F}$, then $q \in \mathcal{P}$.
Note that always $w(t_j) \leq f(t_j)$.
Thus a relaxation of $W$ is the convex set $\widetilde{W} \supseteq W$,
such that $(\pi,w) \in \widetilde{W}$ if:
\begin{align*}
 q \in & \mathcal{P} \\
  q_j = & \sum_{t_j \in T_j} w(t_j)  \quad  &\forall j \in[m] \\
  w(t_j) \leq & \pi(t_j) \leq f(t_j) &\forall j\in[m], t_j \in T_j\\
\end{align*}

%Since $\sum_{t_j \in T_j} w(t_j) \leq \sum_{t_j \in T_j} f(t_j) = 1$, 
%We remind that an element $w \in W$ with additional auxiliary variables $q=\{q_j\}_{j\in[m]}$ if there exists $\pi' \in \Pi'$ such that
%\begin{align*}
%w_j(t_j) = \sum_{\substack{t' \in T:\\t_j'=t_j}} \sum_{[j] \subseteq S} \pi'(t',S) \\
%q_j = \sum_{t_h\in T_j} w(t_j) \quad \forall j \in[m]
%\end{align*}
%That is, $q_j$ is the probability that we allocate item $j$ according to allocation rule $\pi' \in \Pi'$.
%Since allocation rule always allocate bundles that are in $\mathcal{F}$,
%$q \in \mathcal{P}$.

%One way to interpret convex set $\widetilde{W}$,
%is that 
%is that $q_j$ is the probability that we allocate item $j$ to the agent regardless if we only allocate items that are within constraints $\mathcal{F}$,
%and we only care about satisfying feasibility %constraints $\mathcal{F}$ in expectation.
%Observe that $W \subseteq \widetilde{W}$.
Combining the fact that $W\subseteq \widetilde{W}$ and that $bq \cdot \widetilde{W} \subseteq \widehat{W}$,
implies the first part of the proof.



Now we are going to show how to use the definition of $(b,c)$-balanced CRS to prove that $\widehat{W} \subseteq W$.
More specifically we are going to show how to get a joint distribution over allocation $\sigma'\in \Sigma'$ for any $w \in \widehat{W}$.


Let $(\pi,w)\in \widehat{W}$.
We describe now when we choose to activate an item $j$.
First we sample the type $t_j \sim D_j$, and we activate item $j$ with probability $\frac{w(t_j)}{cf(t_j)} \leq 1$.
Note that the activation probability of item $j$ is:
$$
\sum_{t_j\in T_j} f(t_j)\frac{w(t_j)}{cf(t_j)} \leq q_j
$$
Let $\pi_q(A)$ be the distribution over items of the CRS on vector of activation probabilities $q$ when set $A$ is active.
Because CRS $\pi$ is $(b,c)$-balanced,
we can include item $j$ when it is activate with probability at least $c$ and the set of outputted items are a subset of the active items and are in $\mathcal{F}$.
Thus there exists an allocation $\sigma' \in \Sigma'$ such that for all $j\in[m]$ it allocates item $j$ when agent has type $t_j \in T_j$ such that:
%the probability that the agent has type for the $j$-th item equal to $t_j$
%, conditioned on that it is activated with probability $\frac{w(t_j)}{cf(t_j)}$ and conditioned on the two previous scenarios it is included in the final set of outputted items with probability $c$:
$$
\sum_{\substack{t' \in T:\\t_j'=t_j}} \sum_{[j] \subseteq S}f(t') \sigma'(t',S) \geq  f(t_j) \cdot \frac{w(t_j) }{c f(t_j)} \cdot c = w(t_j)
$$
where $f(t_j)\cdot \frac{w(t_j)}{cf(t_j)}$ is just that the agent has type $t_j$ for the item and the item is activated, and the factor $c$ is the probability that the item $j$ is included in the final allocation.
Notice that constraints on $\pi$ relative to $w$ on polytopes $W$ and $\widehat{W}$ are the same.
Thus $\sigma'$ implies that $w\in W$,
which proves that $\widehat{W} \subseteq W$.


Now we show how to construct a separation oracle for $\widehat{W}$,
given access to a demand oracle for $v(\cdot,\cdot)$.
Note that we can rewrite $\widehat{W}$ in the following way:
\begin{align*}
    & \left\{\sum_{t_j \in T_j}w(t_j) \right\}_{j\in[m]} \in bc\cdot P \\
    & w(t_j) \leq c f(t_j) & \forall j\in[m], t_j \in T_j\\
    & w(t_j) \leq \pi(t_j) \leq  f(t_j) & \forall j\in[m], t_j \in T_j\\
\end{align*}

Suppose we are given a vector $w$ and we want to see if $w \in \widehat{W}$.
If $w \notin \widehat{W}$,
we want to output a separating hyperplane.
Given $w$ as input,
it is easy to check if $w(t_j) \leq c\cdot f(t_j)$ and if $w(t_j) \leq \pi(t_j) \leq f(t_j)$. Moreover, if the constraints are not satisfied, it directly gives us a separating hyperplane between $(\pi_i,w_i)$ and $\widehat{W}_i$. Thus by replacing $bc \cdot \hat{q}_j = \sum_{t_j\in T_j}w(t_j)$, it is enough to design a separating oracle for the convex set $\cP$. 

Since $P$ is the convex hull of the characteristic vectors in $\mathcal{F}$,
each vertex of $P$ is a characteristic vector of $\mathcal{F}$.
By equivalence of separation and optimization, it is enough to design a optimization algorithm for convex set $P$,
or equivalently for any vector $\hat{q}$,
we want to find $\max_{S \in \mathcal{F}} \sum_{j\in S}\hat{q}_j$.
Consider an arbitrary $t\in T$, such that $V_j(t) >0$ and w.l.o.g. we can assume that $\hat{q}\geq 0$ (since we can just replace negative entries of $\hat{q}$ with $0$, since constrains in $\mathcal{F}$ are downward closed)
and that $\hat{q} \leq \min_{j\in[m]}V_j(t_j)$.
Note that the optimization problem above,
is equivalent to querying the demand oracle on type $t$ with price for the $j$-th item equal to $V_j(t) - \hat{q}_j$.
\end{proof}

}

\notshow{
\subsection{Sampling $W$}
In this section,
we are going to show how to use ideas from \cite{CaiDW12} \todo{Should I cite the unpublished manuscript?}.

\begin{definition}
For two sets $A,B \subseteq \mathbb{R}^d$,
we denote by $A+B$ the Minkowski addition of set $A$ and set $B$ where:
$$A+B = \{a + b : a \in A\land b \in B\}
$$

Note that if both $A$ and $B$ are convex, then $A+B$ is also convex.
\end{definition}


\begin{definition}[\todo{Should I cite the manuscript?}]
Consider a set of $N$ (where $N$ is a finite number) convex sets $\mathcal{P}_N=\{P_i\}_{i\in [N]}$ and a distribution $\mathcal{D}_N=\{p_i\}_{i\in[N]}$ over the elements in $[N]$.
The polytope $\mathcal{P}$ defined as:
$$
\mathcal{P} = \sum_{i\in[N]}p_i P_i
$$
is called the mixture of $\mathcal{P}_N$ over distribution $\mathcal{D}_N$.
\end{definition}


\begin{theorem}[\todo{What should I cite?}]\label{thm:approx mixture}
Let $\mathcal{P}$ be a mixture of $\mathcal{P}_N=\{P_i\}_{i\in[N]}$ over distribution $\mathcal{D}_N$,
where $P_i\subseteq \mathbb{R}^d$ and $P_i$ is a closed convex polytope for $i\in[N]$.
We further assume that for all $i\in[N]$,
the bit complexity of each corner of $P_i$ is at most $b$.
For $\epsilon > 0$ and $\mathbb{N} \ni k \geq \max\left(\log\left( \frac{1}{\epsilon} \right), \Omega(d^4(b + \log\left( \frac{1}{\epsilon}\right))\right)$,
let $\mathcal{D}'_N$ be the empirical distribution induced by $\frac{8kd}{\epsilon^2}$ samples from $\mathcal{D}_N$.
Let $\mathcal{P}'$ be the mixture of of $\mathcal{P}_N=\{P_i\}_{i\in[N]}$ over distribution $\mathcal{D}'_N$.
With probability at least $1-2de^{-2dk}$ we have that
\begin{enumerate}
    \item For all $q\in \mathcal{P}$,
    there exists a $q'\in \mathcal{P}'$ such that $||q-q'||_\infty \leq \epsilon$
    \item For all $q'\in \mathcal{P}'$,
    there exists a $q\in \mathcal{P}$ such that $||q-q'||_\infty \leq \epsilon$
\end{enumerate}
\end{theorem}


Given the framework from \todo{what should I cite?},
we are going to show how to optimize over an approximation of polytope $W \in [0,1]^{2\sum_{j\in[m]}|T_j|}$.
For a vector $x \in [0,1]^{\sum_{j\in[m]}|T_j|}$,
we index $x$ in the following way.
For each $j\in[m]$ and $t_j \in T_j$,
we use $x_{t_j}$ to denote an element of $x$.


For any $t \in T$,we are going to define a polytope $W_t \in [0,1]^{2\sum_{j\in[m]}|T_j|}$.
An element $w\in W_t$ if there exists a joint distribution over bundles and selected additive function $\sigma \in  \Delta^{2^m\cdot K}$ such that %\argyrisnote{and a function $k(\cdot,\cdot): T \times 2^{[m]} \rightarrow [K]$} such that:
%$$
%w_{t'_j}=
%\begin{cases}
%\sum_{S:j\in S} \pi_S\frac{\gamma_j^S(t)}{V_j(t_j)}, \quad&\text{if $t'_j=t_j$}\\
%0,& \text{o.w} 
%\end{cases}
%$$
\begin{align*}
\pi(t'_j)=&
\begin{cases}
\sum_{[j]\subseteq S} \sigma(S), \quad&\text{if $t'_j=t_j$}\\
0,& \text{o.w} 
\end{cases}\\
w(t'_j)=&
\begin{cases}
\sum_{[j]\subseteq S}\sum_{k\in[K]} \sigma(S,k)\frac{\alpha_j^k(t_j)}{V_j(t_j)}, \quad&\text{if $t'_j=t_j$}\\
0,& \text{o.w} 
\end{cases}
\end{align*}

%where we denote by $\pi_S$ the probability that we award exactly bundle $S$ to the agent.
Note that $W$ is the convex hull finite many deterministic allocation rules and deterministic choice of the activated additive function.
Thus $W$ is a convex polytope.
%\todo{We have to argue that when the function is XOS we really have polytopes? I think it is enough to note that this is true, since we have finite many types and finite many possible allocations.}
\todo{Is it ok to argue that if each $\alpha_j^k(t)$ has bit complexity $b$, then there cannot be infinity many additive functions in the XOS definition in the range $[0,H]$?}

\begin{observation}\label{obs:mix}
Polytope $W$ is mixture of $\{W_t\}_{t\in T}$ over distribution $\{f(t)\}_{t \in T}$
\end{observation}

Thus a collarly of Theorem~\ref{thm:approx mixture} is that with enough samples we can find a polytope approximately close to $W$ \todo{we have to make assumption about the bit complexity of the additive functions within XOS I think?}.
For now on,
we are only going to focus on polytope $\mathcal{P}'_k$ which is a mixture of $\{W_t\}_{t\in T}$ over the empirical distribution $\mathcal{D}'$ induced by $k$ samples from $\mathcal{D}$.
An important question now is how can we get a separation oracle for $\mathcal{P}'_k$.
}

\notshow{
\begin{lemma}\label{lem:separate}
Given access to a adjustable utility oracle for the agent,
we can get a separating oracle for $\mathcal{P}'_k$. \todo{How we should name this adjusted weight value oracle?}
\end{lemma}


\begin{proof}
By equivalence of separation and optimization,
it is enough to design an optimization algorithm over linear objectives for polytope $\mathcal{P}'_k$.
Since $\mathcal{P}'_k$ is the Minkowski addition of at most $k$ polytopes in $\{W_t\}_{t\in T}$,
it is enough to design an optimization algorithm for linear objectives for each polytope $W_t$, where $t \in T$.
Consider we want to maximize the objective:
\begin{align*}
    \max c_\pi^T\pi + c_w^T w \\
    s.t.: (\pi,w) \in W_t
\end{align*}
Note that this is equivalent to the following program:
\begin{align*}
    \max &\sum_{j\in[m]} \sum_{[j] \subseteq S} \left(c_{w}(t_j)\cdot \sum_{k\in[K]}\sigma(S,k)\frac{\alpha_j^k(t_j)}{V_j(t_j)} + c_\pi(t_j) \sigma(S) \right)\\
    s.t.:& \sigma \in \Delta^{2^{[m]}}
\end{align*}
Observe that the vertices of the feasibility constraints are the characteristic vectors of $2^{2Km}$.
Thus the problem is equivalent to:
\begin{align*}
    \max_{\substack{S \subseteq 2^{[m]}\\ S' \subseteq 2^[m]: S' \cap S = \emptyset\\k \in [K]}} \sum_{j\in S}
    \left( \frac{c_w(t_j)}{V_j(t_j)}\alpha_j^k(t) + c_\pi(t_j)\right)  + \sum_{j\in S'} c_\pi(t_j)  
\end{align*}
W.l.o.g. we can assume that for each additive function that the buyer has, we also have another additive function where we can replace any subset of coefficients with $0$.
Thus the program above can be decomposed to:
\begin{align*}
    \max_{S \subseteq 2^{[m]}}\left(\sum_{\substack{j\in S\\c_w(t_j)>0 }}
    \left( \frac{c_w(t_j)}{V_j(t_j)}\alpha_j^k(t) + c_\pi(t_j)\mathds{1}[c_\pi(t_j) < 0]\right)\right)
    +
    \sum_{\substack{j\in[m]\\c_\pi(t_j) \geq 0}} c_\pi(t_j)
\end{align*}

%Notice that if for some $j\in[m]$,
%$c_w(t_j)<0$ and $c_\pi(t_j)>0$,
%then we can give the item to the buyer and assign them a value $0$ for it.
%If for some $j\in[m]$,
%$c_w(t_j)<0$ and $c_\pi(t_j)<0$,
%then we do not give them the item.
%If $c_w(t_j)>0$ and $c_\pi(t_j)>0$,
%we definitely give the item to the buyer and we only care about optimizing the term that to $c_w(t_j)$.



\todo{we need to make it more formal}.
Observe that we can optimize the objective above with a utility?? oracle by properly adjusting the weight for the value that each agent has for the $j$-th item by $\frac{c_w(t_j)}{V_j(t_j)}$ and setting price for the $j$-th item equal to $c\pi(t_j)\mathds{1}[c\pi(t_j) < 0]$.
\end{proof}
}

\begin{lemma}\label{lem:optimize}
For any $t_i\in \cT_i$,
given access to a adjustable utility oracle $\dem(t_i,\cdot)$ for the agent,
we can optimize over $W_t$. \todo{How we should name this adjusted weight value oracle?}
\end{lemma}

\begin{proof}
By equivalence of separation and optimization,
it is enough to design an optimization algorithm over linear objectives for polytope $\mathcal{P}'_k$.
Since $\mathcal{P}'_k$ is the Minkowski addition of at most $k$ polytopes in $\{W_t\}_{t\in T}$,
it is enough to design an optimization algorithm for linear objectives for each polytope $W_t$, where $t \in T$.
Consider we want to maximize the objective:
\begin{align*}
    \max c_\pi^T\pi + c_w^T w \\
    s.t.: (\pi,w) \in W_t
\end{align*}
Note that this is equivalent to the following program:
\begin{align*}
    \max &\sum_{j\in[m]} \sum_{[j] \subseteq S} \left(c_{w}(t_j)\cdot \sum_{k\in[K]}\sigma(S,k)\frac{\alpha_j^k(t_j)}{V_j(t_j)} + c_\pi(t_j) \sigma(S) \right)\\
    s.t.:& \sigma \in \Delta^{2^{[m]}}
\end{align*}
Observe that the vertices of the feasibility constraints are the characteristic vectors of $2^{2Km}$.
Thus the problem is equivalent to:
\begin{align*}
    \max_{\substack{S \subseteq 2^{[m]}\\ S' \subseteq 2^[m]: S' \cap S = \emptyset\\k \in [K]}} \sum_{j\in S}
    \left( \frac{c_w(t_j)}{V_j(t_j)}\alpha_j^k(t) + c_\pi(t_j)\right)  + \sum_{j\in S'} c_\pi(t_j)  
\end{align*}
W.l.o.g. we can assume that for each additive function that the buyer has, we also have another additive function where we can replace any subset of coefficients with $0$.
Thus the program above can be decomposed to:
\begin{align*}
    \max_{S \subseteq 2^{[m]}}\left(\sum_{\substack{j\in S\\c_w(t_j)>0 }}
    \left( \frac{c_w(t_j)}{V_j(t_j)}\alpha_j^k(t) + c_\pi(t_j)\mathds{1}[c_\pi(t_j) < 0]\right)\right)
    +
    \sum_{\substack{j\in[m]\\c_\pi(t_j) \geq 0}} c_\pi(t_j)
\end{align*}

%Notice that if for some $j\in[m]$,
%$c_w(t_j)<0$ and $c_\pi(t_j)>0$,
%then we can give the item to the buyer and assign them a value $0$ for it.
%If for some $j\in[m]$,
%$c_w(t_j)<0$ and $c_\pi(t_j)<0$,
%then we do not give them the item.
%If $c_w(t_j)>0$ and $c_\pi(t_j)>0$,
%we definitely give the item to the buyer and we only care about optimizing the term that to $c_w(t_j)$.



\todo{we need to make it more formal}.
Observe that we can optimize the objective above with a utility?? oracle by properly adjusting the weight for the value that each agent has for the $j$-th item by $\frac{c_w(t_j)}{V_j(t_j)}$ and setting price for the $j$-th item equal to $c\pi(t_j)\mathds{1}[c\pi(t_j) < 0]$.
\end{proof}

\notshow{
We conclude with the main theorem of this section.
\begin{theorem}
Let $k=\max\left(\log\left( \frac{1}{\epsilon} \right), \Omega(d^4(b + \log\left( \frac{1}{\epsilon}\right))\right)$ and $W_k$ be a mixture of $\{W_t\}_{t\in T}$ over the empirical distribution $\mathcal{D}_k$ induced by $k$ samples from $\mathcal{D}$.
Consider the polytope $\widehat{W}= W_k - \epsilon$
% such that $(\widehat{\pi},\widehat{w})\in \widehat{W}$ if there exists a $(\pi_k,w_k)\in W_k$ such that for all $j\in[m]$ and $t_j \in T_j$:
Then for each $(\widehat{\pi},\widehat{w}) \in \widehat{W}$,
there exists a $(\pi,w) \in W$ such that for all $j\in[m]$ and $t_j \in T_j$:
\begin{align*}
\widehat{\pi}(t_j) \leq& \pi_k(t_j) \\
\widehat{w}(t_j) \leq& w_k(t_j)
\end{align*}

and for each $(\widehat{\pi},\widehat{w}) \in \widehat{W}$,
there exists a $(\pi,w) \in W$ such that for all $j\in[m]$ and $t_j \in T_j$:
\begin{align*}
\pi_k(t_j)-2\epsilon \leq &\widehat{\pi}(t_j)  \\
w_k(t_j)-2\epsilon\leq &\widehat{w}(t_j)
\end{align*}

Moreover given access to \todo{adjustable demand oracle},
we can get a separation oracle for $\widehat{W}$ in a efficient manner.
\end{theorem}

\begin{proof}
The first part of the proof follows by combination of Theorem~\ref{thm:approx mixture} and Observation~\ref{obs:mix}.

Notice that in order to get a separation oracle for $\widehat{W}$,
it is enough to get a separation oracle for $W_k$.
The rest of the proof follows by Lemma~\ref{lem:separate}. 
\end{proof}
}

\subsection{Accessing Marginal Reduced Form Polytope for XOS Valuation}


\mingfeinote{Formal Definiton of the polytope $W_i$. Move it before stating the LP.

Mingfei: We need a name for the polytope.

}

\begin{definition}\label{def:W_i}
For every $i\in [n]$, the polytope $W_i\subseteq [0,1]^{2\cdot \sum_j|\cT_{ij}|}$ is defined as follows. Let $\pi_i=(\pi_{ij}(t_{ij}))_{j,t_{ij}\in \cT_{ij}}$ and $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}\in \cT_{ij}}$. Then $(\pi_i,w_i)\in W_i$ if and only if there exist a number $\sigma_S^{(k)}(t_i)\in [0,1]$ for every $t_i\in \cT_i, S\subseteq [m],k\in [K]$, such that
\begin{enumerate}
    \item $\sum_{S,k}\sigma_S^{(k)}(t_i)\leq 1$, $\forall t_i\in \cT_i$.
    \item $f_{ij}(t_{ij})\geq\pi_{ij}(t_{ij})\geq f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})$, for all $i,j,t_{ij}\in \cT_{ij}$.
    \item $w_{ij}(t_{ij})\leq f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}$, for all $i,j,t_{ij}\in \cT_{ij}$.
\end{enumerate}
\yangnote{Yang: why are the $\pi$'s and $w$'s define using inequalities?}
\end{definition}

\argyrisnote{Argyris: Hide the following proposition?}
\begin{proposition}[Polytope $W_i$ for constrained-additive valuation]\label{def:W_i-constrained-add}
For every $i\in [n]$, suppose $v_i(\cdot,\cdot)$ is constrained-additive with feasibility constraint $\cF$. Then $(\pi_i,w_i)\in W_i$ if and only if there exist a number $\sigma_S^{(k)}(t_i)\in [0,1]$ for every $t_i\in \cT_i, S\subseteq [m], k\in [K]$ such that
\begin{enumerate}
    \item $\sum_{S\in \cF,k}\sigma_S^{(k)}(t_i)\leq 1$, $\forall t_i\in \cT_i$.
    \item $f_{ij}(t_{ij})\geq\pi_{ij}(t_{ij})\geq f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})$, for all $i,j,t_{ij}\in \cT_{ij}$.
    \item $w_{ij}(t_{ij})\leq f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S\in \cF:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\cdot \ind[S\in \cF]$, for all $i,j,t_{ij}\in \cT_{ij}$.
\end{enumerate}
\yangnote{Yang:why is this is a proposition? What are we proving here? Also, why do we have $\sigma^{(k)}$ for constrained additive?}
\end{proposition}

\vspace{.3in}

Let $T=\sum_{i,j}|\cT_{ij}|$. We consider the following two polytopes $W_{i,\eps}^f$ and $W_{i, \eps}^r$.

\begin{definition}\label{def:welfare frequent}
For every $i\in [n]$, we consider the polytope $W_{i,\eps}^f$ with parameter $\eps>0$. $(\pi_i^f,w_i^f)\in W_{i,\eps}^f$,
if there exists a $(\pi_i,w_i)\in W_i$ such that:
\begin{align*}
    w^f_{ij}(t_{ij}) =
\begin{cases}
w_{ij}(t_{ij}), \quad & \text{ if $f_{ij}(t_{ij}) \geq \eps$}\\
0 & \text{ o.w.}
\end{cases}\\
\pi^f_{ij}(t_{ij}) =
\begin{cases}
\pi_{ij}(t_{ij}), \quad & \text{ if $f_{ij}(t_{ij}) \geq \eps$}\\
0 & \text{ o.w.}
\end{cases}
\end{align*}

\notshow{
Note that $W_{i,\eps}\subseteq W_i$ and if $(\pi_i^f,w_i^f)\in W_{i,\eps}^f$,
then for any $(\pi_i',w_i')$ such that
\begin{align*}
    &0 \leq w'_{ij}(t_{ij}) \leq w^f_{ij}(t_{ij}) \land f_i(t_{ij}) \geq \pi'_{ij}(t_{ij}) \geq \pi^f_{ij}(t_{ij}) \\
    \lor \quad & w'_{ij}(t_{ij}) = \pi'_{ij}(t_{ij}) = 0
\end{align*}

then $(\pi'_i, w'_i) \in W_{i,\eps}^f$.
}
\end{definition}


%We also consider the following polytope:
\begin{definition}\label{def:welfare rare}
Let $T_i = \sum_{j\in[m]}|\cT_{ij}|$. \mingfeinote{Replace it by $T = \sum_{i,j}|\cT_{ij}|$.}
We consider the polytope $W_{i,\eps}^r$ with parameter $\eps < \nicefrac{1}{T}$, \yangnote{What is $T$? Do you mean $T_i$?}such that $(\pi_i^r,w_i^r)\in W_{i,\eps}^r$ if and only if for every $t_{ij}$ it holds that
\begin{align*}
    0 \leq w_{ij}^r(t_{ij}) \leq \pi_{ij}^r(t_{ij}) \leq \left(1-\eps \cdot T \right)\cdot\min(\eps,f_{ij}(t_{ij}))
\end{align*}
\end{definition}

Clearly the first polytope $W_{i,\eps}^f\subseteq W_i$. We prove in the following lemma that the second polytope $W_{i,\eps}^r \subseteq W_i, \forall \eps<\nicefrac{1}{T}$. 

\begin{lemma}\label{lem:welfare rare}
$W_{i,\eps}^r \subseteq W_i$, for all $\eps < \nicefrac{1}{T}$.
\end{lemma}
\begin{proof}

For any $(\pi_i,w_i)\in W_{i,\eps}^r$, we will prove that $(\pi_i'=\pi_i,w_i'=\pi_i)\in W_i$. Then $(\pi_i,w_i)\in W_i$ since $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})$ for any $j,t_{ij}$.

To prove $(\pi_i',w_i')\in W_i$, we consider the following set of numbers $\{\sigma_{S}^{(k)}(t_i)\}_{t_i,S,k}$ (see \Cref{def:W_i}): For each $j\in [m], t_{ij}\in \cT_{ij}$, let $c_j(t_{ij})=\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right)$; let 
$$p_j(t_{ij})=\frac{\pi_{ij}(t_{ij})}{f_{ij}(t_{ij})\cdot \sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))}$$ 


For every $t_i$, define
\begin{align*}
\sigma_{S}^{(k)}(t_i)=
\begin{cases}
p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'})), &\text{if } S=\{j\}\wedge k=\argmax_{k'}\alpha_{ij}^{(k')}(t_{ij})\\
0, &\text{o.w.}
\end{cases}
\end{align*}

For every $j$, let $C_j(t_{ij})$ be the independent Bernoulli random variable that activates with probability $c_j(t_{ij})$. Then for every $j$, 
$$
\Pr_{C_j(t_{ij}), t_{ij}\sim D_{ij}}\left[C_j(t_{ij})=1\right] \leq \sum_{t_{ij}\in \cT_{ij}} f_{ij}(t_{ij})\cdot\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right) \leq \eps \cdot |\cT_{ij}|
$$
By union bound,
$$\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))=\Pr[C_{j'}(t_{ij'})=0,\forall j'\not=j]\geq 1-\sum_j\Pr[C_j(t_{ij})=1]\geq 1-\eps\cdot T$$

Now we will prove that $(\pi_i',w_i')\in W_i$ by verifying all three inequalities in \Cref{def:W_i}. For the first inequality, since $(\pi_i,w_i)\in W_{i,\eps}^r$, $0 \leq w_{ij}(t_{ij}) \leq \pi_{ij}(t_{ij}) \leq \left(1-\eps \cdot T \right)\cdot f_{ij}(t_{ij})\cdot c_j(t_{ij})$. Thus $p_j(t_{ij})\leq 1$ for every $j,t_{ij}$. We have that $\sum_{S,k}\sigma_S^{(k)}(t_i)=\sum_jp_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))\leq \sum_j c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))$. We notice that $\sum_j c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))$ is exactly the probability of there exists a unique $C_j(t_{ij})=1$. Thus $\sum_{S,k}\sigma_S^{(k)}(t_i)\leq 1$.

The second inequality: 
\begin{align*}
&f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\\
=&f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))=\pi_{ij}(t_{ij})
\end{align*}

The third inequality:
\begin{align*}
&f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_S^{(k)}(t_{ij},t_{i,-j})\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}\\
=&f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot p_j(t_{ij})\cdot c_j(t_{ij})\cdot \prod_{j'\not=j}(1-c_{j'}(t_{ij'}))\cdot \frac{\max_k\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}=\pi_{ij}(t_{ij})=w_{ij}'(t_{ij})
\end{align*}

By \Cref{def:W_i}, $(\pi_i',w_i')\in W_i$. Thus $(\pi_i,w_i)\in W_i$. We finish our proof.

\notshow{
The old proof:

We consider the following allocation rule $\sigma_{S}^k(t_i)$ parametrised by variables $\{p_{j,t_{ij}}\in[0,1]\}_{j\in[m],t_{ij}\in T_{ij}}$.
We are going to prove that $W_{i,\epsilon}^r\subseteq W_i$.
When an agent with type $t_i$ appears, the mechanism works in the following way.
For each $j\in[m]$, let 
$$C(j) \sim Ber\left( \min\left(\frac{\epsilon}{f_{ij}(t_{ij})},1 \right)\right)$$
If there exists only one $j^*\in[m]$ such that $C(j^*)=1$,
then allocate only the $j^*$-th item to the agent activating the additive function $k^*\in[K]$ such that $\alpha^{k*}_{j^*}=V_{ij}(t_{ij})$.
%with probability $p_{j,t_{ij}}$.
Note that:
$$
\Pr_{\substack{t_{ij}\sim D_{ij}\\C(j) \sim Ber\left( \min\left(\frac{\epsilon}{f_{ij}(t_{ij})},1) \right)\right) }}\left[C_j=1  \right] \leq \sum_{t_{ij}\in \cT_{ij}} f_{ij}(t_{ij})\cdot\min\left(\frac{\eps}{f_{ij}(t_{ij})},1 \right) \leq \eps \cdot |\cT_{ij}|
$$
Thus by union bound, $\Pr[C_j=0,\forall j]\geq 1-\sum_j\Pr[C_j=1]\geq 1-\eps\cdot T$.
%the probability that there is no $j\in[m]$ such that $C(j)=1$ is at least $1-\epsilon \cdot M$.
Thus under this allocation we have that
\begin{align*}
    w_{ij}(t_{ij}) = \pi_{ij}(t_{ij}) \geq (1-\epsilon\cdot M)  \min\left(\frac{\epsilon}{f_{ij}(t_{ij})}, 1 \right)f_{ij}(t_{ij}) =
    (1-\epsilon\cdot M)  \min\left(\epsilon, f_{ij}(t_{ij})\right)
\end{align*}
Thus for any target 
$$\{\hat{\pi}_{ij}(t_{ij})\leq (1-\epsilon \cdot M)\min(\epsilon,f_{ij}(t_{ij})\}_{j\in[m],t_{ij}\in T_{ij}}$$ 
there exists a set of variables $\{p_{j,t_{ij}} \in [0,1]\}_{j\in[m],t_{ij}\in T_{ij}}$ such that when the agent has type $t_{i}$, then with probability $p_{j,t_{ij}}$ we set $C(j)=0$ and then run the mechanism as we described it.
This allocation distribution ensures that:
\begin{align*}
    w_{ij}(t_{ij}) = \pi_{ij}(t_{ij}) =\hat{\pi}_{ij}(t_{ij})
\end{align*}
Thus we proved that for every $(\pi,w)$ such that:
\begin{align*}
    w_{ij}(t_{ij}) = \pi_{ij}(t_{ij}) \leq
    (1-\epsilon\cdot M)  \min\left(\epsilon, f_{ij}(t_{ij})\right)
\end{align*}
$(\pi,w_i)\in  W_i$.
Observe that for each $(\pi',w_i')$ such that:
\begin{align*}
    w_{ij}'(t_{ij})\leq w_{ij}(t_{ij}) \\
    \pi_{ij}'(t_{ij})\geq \pi_{ij}(t_{ij})
\end{align*}

then $(\pi',w')\in W_i$.
This concludes that $W_{i,\eps}^r \subseteq W_i$ for all $\epsilon < \frac{1}{T}$.}
\end{proof}

Now we consider the polytope $\frac{1}{2}W_{i,\eps}^f + \frac{1}{2}W_{i, \eps}^r$. We prove in the following lemma that it approximates $W_i$ with a multiplicative ratio.

\begin{lemma}
For any $0\leq \eps<\frac{1}{T}$, then $\frac{1-\eps\cdot T}{2}W_i \subseteq \frac{1}{2}W_{i,\eps}^f + \frac{1}{2}W_{i, \eps}^r \subseteq  W_i$.
\end{lemma}
\begin{proof}
$\frac{1}{2}W_{i,\epsilon}^f + \frac{1}{2}W_{i, \epsilon}^r \subseteq  W_i$ directly comes from Definition~\ref{def:welfare frequent} and Lemma~\ref{lem:welfare rare}.

Now we are going to show that for each $(\pi_i,w_i) \in \frac{1-\eps \cdot T}{2}\cdot W_i$,
then $(\pi_i,w_i) \in \frac{1}{2}W_{i,\eps}^f + \frac{1}{2}W_{i, \eps}^r$.
We consider the following vector $(\pi_{i}^f, w_{i}^f)$:
\begin{align*}
\pi_{ij}^f(t_{ij})=
\begin{cases}
\pi_{ij}(t_{ij}), \quad&\text{if $f_{ij}(t_{ij})\geq \epsilon$}\\
0,& \text{o.w} 
\end{cases}    \\
w_{ij}^f(t_{ij})=
\begin{cases}
w_{ij}(t_{ij}), \quad&\text{if $f_{ij}(t_{ij})\geq \epsilon$}\\
0,& \text{o.w} 
\end{cases}
\end{align*}

Then by \Cref{def:welfare frequent}, $(\pi_{i}^f, w_{i}^f)\in \frac{1-\eps\cdot T}{2}W_{i,\eps}^f\subseteq \frac{1}{2}W_{i,\eps}^f$. We consider another vector $(\pi_{i}^r, w_{i}^r)$ %$(\pi_{i}^r, w_{i}^r)\in  \frac{1}{2}W_{i,\eps}^r$ 
such that:
\begin{align*}
\pi_{ij}^r(t_{ij})=
\begin{cases}
\pi_{ij}(t_{ij}), \quad&\text{if $f_{ij}(t_{ij})< \eps$}\\
0,& \text{o.w} 
\end{cases}    \\
w_{ij}^r(t_{ij})=
\begin{cases}
w_{ij}(t_{ij}), \quad&\text{if $f_{ij}(t_{ij}) < \eps$}\\
0,& \text{o.w} 
\end{cases}
\end{align*}
We notice that since $(\pi_i,w_i)\in \frac{1-\eps \cdot T}{2}\cdot W_i$, we have $w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})\leq \frac{1-\eps \cdot T}{2}\cdot f_{ij}(t_{ij})$. Thus $w_{ij}^r(t_{ij})\leq \pi_{ij}^r(t_{ij})\leq \frac{1-\eps \cdot T}{2}\cdot f_{ij}(t_{ij})\cdot \ind[f_{ij}(t_{ij})<\eps]$. Thus $(\pi_{i}^r, w_{i}^r)\in \frac{1}{2}W_{i,\eps}^r$. Now observe that $(\pi_i,w_i) = (\pi^f_i + \pi^r_i,w^f_i + w^r_i)\in \frac{1}{2}W_{i,\eps}^f + \frac{1}{2}W_{i, \eps}^r$,
which concludes the proof.
\end{proof}


\begin{definition}\label{def:welfare frequent-t_i}
For any $i, t_i \in \cT_i$ and $\eps>0$, we define the polytope $W^f_{i,\eps}(t_i) \subseteq [0,1]^{2\cdot \sum_j|\cT_{ij}|}$ as follows.
An element $(\pi_i^f,w_i^f)\in W^f_{i,\eps}(t_i)$ if there exists a number $\sigma_S^k\in[0,1]$ for all $S \subseteq [m],k\in [K]$, such that for any $j,t_{ij}'\in \cT_{ij}$,
\begin{align*}
&\sum_{S \subseteq [m]}\sum_{k \in [K]} \sigma_S^k \leq 1\\
&\pi_{ij}^f(t_{ij}')\geq
\sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^k\cdot \ind[t_{ij}'=t_{ij} \land f_{ij}(t_{ij})\geq \eps]\\
&w_{ij}^f(t_{ij}')\leq \sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^k\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}\cdot\ind[t_{ij}'=t_{ij}\land f_{ij}(t_{ij})\geq \eps]
%\begin{cases}
%\sum_{\{j\}\subseteq S \subseteq[m]}\sum_{k\in[K]} \sigma_S^k\frac{\alpha_j^k(t_j)}{V_j(t_j)}, \quad&\text{if $t'_j=t_j \land f_{ij}(t_{ij})\geq \eps$}\\
%0,& \text{o.w} 
%\end{cases}
\end{align*}
\end{definition}
\yangnote{Yang:$\pi_{ij}^f$ has no upper bound?}
\mingfeinote{It's bounded by 1 if $t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij})\geq \eps$. We can use the following definition:

An element $(\pi_i^f,w_i^f)\in W^f_{i,\eps}(t_i)$ if there exists a number $\sigma_S^k\in[0,1]$ for all $S \subseteq [m],k\in [K]$ such that
$\sum_{S \subseteq [m]}\sum_{k \in [K]} \sigma_S^k \leq 1$, and for any $j,t_{ij}'\in \cT_{ij}$,
\begin{itemize}
\item If $t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij})\geq \eps$, then $$\sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^k\leq \pi_{ij}^f(t_{ij}')\leq 1, \quad
w_{ij}^f(t_{ij}')\leq \sum_{S:j\in S} \sum_{k \in [K]} \sigma_S^k\cdot \frac{\alpha_{ij}^{(k)}(t_{ij})}{V_{ij}(t_{ij})}.$$
\item Otherwise, $\pi_{ij}^f(t_{ij}')=w_{ij}^f(t_{ij}')=0$.
\end{itemize}

}

%where we denote by $\pi_S$ the probability that we award exactly bundle $S$ to the agent.
Note that $W$ is the convex hull finite many deterministic allocation rules and deterministic choice of the activated additive function.
Thus $W$ is a convex polytope.
%\todo{We have to argue that when the function is XOS we really have polytopes? I think it is enough to note that this is true, since we have finite many types and finite many possible allocations.}
\todo{Is it ok to argue that if each $\alpha_j^k(t)$ has bit complexity $b$, then there cannot be infinity many additive functions in the XOS definition in the range $[0,H]$?}

\begin{observation}\label{obs:W_i(t_i)-1}
Let $\textbf{0}$ be the vector with 0 in all entries. For any $t_i$ and $\pi_i^f\in [0,1]^{\sum_j|\cT_{ij}|}$such that $\pi_{ij}^f(t_{ij}')\leq \ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij})\geq \eps]$, $(\pi_i^f,\textbf{0})\in W_{i,\eps}^f(t_i)$. 
\end{observation}
\begin{proof}
Choosing $\sigma_{S}^k=0$ for all $S,k$ finishes the proof.
\end{proof}


\begin{observation}\label{obs:W_i(t_i)-2}
Fix any $t_i$. For any $j$, $S_j\subseteq |\cT_{ij}|$, $(\pi,w)\in W_{i,\eps}^f(t_i)$, define $(\pi',w')\in [0,1]^{2\cdot \sum_{j}|\cT_{ij}|}$ as: $$\pi_{j}'(t_{ij}')=\pi_j(t_{ij}')\cdot\ind[t_{ij}\in S_j],\quad w_{j}'(t_{ij}')=w_j(t_{ij}')\cdot\ind[t_{ij}\in S_j].$$ 
Then $(\pi',w')\in W_{i,\eps}^f(t_i)$. 
\end{observation}

\begin{proof}
Let $\{\sigma_{S}^k\}_{S,k}$ be the set of numbers associated with $(\pi,w)$. Let $S'=\{j\mid t_{ij}\in S_j\}$. The observation then directly follows by choosing $(\sigma_{S}^{k})'=\sigma_{S\cap S'}^k$.
\end{proof}

\notshow{
\begin{observation}\label{obs:W_i(t_i)-2}
Let $L\geq 1$ be any integer. Suppose for every $j$, there exists a partition for $\cT_{ij}$: $\cT_{ij}=\cup_{\ell\in [L]}S_j^{(\ell)}$. Suppose $(\pi^{(\ell)},w^{(\ell)})\in W_{i,\eps}^f(t_i),\forall \ell\in [L]$. Define $(\pi,w)\in [0,1]^{2\cdot \sum_{j}|\cT_{ij}|}$ as: $$\pi_{j}(t_{ij})=\sum_{\ell}\pi_j^{(\ell)}(t_{ij})\cdot \ind[t_{ij}\in S_j^{(\ell)}],\quad w_{j}(t_{ij})=\sum_{\ell}w_j^{(\ell)}(t_{ij})\cdot \ind[t_{ij}\in S_j^{(\ell)}].$$ 
Then $(\pi,w)\in W_{i,\eps}^f(t_i)$.
\end{observation}
%\begin{proof}
%For every $\ell\in [L]$, 
%\end{proof}
}

\begin{definition}
For any two sets $A,B \subseteq \mathbb{R}^d$,
we denote by $A+B$ the \emph{Minkowski addition} of set $A$ and set $B$ where:
$$A+B = \{a + b : a \in A\land b \in B\}
$$

Note that if both $A$ and $B$ are convex, then $A+B$ is also convex.
\end{definition}


\begin{definition}[\todo{Should I cite the manuscript?}]
Consider a set of $N$ (where $N$ is a finite number) convex sets $\mathcal{P}_N=\{P_i\}_{i\in [N]}$ and a distribution $\mathcal{D}_N=\{p_i\}_{i\in[N]}$ over the elements in $[N]$.
The polytope $\mathcal{P} = \sum_{i\in[N]}p_i P_i$
is called the mixture of $\mathcal{P}_N$ over distribution $\mathcal{D}_N$.
\end{definition}


\begin{observation}\label{obs:mix}
For any $\eps>0$ and $t_i \in \cT_i$, $W_{i,\eps}^f$ is mixture of $\{W^f_{i,\eps}(t_i)\}_{t_i\in \cT_i}$ over distribution $D_i$. Recall that $D_i$ is the distribution for buyer $i$'s type $t_i$.
%$\{f_i(t_i)\}_{t_i \in T_i}$.
\end{observation}

\notshow{
\begin{observation}\label{obs:combine}
Let $W^f_{i,B}$ be a mixture of $\{W^f_{i,t_i,\epsilon}\}_{t_i\in T_i}$ over distribution $B$.
Then if $(\pi_i,w_i) \in W^f_{i,B}$,
then for any $(\pi_i',w_i')$ such that 
\begin{align*}
    &0 \leq w'_{ij}(t_{ij}) \leq w_{ij}(t_{ij}) \land \Pr_{t'_{ij}\sim B_{ij}}[t_{ij}'=t_{ij}] \geq \pi'_{ij}(t_{ij}) \geq \pi_{ij}(t_{ij}) \\
    \lor \quad & w'_{ij}(t_{ij}) = \pi'_{ij}(t_{ij}) = 0
\end{align*}
then $(\pi'_i, w'_i) \in W_{i,D}$.
\end{observation}

}



\begin{theorem}[\todo{What should I cite?}]\label{thm:approx mixture}
Let $\mathcal{P}$ be a mixture of $\mathcal{P}_N=\{P_i\}_{i\in[N]}$ over distribution $\mathcal{D}_N$,
where $P_i\subseteq \mathbb{R}^d$ and $P_i$ is a closed convex polytope for $i\in[N]$.
We further assume that for all $i\in[N]$,
the bit complexity of each corner of $P_i$ is at most $b$.
For $\eps > 0$ and integer $k \geq \max\left(\log\left( \frac{1}{\eps} \right), \Omega(d^4(b + \log\left( \frac{1}{\eps}\right))\right)$,
let $\mathcal{D}'_N$ be the empirical distribution induced by $\frac{8kd}{\epsilon^2}$ samples from $\mathcal{D}_N$.
Let $\mathcal{P}'$ be the mixture of of $\mathcal{P}_N=\{P_i\}_{i\in[N]}$ over distribution $\mathcal{D}'_N$.
With probability at least $1-2de^{-2dk}$ we have that
\begin{enumerate}
    \item For all $q\in \mathcal{P}$,
    there exists a $q'\in \mathcal{P}'$ such that $||q-q'||_\infty \leq \eps$
    \item For all $q'\in \mathcal{P}'$,
    there exists a $q\in \mathcal{P}$ such that $||q-q'||_\infty \leq \eps$
\end{enumerate}
\end{theorem}









\begin{theorem}\label{thm:multi-approx-mixture}
For every $i$, $0 < \eps < 1/T$ and $\delta\in (\eps T,1)$, let $\widehat{D}_i$ be the empirical distribution induced by $k\geq $ \mingfeinote{sth.} independent samples from $D_i$. Let $\widehat{W}_{i,\eps}^f$ be the mixture of $\{W_{i,\eps}^f(t_i)\}_{t_i\in T_i}$ over the empirical distribution $\widehat{D}_i$.
%induced by $k$ samples from $D$ 
%\todo{ need enough samples so that the additive error is $\epsilon'$}.
Consider the polytope $\widehat{W}_i = \frac{1}{2}\widehat{W}_{i,\eps}^f + \frac{1}{2}W^r_{i,\eps}$. Then with probability \mingfeinote{add prob.}, both of the following are satisfied \yangnote{Yang: I believe with the statement here, we can guarantee to solve the program within a constant factor. But 
does this imply that $\widehat{W}_i$ is sandwiched between $a W_i$ and $b W_i$?  }\argyrisnote{Argyris: I don't think it implies that $\widehat{W}_i$ can be sandwiched, but I think that we can "round" each coordinate of the element of $\widehat{W}_i$ (by multiplying each coordinate with a constant) such that the rounded element is in $W_i$}: 
\begin{enumerate}
    \item For each $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$,
there exists a $(\pi_i,w_i) \in \frac{1}{2}W^f_{i,\eps} +\frac{1}{2}W^r_{i,\eps}$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:
$$\frac{{\pi}_{ij}(t_{ij})}{\widetilde{\pi}_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}],\quad \frac{{w}_{ij}(t_{ij})}{\widetilde{w}_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}]$$
%\argyrisnote{maybe the multiplicative approximation is a different constant}
%\begin{align*}
%\frac{\epsilon-\epsilon'}{\epsilon}\pi_{ij}(t_{ij})\leq \widehat{\pi}_{ij}(t_{ij}) \leq& \frac{\epsilon + \epsilon'}{\epsilon}\pi_{ij}(t_{ij}) %\\
%\frac{\epsilon + \epsilon'}{\epsilon}w_{ij}(t_{ij})\leq \widehat{w}_{ij}(t_{ij}) \leq& \frac{\epsilon + \epsilon'}{\epsilon}w_{ij}(t_{ij}) \\
%\end{align*}
\item For each $(\pi_i,w_i) \in \frac{1}{2}W^f_{i,\eps} +\frac{1}{2}W^r_{i,\eps}$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:
%\begin{align*}
%\frac{\epsilon-\epsilon'}{\epsilon}\pi_{ij}(t_{ij})\leq \widehat{\pi}_{ij}(t_{ij}) \leq& \frac{\epsilon + \epsilon'}{\epsilon}\pi_{ij}(t_{ij}) %\\
%\frac{\epsilon + \epsilon'}{\epsilon}w_{ij}(t_{ij})\leq \widehat{w}_{ij}(t_{ij}) \leq& \frac{\epsilon + \epsilon'}{\epsilon}w_{ij}(t_{ij}) \\
%\end{align*}

$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}]$$
\end{enumerate}
\end{theorem}

\begin{proof}
\todo{Conditioning on the probability that the sampled polytope is accurate}.
Let $\eps'=\delta\cdot \eps$. We are going to show that for each $(\pi_i,w_i) \in \frac{1}{2}W^f_{i,\eps} +\frac{1}{2}W^r_{i,\eps}$,
there exists a $(\widetilde{\pi}_i,\widetilde{w}_i) \in \widehat{W}_i$ that satisfies the second condition. The other direction is similar.

For every $j,t_{ij}$, let $\widehat{f}_{ij}(t_{ij})=\Pr_{t_i'\sim \widehat{D}_i}[t_{ij}'=t_{ij}]$ be the marginal probability of $t_{ij}$ when $t_i\sim \widehat{D}_i$. We first prove the following lemma using \Cref{thm:approx mixture}. 

\begin{lemma}\label{lem:f_hat and f} \yangnote{Why does this require Theorem~\ref{thm:approx mixture}? This follows from Chernoff+union bound directly.} \argyrisnote{Argyris: I think we could, but we need to take a union-bound that we can avoid with this approach.}
For every $t_{ij}$ such that $f_{ij}(t_{ij})\geq \eps$, we have $\frac{\widehat{f}_{ij}(t_{ij})}{f_{ij}(t_{ij})}\in [1-\delta,1+\delta]$.
\end{lemma}
\begin{proof}

For any $t_i$, consider the following vector $(\pi_{i}^{(t_i)},w_i^{(t_i)})$ such that $\pi_{ij}^{(t_i)}(t_{ij}')=\ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij})\geq \eps], w_{ij}^{(t_i)}(t_{ij}')=0$. By \Cref{def:welfare frequent-t_i}, we have $(\pi_{i}^{(t_i)},w_i^{(t_i)})\in W_{i,\eps}^f(t_i)$ by considering the set of numbers $\{\sigma_S^{(k)}\}_{S,k}$ such that $\sigma_S^{(k)}=\ind[S=[m]\wedge k=\argmax_{k'}\alpha_{ij}^{(k')}(t_{ij})]$. Now let $(\pi_{i},w_i)=\sum_{t_{i}\in \cT_i}f_i(t_i)\cdot (\pi_{i}^{(t_i)},w_i^{(t_i)})$. Since $W_{i,\eps}^f$ is a mixture of $W_{i,\eps}^f(t_i)$ over $t_i\sim D_i$. Thus $(\pi_{i},w_i)\in W_{i,\eps}^f$. Moreover, $w_{ij}(t_{ij})=0$ and $$\pi_{ij}(t_{ij})=\sum_{t_i'\in \cT_i}f_i(t_i')\cdot \ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij}')\geq \eps]=f_{ij}(t_{ij})\cdot \ind[f_{ij}(t_{ij})\geq \eps]$$  

Similarly, let $(\widehat\pi_{i},\widehat w_i)=\sum_{t_{i}\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\pi_{i}^{(t_i)},w_i^{(t_i)})$. Then $(\widehat\pi_{i},\widehat w_i)\in \widehat{W}_{i,\eps}^f$. Moreover, $\widehat w_{ij}(t_{ij})=0$ and $$\widehat\pi_{ij}(t_{ij})=\sum_{t_i'\in \cT_i}\Pr_{x\sim \widehat{D}_i}[x=t_i']\cdot \ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij}')\geq \eps]=\widehat f_{ij}(t_{ij})\cdot \ind[f_{ij}(t_{ij})\geq \eps]$$   

Now by \Cref{thm:approx mixture}, there exists $(\pi_{i}',w_i')\in \widehat W_{i,\eps}^f$, such that $||\pi_i-\pi_i'||_{\infty}<\eps'$. Thus for $t_{ij}$ such that $f_{ij}(t_{ij})\geq \eps$, we have $$(1-\delta)f_{ij}(t_{ij})\leq f_{ij}(t_{ij})-\eps'=\pi_{ij}(t_{ij})-\eps'\leq \pi_{ij}'(t_{ij})\leq\widehat{f}_{ij}(t_{ij})$$

the last inequality is because: since $\widehat W_{i,\eps}^f$ is a mixture of $\widehat W_{i,\eps}^f(t_i)$ over $t_i\sim \widehat D_i$, $$\pi_{ij}'(t_{ij})\leq \sum_{t_{i'}\in \cT_i}\Pr_{x\sim \widehat{D}_i}[x=t_i']\cdot \ind[t_{ij}=t_{ij}']=\widehat{f}_{ij}(t_{ij}).$$

On the other hand, again by \Cref{thm:approx mixture}, there exists $(\pi_{i}'',w_i'')\in W_{i,\eps}^f$, such that $||\widehat\pi_i-\pi_i''||_{\infty}<\eps'$. Thus for $t_{ij}$ such that $f_{ij}(t_{ij})\geq \eps$, we have $$\widehat f_{ij}(t_{ij})=\widehat\pi_{ij}(t_{ij})\leq \pi_{ij}''(t_{ij})+\eps'\leq (1+\delta)\cdot f_{ij}(t_{ij})$$
the last inequality uses the fact that $\pi_{ij}''(t_{ij})\leq f_{ij}(t_{ij})$ and $f_{ij}(t_{ij})\geq \eps$.

\notshow{
By noting that for each $j\in[m]$ and $t_{ij}\in T_{ij}$ such that $f_{ij}(t_{ij}) \geq \epsilon$,
then the element $(\pi_{i,t_{ij}},w_{i,t_{ij}})$ such that
\begin{align*}
    \pi_{i,t_{ij}}(t_{ij}') = w_{i,t_{ij}}(t_{ij}') = 
    \begin{cases}
    f_{ij}(t_{ij}) \quad &\text{if $t_{ij}'= t_{ij}$}\\
    0 & \text{ o.w.}
    \end{cases}
\end{align*}
$(\pi_{i,t_{ij}},w_{i,t_{ij}})\in W^f_{i,\epsilon}$.
Similarly for each $j\in[m]$ and $t_{ij}\in T_{ij}$ such that $f_{ij}(t_{ij}) \geq \epsilon$,
then the element $(\widehat{\pi}_{i,t_{ij}},\widehat{w}_{i,t_{ij}})$ such that
\begin{align*}
    \widehat{\pi}_{i,t_{ij}}(t_{ij}') = \widehat{w}_{i,t_{ij}}(t_{ij}') = \begin{cases}
    \Pr_{t_{ij}'\sim \widehat{D}_{j}}\left[t_{ij}'=t_{ij} \right] \quad &\text{if $t_{ij}'= t_{ij}$}\\
    0 & \text{ o.w.}
    \end{cases}
\end{align*}
$(\widehat{\pi}_{i,t_{ij}},\widehat{w}_{i,t_{ij}})\in \widehat{W}^f_{i,\epsilon}$.
A consequence of Theorem~\ref{thm:approx mixture} is that for each $j\in[m]$ and $t_{ij}\in T_{ij}$ such that $f_{ij}(t_{ij}) \geq \epsilon$,
then 
$$ f_{ij}(t_{ij}) - \frac{\epsilon'}{\epsilon}f_{ij}(t_{ij})\leq f_{ij}(t_{ij}) - \epsilon' \leq \Pr_{t_{ij}'\sim \widehat{D}_{j}}\left[t_{ij}'=t_{ij} \right]\leq f_{ij}(t_{ij}) + \epsilon' \leq f_{ij}(t_{ij}) + \frac{\epsilon'}{\epsilon}f_{ij}(t_{ij})$$
}
\end{proof}


%is close to $(\pi,w_i)$ in a multiplicative sense, since the other directions is similar.

Back to the proof of \Cref{thm:multi-approx-mixture}. Since $(\pi_i,w_i) \in \frac{1}{2}W^f_{i,\eps} +\frac{1}{2}W^r_{i,\eps}$,
we can decompose $(\pi_i,w_i) = \frac{1}{2}(\pi_i^f,w_i^f) + \frac{1}{2}(\pi_i^r,w_i^r)$ such that $(\pi_i^f,w_i^f) \in W^f_{i,\eps}$ and $(\pi_i^r,w_i^r) \in W^r_{i,\eps}$.
For every $j\in [m]$, we partition $\cT_{ij}$ into four disjoint sets: 
%such that the polytope $\in \frac{1}{2}W^f_{i,\epsilon}$ has (possibly) non-zero elements into the following two disjoint sets:
\begin{align*}
S_{j}^{(1)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land \eps < w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij})  \} \\
S_j^{(2)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land w_{ij}(t_{ij})\leq \eps < \pi_{ij}(t_{ij})  \} \\
S_j^{(3)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) \geq \eps \land w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij}) \leq \eps \}\\
S_j^{(4)}=&\{t_{ij}\in \cT_{ij} : f_{ij}(t_{ij}) <\eps\}
\end{align*}

%Recall that for each $t_{ij}\in T_{ij}$ such that $f_{ij}(t_{ij}) < \epsilon$, then for each $(\pi_i^a,w_i^a) \in W^f_{i,\epsilon}$ and $(\pi_i^b,w_i^b) \in \widehat{W}^f_{i,\epsilon}$,
%then $\pi^a_{ij}(t_{ij})=w^a_{ij}(t_{ij})=\pi^b_{ij}(t_{ij})=w^b_{ij}(t_{ij})=0$.

%\begin{align*}
%S_{+}=&\cup_{j\in[m]}\{t_{ij}\in T_{ij} : \epsilon < w_{ij}(t_{ij})  \} \\
%S_{-}=&\cup_{j\in[m]}\{t_{ij}\in T_{ij} :  w_{ij}(t_{ij})\leq \leq \epsilon \}
%\end{align*}



By Theorem~\ref{thm:approx mixture}, there exists a $(\widehat{\pi}^f_{i},\widehat{w}^f_i)\in \widehat{W}^f_{i,\eps}$ such that for all $j\in[m]$ and $t_{ij} \in \cT_{ij}$:
\begin{align*}
\pi^f_{ij}(t_{ij}) - \eps'\leq \widehat{\pi}^f_{ij}(t_{ij}) \leq \pi^f_{ij}(t_{ij}) + \eps' \\
w^f_{ij}(t_{ij}) - \eps'\leq \widehat{w}^f_{ij}(t_{ij}) \leq w^f_{ij}(t_{ij}) + \eps'
\end{align*}

Let $a=1-\eps\cdot T>0$. Now consider the following vector $(\widetilde{\pi}^f_i,\widetilde{w}^f_i) \in [0,1]^{2\sum_{j\in[m]}|\cT_{ij}|}$:
\begin{align*}
\widetilde{\pi}^f_{ij}(t_{ij}) =&
\begin{cases}
\widehat{\pi}_{ij}^f(t_{ij}) \quad & \text{ if $t_{ij}\in S_j^{(1)}$} \\
\min\left( \widehat{f}_{ij}(t_{ij}) ,a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))\right)  \quad & \text{ if $t_{ij}\in S_j^{(2)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\widetilde{w}^f_{ij}(t_{ij}) =&
\begin{cases}
\widehat{w}_{ij}^f(t_{ij}) \quad & \text{ if $t_{ij}\in S_j^{(1)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\end{align*}
\yangnote{What's $a$?}
%By Observation~\ref{obs:combine} we have that 
\mingfeinote{$a=1-\eps\cdot T$. Originally it was right after lemma 15. Now I move it right before the definition of $(\widetilde{\pi}^f_i,\widetilde{w}^f_i)$.}

\begin{lemma}
$(\widetilde{\pi}^f_i,\widetilde{w}^f_i) \in \widehat{W}_{i,\eps}^f$.
\end{lemma}
%We will prove that  
%Let $\eta_i\in [0,1]^{\sum_{j\in [m]}|\cT_{ij}|}$ be the vector such that 
\begin{proof}
Since $(\widehat{\pi}^f_{i},\widehat{w}^f_i)\in \widehat{W}^f_{i,\eps}$, for every $t_i$, there exists $(\widehat{\pi}^{(t_i)},\widehat{w}^{(t_i)})\in W_{i,\eps}^f(t_i)$, such that $(\widehat{\pi}^f_{i},\widehat{w}^f_i)=\sum_{t_i\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\widehat{\pi}^{(t_i)},\widehat{w}^{(t_i)})$. Define $(\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})$ as follows:

\begin{align*}
\widetilde{\pi}^{(t_i)}_j(t_{ij}') =&
\begin{cases}
\widehat{\pi}^{(t_i)}_j(t_{ij}) \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(1)}$} \\
\min\left(1 ,a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))/\widehat{f}_{ij}(t_{ij})\right)  \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(2)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\widetilde{w}^{(t_i)}_{j}(t_{ij}') =&
\begin{cases}
\widehat{w}_{j}^{(t_i)}(t_{ij}) \quad & \text{ if $t_{ij}=t_{ij}'\wedge t_{ij}\in S_j^{(1)}$} \\
0 \quad & \text{ o.w.}
\end{cases}\\
\end{align*}

By \Cref{obs:W_i(t_i)-1} and \Cref{obs:W_i(t_i)-2}, we have $(\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})\in W_{i,\eps}^f(t_i)$. Since $\widehat{W}_{i,\eps}^f$ is a mixture of $W_{i,\eps}^f(t_i)$ over distribution $\widehat{D}_i$, we have that $(\widetilde{\pi}^f_{i},\widetilde{w}^f_i)=\sum_{t_i\in \cT_i}\Pr_{t_i'\sim \widehat{D}_i}[t_i'=t_i]\cdot (\widetilde{\pi}^{(t_i)},\widetilde{w}^{(t_i)})$ is in $\widehat{W}_{i,\eps}^f$. 
\end{proof}

%For any $t_i$, consider the following vector $(\pi_{i}^{(t_i)},w_i^{(t_i)})$ such that $\pi_{ij}^{(t_i)}(t_{ij}')=\ind[t_{ij}'=t_{ij}\wedge f_{ij}(t_{ij})\geq \eps], w_{ij}^{(t_i)}(t_{ij}')=0$. By \Cref{def:welfare frequent-t_i}, we have $(\pi_{i}^{(t_i)},w_i^{(t_i)})\in W_{i,\eps}^f(t_i)$ by considering the set of numbers $\{\sigma_S^{(k)}\}_{S,k}$ such that $\sigma_S^{(k)}=\ind[S=[m]\wedge k=\argmax_{k'}\alpha_{ij}^{(k')}(t_{ij})]$.



Now we consider another vector $(\widetilde{\pi}^r_i,\widetilde{w}^r_i)$: 
%\in W_{i,\epsilon}^r$:
\begin{align*}
(\widetilde{\pi}^r_{ij}(t_{ij}),\widetilde{w}^r_{ij}(t_{ij})) =&
\begin{cases}
({\pi}_{ij}^r(t_{ij}),w^r_{ij}(t_{ij})) \quad & \text{ if $t_{ij}\in S_{j}^{(1)}\cup S_{j}^{(4)}$} \\ 
(a\cdot w_{ij}(t_{ij}),a\cdot w_{ij}(t_{ij}))  \quad & \text{ if $t_{ij}\in S_{j}^{(2)}$} \\
(a\cdot{\pi}_{ij}(t_{ij}),a\cdot w_{ij}(t_{ij})) \quad & \text{ if $t_{ij}\in S_{j}^{(3)}$} \\
%(\pi_{ij}^r(t_{ij}) \quad & \text{ if $t_{ij}\in S_{j}^{(4)}$}
\end{cases}
%\widetilde{w}^r_{ij}(t_{ij}) %=&
%\begin{cases}
%{w}_{ij}^r(t_{ij}) \quad & %\text{ if $t_{ij}\in S_{++}$} \\
%w_{ij}(t_{ij})  \quad & \text{ if $t_{ij}\in S_{+-}$} \\
%{w}_{ij}(t_{ij}) \quad & \text{ if $t_{ij}\in S_{--}$} \\
%w_{ij}^r(t_{ij}) \quad & \text{ o.w.}
%\end{cases}
\end{align*}

For every $j,t_{ij}$, clearly $\widetilde{\pi}_{ij}^r(t_{ij})\geq \widetilde{w}_{ij}^r(t_{ij})$ since $\pi_{ij}^r(t_{ij})\geq w_{ij}^r(t_{ij})$ and $\pi_{ij}(t_{ij})\geq w_{ij}(t_{ij})$. Moreover, if $t_{ij}\in S_j^{(1)}\cup S_j^{(4)}$, $\widetilde{\pi}_{ij}^r(t_{ij})=\pi_{ij}^r(t_{ij})\leq a\cdot \min\{\eps,f_{ij}(t_{ij})\}$. If $t_{ij}\in S_j^{(2)}\cup S_j^{(3)}$, by definition of $S_j^{(2)}$ and $S_j^{(3)}$, we have that $\widetilde\pi_{ij}^r(t_{ij})\leq a\cdot\eps=a\cdot \min\{\eps,f_{ij}(t_{ij})\}$. Thus $(\widetilde{\pi}^r_i,\widetilde{w}^r_i)\in W_{i,\eps}^r$. Now define $(\widetilde{\pi},\widetilde{w})=\frac{1}{2}(\widetilde{\pi}^f_i,\widetilde{w}^f_i) + \frac{1}{2}(\widetilde{\pi}^r_i,\widetilde{w}^r_i)$. Then $(\widetilde{\pi}_i,\widetilde{w}_i)\in \widehat{W}_i$.
We remain to prove that $(\widetilde{\pi}_i,\widetilde{w}_i)$ satisfies:
%is close to $({\pi}_i,{w}_i)$ in a multiplicative sense.
%We are going to take cases.

$$\frac{\widetilde{\pi}_{ij}(t_{ij})}{\pi_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}],\quad \frac{\widetilde{w}_{ij}(t_{ij})}{w_{ij}(t_{ij})}\in [\frac{1-\delta}{2},1+\frac{\delta}{2}]$$

We will verify all cases depending on which set $t_{ij}$ is in. First observe that for $t_{ij}\in S_j^{(1)}$, $\eps<w_{ij}(t_{ij}) \leq \pi_{ij}(t_{ij})$. We have $$-\frac{\delta}{2}\cdot \pi_{ij}(t_{ij})\leq-\frac{\eps'}{2}\leq\widetilde\pi_{ij}(t_{ij})-\pi_{ij}(t_{ij})=\frac{1}{2}(\hat\pi_{ij}^f(t_{ij})-\pi_{ij}^f(t_{ij}))\leq\frac{\eps'}{2}\leq \frac{\delta}{2}\cdot \pi_{ij}(t_{ij})$$
Similarly, 
$$-\frac{\delta}{2}\cdot w_{ij}(t_{ij})\leq-\frac{\eps'}{2}\leq\widetilde {w}_{ij}(t_{ij})-w_{ij}(t_{ij})=\frac{1}{2}(\hat{w}_{ij}^f(t_{ij})-w_{ij}^f(t_{ij}))\leq\frac{\eps'}{2}\leq \frac{\delta}{2}\cdot w_{ij}(t_{ij})$$

%\begin{align*}
%{\pi}_{ij}(t_{ij}) - \frac{\epsilon'}{2\epsilon}{\pi}_{ij}(t_{ij}) \leq {\pi}_{ij}(t_{ij}) - \frac{\epsilon'}{2}\leq  \widetilde{\pi}_{ij}(t_{ij})  \leq {\pi}_{ij}(t_{ij}) + \frac{\epsilon'}{2} \leq {\pi}_{ij}(t_{ij}) + \frac{\epsilon'}{2\epsilon}{\pi}_{ij}(t_{ij}) \\
%{w}_{ij}(t_{ij}) - \frac{\epsilon'}{2\epsilon}{w}_{ij}(t_{ij}) \leq {w}_{ij}(t_{ij}) - \frac{\epsilon'}{2}\leq  \widetilde{w}_{ij}(t_{ij})  \leq {w}_{ij}(t_{ij}) + \frac{\epsilon'}{2} \leq {w}_{ij}(t_{ij}) + \frac{\epsilon'}{2\epsilon}{w}_{ij}(t_{ij}) \\
%\end{align*}

For $t_{ij}\in S_j^{(2)}$,
we have
$
\widetilde{w}_{ij}(t_{ij}) = \frac{a}{2}\cdot {w}_{ij}(t_{ij})
$.
For $\widetilde{\pi}_{ij}(t_{ij})$, when $\widehat{f}_{ij}(t_{ij}) \geq a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))$,
$
\widetilde{\pi}_{ij}(t_{ij}) = \frac{a}{2}\cdot {\pi}_{ij}(t_{ij})
$.
Moreover, since $(\pi_i,w_i) \in \frac{1}{2}W^f_{i,\eps} +\frac{1}{2}W^r_{i,\eps}\subseteq W_i$, we have $\pi_{ij}(t_{ij})-w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij}) \leq f_{ij}(t_{ij})$. Also by \Cref{lem:f_hat and f}, $\widehat{f}_{ij}(t_{ij}) \geq (1-\delta)f_{ij}(t_{ij})$. Thus if $\widehat{f}_{ij}(t_{ij}) < a\cdot(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}))$,
then
$$
\left(1-\delta\right)\left(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}) \right)\leq \left(1-\delta \right)f_{ij}(t_{ij})\leq \widehat{f}_{ij}(t_{ij})
$$


%If $\Pr_{t_{ij}'\sim \widehat{D}_j} \left[ t_{ij}'=t_{ij} \right] < \pi_{ij}(t_{ij}) - w_{ij}(t_{ij})$,
%then 
%by combining the fact that $f_{ij}(t_{ij})\geq \epsilon $ and $f_{ij}(t_{ij}) - \epsilon' \leq \Pr_{t_{ij}'\sim \widehat{D}_{j}}\left[t_{ij}'=t_{ij} \right]\leq f_{ij}(t_{ij}) + \epsilon'$ we can infer that
%$$
%f_{ij}(t_{ij}) - \frac{\epsilon'}{\epsilon}f_{ij}(t_{ij}) \leq f_{ij}(t_{ij}) - \epsilon' \leq \Pr_{t_{ij}'\sim \widehat{D}_{j}}\left[t_{ij}'=t_{ij} \right]\leq f_{ij}(t_{ij}) + \epsilon' \leq f_{ij}(t_{ij}) + \frac{\epsilon'}{\epsilon}f_{ij}(t_{ij})
%$$

%Moreover we have that $\pi_{ij}(t_{ij}) - w_{ij}(t_{ij})\leq \pi_{ij}(t_{ij}) \leq f_{ij}(t_{ij})$.
Thus
\begin{align*}
    \widetilde{\pi}_{ij}(t_{ij}) = \frac{1}{2} \left(\widehat{f}_{ij}(t_{ij}) + a\cdot w_{ij}(t_{ij})\right) \geq \frac{1}{2} \left(1-\delta\right)(\pi_{ij}(t_{ij}) - w_{ij}(t_{ij})) + \frac{a}{2}w_{ij}(t_{ij}) \geq \frac{1-\delta}{2} \pi_{ij}(t_{ij}),
\end{align*}
where the last inequality uses the fact that $a\geq 1-\delta$. On the other hand,
\begin{align*}
    \widetilde{\pi}_{ij}(t_{ij})<\frac{a}{2} (\pi_{ij}(t_{ij}) - w_{ij}(t_{ij}) + w_{ij}(t_{ij})) \leq \frac{a}{2} \pi_{ij}(t_{ij})
\end{align*}

For $t_{ij}\in S_j^{(3)}$, we have $\widetilde{\pi}_{ij}(t_{ij}) = \frac{a}{2}\cdot {\pi}_{ij}(t_{ij})$ and $\widetilde{w}_{ij}(t_{ij}) = \frac{a}{2}\cdot {w}_{ij}(t_{ij})$. 
%\begin{align*}
%\widetilde{\pi}_{ij}(t_{ij}) = \frac{1}{2} {\pi}_{ij}(t_{ij}) \\
%\widetilde{w}_{ij}(t_{ij}) = \frac{1}{2} {w}_{ij}(t_{ij})
%\end{align*}
For $t_{ij}\in S_j^{(4)}$, since $f_{ij}(t_{ij})<\eps$, $w_{ij}^f(t_{ij})=\pi_{ij}^f(t_{ij})=0$. Thus $\widetilde{\pi}_{ij}(t_{ij})=\frac{1}{2}\pi_{ij}^r(t_{ij})=\pi_{ij}(t_{ij})$, and $w_{ij}(t_{ij})=\frac{1}{2}w_{ij}^r(t_{ij})=w_{ij}(t_{ij})$. 
%\begin{align*}
%\widetilde{\pi}_{ij}(t_{ij}) =  {\pi}_{ij}(t_{ij}) \\
%\widetilde{w}_{ij}(t_{ij}) = {w}_{ij}(t_{ij})
%\end{align*}
\end{proof}





\notshow{
\begin{observation}
Let $(\pi_i,w_i)\in W_{\neg \epsilon}$,
then the element $(\pi_i',w_i')\in W_{\neg \epsilon}$ such that:
\begin{align*}
    w_{ij}'(t_{ij}) \geq &w_{ij}(t_{ij}) \\
    \pi_{ij}'(t_{ij}) \leq &\pi_{ij}(t_{ij})
\end{align*}
or
\begin{align*}
    w_{ij}'(t_{ij}) = \pi_{ij}'(t_{ij}) =0
\end{align*}

Let $\hat{W}_{\neg \epsilon}$ be the sampled induced polytope by $W_{\neg \epsilon}$,
then the property holds.
\end{observation}









\begin{theorem}
Let $\hat{W}_{\neg c\cdot \epsilon}$ be the sampled polytope induced by $W_{\neg c\cdot \epsilon}$ with additive error $c \cdot \epsilon$ where $c\in[0,1]$.
Consider the polytope $\hat{W} = \frac{1}{2}\hat{W}_{\neg c\cdot \epsilon} + \frac{1}{2}W_{\epsilon}$.
Then for each $(\widehat{\pi},\widehat{w}) \in \widehat{W}$,
there exists a $(\pi,w) \in \frac{1}{2}W_{\neg\epsilon} +\frac{1}{2}W_\epsilon$ such that for all $j\in[m]$ and $t_j \in T_j$:
\begin{align*}
\frac{c-1}{c}\pi_{ij}(t_{ij})\leq \widehat{\pi}_{ij}(t_{ij}) \leq& \frac{c+1}{c}\pi_{ij}(t_{ij}) \\
\frac{c-1}{c}w_{ij}(t_{ij})\leq \widehat{w}_{ij}(t_{ij}) \leq& \frac{c+1}{c}w_{ij}(t_{ij}) \\
\end{align*}

and for each $(\widehat{\pi},\widehat{w}) \in \widehat{W}$,
there exists a $(\pi,w) \in W$ such that for all $j\in[m]$ and $t_j \in T_j$:
\begin{align*}
\frac{c-1}{c}\pi_{ij}(t_{ij})\leq \widehat{\pi}_{ij}(t_{ij}) \leq& \frac{c+1}{c}\pi_{ij}(t_{ij}) \\
\frac{c-1}{c}w_{ij}(t_{ij})\leq \widehat{w}_{ij}(t_{ij}) \leq& \frac{c+1}{c}w_{ij}(t_{ij}) \\
\end{align*}
\end{theorem}

\begin{proof}
We are only going to prove the case where if $(\pi,w) \in \frac{1}{2}W_{\neg\epsilon} +\frac{1}{2}W_\epsilon$,
then there exists a $(\hat{\pi},\hat{w}) \in \frac{1}{2}\hat{W}_{\neg\epsilon} +\frac{1}{2}W_\epsilon$ such that for all $j\in[m]$ and $t_j \in T_j$:
\begin{align*}
\frac{c-1}{c}\pi_{ij}(t_{ij})\leq \widehat{\pi}_{ij}(t_{ij}) \leq& \frac{c+1}{c}\pi_{ij}(t_{ij}) \\
\frac{c-1}{c}w_{ij}(t_{ij})\leq \widehat{w}_{ij}(t_{ij}) \leq& \frac{c+1}{c}w_{ij}(t_{ij}) \\
\end{align*}

Note that each $w \in  \frac{1}{2}W_{\neg\epsilon} +\frac{1}{2}W_\epsilon$,
can be decomposed into two vectors $w_{\neg c\cdot  \epsilon} \in \frac{1}{2}W_{\neg c \cdot \epsilon}$ and $w_{epsilon} \in \frac{1}{2}W_{\epsilon}$. 
By Theorem~\ref{thm:approx mixture},
for each $(\pi_{\neg c \cdot \epsilon},w_{\neg c \cdot \epsilon})\in W_{\neg c \cdot \epsilon}$
there exists a point $(\widetilde{\pi}_{\neg c \cdot \epsilon},\widetilde{w}_{\neg c \cdot \epsilon})\in \hat{W}_{\neg c \cdot \epsilon}$ such that for all $j\in[m]$ and $t_{ij}\in T_{ij}$:
\begin{align*}
\pi_{ij}(t_{ij})- c \cdot \epsilon \leq \widetilde{\pi}_{ij}(t_{ij}) \leq& \pi_{ij}(t_{ij}) + c \cdot \epsilon \\
w_{ij}(t_{ij})- c \cdot \epsilon \leq \widetilde{w}_{ij}(t_{ij}) \leq& w_{ij}(t_{ij}) + c \cdot \epsilon
\end{align*}


Now we are going to show how to construct the requested point based on $(\widetilde{\pi},\widetilde{w})$.
Note that for each $j\in[m]$ and $t_{ij}\in T_{ij}$ such that  $\epsilon \leq \pi_{ij}(t_{ij}) \leq w_{ij}(t_{ij})$, we have that:
\begin{align*}
\frac{c-1}{c}\pi_{ij}(t_{ij})\leq \widehat{\pi}_{ij}(t_{ij}) \leq& \frac{c+1}{c}\pi_{ij}(t_{ij}) \\
\frac{c-1}{c}w_{ij}(t_{ij})\leq \widehat{w}_{ij}(t_{ij}) \leq& \frac{c+1}{c}w_{ij}(t_{ij}) \\
\end{align*}
and we are not going to modify them.
Now we turn our attention in the case where $\pi_{ij}(t_{ij}) \leq w_{ij}(t_{ij}) < \epsilon$
\end{proof}
}


\notshow{
\subsection{OCRS \argyrisnote{(I don't think it is needed)}}
\begin{definition}[Definition~1.2 and Definition~1.4  \cite{FeldmanSZ21}]\label{def:ocrs}
We assume that the buyer's valuation is additive over $m$ heterogeneous items with feasibility constraints $\mathcal{F} \subseteq 2^{[m]}$.
Let $Q$ be the convex hull of vectors in $\mathcal{F}$.
Each item $j\in[m]$ can be active or inactive independent of each,
where the $j$-th item can be activated with probability $q_j$.
Our goal is to collect a subset of active elements w.r.t. feasibility constraints $\mathcal{F}$. 

A greedy Online Contention Resolution Scheme (greedy OCRS),
takes as input the vector of activation probabilities $q \in Q$, and outputs a downward-closed family of feasibility constraints $\mathcal{F}_q \subseteq \mathcal{F}$.
Then it iterates over items in $[m]$ in a (possible arbitrary) order and decides to include item $j\in[m]$,
if $j$ is active and by adding it to the already selected items,
we are still feasible w.r.t. $\mathcal{F}_q$.


Given vector $q$,
greedy OCRS could output a distribution over feasibility constraints,
in which case we call this OCRS greedy randomised OCRS.
\end{definition}


Another useful definition is the following.

\begin{definition}[Definition~1.8 \cite{FeldmanSZ21}]
Using the same notation as in Definition~\ref{def:ocrs},
consider we have an OCRS for feasibility constraints $\mathcal{F}$. Given vector of activation probabilities $q \in b \cdot Q$
where $b \in[0,1]$,
we define by $A(q)$ the distribution over active items w.r.t. proabiblities activation vector $q$ and by $\mathcal{D}_{\mathcal{F}}$ the distribution over subset of feasibility constraints generated by the greedy (possibly randomsed OCRS) for $q$.
We say that the greedy (possibly randomized) OCRS is $(b,c)$-selectable,
for $c\in[0,1]$,
if it holds that for each item $j\in[m]$:

$$
\Pr_{\substack{\mathcal{F}_q \sim \mathcal{D}_\mathcal{F}\\A \sim A(q)}}\left[S\cup \{j\}\in \mathcal{F}_q \quad \forall S \subseteq A \land S \in \mathcal{F}_q \right] \geq c
$$
\end{definition}


\argyrisnote{I don't think OCRS is needed.}
}

==> prelim.tex <==
\section{Preliminaries}\label{sec:prelim}

%\todo{Define $\prev$. Define the RPP which allows randomized prices. Mention that $\prev$ is clearly achieved by deterministic prices.}\argyrisnote{I would suggest making this comment in intro since we spent a pargraph describing the mechanisms.}


We focus on revenue maximization in the combinatorial auction with $n$ independent bidders and $m$ heterogeneous items. We denote bidder $i$'s type $t_i$ as $\{t_{ij}\}_{j\in [m]}$, where $t_{ij}$ is bidder $i$'s private information about item $j$. For each $i$, $j$, we assume $t_{ij}$ is drawn independently from the distribution $D_{ij}$. 
Let $D_i=\times_{j=1}^m D_{ij}$ be the distribution of bidder $i$'s type and $D=\times_{i=1}^n D_i$ be the distribution of the type profile.  %Except for \Cref{sec:sample access},
We only consider discrete distributions in this paper. We use $\cT_{ij}$ (or $\cT_i, \cT$) and $f_{ij}$ (or $f_i, f$) to denote the support and the probability mass function of $D_{ij}$ (or $D_i, D$). For notational convenience, we let  $t_{-i}$ to be the types of all bidders except $i$ and $t_{<i}$ (or $t_{\leq i})$ to be the types of the first $i-1$ (or $i$) bidders. Similarly, we define $D_{-i}$, $\cT_{-i}$
  and $f_{-i}$ for the corresponding distribution, support of the distribution, and probability mass function. 

\vspace{-.15in}
\paragraph{Valuation Functions.} For every bidder $i$, denote her valuation function as $v_i(\cdot,\cdot):\cT_i\times 2^{[m]}\to \mathbb{R}_+$. For every $t_i\in \cT_i,S\subseteq 2^{[m]}$, $v_i(t_i,S)$ is bidder $i$'s value for receiving a set $S$ of items, when her type is $t_i$. In the paper, we are interested in constrained-additive and XOS valuations. For every $i\in [n]$, bidder $i$'s valuation $v_i(\cdot,\cdot)$ is \emph{constrained-additive} if the bidder can receive a set of items subject to some downward-closed feasibility constraint $\cF_i$. Formally, $v_i(t_i,S)=\max_{R \in 2^S\cap \cF}\sum_{j\in R} t_{ij}$ for every type $t_i$ and set $S$. It contains classic valuations such as additive ($\cF_i=2^{[m]}$) and unit-demand ($\cF_i=\cup_{j\in[m]}\{j\}$). For constrained-additive valuations, we use $t_{ij}$ to denote bidder $i$'s value for item $j$. For every $i\in [n]$, bidder $i$'s valuation $v_i(\cdot,\cdot)$ is \emph{XOS (or fractionally-subadditive)} if each $t_{ij}$ represents a set of $K$ non-negative numbers $\{\alpha_{ij}^{(k)}(t_{ij})\}_{k\in[K]}$, for some integer $K$, and $v_i(t_i,S) = \max_{k\in[K]} \sum_{j\in S}\alpha_{ij}^{(k)}(t_{ij})$, for every type $t_i$ and set $S$. We denote by $V_{ij}(t_i)=v_i(t_i,\{j\})$ the value for a single item $j$. Since the value of the bidder for item $j$ only depends on $t_{ij}$, we denote $V_{ij}(t_{ij})$ as~the~singleton~value.


%When bidder $i$'s type is $t_i$, her valuation for a set of items $S$ is denoted by $v_i(t_i,S)$.

%We denote as $D_i =\prod_{j\in[m]}D_{ij}$ the product distribution over types that the $i$-th bidder is sampled from and by $D=\prod_{i\in[n]}D_i$ the product distribution of type profiles that all agents are sampled from.
%We denote by $\cT_{ij}$ (and $\cT_{i}, \cT$ resp.) the support of $D_{ij}$ (and $D_i$, $D$ resp.).
%Given a bidder's type $t_i\in \cT_i$, we denote by $t_{i-j}$ all the types of the bidder, except for item $j$.
%We denote by $f_{ij}(t_{ij})=\Pr_{t_{ij}'\sim D_{ij}}\left[t_{ij}'=t_{ij}\right]$,$f_{i}(t_{i})=\Pr_{t_{i}'\sim D_{i}}\left[t_{i}'=t_{i}\right]$ and $f(t) = \Pr_{t'\sim D}\left[t'=t\right]$.
%We denote as $D_{i-j}$ the distribution over types for bidder $i$, by excluding the type for item $j$, by $\cT_{i-j}$ the support of distribution $D_{i-j}$ and by $f(t_{i-j})=\Pr_{t_{i-j}'\sim D_{i-j}}\left[t_{i-j}'=t_{i-j}\right]$.
%Similarly given a type profile $t\in \cT$, we denote $t_{-i}$ the type profiles of all agent excluding agent $i$, $D_{-i}$ the distribution over type profiles excluding agent $i$, $\cT_{-i}$ the support of $\cT_{-i}$ and $f_{-i}(t_{-i})=\Pr_{t_{-i}'\sim D_{-i}}\left[t_{-i}'=t_{-i} \right]$. When the $i$-th bidder has type $t_i$,
%then we denote her value for the set of items $S\subseteq[m]$ as $v_i(t_i,S)$.
%the support over types that the $i$-th bidder has for the $j$-th. Similarly we denote by $\cT_i = \supp( D_i)$ the support over  and $\cT= \supp( D)$

%We consider several classes of bidder's valuation


\notshow{
\begin{definition}
%We consider several interesting classes of bidder's valuation
For every bidder $i$, we consider 
\begin{itemize}
\item \textbf{Constrained Additive:} Given a set of downward closed feasibility constraints $\cF$,
$v_i(t_i,S)=\max_{R\subseteq S,R \in \cF}\sum_{j\in R} t_{ij}$,
where we abuse the notation and denote by $v_i(t_{ij},\{j\})=t_{ij}$.
When $\cF=\cup_{j\in[m]}\{j\}$, that is a bidder is interested in buying at most one item, the valuation is called unit demand. When $\cF=2^{[m]}$, the valuation is called additive.
\item \textbf{XOS:} For a finite number $K$, each type represents a set of $K$ non-negative numbers $t_{ij}=\{a_{ij}^{(k)}(t_{ij})\}_{k\in[K]}$.
Moreover $v_i(t,S) = \max_{k\in[K]} \sum_{j\in S}a_{ij}^{(k)}(t_{ij})$ and we denote by $V_{ij}(t)=v(t,\{j\})$. Since the value of the agent for the $j$-th item only depends on $t_{ij}$, we overuse notation and also denote $V_{ij}(t_{ij})=v(t,\{j\})$.
%\item \textbf{Subadditive:} For all $S_1,S_2\subseteq[m]$ we have $v(t,S_1\cup S_2)\leq v(t,S_1) + v(t,S_2)$.
\end{itemize}
\end{definition}
%It is well known that the class of subadditive functions contains the class of XOS functions and the class of XOS functions contain the class of Constraint Additive functions.
%We need to introduce some additional definitions.
%More importantly we need to define what a Separation Oracle is.
}

\vspace{-.15in}
\paragraph{Mechanisms.} A mechanism $\cM$ can be described as a tuple $(\sigma,p)$, where $\sigma$ is the \emph{interim allocation} rule of $\cM$ and $p$ stands for the payment rule. Formally, for every bidder $i$, type $t_i$ and set $S$, $\sigma_{iS}(t_i)$ is the interim probability that bidder $i$ with type $t_i$ receives exact bundle $S$.  
%To ease notations, for every bidder $i$ and types $t_i$, we use $p_i(t_i)=\E_{t_{-i}}[p_i(t_i,t_{-i})]$ as the interim price paid by bidder $i$ and $\sigma_{iS}(t_i)=\E_{t_{-i}}[x_{iS}(t_i,t_{-i})]$ as the interim probability of receiving the exact bundle $S$.
We use standard concepts of BIC, DSIC and IR for mechanisms. See~\Cref{appx:prelim} for the formal definitions. For any BIC and IR mechanism $\cM$, denote $\rev(\cM)$ the revenue of $\cM$. Denote $\opt$ the optimal revenue among all BIC and IR mechanisms.
Throughout this paper, the two classes of simple mechanisms we focus on are \emph{rationed posted price} (RPP) mechanisms and \emph{two-part tariff} (TPT) mechanisms, which are both described in \Cref{sec:intro}. We denote $\prev$ the optimum revenue achievable among all RPP mechanisms.  
\notshow{

Relevant to our work is to measure the bit complexity of the problems that we are facing.
In the following definitions we show how we measure the bit complexity of the problem when the bidder's type are Constraint Additive or XOS.
\begin{definition}[Bit Complexity of Instance]
Given a product distribution $D=\prod_{i\in[n]}$ over types for constraint additive or XOS valuation and let $T=\sum_{i\in[n]}\sum_{j\in[m]}\sum_{t_{ij}\in\cT_{ij}}|\cT_{ij}|$.
\begin{itemize}
\item Denote as $b_f$ the bit complexity of elements in $\{f_{ij}(t_{ij})\}_{i\in[n],j\in[m],t_{ij}\in\cT_{ij}}$.
\item If the valuations of the bidders are constraint additive, denote as $b_v$ the bit complexity of elements in $\{t_{ij}\}_{i\in[n],j\in[m],t_{ij}\in\cT_{ij}}$.
\item If the valuations of the bidders are XOS, denote as $b_v$ the bit complexity of elements in $\{\alpha^{(k)}_{ij}\}_{i\in[n],j\in[m],k\in[K],t_{ij}\in\cT_{ij}}$.
\end{itemize}
We refer to the value $\max(b_l,b_f)$ as the bit complexity of the instance.
\end{definition}}
\vspace{-.15in}
\paragraph{Access to the Bidders' Valuations.} We define several ways to access a bidder's valuation. 
\begin{definition}[Value and Demand Oracle]\label{def:value and demand oracle}
A \emph{value oracle} for a valuation $v(\cdot,\cdot)$ takes a type $t$ and a set of items $S\subseteq[m]$ as input, and returns the bidder's value $v(t,S)$ for the bundle $S$. A \emph{demand oracle} for a valuation $v(\cdot,\cdot)$ takes a type $t
$ and a  collection of non-negative prices $\{p_j\}_{j\in[m]}$ as input, and returns a utility-maximizing bundle, i.e. $S^*\in \arg\max_{S\subseteq [m]} \left(v(t,S) - \sum_{j\in S}p_j\right)$. In this paper, we use $\dem_i(\cdot,\cdot)$ to denote the demand oracle for bidder $i$'s valuation  $v_i(\cdot,\cdot)$.
\end{definition}
For constrained-additive valuations, our result only requires query access to a value oracle and a \emph{demand oracle} for every bidder $i$'s valuation $v_i(\cdot,\cdot)$. For XOS valuations, we need a stronger demand oracle that allows ``scaled types'' as input. We refer to the stronger oracle as the \emph{adjustable demand oracle}. 

\begin{definition}[Adjustable Demand Oracle]\label{def:adjustable demand oracle}
An \emph{adjustable demand oracle} for an XOS valuation $v(\cdot,\cdot)$
takes a type $t$, a collection of non-negative coefficients  $\{b_j\}_{j\in[m]}$, and a collection of non-negative prices $\{p_j\}_{j\in[m]}$ as input. For every item $j$, $b_j$ is a scaling factor for $t_{ij}$, meaning that each of the $K$ numbers $\{\alpha_{ij}^{(k)}(t_{ij})\}_{k\in[K]}$, i.e. the contribution of item $j$ under each additive function, is multiplied by $b_j$. The oracle outputs a favorite bundle $S^*$ with respect to the adjusted contributions and the prices $\{p_j\}_{j\in[m]}$, as well as the additive function $\{\alpha_{ij}^{(k^*)}(t_{ij})\}_{j\in [m]}$ for some $k^*\in [K]$ that achieves the highest value on $S^*$. %\argyrisnote{Argyris: Maybe change the previous sentence to: as well as the coefficients of the additive function $\{\alpha_{ij}^{(k^*)}(t_{ij})\}$, where $k^*\in [K]$  that achieves this value for $S^*$.} 
Formally, 
%and outputs a subset of items $S^*\subseteq[m] $ and $k^*\in[K]$ such that .
$
(S^*,k^*) \in \argmax_{S\subseteq [m],k\in[K]} \left\{\sum_{j\in S}b_j \alpha_{ij}^{(k)}(t_{ij}) - \sum_{j\in S}p_j\right\}.
$
%\argyrisnote{Argyris: Maybe we change it to:
%$$
%(S^*,\{\alpha_{ij}^{(k^*)}(t_{ij})\}_{j\in S^*}) \in \argmax_{S\subseteq [m],k\in[K]} \left\{\sum_{j\in S}b_j \alpha_{ij}^{(k)}(t_{ij}) - \sum_{j\in S}p_j\right\}.
%$$
%}
We use  $\adem_i(\cdot,\cdot,\cdot)$ to denote the adjustable demand oracle for bidder $i$'s XOS valuation $v_i(\cdot,\cdot)$.
\end{definition}

%\todo[inline]{Add discussion about adjustable demand oracles}
\vspace{-.05in}
The adjustable demand oracle can be viewed as a generalization of the demand oracle for XOS valuations. In the above definition, if every coefficient $b_j$ is 1, then the adjustable demand oracle outputs the utility-maximizing bundle $S^*$ (as in the demand oracle) and the additive function that achieves the value for this set. For general $b_j$'s, the oracle accommodates a different coefficient across items, which is multiplied with all bidders' contribution for this item. The output bundle $S^*$ maximizes the adjusted utility.\footnote{ {Note that for every collection of scaling factors, the query to the adjusted demand oracle is simply a demand query for a different XOS valuation. If all additive functions of $t_i$ are explicitly given, then the adjusted demand oracle can be simulated in~time~$O(mK)$.}}

\vspace{-.05in}
\begin{definition}[Bit Complexity of an Instance]\label{def:bit complexity}
%Given a product distribution $D=\prod_{i\in[n]}$ over types for constrained-additive or XOS valuation and let $T=\sum_{i\in[n]}\sum_{j\in[m]}\sum_{t_{ij}\in\cT_{ij}}|\cT_{ij}|$.
Given any instance of our problem represented as the tuple $(\cT,D,v=\{v_i(\cdot,\cdot)\}_{i\in [n]})$,  
%\begin{itemize}
%\item 
Denote as $b_f$ the bit complexity of elements in $\{f_{ij}(t_{ij})\}_{i\in[n],j\in[m],t_{ij}\in\cT_{ij}}$.
%\item 
For constrained-additive valuations, denote as $b_v$ the bit complexity of elements in $\{t_{ij}\}_{i\in[n],j\in[m],t_{ij}\in\cT_{ij}}$. For XOS valuations, denote as $b_v$ the bit complexity of elements in $\{\alpha^{(k)}_{ij}(t_{ij})\}_{i\in[n],j\in[m],t_{ij}\in\cT_{ij}, k\in[K]}$.
%\end{itemize}
We define the value $\max(b_v,b_f)$ to be the bit complexity of the instance.
\end{definition}


%%%%%%END of this section %%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\notshow{
\begin{definition}[\todo{Is demand oracle folklore?} Demand Oracle for Constraint Additive Valuation $v_i(\cdot,\cdot)$]
Consider a set of non-negative prices $\{p_j\}_{j\in[m]}$ and a type $t_i\in \cT_i$ for bidder $i$,
a demand oracle $\dem(\cdot,\cdot)$ for a constraint additive valuation $v_i(\cdot,\cdot)$,
takes an input the bidder's type, the price vector and returns the utility maximizing bundle.
More formally, $\dem(t_i,\{p_j\}_{j\in[m]})$ outputs an a subset $S\subseteq [m] $ such that
$$
S\in \arg\max_{S\subseteq [m]} v_i(t_i,S) - \sum_{j\in S}p_j
$$
\end{definition}

However,
when we try to compute a simple mechanism for bidders with XOS valuations,
we will need to have access to a demand oracle that can alter the weight that the agent can have for different items.
We call this oracle the adjustable demand oracle and it is defined below.
}
















\notshow{

\section{XOS Valuation}

\begin{definition}
Let $\DD_i$ be a product distribution over types of the $i$-th agent over $m$ heterogeneous items.
We denote by $T_i$ the support of $\DD_i$. The valuation of the bidder for the items is XOS.
We consider only anonymous posted price mechanisms with entry fee.


For each bidder,
we assume access to a demand oracle $\dem_i(\cdot,\cdot): T \times \R^m\rightarrow \mathbb{R}$,
that is, for a type $t \in T$ and a set of prices the item $\{p_j\}_{j \in[m]}$,
$\dem_i(t,\{p_j\}_{j\in[m]})$ is the maximum utility of the $i$-th agent with realized type $t$ that she can get under those prices.
%Moreover, for each bidder we assume access to a value oracle
%we denote by $\val(\DD)$ the expected value that the agent has for the whole bundle.
Moreover we assume sample access to the agents distribution. \argyrisnote{I think it would be usefull to specify the model we are working on.
I don't think we lose anything by considering sample access to the distribution.}
\yangnote{Yang: We don't have multiplicative approximation if we assume only sample access. I will suggest work with the explicit model first, then in the end have a section discuss how our results can be used to derive results under the sample accesss model.}
\end{definition}


Let $\M(\{\sigma_{i,S}(\cdot)\}_{i\in[n], S \subseteq 2^{[m]}})$ be any BIC mechanism,
where by $\sigma_{i,S}(t_i)$ is the probability that the $i$-th agent with type $t_i \in T_i$ receives exactly bundle $S$.
Let $\epsilon = \sup_{\substack{i\in[n],j\in[m]\\t_{i,j} \in T_{i,j}}}f_i(t_{i,j})$.
Note that given supports $\{T_{i,j}\}_{i\in[n],j\in[m]}$ such that $\epsilon = \sup_{\substack{i\in[n],j\in[m]\\t_{i,j} \in T_{i,j}}}f_i(t_{i,j})$,
we can construct $\{T'_{i,j}\}_{i\in[n],j\in[m]}$ such that $\epsilon' = \sup_{\substack{i\in[n],j\in[m]\\t_{i,j} \in T'_{i,j}}}f_i(t_{i,j})$ and $|T'_{i,j}| \leq \left\lceil\frac{\epsilon}{\epsilon'}\right\rceil|T_{i,j}|$ by subdividing each $t_{i,j}\in T_{i,j}$ to $\{t_{i,j}^{(i)}\}_{i \in \left[\left\lceil\frac{\epsilon}{\epsilon'}\right\rceil\right]}\subseteq T_{i,j}'$. \yangnote{Yang: Could you make the notation consistent? Sometimes it's $T_{i,j}$ and sometimes it's $\cT_{ij}$. Also, what does $t_{i,j}^{(i)}$ mean?}
%We only consider mechanisms such that each item is allocated with probability at most $\frac{1}{2}$. 
%Note that the optimal revenue among the mechanisms that we consider is at least half the optimal revenue when we place no restriction on the probability that an item is allocated.


%\argyrisnote{Variables: $\pi_{i,j}(t_{i,j})$, $\delta_i$, $\lambda_{i,j}(1,t_{i,j},\beta),\lambda_{i,j}(0,t_{i,j},\beta)$.}

%\argyrisnote{$\lambda_{i,j}(1,t_{i,j},\beta)$: Prob. of allocating item $j$ and choosing the threshold $\beta$, when the bidder reports $t_{ij}$.}

%\argyrisnote{The following LP is before taking the convex hull. We want to take the convex hull for every $i,j,t_{i,j}$ and $\beta$.}

%\argyrisnote

Let $W_{i}$ be the polytope of feasible welfares normalised to $[0,1]$ for the $i$-th agent.
That is,
there exists an allocation $\pi_i$, such that $w_{i,j}(t_{i,j})V_{i,j}(t_{i,j}) = \sum_{\substack{t_i'\in T_i \\t_{i,j}' = t_{i,j}}} f_i(t_{i,-j})\pi_{i}(t_{i},S)p_i(t_i, S,j)$,
where $p_i(t_i,S,j)$ is the supporting price for item $j$, when the $i$-th agent has type $t_i$ and receives set $S$. \yangnote{Yang: the definition of $W_i$ is different from later sections.}
%Let $W_i$ be a mixture of polytopes $\{W_{t}\}_{ t \in T}$ with distribution $\{f(t)\}_{t \in T}$.

}

==> program.tex <==
\section{XOS Valuation}

\begin{definition}
Let $\DD_i$ be a product distribution over types of the $i$-th agent over $m$ heterogeneous items.
We denote by $T_i$ the support of $\DD_i$. The valuation of the buyer for the items is XOS.
We consider only anonymous posted price mechanisms with entry fee.


For each buyer,
we assume access to a demand oracle $\dem_i(\cdot,\cdot): T \times \R^m\rightarrow \mathbb{R}$,
that is, for a type $t \in T$ and a set of prices the item $\{p_j\}_{j \in[m]}$,
$\dem_i(t,\{p_j\}_{j\in[m]})$ is the maximum utility of the $i$-th agent with realized type $t$ that she can get under those prices.
%Moreover, for each buyer we assume access to a value oracle
%we denote by $\val(\DD)$ the expected value that the agent has for the whole bundle.
Moreover we assume sample access to the agents distribution. \argyrisnote{I think it would be usefull to specify the model we are working on.
I don't think we lose anything by considering sample access to the distribution.}
\end{definition}


Let $\M(\{\sigma_{i,S}(\cdot)\}_{i\in[n], S \subseteq 2^{[m]}})$ be any BIC mechanism,
where by $\sigma_{i,S}(t_i)$ is the probability that the $i$-th agent with type $t_i \in T_i$ receives exactly bundle $S$.
Let $\epsilon = \sup_{\substack{i\in[n],j\in[m]\\t_{i,j} \in T_{i,j}}}f_i(t_{i,j})$.
Note that given supports $\{T_{i,j}\}_{i\in[n],j\in[m]}$ such that $\epsilon = \sup_{\substack{i\in[n],j\in[m]\\t_{i,j} \in T_{i,j}}}f_i(t_{i,j})$,
we can construct $\{T'_{i,j}\}_{i\in[n],j\in[m]}$ such that $\epsilon' = \sup_{\substack{i\in[n],j\in[m]\\t_{i,j} \in T'_{i,j}}}f_i(t_{i,j})$ and $|T'_{i,j}| \leq \left\lceil\frac{\epsilon}{\epsilon'}\right\rceil|T_{i,j}|$ by subdividing each $t_{i,j}\in T_{i,j}$ to $\{t_{i,j}^{(i)}\}_{i \in \left[\left\lceil\frac{\epsilon}{\epsilon'}\right\rceil\right]}\subseteq T_{i,j}'$.
%We only consider mechanisms such that each item is allocated with probability at most $\frac{1}{2}$. 
%Note that the optimal revenue among the mechanisms that we consider is at least half the optimal revenue when we place no restriction on the probability that an item is allocated.


%\argyrisnote{Variables: $\pi_{i,j}(t_{i,j})$, $\delta_i$, $\lambda_{i,j}(1,t_{i,j},\beta),\lambda_{i,j}(0,t_{i,j},\beta)$.}

%\argyrisnote{$\lambda_{i,j}(1,t_{i,j},\beta)$: Prob. of allocating item $j$ and choosing the threshold $\beta$, when the buyer reports $t_{ij}$.}

%\argyrisnote{The following LP is before taking the convex hull. We want to take the convex hull for every $i,j,t_{i,j}$ and $\beta$.}

%\argyrisnote

Let $W_{i}$ be the polytope of feasible welfares normalised to $[0,1]$ for the $i$-th agent.
That is,
there exists an allocation $\pi_i$, such that $w_{i,j}(t_{i,j})V_{i,j}(t_{i,j}) = \sum_{\substack{t_i'\in T_i \\t_{i,j}' = t_{i,j}}} f_i(t_{i,-j})\pi_{i}(t_{i},S)p_i(t_i, S,j)$,
where $p_i(t_i,S,j)$ is the supporting price for item $j$, when the $i$-th agent has type $t_i$ and receives set $S$.
%Let $W_i$ be a mixture of polytopes $\{W_{t}\}_{ t \in T}$ with distribution $\{f(t)\}_{t \in T}$.


\section{Main Program}
%\argyrisnote{Do we agree that the first among the two programs is the one we are going to focus on?}

The variables in the LP are as follows:
\begin{enumerate}
    \item $\pi_{ij}(t_{ij})$, for all $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We denote $\pi_i=(\pi_{ij}(t_{ij}))_{j,t_{ij}}$ the vector of all variables associated with buyer $i$.
    \item $w_{ij}(t_{ij})$, for all $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We denote $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}}$ the vector of all variables associated with buyer $i$.
    \item $\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij}),\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})$, for all $i,j$ and $t_{ij}\in \cT_{ij}$, $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta_i$.
    \item $\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij}), \hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$, for all $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta_i$, %denoting the joint distribution over $\cV_{ij}\times \Delta_i$.
    \item $d_i$, for all $i\in [n]$.
\end{enumerate} \todo{To add some explanation of the variables.} In the LP, we will abuse the notations and let $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})+\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})$, $\lambda_{ij}(t_{ij},\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$. Similarly, let $\hat\lambda_{ij}(\beta_{ij},\delta_{ij})=\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})+\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}^{(r)}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}(\beta_{ij},\delta_{ij})$. 

%Let $W_{i}$ be the polytope of feasible normalized welfare for buyer $i$.
%That is, $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}}$ is in $W_i$ if and only if there exists an allocation (for buyer $i$) $\{\sigma_{iS}(\cdot)\}_{S\subseteq [m]}$, such that $$w_{ij}(t_{ij})\cdot V_{ij}(t_{ij}) = \sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\sigma_{iS}(t_{ij},t_{i,-j})\cdot\gamma_{ij}^{S}(t_i),$$
%where $\gamma_{ij}^{S}(t_i)$ is buyer $i$'s supporting price for item $j$ with respect to set $S$. \todo{Add a definition $\gamma_{ij}^S(t_i)=\alpha_{ij}^{k(t_i,S)}$.}
%\mingfeinote{Add definition of ``supporting price''. Should be $\alpha_j^k$ instead.} \argyrisnote{I think it should be $\alpha_j^k$ instead.}


\argyrisnote{
LP, we will abuse the notations and let  $\lambda_{ij}(t_{ij},\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$. Similarly, let $\hat\lambda_{ij}(\beta_{ij},\delta_{ij})=\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})+\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}^{(r)}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}(\beta_{ij},\delta_{ij})$. 

\begin{align*}
    (P)
    &\quad\text{maximize  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \\
    &\sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} \lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})\leq \beta_{ij} + \delta_{ij}]\\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    s.t.\quad & (1)\quad (\pi_i,w_i) \in W_i & \forall i \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    & (2)\quad f_{ij}(t_{ij})\cdot\sum_{\beta_{ij}\in \cV_{ij}} \lambda_{ij}(t_{ij},\beta_{ij}) = w_{ij}(t_{ij}) & \forall i,j,t_{ij}\in \cT_{ij}\\
    &(3) \quad \sum_i\sum_{t_{ij}\in \cT_{ij}}\pi_{ij}(t_{ij})\leq 1 & \forall j\\
    &(4) \quad \sum_{i\in[n]}\sum_{\beta_{ij} \in \cV_{ij}} \hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})> \beta_{ij}] & \forall j\\
    &\qquad\qquad\qquad\qquad\quad +\hat\lambda_{ij}^{(r)}(\beta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})=\beta_{ij}] \leq \frac{1}{2}\\
    & (5)\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \lambda_{ij}(t_{ij},\beta_{ij}) \leq  \hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})> \beta_{ij}] & \forall i,j,\beta_{ij}\in \cV_{ij}\\
    &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad+\hat\lambda_{ij}^{(r)}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\beta_{ij}]\\
    & (6)\quad\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}(\beta_{ij}, \delta_{ij}) & \forall i,j, t_{ij},\beta_{ij},\delta_{ij}\\
    %& \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) &\forall i\in[n], j \in[m] \\
    & (7)\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\ \delta_{ij} \in \Delta_i}} \delta_{ij}\cdot \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \leq d_i  & \forall i,j\\
    & (8)\quad\sum_{i\in[n]} d_i \leq 8\cdot \prev \text{\todo{Change the constant if needed.}}\\
    &(9)\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) = 1 & \forall i,j\\
     & w_{ij}(t_{ij})\geq 0,\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})\geq 0 & \forall i,j,t_{ij},\beta_{ij},\delta_{ij}
\end{align*}
}
\argyrisnote{I guess we define as $\Delta_i$ to be the geometric discretization of $[\frac{\prev}{n},\prev]$? I think we should drop the subscript $i$ then and replace constraint (7) with $16\prev$?}

Let $\optlp$ be the maximum objective of $(P)$. 


\notshow{
\begin{align*}
    (P) = 
    \max& \frac{1}{2} \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{i,j}\in T_{i,j}}  f_{i,j}(t_{i,j})\cdot V_{i,j}(t_{i,j})\cdot
    \\
    &\quad \quad\sum_{\substack{\beta\in V_{i,j}(T_{i,j})\\\delta \in \Delta V_{i}}} \lambda_{i,j}(t_{i,j},\beta, \delta)\cdot \mathds{1}[V_{i,j}(t_{i,j}) \leq \beta + \delta]\\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    s.t.\quad & w_i \in W_i  \text{\argyrisnote{ I think we only need this since always $w_{i,j}(t_{i,j}) \leq \pi_{i,j}(t_{i,j})$?}} & \forall i \in[n] \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    & \sum_{\beta\in V_{i,j}(T_{i,j})} \lambda_{i,j}(t_{i,j},\beta) = w_{i,j}(t_{i,j}) & \forall i\in[n],j\in[m],t_{i,j}\in T_{i,j}\\
    &\sum_{i\in[n]}\sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta) \cdot \Pr_{t\sim D_{i,j}}[t \geq \beta] \leq \frac{1}{2} + n\cdot \epsilon & \forall j \in[m] \\
    %& \sum_{i\in[n]}\sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})\cdot \pi_{i,j}(t_{i,j}) \leq 1, & \forall j \in[m] \\
    &\frac{1}{2} \sum_{t_{i,j} \in T_{i,j}} f_{i,j}(t_{i,j}) \lambda_{i,j}(t_{i,j},\beta) \leq  \lambda'_{i,j}(\beta) \left(\Pr_{t_{i,j}\sim D_{i,j}}[t_{i,j} \geq \beta] + \epsilon_{i,j,\beta} \right) & \forall i\in[n],j\in[m], \beta \in V_{i,j}(T_{i,j})\\
    &\sum_{\beta \in V_{i,j(T_{i,j}})} \epsilon_{i,j,\beta}\leq \epsilon
    & \forall i\in[n],j\in[m]\\
    & \lambda_{i,j}(t_{i,j},\beta, \delta) \leq \lambda_{i,j}'(\beta, \delta) & \forall i\in[n], j \in[m], t_{i,j} \in T_{i,j}\\ 
    & \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) &\forall i\in[n], j \in[m] \\
    & \sum_{\delta \in \Delta V_i} \delta \lambda_{i}'(\delta) \leq \delta_i  & \forall i \in [n]\\
    & \sum_{i\in[n]} \delta_i \leq O(1) \cdot \srev \\
     & \forall i \in[n],j\in [m],t\in T_{i,j},\beta,\gamma \in V_{i,j}(t_{i,j})\\
\end{align*}

}

\begin{lemma}\cite{CaiZ17}\label{lem:caiz17}
Given any BIC, IR mechanism $\cM$, there exist non-negative numbers $\{\tilde{\beta}_{ij}\}_{i,j}, \{c_i\}_{i\in[n]}$ and $r\in [0,1]$ such that
\begin{enumerate}
    \item $\sum_i \left(\Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde\beta_{ij}]+r\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde\beta_{ij}]\right)\leq \frac{1}{2}$.
    \item $\frac{1}{2}\cdot\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\sigma_{iS}(t_i)= \Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde\beta_{ij}]+r\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde\beta_{ij}]$.
    \item $\rev(\cM)\leq 28\cdot \prev+4\cdot\core(\cM,\tilde{\beta},\vec{c})$.
    \item $\core(\cM,\tilde{\beta},\vec{c})\leq 64\cdot \prev + 8\cdot \aperev$.
    \item $\sum_ic_i\leq 8\cdot \prev$.
\end{enumerate}

Here $\sigma_{iS}(t_i)$ is the ex-ante probability for buyer $i$ obtaining exactly set $S$ in $\cM$, when her type is $t_i$. $\core(\cM,\tilde{\beta},\vec{c})$ is the welfare of $\cM$ truncated at $\tilde{\beta}_{ij}+c_i$ for every $i,j$, with rebate ratio $r$ (see the remark below). Formally, $$\core(\cM,\tilde{\beta},\vec{c})=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}\gamma_{ij}^S(t_i)\cdot \left(\ind[V_{ij}(t_{ij})< \tilde{\beta_{ij}}+c_i]+r\cdot \ind[V_{ij}(t_{ij})= \tilde{\beta_{ij}}+c_i] \right)$$
\end{lemma}
\argyrisnote{I think the first two constraints are not immediately implied by the paper, but they are implied by the proof of Lemma~5 in \cite{CaiZ17}. Could this be an issue? I also think that $\sum_i c_i$ could be $8\prev + \epsilon$ since rebate might also be used there, so maybe we can relax (5) to $\sum_i c_i < 9 \prev$? I also think if we change the notation of $W_i$ to be the one with the $\alpha_j^k$, we might also need to include information about them.}

%\mingfeinote{See if you think the following remark is enough. To make the notation consistent, we can add a line say $\gamma_{ij}^S(t_i)=\alpha_{ij}^{k(t_i,S)}$.}

Remark: \mingfeinote{A remark about the rebate ratio r.}

We will show in the following lemma that the tuple $(\cM,\{\tilde{\beta}_{ij}\}_{i,j}, \{c_i\}_{i\in[n]})$ stated in \Cref{lem:caiz17} corresponds to a feasible solution whose objective equals to $\core(\cM,\tilde{\beta},\vec{c})$. 

\begin{lemma}\label{lem:bound rev by opt}
For any BIC, IR mechanism $M$, $\rev(M)\leq 28\cdot \prev+4\cdot\optlp$.
\end{lemma}
\begin{proof}
For every $i,t_i,S$, let $\hat\sigma_{iS}(t_i)$ be the ex-ante probability for buyer $i$ obtaining exactly set $S$ in $\cM$, when her type is $t_i$. Consider the following choice of variables of $(P)$ from the tuple $(\cM,\{\tilde{\beta}_{ij}\}_{i,j}, \{c_i\}_{i\in[n]})$ stated in \Cref{lem:caiz17}. For every $i,j,t_{ij}$, let $$\pi_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{iS}(t_{ij},t_{i,-j})$$
$$w_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{iS}(t_{ij},t_{i,-j})\cdot\frac{\gamma_{ij}^{S}(t_i)}{V_{ij}(t_{ij})}.$$ 
\argyrisnote{Should we say something about $\gamma_{ij}^S(\cdot)$? Like that they are $1$-supporting prices? fix: where $\gamma_{ij}^S(t_i)$ is equal to $\alpha_{ij}^{k(t_i,S)}(t_{ij})$, where $k(t_i,S)=\arg\max_{k\in[K]}\left(\sum_{j\in S}\alpha^k_{ij}(t_{ij}) \right)$.}
All of $\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij}), \lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})$ and $\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$ will be non-zero only if $\beta_{ij}=\tilde{\beta}_{ij}$ and $\delta_{ij}=c_i$. Moreover, $\lambda_{ij}^{(r)}(t_{ij},\tilde{\beta}_{ij},c_i)=r\cdot w_{ij}(t_{ij})/f_{ij}(t_{ij})$; $\lambda_{ij}^{(n)}(t_{ij},\tilde{\beta}_{ij},c_i)=(1-r)\cdot w_{ij}(t_{ij})/f_{ij}(t_{ij})$; $\hat\lambda_{ij}^{(r)}(\tilde{\beta}_{ij},c_i)=r$; $\hat\lambda_{ij}^{(n)}(\tilde{\beta}_{ij},c_i)=1-r$; $d_i=c_i$.
%\argyrisnote{Shouldn't it be $\lambda_{ij}^{(r)}(t_{ij},\tilde{\beta}_{ij},c_i)=r\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}$ and; $\lambda_{ij}^{(n)}(t_{ij},\tilde{\beta}_{ij},c_i)=(1-r)\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}$ and 
\argyrisnote{whether or not $d_i=c_i$ depends on the discretization we choose, right?}

We show that this is indeed a feasible solution of $(P)$ by verifying each constraint. 
%(1) comes directly from the definition of the polytope $W_i$; 
We first prove that $(\pi_i,w_i)\in W_i$ for every $i$. For every $t_i$, consider the mapping $\sigma_{iS}^{(k)}(t_i)=\hat\sigma_{iS}(t_i)\cdot \ind[k=\argmax_{k'\in [K]}\sum_{j\in S}\alpha_{ij}^{(k')}(t_{ij})]$ (we break ties arbitrarily). Thus by the definition of $\gamma_{ij}^S$, we have $\hat\sigma_{iS}(t_i)\cdot \gamma_{ij}^S(t_i)=\sum_{k}\sigma_{iS}^{(k)}(t_i)\cdot \alpha_{ij}^{(k)}(t_i)$. Then clearly $(\pi_i,w_i)$ satisfies all of the conditions in \Cref{def:W_i}.

For (2), LHS equals to $f_{ij}(t_{ij})(\lambda_{ij}^{(r)}(t_{ij},\tilde{\beta}_{ij},c_i)+\lambda_{ij}^{(n)}(t_{ij},\tilde{\beta}_{ij},c_i))=w_{ij}(t_{ij})$; (3) follows from the fact that in $\cM$, each item $j$ can be allocated to at most one buyer for every type profile. Thus
$$\sum_i\sum_{t_{ij}}\pi_{ij}(t_{ij})=\sum_i\sum_{t_i}f_i(t_i)\sum_{S:j\in S}\hat\sigma_{iS}(t_i)\leq 1$$
(4) comes from property 1 of \Cref{lem:caiz17}. For (5), we only have to verify the constraint for $\beta_{ij}=\tilde{\beta}_{ij}$. LHS equals to $\frac{1}{2}\sum_{t_{ij}}w_{ij}(t_{ij})$. %\argyrisnote{Isn't it equal to $\frac{1}{2}\sum_{t_{ij}} w_{ij}(t_{ij})$}. 
We notice that $\gamma_{ij}^S(t_i)\leq V_{ij}(t_{ij})$ for all $i,j,S$. Thus  
$$\sum_{t_{ij}}w_{ij}(t_{ij})\leq \sum_{t_{ij}}f_{ij}(t_{ij})\cdot \sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\hat\sigma_{iS}(t_{ij},t_{i,-j})=\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\hat\sigma_{iS}(t_i)$$

Since $r\in [0,1]$, by property 2 of \Cref{lem:caiz17}, we have

$$LHS\leq \frac{1}{2}\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\hat\sigma_{iS}(t_i)=\Pr_{t_{ij}}[V_{ij}(t_{ij})>\tilde{\beta}_{ij}]+r\cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\tilde{\beta}_{ij}]$$

For (6), since $\gamma_{ij}^S(t_i)\leq V_{ij}(t_{ij})$ for all $i,j,S$ and $\sum_{S\in [m]}\hat\sigma_{iS}(t_i)\leq 1$, we have $w_{ij}(t_{ij})\leq f_{ij}(t_{ij})$. Thus 
$$\lambda_{ij}^{(r)}(t_{ij},\tilde{\beta}_{ij},c_i)=r\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}\leq r= \hat\lambda_{ij}^{(r)}(\tilde{\beta}_{ij},c_i).$$ 
%\argyrisnote{Maybe change it to:
%For (6), since $w_{ij}(t_i)\leq f_{ij}(t_{ij})$ for all $i,j,S$, we have  
%$$\lambda_{ij}^{(r)}(t_{ij},\tilde{\beta}_{ij},c_i)=r\cdot \frac{w_{ij}(t_{ij})}{f_{ij}(t_{ij})}\leq r= \hat\lambda_{ij}^{(r)}(\tilde{\beta}_{ij},c_i).$$ }
Similarly $\lambda_{ij}^{(n)}(t_{ij},\tilde{\beta}_{ij},c_i)\leq 1-r=\hat\lambda_{ij}^{(n)}(\tilde{\beta}_{ij},c_i)$. (7) and (9) are straightforward since $\hat\lambda_{ij}(\beta_{ij},\delta_i)=\ind[\beta_{ij}=\tilde{\beta}_{ij}\wedge \delta_{ij}=c_i]$. And last, (8) comes from property 5 of \Cref{lem:caiz17}. Thus the solution is feasible. We are left to show that the objective of the above solution equals to $\core(\cM,\tilde{\beta},\vec{c})$. In fact, by the definition of $w_{ij}(t_{ij})$,   

$$\core(\cM,\tilde{\beta},\vec{c})=\sum_i\sum_j\sum_{t_{ij}}f_{ij}(t_{ij})\cdot w_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot \left(\ind[V_{ij}(t_{ij})< \tilde{\beta_{ij}}+c_i]+r\cdot \ind[V_{ij}(t_{ij})= \tilde{\beta_{ij}}+c_i] \right)$$ 
%\argyrisnote{I think also $c_i$ might have a rebate? In that case the definition of core might change? I think everything is fine if we double the value of $c_i$. I also think that this is not due to property 3 of \Cref{lem:caiz17}.}

This is exactly the objective of $(P)$ since $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=w_{ij}(t_{ij})\cdot \ind[\beta_{ij}=\tilde{\beta}_{ij}\wedge \delta_{ij}=c_i]$ and $\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})=r\cdot w_{ij}(t_{ij})\cdot \ind[\beta_{ij}=\tilde{\beta}_{ij}\wedge \delta_{ij}=c_i]$. The proof is done according to property 3 of \Cref{lem:caiz17}. 
\end{proof}

%\argyrisnote{Note about the above lemma: Maybe we need to rebate when using the $c_i$, I think we can avoid that in the LP by relaxing the (5) constraint to be $\sum_i c_i \leq 16 \prev$? I also think we need to rethink the the argument in the proof that uses the definition of polytope $W_i$.}



Now we will connect the objective of $(P)$ to the revenue of simple mechanisms. In \cite{CaiZ17}, they proved that for any BIC and IR mechanism $\cM$, $\core(\cM,\tilde\beta,\vec{c})$ can be bounded by a constant number of $\prev$ and $\aperev$ (see property 4 of \Cref{lem:caiz17}). In our paper, we generalize their result, proving that for any feasible solution of $(P)$, its objective can be bounded by the revenue of simple mechanisms. And moreover, the mechanism can be computed efficiently. 

Let $(w,\lambda^{(r)},\lambda^{(n)},\hat\lambda^{(r)},\hat\lambda^{(n)}, d=(d_i)_{i\in [n]})$ be any fixed feasible solution of $(P)$. We need the following definition.

\begin{definition}\label{def:Q_j}
%Given an optimal solution %$\{\lambda_{i,j}(\beta)\}_{\beta \in V_{i,j}(T_{i,j})}$,
%of the program above,
Let $(w,\lambda^{(r)},\lambda^{(n)},\hat\lambda^{(r)},\hat\lambda^{(n)}, d=(d_i)_{i\in [n]})$ be any feasible solution of $(P)$. 
For any $i,j,\beta_{ij}\in \cV_{ij},\delta_{ij}\in \Delta_i$, define

$$g_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})<\beta_{ij} + \delta_{ij}]+\lambda_{ij}^{(r)}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})=\beta_{ij} + \delta_{ij}]$$

%We denote by $B_{i,j} \times \Delta_{i,j}$ a coupled distribution over $V_{i,j}(T_{i,j}) \times \Delta_{i}$ such that: $\Pr_{(\beta,\delta) \sim B_{i,j} \times \Delta_{i,j}}[\beta = a \land \delta = b]= \lambda'_{i,j}(\beta_{i,j}=a, \delta_{i,j} = b)$.
For every $j\in [m]$, define 
$$Q_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}}g_{ij}(t_{ij},\beta_{ij},\delta_{ij})
$$
\end{definition}

With the above definition, the objective function of $(P)$ can also be written as $2\cdot \sum_{j}Q_j$.

\begin{theorem}\label{thm:bounding-lp-simple-mech}
Let $(w,\lambda^{(r)},\lambda^{(n)},\hat\lambda^{(r)},\hat\lambda^{(n)}, d=(d_i)_{i\in [n]})$ be any feasible solution of $(P)$. Then its objective $2\cdot \sum_{j\in [m]}Q_j$ is bounded by $O(1)\cdot \rev(\cM_1)+O(1)\cdot \rev(\cM_2)$ \mingfeinote{Add the constant}, for some \mingfeinote{restricted SPM} $\cM_1$ and some \mingfeinote{SPEM} $\cM_2$. Moreover, both $\cM_1$ and $\cM_2$ can be computed in time\mingfeinote{Add time and query complexity}.
\end{theorem}
\argyrisnote{We can bound any SPEM mechanism by $\prev$, since its just a BIC mechanism designed for UD buyers?}


The rest of this section is dedicated to the proof of \Cref{thm:bounding-lp-simple-mech}. By constraint (9), for every $i,j$, $\hat\lambda_{ij}(\cdot,\cdot)$ can be viewed as a joint distribution $\cC_{ij}$ over $\cV_{ij}\times \Delta_{i}$, i.e. $\Pr_{(\beta_{ij},\delta_{ij}) \sim \cC_{ij}}[\beta_{ij} = a \land \delta_{ij} = b]= \hat\lambda_{ij}(\beta_{i,j}=a, \delta_{ij} = b)$. Denote $\cB_{ij}$ the marginal distribution of $\beta_{ij}$ with respect to $\cC_{ij}$. Inspired by the ``shifted core'' technique by Cai and Zhao~\cite{CaiZ17}, we need further definitions that describes the welfare contribution for each item, under a different (randomized) threshold.  

\mingfeinote{Add a discussion to assume that we will work on continuous distributions in the rest of the proof.}
\argyrisnote{Just to see if I understand correctly, you also turn discrete $\beta_{i,j}$ with rebate into a continuous single point $\beta_{i,j}$ without rebate, right? Essentially you are transferring the solution of (P) to a solution of a continuous distribution version of (P)?}

\begin{definition}\label{def:hatQ_j}
For every $i\in [n]$, define %$\tau_i\geq 0$ such that
$$\tau_i = \inf_{x\geq 0}\left\{ \sum_{j\in[m]} \Pr_{t_{ij}\sim \cD_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j + x)]\leq \frac{1}{2}\right\}$$
%$$\sum_{j\in[m]} \Pr_{t_{ij}\sim \cD_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j + \tau_i)]= \frac{1}{2}$$

%\argyrisnote{or maybe we could use the following definition since we are dealing with a discrete distribution (I don't think its nessessary though):}
%$$\tau_i = \inf_{x\in \cup_{j\in[m]} \{V_{i,j}(T_{i,j}\}} \sum_{j\in[m]} \Pr_{t_{i,j}\sim D_{i,j},\beta \sim B_{i,j}}[V_{i,j}(t_{i,j}) \geq \max(\beta, Q_j + x)]\leq \frac{1}{2}$$

Then for every $j\in [m]$, define
$$\hat Q_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}}g_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]$$
\end{definition}

%\argyrisnote{Should't it be $\inf_{\tau\geq 0}\sum_{j\in[m]} \Pr_{t_{ij}\sim \cD_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j + \tau_i)] \leq \frac{1}{2}$? It could be the case that  that $\sum_{j\in[m]} \Pr_{t_{ij}\sim \cD_{ij},\beta_{ij} \sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j)]< \frac{1}{2}$}
%\mingfeinote{I changed the definition.}

We prove in \Cref{lem:Q and Q-hat} that $\sum_j\hat{Q}_j$ are close to $\sum_jQ_j$. Before giving the proof, we first prove a useful lemma that analyzes the revenue of RSPM. It's a generalization of Lemma 17 of \cite{CaiZ17}, which allows randomized posted prices.  

\begin{lemma}\label{lem:prev-useful}\cite{CaiZ17}
%For every $i,j$, let $\cG_{ij}$ be a joint distribution over $\cV_{ij}\times \mathbb{R}_+$, whose marginal distribution on $\beta_{ij}\in \cV_{ij}$ is $\cB_{ij}$. In other words, $\Pr_{(\beta_{ij},x_{ij})\sim \cG_{ij}}[\beta_{ij}=b]=\Pr_{\beta_{ij}\sim \cB_{ij}}[\beta_{ij}=b]$ for every $b\in \cV_{ij}$.
For every $i,j$, let $\cG_{ij}$ be any distribution over $\mathbb{R}_+$. All $\cG_{ij}$s are independent. Suppose both of the following two inequalities are satisfied, for some $a,b\in (0,1)$:
\begin{enumerate}
\item $\sum_{i\in [n]} \Pr_{t_{ij}\sim \cD_{ij},x_{ij}\sim \cG_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\leq a,\forall j\in [m]$.
\item
$\sum_{j\in [m]} \Pr_{t_{ij}\sim \cD_{ij},x_{ij}\sim \cG_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\leq b,\forall i\in [n]$.
\end{enumerate}
Then
\begin{equation*}
\sum_i\sum_j \E_{x_{ij}\sim \cG_{ij}}\left[x_{ij}\cdot \Pr_{t_{ij}\sim \cD_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\right]\leq \frac{1}{(1-a)(1-b)}\cdot \prev.
\end{equation*}
\end{lemma}

\begin{proof}
Consider an RSPM that sells item $j$ to buyer $i$ at price $x_{ij}\sim \cG_{ij}$. The mechanism
visits the buyers in some arbitrary order. For every $i,j$ and every realized $x_{ij}$, we will bound the probability of buyer $i$ purchasing item $j$, over the randomness of $\{\cD_{i',j'}\}_{i',j'}$ and $\{\cG_{i',j'}\}_{(i',j')\neq (i,j)}$. 
Notice that when it is buyer $i$'s turn, she purchases exactly item $j$ and pays $x_{ij}$ if all of the following three conditions hold: (i) $j$ is still available, (ii) $V_i(t_{ij})\geq x_{ij}$ and (iii) $\forall k\neq j, V_i(t_{ik})< x_{ik}$. The second condition means buyer $i$ can afford item $j$. The third condition means she cannot afford any other item $k\neq j$. Therefore, buyer $i$ purchases exactly item $j$.

Now let us compute the probability that all three conditions hold, when $t_{ij}\sim \cD_{ij}$ and $x_{ij}\sim \cG_{ij}$ for all $i,j$. Since every buyer's valuation is subadditive over the items, item $j$ is purchased by someone else only if there exists a buyer $k\neq i$ who has $V_k(t_{kj})\geq x_{kj}$. %Because $x_{kj}\geq 0$ for all $k$, 
By the union bound, the event described above happens with probability at most $\sum_{k\neq i} \Pr_{t_{kj},x_{kj}}\left[V_k(t_{kj})\geq x_{kj}\right]$, which is less than $a$ by Inequality 1 of the statement. Therefore, condition (i) holds with probability at least $1-a$. Clearly, condition (ii) holds with probability $\Pr_{t_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]$. Finally, condition (iii) holds with at least probability $1-b$, because the probability that there exists any item $k\neq j$ such that $V_i(t_{ik})\geq x_{ik}$ is no more than $\sum_{k\neq j}\Pr_{t_{ik},x_{ik}}[V_i(t_{ik})\geq x_{ik}]\leq b$ (Inequality 2 of the statement). Since the three conditions are independent, buyer $i$ purchases exactly item $j$ with probability at least $(1-a)(1-b)\cdot \Pr_{t_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]$. So the expected revenue of this mechanism is at least $(1-a)(1-b)\cdot \E_{x_{ij}\sim \cG_{ij}}\left[x_{ij}\cdot \Pr_{t_{ij}\sim \cD_{ij}}\left[V_i(t_{ij})\geq x_{ij}\right]\right]$.
\end{proof}

A direct corollary of \Cref{lem:prev-useful} is that $\sum_i \tau_i$ can be bounded using $\prev$.

\begin{lemma}\label{lem:bounding tau_i}
$\sum_i \tau_i\leq 8\cdot \prev$.
\end{lemma}
\begin{proof}
By constraint (4) of $(P)$, for every $j$,%\argyrisnote{(4) you mean?} 
$$\sum_{i}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\leq \sum_{i}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij})\geq \beta_{ij}]=\sum_{i}\sum_{\beta_{ij}}\hat\lambda_{ij}(\beta_{ij})\Pr_{t_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}]\leq \frac{1}{2}$$
%\argyrisnote{I think there is one extra ]}


By the definition of $\tau_i$, for every $i$ we have
$$\sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]\leq\frac{1}{2}$$
%\argyrisnote{I think it should be $\leq$? Either $\tau_i=0$ or $\sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]=\frac{1}{2}$, right? So the following statement still holds.}

Thus by \Cref{lem:prev-useful}, 
\begin{align*}
4\cdot \prev\geq& \sum_{i,j} 
\E_{\beta_{ij}\sim\cB_{ij}}\left[\max(\beta_{ij}, Q_j+\tau_i)\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\right]\\
\geq & \sum_{i}\tau_i\sum_j\E_{\beta_{ij}\sim\cB_{ij}}\left[\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\right]\\
=&\frac{1}{2}\sum_i \tau_i,
\end{align*}
{The last equality comes from the fact that by the definition of $\tau_i$, $\sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]=\frac{1}{2}$ for all $i$ such that $\tau_i>0$. We finish the proof.}
\end{proof}

In the following lemma, we prove that the difference between $\sum_j Q_j$ and $\sum_j \hat{Q}_j$ can be bounded using $\prev$ and the revenue of some restricted SPEM that can be efficiently computed.

\begin{lemma}\label{lem:Q and Q-hat}
For every $j\in [m]$, $Q_j\geq \hat{Q}_j$. 
Moreover, there exists a \mingfeinote{restricted SPEM} $\cM$ such that
$$\sum_{j\in [m]}Q_j\leq \sum_{j\in [m]}\hat{Q}_j+44\cdot \prev+8\cdot\rev(\cM).$$
%$\cM$ can be computed in time \mingfeinote{Add time and query complexity}.
%\argyrisnote{Work In Progress}

\mingfeinote{
Moreover,
$$\sum_{j\in [m]}Q_j\leq \sum_{j\in [m]}\hat{Q}_j+256\cdot \prev.$$}
\end{lemma}

\begin{proof}

For every $j$, it's clear that $\hat{Q}_j\leq Q_j$ by the definition of $\hat{Q}_j$. It remains to bound $\sum_j(Q_j-\hat{Q}_j)$. 

\begin{align*}
    &2\sum_{j\in [m]} \left(Q_j - \hat{Q}_j \right) \\
    = & \sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) V_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\
    \delta_{ij} \in \Delta_i}} \lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}] \\
    \leq & \sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\
    \delta_{ij} \in \Delta_i}} \left(\beta_{ij}+(V_{ij}(t_{ij})-\beta_{ij})^+\right)\cdot\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\\
    \leq & \sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\beta_{ij}\in \cV_{ij}} \beta_{ij}\cdot\lambda_{ij}(t_{ij},\beta_{ij})\\
    &+\sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\
    \delta_{ij} \in \Delta_i}} (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\\
\end{align*}

\argyrisnote{In the continuous setting we don't use $g_{ij}(t_{ij},\beta_{ij},\delta_{ij})$, right?}
Here the first equality uses the fact that $g_{ij}(t_{ij},\beta_{ij},\delta_{ij})$ and $g_{ij}(t_{ij},\beta_{ij},\delta_{ij})\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]$ can differ only when $V_{ij}(t_{ij})>Q_j+\tau_i \wedge V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}$. In the last inequality, we drop the indicator $\ind[V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}]$ for the first term and use the fact that $\sum_{\delta_{ij}\in \Delta_i}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\lambda_{ij}(t_{ij},\beta_{ij})$.

We bound the first term:
\begin{equation}\label{inequ:Q and Q_hat-term1}
\begin{aligned}
&\sum_{j} \sum_{i}  \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot \sum_{\beta_{ij}\in \cV_{ij}} \beta_{ij} \cdot \lambda_{ij}(t_{ij},\beta_{ij})\\
%=&\sum_{j\in[m]} \sum_{i\in[n]} 
%\sum_{\beta\in V_{i,j}(T_{i,j}) } %\beta
%\sum_{\substack{t_{i,j}\in T_{i,j}:\\V_{i,j}(t_{i,j}) \geq Q_j^*+\tau_i}}  f_i(t_{i,j})  \cdot \lambda_{i,j}(t_{i,j},\beta)\\
= & \sum_{i,j} \sum_{\beta_{ij}\leq Q_j+\tau_i} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})
+
\sum_{i,j}\sum_{\beta_{ij}> Q_j+\tau_i} \beta_{ij} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})\cdot  \lambda_{ij}(t_{ij},\beta_{ij})\\
\leq &\sum_{i,j}
\sum_{\beta_{ij}\leq Q_j + \tau_i} \hat\lambda_{ij}(\beta_{ij}) \cdot \beta_{ij}
\sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j+\tau_i} f_{ij}(t_{ij})
+ 
\sum_{i,j}
\sum_{\beta_{ij} > Q_j + \tau_i} 
2\hat\lambda_{ij}(\beta_{ij})\cdot\beta_{ij}\cdot\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \beta_{ij}]\\
\leq & 2\sum_{i,j} 
\sum_{\beta_{ij}\in \cV_{ij}} \hat\lambda_{ij}(\beta_{ij}) \cdot \beta_{ij}\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\\
= & 2\sum_{i,j} 
\E_{\beta_{ij}\sim \cB_{ij}}\left[  \beta_{ij}\cdot
\Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]\right]\\
\leq & 8\cdot\prev
\end{aligned}
\end{equation}

Here the first inequality comes from constraint (5) and (6) of $(P)$. For the last inequality, we notice that by constraint (4) of $(P)$, for every $j$, 
$$\sum_{i}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]\leq \sum_{i}\Pr_{\substack{t_{ij}\sim D_{ij}\\\beta_{ij}\sim \cB_{ij}}}[V_{ij}(t_{ij})\geq \beta_{ij}]=\sum_{i}\sum_{\beta_{ij}}\hat\lambda_{ij}(\beta_{ij})\Pr_{t_{ij}}[V_{ij}(t_{ij})\geq \beta_{ij}]\leq \frac{1}{2}$$

By the definition of $\tau_i$, for every $i$ we have
$$\sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]\leq\frac{1}{2}$$

The last inequality then follows from \Cref{lem:prev-useful}. For the second term, we have

\begin{align*}
&\sum_{j} \sum_{i} \sum_{t_{ij}:V_{ij}(t_{ij}) \geq Q_j + \tau_i} f_{ij}(t_{ij}) \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\\
\leq & \sum_{j} \sum_{i} \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} \hat\lambda_{ij}(\beta_{ij}, \delta_{ij})\cdot\sum_{t_{ij}} f_{ij}(t_{ij})  (V_{ij}(t_{ij})-\beta_{ij})\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij} \wedge V_{ij}(t_{ij})\geq \max(\beta_{ij}, Q_j + \tau_i)]\\
= & \sum_{i,j}\E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}}\left[\sum_{t_{ij}}f_{ij}(t_{ij})u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right],
\end{align*}

where
$$u_{ij}(t_{ij},\beta_{ij},\delta_{ij})=(V_{ij}(t_{ij})-\beta_{ij})\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij} \wedge V_{ij}(t_{ij})\geq \max(\beta_{ij}, Q_j + \tau_i)]$$

We notice that by the definition of $\tau_i$,

\begin{equation}\label{inequ:Q and Q_hat-1} 
\sum_j\Pr_{t_{ij}\sim D_{ij},(\beta_{ij},\delta_{ij})\sim \cC_{ij}}[u_{ij}(t_{ij},\beta_{ij},\delta_{ij})>0]\leq \sum_{j}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[V_{ij}(t_{ij}) \geq \max(\beta_{ij}, Q_j+\tau_i)]]\leq\frac{1}{2}    
\end{equation}

Denote $\cC_i=\times_{j=1}^m \cC_{ij}$ and $\beta_{i}=(\beta_{ij})_{j\in [m]}, \delta_{i}=(\delta_{ij})_{j\in [m]}$, we have  
\begin{align*}
    &\sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_{t_i}f_i(t_i)\cdot\max_j u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]\\
\geq & \sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_j\sum_{t_{ij}}f_{ij}(t_{ij})\cdot u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot \prod_{k\not=j}\Pr_{t_{ik}\sim D_{ik}}[u_{ik}(t_{ik},\beta_{ik},\delta_{ik})=0]\right]\\
=&\sum_{i}\sum_j\E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}}\left[\sum_{t_{ij}}f_{ij}(t_{ij})\cdot u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot \prod_{k\not=j}\Pr_{t_{ik}\sim D_{ik},(\beta_{ik},\delta_{ik})\sim \cC_{ik}}[u_{ik}(t_{ik},\beta_{ik},\delta_{ik})=0]\right]\\
\geq & \frac{1}{2}\cdot \sum_{i,j}\E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}}\left[\sum_{t_{ij}}f_{ij}(t_{ij})u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]
\end{align*}

Here the equality uses the fact that all $\cC_{ij}$s are independent. The last inequality comes from Inequality~\eqref{inequ:Q and Q_hat-1} and union bound. Now the second term is bounded by \begin{align*}
& 2\cdot \sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_{t_i}f_i(t_i)\cdot\max_j u_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]\\
\leq & 2\cdot \sum_{i}\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\sum_{t_i}f_i(t_i)\cdot\max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]
\end{align*}

\begin{definition}
For every $i,j,t_i\in \cT_i, S\subseteq [m]$, let 
$$\eta_i(t_i,S)=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]$$
%\mingfeinote{For every $i,j,t_i\in \cT_i,\beta_i\in \times_j\cV_{ij}, \delta_i\in \Delta_i^{n}, S\subseteq [m]$, let 
%$$\eta_i(t_i,\beta_i,\delta_i,S)=\max_{j\in S}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}$$
%}
\end{definition}

\begin{lemma}\label{lem:eta-lipschitz}
For every $i$, $\eta_i(\cdot, \cdot)$ is subadditive over independent items and $d_i$-Lipschitz. Note that $d_i$ is the variable in $(P)$.
%\mingfeinote{For every $i,t_i,\beta_i,\delta_i$, $\eta_i(t_i,\beta_i,\delta_i,\cdot)$ is monotone, subadditive, has no externalities, and it's $\delta_i$-Lipschitz.}
\end{lemma}

\begin{proof}

For every $i,j,t_{ij},\beta_{ij},\delta_{ij}$, denote $h_{ij}(t_{ij},\beta_{ij},\delta_{ij})=(V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]$.

We will first verify that for each $t_i\in T_i$, $\eta_i(t_i,\cdot)$ is monotone, subadditive and has no externalities.

Monotonicity: Let $S_1\subseteq S_2 \subseteq [m]$.
Then:
\begin{align*}
\eta_i(t_i,S_1)=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_1}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right] 
\leq  \E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_2}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right]
=  \eta_i(t_i,S_2)
\end{align*}

Subadditivity: For any set $S_1,S_2,S_3\subseteq [m]$ such that $S_1 \cup S_2 = S_3$,
it holds that:
\begin{align*}
\eta_i(t_i,S_3)&=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_3}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right] \\
&\leq\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\bigg[\max_{j\in S_1}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} + \max_{j\in S_2}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\bigg] \\
&=\eta_i(t_i,S_1) + \eta_i(t_i,S_2)
\end{align*}
The first inequality follows because $S_1\cup S_2=S_3$.

No externalities: for every $S\subseteq [m]$ and $t_i,t_i'\in \cT_i$ such that $t_{ij}=t_{ij}'$ for every $j\in S$, we have
$$\eta_i(t_i,S)=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\}\right]=\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S}\left\{ h_{ij}(t_{ij}',\beta_{ij},\delta_{ij})\right\}\right]=\eta_i(t_i',S)$$

Now we are going to prove that $\eta_i(\cdot,\cdot)$ is $d_i$-Lipschitz.
For $t_i,t_i'\in \cT_i$ and $X,Y \subseteq[m]$,
let $Z = \{j \in X\cap Y \land t_{ij}=t_{ij}'\}$.
It is enough to show that:
\begin{align*}
\eta_i(t_i,X) - \eta_i(t_i',Y) \leq  (m-|Z|)\cdot d_i \\
\eta_i(t'_i,Y) - \eta_i(t_i,X) \leq (m-|Z|)\cdot d_i
\end{align*}
We are only going to show $\eta_i(t_i,X) - \eta_i(t_i',Y) \leq  (m-|Z|)\cdot d_i $,
since the other case is similar.
Because $\eta_i(t_i,\cdot)$ is monotone, it is enough to prove that:
$$
\eta_i(t_i,X) - \eta_i(t_i',Y) \leq \eta_i(t_i,X) - \eta_i(t_i',Z) \leq  (m-|Z|)\cdot d_i 
$$
For each $j \in Z$, $t_{ij} =t_{ij}'$, which implies that $\eta_i(t_i',Z) = \eta_i(t_i,Z)$.
Note that:
\begin{align*}
&\eta_i(t_i,X) - \eta_i(t_i',Z)\\ 
= & \eta_i(t_i,X) - \eta_i(t_i,Z)\\
= & \E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\big[\max_{j\in X}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} - \max_{j\in Z}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} \big] \\
\leq & \E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\big[\max_{j\in Z}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} +\sum_{j\in X \backslash Z} h_{ij}(t_{ij},\beta_{ij},\delta_{ij}) - \max_{j\in Z}\left\{ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right\} \big] \\
= &  \E_{(\beta_{i},\delta_{i})\sim \cC_{i}} \left[\sum_{j\in X \backslash Z} h_{ij}(t_{ij},\beta_{ij},\delta_{ij}) \right]\\
= &  \sum_{j\in X \backslash Z} \E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}} \left[ h_{ij}(t_{ij},\beta_{ij},\delta_{ij})\right]\\
\leq &  \sum_{j\in X \backslash Z} \E_{(\beta_{ij},\delta_{ij})\sim \cC_{ij}} \left[ \delta_{ij} \right]\\
\leq & (|X|-|Z|)d_i \leq (m-|Z|)d_i
\end{align*}
Here the second last inequality follows by constraint (7) of (P). We finish the proof.
\end{proof}

\begin{lemma}\label{lemma:concentrate}\cite{CaiZ17}
Let $g(t,\cdot)$ with $t\sim D=\prod_j D_j$ be a function drawn from a distribution that is  subadditive over independent items of ground set $I$. If $g(\cdot,\cdot)$ is $c$-Lipschitz, then if we let $a$ be the median of the value of the grand bundle $g(t,I)$, i.e. $a=\inf\left\{x\geq 0: \Pr_t[g(t,I)\leq x]\geq \frac{1}{2}\right\}$,
$$\mathds{E}_t[g(t,I)]\leq 2a+\frac{5c}{2}.$$
\end{lemma}

To finish the proof of \Cref{lem:Q and Q-hat}, we will bound $\sum_i\sum_{t_i}f_i(t_i)\cdot \eta_i(t_i,[m])$ by the revenue of some restricted SPEM. Consider the restricted SPEM $\cM$ \todo{To add definition in the prelim. Only allow the buyer to buy one item.} with posted price $\beta_{ij}\sim \cB_{ij}$ for buyer $i$ and item $j$. Let $S_i(t_{<i},\beta_{<i})$ be the random set of available items when buyer $i$ comes to the auction. Then by union bound, for every item $j$,

$$\Pr[j\in S_i(t_{<i},\beta_{<i})]\geq 1-\sum_{k<i}\Pr_{t_{ij}\sim D_{ij},\beta_{ij}\sim \cB_{ij}}[t_{ij}\geq \beta_{ij}]\geq \frac{1}{2}$$
%\argyrisnote{Maybe we should mention that $\Pr_{\beta_{ij}\sim \Beta_{ij}}[t_{ij}\geq \beta_{ij}]$ that }

Consider the following entry fee function in $\cM$: $\xi_i(S_i(t_{<i},\beta_{<i}))=\Med_{t_i\sim D_i}\{\eta_i(t_i,S_i(t_{<i},\beta_{<i}))\}$\footnote{Here $\Med_x[h(x)]$ denotes the median of a non-negative function $h(x)$ on random variable $x$, i.e.
$\Med_x[h(x)]=\inf\{a\geq 0:\Pr_{x}[h(x)\leq a]\geq\frac{1}{2}\}$.
}. We notice that for every $t_{<i},\beta_{<i}$, after seeing the remaining item set $S_i(t_{<i},\beta_{<i})$, buyer $i$'s expected utility if she pays the entry fee is:
$$\E_{(\beta_{i},\delta_{i})\sim \cC_{i}}\left[\max_{j\in S_i(t_{<i},\beta_{<i})}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\right\}\right]\geq \eta_i(t_i,S_i(t_{<i},\beta_{<i}))$$

Thus the buyer will accepts the entry fee with probability at least $1/2$. Hence

\begin{equation}\label{inequ:Q and Q_hat-term2}
\begin{aligned}
\rev(\cM) & \geq  \frac{1}{2}\sum_i\E_{t_{<i},\beta_{<i}}[\xi_i(S_i(t_{<i},\beta_{<i}))]\geq \frac{1}{2}\cdot \sum_i(\frac{1}{2}\E_{t_i,t_{<i},\beta_{<i}}[\eta_i(t_i,S_i(t_{<i},\beta_{<i}))]-\frac{5}{4}d_i)\\
 & \geq \frac{1}{2}\cdot \sum_i(\frac{1}{4}\E_{t_i}[\eta_i(t_i,[m])]-\frac{5}{4}d_i) \geq\frac{1}{8}\cdot \sum_i \E_{t_i}[\eta_i(t_i,[m])]-5\cdot \prev 
\end{aligned}
\end{equation}

%\argyrisnote{Is it $\delta$ instead of $\theta$?We lose a factor of $2$ in the second inequality because each item is available with probability at least $\frac{1}{2}$?}
%\mingfeinote{Changed the proof a little. See if you agree now.}

%\argyrisnote{Should we also take expectation over $t_i\sim D_i$ in the first term above?}
%\mingfeinote{In the first term, $\xi_i$ is the $\Med_{t_i}$, the median over $t_i\sim D_i$.}

Here the second inequality is obtained by applying \Cref{lemma:concentrate} to function $\eta_i(t_i,\cdot)$ and ground set $I=S_i(t_{<i},\beta_{<i})$ for every $t_{<i},\beta_{<i}$. The last inequality comes from constraint (8) of $(P)$. The third inequality comes from the following:  

%For every $i,j,t_{ij},\beta_{ij},\delta_{ij}$, denote $h_{ij}(t_{ij},\beta_{ij},\delta_{ij})=(V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]$. Then for every $t_i,\beta_i,\delta_i$,

Fix any $t_i,\beta_i,\delta_i$. Let $j^*=\argmax_{j\in [m]}(V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]$. Then 

%\argyrisnote{You cannot fix $\beta_i,\delta_i$ right? $\eta$ takes expectation over them?} \mingfeinote{$t_i,\beta_i,\delta_i$ are fixed only for the following inequality.}
\begin{align*}
&\E_{t_{<i},\beta_{<i}}\left[\max_{j\in S_i(t_{<i},\beta_{<i})}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\right]\\
\geq & \E_{t_{<i},\beta_{<i}}\left[\max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\cdot \ind[j^*\in S_i(t_{<i},\beta_{<i})]\right]\\
= & \max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}\cdot \Pr_{t_{<i},\beta_{<i}}[j^*\in S_i(t_{<i},\beta_{<i})]\\
\geq & \frac{1}{2}\cdot \max_{j\in [m]}\left\{ (V_{ij}(t_{ij})-\beta_{ij})^+\cdot\mathds{1}[V_{ij}(t_{ij}) \leq \beta_{ij}+ \delta_{ij}]\right\}
\end{align*}

Taking expectation over $t_i$ and $(\beta_i,\delta_i)\sim \cC_i$ on both sides, we have 
$$\E_{t_i,t_{<i},\beta_{<i}}[\eta_i(t_i,S_i(t_{<i},\beta_{<i}))]\geq \frac{1}{2}\E_{t_i}[\eta_i(t_i,[m])],$$

%By \Cref{lem:eta-lipschitz}, for every $i,t_i$, $\eta_i(t_i,\cdot)$ is an XOS function. Denote $\{a_j\}_{j\in [m]}$ the supporting price of $\eta_i(t_i,\cdot)$ for set $[m]$. Then

%$$\E_{t_{<i},\beta_{<i}}[\eta_i(S_i(t_{<i},\beta_{<i}))]\geq\E_{t_{<i},\beta_{<i}}\left[\sum_{j\in S_i(t_{<i})}a_j\right]=\sum_j a_j\cdot \Pr_{t_{<i},\beta_{<i}}[j\in S_i(t_{<i},\beta_{<i})]\geq \frac{1}{2}\sum_j\theta_j=\frac{1}{2}\eta(t_i,[m])$$
 
which is exactly the third inequality of \eqref{inequ:Q and Q_hat-term2}. By combining Inequalities \eqref{inequ:Q and Q_hat-term1} and \eqref{inequ:Q and Q_hat-term2}, we have
$$2\sum_j(Q_j - \hat{Q}_j) \leq 88\cdot\prev + 16\cdot\rev(\cM)$$

\mingfeinote{
Finally, since in $\cM$, each buyer is restricted to purchase at most one item, it can be treated as a BIC and IR mechanism in the unit-demand setting. By \cite{ChawlaHMS10,KleinbergW12,CaiDW16}, $\rev(\cM)\leq 24\cdot \prev$. We finish our proof.
}

%\todo{Say that the entry fee can be computed efficiently.}
%\argyrisnote{I don't think it is necessary? as mentioned in the comment after the statement of the theorem.}
%\argyrisnote{
%Also by Combining the mentioned inequalities don't we get that $2\sum_j(Q_j - \hat{Q}_j) \leq 48 \prev + 16 \aperev$?
%Isn't restricted SPEM with entry fee just \prev, where we shift the price of each item by the same number? So the previous bound just becomes $64\prev$?} \mingfeinote{Thanks for pointing it out! I divided the constant by 2. Also, I don't think the restricted SPEM is equivalent to $\prev$ when the posted price are randomized. In $\prev$ the posted price are drawn and given to the buyer before the buyer makes any decision. In restricted SPEM, the buyer has to decide whether to pay this fixed entry fee before seeing the exact posted price.}
%\argyrisnote{Why don't we use a mechanism that shows the items to the buyer and sets entry fee to the $i$-th buyer equal to $\delta_i=\Med_{t_i\sim D_i}\{\eta_i(t_i,S_i(U)\}$?
%The buyer accepts the entry fee with probability at least $\frac{1}{4}$, the probability to accept the entry fee, if all the items are available $\frac{1}{2}$ times the probability that her favourite item is available $\frac{1}{2}$. That way we can covnert the mechanism into a real SPEM that does not depend on which items have been sold, right?}



\notshow{
\begin{align*}
& \sum_{j\in[m]}\sum_{i\in[n]} \sum_{\substack{t_{i,j}\in T_{i,j}\\V_{i,j}(t_{i,j}) \geq Q_j^* + \tau_i}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
\sum_{\delta \in \Delta V_{i}} (V_{i,j}(t_{i,j})-\beta)\cdot
\lambda_{i,j}(t_{i,j},\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \beta ] \\
= & \sum_{j\in[m]}\sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
\sum_{\delta \in \Delta V_{i}} (V_{i,j}(t_{i,j})-\beta)\cdot
\lambda_{i,j}(t_{i,j},\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] \\
\leq & \sum_{j\in[m]} \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] 
\end{align*}


Observe that the quantity above is the sum of the truncated utilities if we pretend that the buyers are additive,
when the price is set to 
%$\max(Q_j + \tau_i, \beta_{i,j})$
$\beta_{i,j}$
of the $i$-th agent for the $j$-th item,
where $\beta_{i,j}$ and the truncation $\delta_{i,j}$ is sampled (independently from the other items and agents, but the distribution between $\beta_{i,j}$ and $\delta_{i,j}$ is coupled) from $B_{i,j} \times \Delta_{i,j}$.
By the constraint of the program,
the expected truncated utility of the $i$-th agent is at most $\delta_i$.
Let

$$u_{ADD} = \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] 
$$

Let $u_{UD}$ be the expected truncated utility if the buyer was unit-demand,
notice that a lower bound of $u_{UD}$ is:
\begin{align*}
u_{UD} \geq & \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) > \max( \beta, Q_j^* + \tau_i) ] \\
& \quad \cdot \prod_{k\neq i}\Pr_{\substack{\beta \sim B_{i,k}\\t_{i,k}\sim D_{i,k}}}[V_{i,k}(t_{i,k}) \leq \max( \beta, Q_k^* + \tau_i) ] \\
\geq & \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
 (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
\lambda_{i,j}'(\beta, \delta)
\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) > \max( \beta, Q_j^* + \tau_i) ] \frac{1}{2} \\
%= & \sum_{i\in[n]} \sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})  \sum_{\beta\in V_{i,j}(T_{i,j})}
% (V_{i,j}(t_{i,j})-\beta) \sum_{\delta \in \Delta V_{i}}
%\lambda_{i,j}'(\beta, \delta)
%\mathds{1}[\delta + \beta \geq V_{i,j}(t_{i,j}) \geq \max( \beta, Q_j^* + \tau_i) ] \frac{1}{2} \\
= & \frac{u_{ADD}}{2}
\end{align*}

Now we are going to show that there exists a simple mechanism that generates revenue close to $u_{UD}$.
Let $B\times \Delta$ be the coupled distribution of $B_i \times \Delta_i$.
Let 
$$u^T_i(t, X) = \E_{(\beta, \delta) \sim B \times \Delta} [ \max_{j \in X} (V_{i,j}(t_{i,j})- \beta_j)\mathds{1}[\delta_{i,j} + \beta_j \geq V_{i,j}(t_{i,j}) \geq \beta_j ]$$

Note that $\sum_{i\in[n]}\E_{t_i \sim \DD_i}[u^T_i(t, [m])] \geq u_{UD}$.



\begin{lemma}
The function $u^T_i(\cdot, \cdot)$ is $\delta_i$-Lipschitz and subadditive over the items.
\end{lemma}

}

%\todo{Since values $\beta$ have been choosen so that each item is sold with probability $\frac{1}{2}$, we can still bound the objective by a simple mechanism.}
%Thus the median and mean of the utility are close,
%so we can find a proper entry fee to get the truncated utility (minus $O(1)Srev$) as revenue.
%Observe that Unit-Demand prices + entry fee is bounded \srev.


\notshow{

\todo{Let $t_i \in T_i$.
We denote by $W_{t_i}$ the the polytope of feasible welfares normalised to $[0,1]$  when the $i$-th agent has type $t_i$ (note that this can be achieved by dividing the supporting price that the agent has for the allocation by $V_{i,j}(t_{i,j})$).
Let $W_i$ be a mixture of polytopes $\{W_{t}\}_{ t \in T}$ with distribution $\{f(t)\}_{t \in T}$.
%Note that the bit complexity of each vertex of each polytope is $O(m)$.
%The bit complexity of each node in the polytope depends on $\max_{i\in[n], t_i \in T_i, j\in[m], S \in 2^{[m]}}b(v_j^S(t_{i,j}))$.
The bit complexity of the polytope depends on the supporting prices, which (I believe) its reasonable to assume that are bounded.

Note that for $t_i \in T_i$,
we can optimize any objective over $W_{t_i}$ by using a demand oracle. 
By sampling we can get a sampling an empirical polytope close to the polytope of $W_i$. Thus we can calculate the value of $(P)$ with respect to the sampled polytope.

Observe that the way $W_i$ is defined here,
is the scaled by $f_i(t_i)$ version of the $W_i$ that was defined in the program

%Thus we lose $\epsilon \cdot n \cdot m \cdot H$ in the objective by sampling in order to get a feasible solution, where $\epsilon$ depends on the number of samples we used to form the empirical polytope and $H$ is the highest value for an item and we can get a feasible solution.
%Since each element is within $\epsilon$ of a feasible, and by reducing the value of $w_{i,j}(t_{i,j})$ by $\epsilon$ we can still get a feasible solution of the original problem, I think we are fine.
}

}

\end{proof}


\subsection{Construction of SPEM}

In this section, we will construct a SPEM whose revenue bounds $\sum_jQ_j$.
%how to bound $\sum_j\hat{Q}_j$ using simple mechanisms that can be computed efficiently. 
%Then \Cref{thm:bounding-lp-simple-mech} follows directly from \Cref{lem:Q and Q-hat} and \Cref{lem:bounding Q-hat}, since the objective of any feasible solution of $(P)$ is represented as $\sum_{j\in [m]}Q_j$.

\begin{definition}[Construction of the SPEM]\label{def:constructed-SPEM}

Denote $\Meff$ the SPEM with deterministic posted price $\theta_{ij}=Q_j$ for every $i,j$. For any type profile $t\in T$ and any buyer $i$, define the entry fee for buyer $i$ as $$\xi_i(S_i(t_{<i})) = \Med_{t_i}\left[\max_{S'\subseteq S_i(t_{<i})}\left(v_i(t_i,S')-\sum_{j\in S'}Q_j\right)\right],$$ where $S_1(t_{<1})=[m]$ and $S_i(t_{<i})$ is the set of items that are not purchased by the first $i-1$ buyers in the SPEM. We notice that the remaining item set only depends on $t_{<i}$ since the posted prices are deterministic $(\theta_{ij}=Q_j)$.
\end{definition}

\begin{lemma}\label{lem:Meff-computation}
The mechanism $\Meff$ in \Cref{def:constructed-SPEM} can be computed efficiently. Formally, for every $i,j$ and $S\subseteq [m]$, both the posted price $\theta_{ij}$ and entry fee $\xi_i(S)$ can be computed in time \mingfeinote{Add time complexity and query complexity to the adjusted demand oracle}.
\end{lemma}


%\begin{lemma}\label{lem:bounding Q-hat}
%Let $\cM$ and $\Meff$ be the mechanism stated in \Cref{lem:Q and Q-hat} and \Cref{def:constructed-SPEM} accordingly. Then $\sum_j \hat{Q}_j\leq O(1)\cdot \prev+O(1)\cdot \rev(\cM) + O(1)\cdot \rev(\Meff)$.
%\end{lemma}

%To prove \Cref{lem:bounding Q-hat}, 
To analyze the revenue of $\Meff$, we require the following definition.

\begin{definition}\label{def:mu}
%For any $i,t_i,\beta_i=(\beta_{ij})_j,\delta_i=(\delta_{ij})_j$, let

%$$C_i(t_i,\beta_i,\delta_i)=\{j\in [m]\mid V_{ij}(t_{ij})\leq \min\{\beta_{ij}+\delta_{ij},Q_j+\tau_i\}\}$$

For any $i,t_i$, let $C_i(t_i)=\{j\in [m]\mid V_{ij}(t_{ij})\leq Q_j+\tau_i\}$. For any $t_i\in \cT_i$ and set $S\subseteq [m]$, let
%$$\mu_i(t_i,S)=\E_{(\beta_i,\delta_i)\sim \cC_i}\left[\max_{S'\subseteq S}\left(v_i(t_i,S'\cap C_i(t_i,\beta_i,\delta_i))-\sum_{j\in S'}Q_j\right)\right]$$ 

$$\mu_i(t_i,S)=\max_{S'\subseteq S}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)$$ 
\end{definition}

\begin{lemma}\label{lem:mu_i lipschitz}
For every $i$, $\mu_i(\cdot, \cdot)$ is subadditive over independent items and $\tau_i$-Lipschitz.
\end{lemma}

\begin{proof}
First we are going to show that $\mu_i(t,\cdot)$ is monotone.
Note that for sets $S_1 \subseteq S_2$ the following holds:
\begin{align*}
    \mu_i(t_i,S_1)=& \max_{S'\subseteq S_1}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    \leq &\max_{S'\subseteq S_2}\left(  v_i(t_i, S'\cap C_i(t_i)) -\sum_{j\in S'}Q_j\right)\\
    = & \mu_i(t_i,S_2)
\end{align*}

Now we are going to show that $\mu_i(t,\cdot)$ is subadditive.
Let $S_1,S_2,S_3\subseteq[m]$ such that $S_1 \cup S_2 = S_3$ and $S_1 \cap S_2 = S_c$.
Let $S_a = S_1 \backslash S_c$ and $S_b=S_2$,
then for any $t_i\in T_i$ we have the following:
\begin{align*}
    \mu_i(t_i,S_3)=& \max_{S'\subseteq S_3}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    \leq &\max_{S'\subseteq S_3}\left(  v_i(t_i,\left(S_a\cap S'\right)\cap C_i(t_i)) + v_i(t_i,\left(S_b\cap S'\right)\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    = & \max_{S'\subseteq S_3}\left(  \left(v_i(t_i,\left(S_a\cap S'\right)\cap C_i(t_i))- \sum_{j\in S_a\cap S'}Q_j \right)+ \left(v_i(t_i,\left(S_b\cap S'\right)\cap C_i(t_i))-\sum_{j\in S_b\cap S'}Q_j\right)\right)\\
    \leq & \max_{S'\subseteq S_a}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right) + \max_{S'\subseteq S_b}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    = & \mu_i(t_i,S_a) + \mu_i(t_i,S_b) \\
    \leq & \mu_i(t_i,S_1) + \mu_i(t_i,S_2)
\end{align*}

The first inequality follows because $v_i(t_i,\cdot)$ is subadditive function and $S_a\cup S_b=S_3$. The second equality follows because $S_a \cap S_b = \emptyset$ and $S_a \cup S_b = S_3$. The final inequality follows from the fact that $S_b =S_2$, $S_1 \supseteq S_a$ and that $\mu_i(t_i,\cdot)$ is monotone.

No externalities: Fix any $S\subseteq [m]$ and $t_i,t_i'\in \cT_i$ such that $t_{ij}=t_{ij}'$. We notice that by the definition of $C_i$, $S\cap C_i(t_i)=S\cap C_i(t_i')$. Since $v_i(\cdot,\cdot)$ has no externalities, $v_i(t_i,S'\cap C_i(t_i))=v_i(t_i',S'\cap C_i(t_i'))$ for every $S'\subseteq S$. Thus $\mu_i(t_i,S)=\mu_i(t_i',S)$.

Now we are going to show that $\mu_i(\cdot,\cdot)$ is $\tau_i$-Lipschitz.
Let $t_i,t_i' \in \cT_i$ and $X,Y \subseteq[m]$ and $c= |\{j \in [m]: j \in X \Delta Y \lor t_{ij} \neq t_{ij}'\}|$, we need to show that:
$$
|\mu_i(t_i,X) - \mu_i(t_i',Y)| \leq c\cdot \tau_i
$$
Let $Z = \{j\mid j \in X\cap Y \land t_{ij}=t_{ij}'\}$.
Since $\mu_i(t_i,\cdot)$ is monotone, in order to show that $\mu_i(\cdot,\cdot)$ is $\tau_i$-Lipschitz,
it is enough to show that
\begin{align*}
\mu_i(t_i,X) - \mu_i(t_i',Y) \leq \mu_i(t_i,X) - \mu_i(t_i',Z) \leq c\cdot \tau_i \\
\mu_i(t'_i,Y) - \mu_i(t_i,X) \leq \mu_i(t'_i,Y) - \mu_i(t_i,Z) \leq c\cdot \tau_i
\end{align*}
We are only going to prove that $\mu_i(t_i,X) - \mu_i(t_i',Z) \leq c\cdot \tau_i$ since the other case is similar.
Because for each $j\in Z$, $t_{i,j}'=t_{i,j}$, then $\mu_i(t_i',Z)= \mu_i(t_i,Z)$.
Observe that $|Z|+c = m$. Thus it is enough to show:
$$
\mu_i(t_i,X) - \mu_i(t_i,Z) \leq (m-|Z|)\cdot \tau_i \Leftrightarrow \mu_i(t_i,X)  \leq (m-|Z|)\cdot \tau_i +  \mu_i(t_i,Z)
$$
We have
\begin{align*}
    \mu_i(t_i,X)=& \max_{S'\subseteq X}\left(v_i(t_i,S'\cap C_i(t_i))-\sum_{j\in S'}Q_j\right)\\
    \leq &\max_{S'\subseteq X}\left(\sum_{j\in S'\backslash Z}\left(v_i(t_i,\{j\}\cap C_i(t_i)) - Q_j \right) +  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right)\right)\\
    \leq &\max_{S'\subseteq X}\left(\sum_{j\in S'\backslash Z}\left(V_{ij}(t_{ij}) - Q_j \right)^+\ind[V_{ij}(t_{ij}) \leq Q_j + \tau_i] +  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right)\right)\\
    = & \max_{S'\subseteq Z}  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right) + \sum_{j\in X\backslash Z}\left(V_{ij}(t_{ij}) - Q_j \right)^+\ind[V_{ij}(t_{ij}) \leq Q_j + \tau_i]\\
    \leq & \max_{S'\subseteq Z}  \left(v_i(t_i,(Z\cap S')\cap C_i(t_i))-\sum_{j\in Z\cap S'}Q_j\right) + (|X| - |Z|)\tau_i\\
    \leq &\mu_i(t_i,Z) +  (m-|Z|)\cdot \tau_i
\end{align*}
The first inequality follows because $v_i(t_i,\cdot)$ is subadditive.
The second inequality follows because $v_i(t_i,\{j\}\cap C_i(t_i)) - Q_j \leq (V_{ij}(t_{ij}) - Q_j)^+\ind[V_{ij}(t_{ij})\leq Q_j + \tau_i]$.
\end{proof}

\begin{lemma}\label{lem:lower bounding mu}
	Let $\cM$ be the restricted SPEM stated in \Cref{lem:Q and Q-hat}. For every type profile $t\in \cT$, let $\textsc{SOLD}(t)$ be the set of items sold in mechanism $\Meff$. Then

\begin{align*}
\E_{t}\left[\sum_{i\in[n]} \mu_i\left(t_i,S_i(t_{< i})\right) \right]&\geq \sum_j \Pr_{t}[j\notin \sold(t)]\cdot(2\hat{Q}_j-Q_j)\\
&\geq \sum_{j} \Pr_t\left[j\notin \sold(t)\right]\cdot Q_j - 88\cdot \prev - 16\cdot \rev(\cM)
\end{align*}

\end{lemma}

\begin{proof}

By the definition of polytope $W_i$, for every buyer $i$ and $t_i\in \cT_i$, there exists an vector of non-negative numbers $\{\sigma_{iS}^{(k)}(t_i)\}_{S\subseteq [m],k\in [K]}$, such that $\sum_{S,k} \sigma_{iS}^{(k)}(t_i)=1$ and
\begin{equation}
\pi_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_{k\in [K]}\sigma_{iS}^{(k)}(t_{ij},t_{i,-j})
\end{equation}

\begin{equation}\label{equ:w and gamma}
w_{ij}(t_{ij})\cdot V_{ij}(t_{ij}) = f_{ij}(t_{ij})\cdot \sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_{ij},t_{i,-j})\cdot\alpha_{ij}^{(k)}(t_{ij})
\end{equation}

%For every $t_i$, define
%$$\hat\gamma_{ij}^S(t_i)=\gamma_{ij}^S(t_i)\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]$$

%Then clearly for every $t_i$ and $S$, $\{\hat\gamma_{ij}^S(t_i)\}_j$ is the supporting price for $v_i(t_i,S\cap C_i(t_i))$. 
We have
\begin{align*}
&\E_{t}\left[\sum_i \mu_i\left(t_i,S_i(t_{< i})\right) \right]\\
\geq & \sum_i \E_{t_i, t_{-i}}\left[\sum_{S\subseteq [m]}\sum_k\sigma_{iS}^{(k)}(t_i)\cdot\mu_i\left(t_i,S_i(t_{<i})\cap S\right)\right]\\
\geq & \sum_i \E_{t_i, t_{-i}}\left[\sum_{S,k}\sigma_{iS}^{(k)}(t_i)\cdot\sum_{j\in S} \ind\left[j\in S_i(t_{<i})\right]\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)^+ \right]\\
=& \sum_i \E_{t_i}\left[\sum_{j\in [m]}\Pr_{t_{-i}}[j\in S_i(t_{<i})]\cdot\sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_i)\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)^+ \right]\\
\geq & \sum_i\sum_j \Pr_{t}[j\notin \sold(t)]\cdot \E_{t_i}\left[\sum_{S: j\in S}\sum_k \sigma_{iS}^{(k)}(t_i)\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)^+\right]\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_i} f_i(t_i)\cdot \sum_{S: j\in S}\sum_k \sigma_{iS}^{(k)}(t_i)\cdot\left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)\\
= & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot\sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_i)\cdot(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j)\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} w_{ij}(t_{ij}) V_{ij}(t_{ij})\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-\sum_j\Pr_t[j\not\in \sold(t)]\cdot Q_j
\end{align*}

%\argyrisnote{I don't see why:
%$\sum_i \sum_{t_{ij}} f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{,%-j}(t_{i,-j})\cdot\sum_{S:j\in S}\sigma_{iS}(t_i)Q_j =Q_j$? We could overallocate the item since we have constraints only on $w_{i,j}$?}

The first inequality is because $\mu_i(t_i,S)$ is monotone in set $S$ for any $i,t_i$ and $\sum_{S,k}\sigma_{iS}^{(k)}(t_i)=1$. For any fixed $i,t_i$ and set $S$, if we let $S'$ be the set of items that are in $S\cap S_i(t_{<i})$ and satisfy that $\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\geq 0$. Clearly $S'\subseteq C_i(t_i)$. Then 
\begin{align*}
\mu_i\left(t_i,S_i(t_{<i})\cap S\right)&\geq v_i(t_i,S')-\sum_{j\in S'}Q_j\\
&= \max_{k'\in [K]}\sum_{j\in S'}\alpha_{ij}^{(k')}(t_{ij})-\sum_{j\in S'}Q_j\geq \sum_{j\in S'} \left(\alpha_{ij}^{(k)}(t_{ij})-Q_j\right)\\
&=\sum_{j\in S'} \left(\alpha_{ij}^{(k)}(t_{ij})\cdot\ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-Q_j\right)~~~~~(S'\subseteq C_i(t_i))
\end{align*} 

This inequality is exactly the second inequality above. The third inequality is because $\Pr_{t_{<i}}[j\in S_i(t_{<i})]\geq \Pr_{t}[j\notin \sold(t)]$ for all $j$ and $i$, as the LHS is the probability that the item is not sold after the seller has visited the first $i-1$ buyers and the RHS is the probability that the item remains unsold till the end of the mechanism $\Meff$. 
%The second last inequality follows from the definition of $\hat\gamma_{ij}^S(t_i)$ and the fact that
The last inequality follows from Equation~\eqref{equ:w and gamma} and constraint (3) of $(P)$:

$$\sum_i\sum_{t_{ij}}f_{ij}(t_{ij})\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sum_k\sigma_{iS}^{(k)}(t_i)=\sum_i\sum_{t_{ij}}\pi_{ij}(t_{ij})\leq 1$$

Now we notice that by \Cref{def:Q_j} and constraint (2) of $(P)$, for every $i,j,t_{ij}$, 

$$\sum_{\beta_{ij},\delta_{ij}}g_{ij}(t_{ij},\beta_{ij},\delta_{ij})\leq \sum_{\beta_{ij},\delta_{ij}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=w_{ij}(t_{ij})/f_{ij}(t_{ij})$$
\argyrisnote{In the continuous version, we do not use $g_{ij}$, right?}
Thus we have

\begin{align*}
&\sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} w_{ij}(t_{ij}) V_{ij}(t_{ij})\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i]-\sum_j\Pr_t[j\not\in \sold(t)]\cdot Q_j\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot \sum_i \sum_{t_{ij}} f_{ij}(t_{ij})V_{ij}(t_{ij})\cdot \ind[V_{ij}(t_{ij})\leq Q_j+\tau_i] \sum_{\beta_{ij},\delta_{ij}}g_{ij}(t_{ij},\beta_{ij},\delta_{ij})-\sum_j\Pr_t[j\not\in \sold(t)]\cdot Q_j\\
= &\sum_j \Pr_{t}[j\notin \sold(t)]\cdot (2\hat{Q}_j-Q_j)~~~~~\text{(\Cref{def:hatQ_j})}\\
= &  \sum_j \Pr_{t}[j\notin \sold(t)]\cdot Q_j-  \sum_j\Pr_{t}[j\notin \sold(t)]\cdot2(Q_j-\hat{Q}_j)\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot Q_j - \sum_j 2(Q_j-\hat{Q}_j )~~~~~{\text{(\Cref{lem:Q and Q-hat}, $Q_j-\hat{Q}_j\geq 0$ for all $j$)}}\\
\geq & \sum_j \Pr_{t}[j\notin \sold(t)]\cdot Q_j- 88\cdot\prev-16\cdot\rev(\cM)~~~~~\text{(\Cref{lem:Q and Q-hat})}
\end{align*}
\end{proof}


\begin{prevproof}{Theorem}{thm:bounding-lp-simple-mech}

For every $i,t_{<i}$, we apply \Cref{lemma:concentrate} with function $\mu_i(t_i,\cdot)$ and ground set $S_i(t_{<i})$. By \Cref{def:mu}, we have
$$\E_{t_i}[\mu_i(t_i,S_i(t_{<i}))]\leq 2\cdot \Med_{t_i}(\mu_i(t_i,S_i(t_{<i})))+\frac{5}{2}\cdot \tau_i$$

We now bound the revenue of $\Meff$. For every buyer $i$ with type $t_i$, her utility for the set $S_i(t_{<i})$ is $\max_{S'\subseteq S_i(t_{<i})}(v_i(t_i,S')-\sum_{j\in S'}Q_j)$. By the definition of $\xi_i(S_i(t_{<i}))$, the buyer will accept the entry fee with probability $\frac{1}{2}$. The revenue of $\Meff$ from the entry fee is
\begin{align*}
\frac{1}{2}\sum_i\E_{t_{<i}}[\xi_i(S_i(t_{<i}))]\geq & \frac{1}{2}\sum_i\E_{t_{<i}}\left[\Med_{t_i}(\mu_i(t_i,S_i(t_{<i})))\right]\\
\geq & \frac{1}{4}\sum_i\E_{t_i,t_{<i}}[\mu_i(t_i,S_i(t_{<i}))]-\frac{5}{8}\cdot \sum_i\tau_i\\
\geq & \frac{1}{4}\sum_{j} \Pr_t\left[j\notin \sold(t)\right]\cdot Q_j - 27\cdot \prev - 4\cdot \rev(\cM)
\end{align*}
The first inequality comes from the fact that $\mu_i(t_i,S)\leq \max_{S'\subseteq S}(v_i(t_i,S')-\sum_{j\in S'}Q_j)$ for all $i,t_{i}$ and $S\subseteq [m]$. The third inequality follows from \Cref{lem:lower bounding mu} and \Cref{lem:bounding tau_i}. We notice that for $\Meff$, the revenue from the posted prices are $\sum_j \Pr[j\in \sold(t)]\cdot Q_j$. Thus
\begin{align*}\rev(\Meff)\geq & \frac{1}{4}\sum_{j} \Pr_t\left[j\notin \sold(t)\right]\cdot Q_j - 27\cdot \prev - 4\cdot \rev(\cM)+\sum_j \Pr[j\in \sold(t)]\cdot Q_j\\
\geq & \frac{1}{4}\cdot \sum_{j\in [m]}Q_j-27\cdot \prev - 4\cdot \rev(\cM)
\end{align*}

Thus
$$2\cdot \sum_jQ_j\leq 216\cdot \prev+32\cdot \rev(\cM)+8\cdot\rev(\Meff)$$

By \Cref{lem:Meff-computation} and \Cref{lem:Q and Q-hat}, both $\cM$ and $\Meff$ can be computed in time \mingfeinote{Add time}. The proof is done.
\end{prevproof}

\notshow{
\section{Backup section (only for checking)}

\begin{align*}
    (P) = 
    \max& \frac{1}{2} \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{i,j}\in T_{i,j}}  f_{i,j}(t_{i,j})\cdot V_{i,j}(t_{i,j})\cdot
    \\
    &\quad \quad\sum_{\substack{\beta\in V_{i,j}(T_{i,j})\\\delta \in \Delta V_{i}}} \lambda_{i,j}(t_{i,j},\beta, \delta)\cdot \mathds{1}[V_{i,j}(t_{i,j}) \leq \beta + \delta]\\
    s.t.\quad & \pi_i \in \Pi_i  & \forall i \in[n] \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    & \sum_{\beta}\lambda_{i,j}(t_{i,j},\beta) = \pi_{i,j}(t_{i,j}) & \forall i\in[n],j\in[m],t_{i,j}\in T_{i,j}\\
    & \sum_{i\in[n]}\sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})\cdot \pi_{i,j}(t_{i,j}) \leq 1, & \forall j \in[m] \\
    & \lambda_{i,j}(t_{i,j},\beta, \delta) \leq \lambda_{i,j}'(\beta, \delta) & \forall i\in[n], j \in[m], t_{i,j} \in T_{i,j}\\ 
    &\sum_{t_{i,j}} f_{i,j}(t_{i,j}) \lambda_{i,j}(t_{i,j},\beta) \leq \frac{1}{2}\cdot \lambda'_{i,j}(\beta) \Pr_{t_{i,j}\sim D_{i,j}}[t_{i,j} \geq \beta] & \forall \beta \in V_{i,j}(T_{i,j})\\
    & \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) \text{(Maybe not needed)} &\forall i\in[n], j \in[m] \\
    & \sum_{\delta \in \Delta V_i} \delta \lambda_{i}'(\delta) \leq \delta_i  & \forall i \in [n]\\
    & \sum_{i\in[n]} \delta_i \leq O(1) \cdot \srev \\
     & \forall i \in[n],j\in [m],t\in T_{i,j},\beta,\gamma \in V_{i,j}(t_{i,j})\\
\end{align*}
}




\section{Old Main Program (for reference only)}
%\argyrisnote{Do we agree that the first among the two programs is the one we are going to focus on?}

The variables in the LP are as follows:
\begin{enumerate}
    \item $\pi_{ij}(t_{ij})$, for all $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We denote $\pi_i=(\pi_{ij}(t_{ij}))_{j,t_{ij}}$ the vector of all variables associated with buyer $i$.
    \item $w_{ij}(t_{ij})$, for all $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We denote $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}}$ the vector of all variables associated with buyer $i$.
    \item $\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij}),\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})$, for all $i,j$ and $t_{ij}\in \cT_{ij}$, $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta_i$.
    \item $\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij}), \hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$, for all $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta_i$, %denoting the joint distribution over $\cV_{ij}\times \Delta_i$.
    \item $d_i$, for all $i\in [n]$.
\end{enumerate} \todo{To add some explanation of the variables.} In the LP, we will abuse the notations and let $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})+\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})$, $\lambda_{ij}(t_{ij},\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$. Similarly, let $\hat\lambda_{ij}(\beta_{ij},\delta_{ij})=\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})+\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}^{(r)}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}(\beta_{ij},\delta_{ij})$. 

%Let $W_{i}$ be the polytope of feasible normalized welfare for buyer $i$.
%That is, $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}}$ is in $W_i$ if and only if there exists an allocation (for buyer $i$) $\{\sigma_{iS}(\cdot)\}_{S\subseteq [m]}$, such that $$w_{ij}(t_{ij})\cdot V_{ij}(t_{ij}) = \sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\sigma_{iS}(t_{ij},t_{i,-j})\cdot\gamma_{ij}^{S}(t_i),$$
%where $\gamma_{ij}^{S}(t_i)$ is buyer $i$'s supporting price for item $j$ with respect to set $S$. \todo{Add a definition $\gamma_{ij}^S(t_i)=\alpha_{ij}^{k(t_i,S)}$.}
%\mingfeinote{Add definition of ``supporting price''. Should be $\alpha_j^k$ instead.} \argyrisnote{I think it should be $\alpha_j^k$ instead.}

\begin{align*}
    (P)
    &\quad\text{maximize  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \\
    &\sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} \left(\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})<\beta_{ij} + \delta_{ij}]+\lambda_{ij}^{(r)}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})=\beta_{ij} + \delta_{ij}]\right)\\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    s.t.\quad & (1)\quad (\pi_i,w_i) \in W_i & \forall i \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    & (2)\quad f_{ij}(t_{ij})\cdot\sum_{\beta_{ij}\in \cV_{ij}} \lambda_{ij}(t_{ij},\beta_{ij}) = w_{ij}(t_{ij}) & \forall i,j,t_{ij}\in \cT_{ij}\\
    &(3) \quad \sum_i\sum_{t_{ij}\in \cT_{ij}}\pi_{ij}(t_{ij})\leq 1 & \forall j\\
    &(4) \quad \sum_{i\in[n]}\sum_{\beta_{ij} \in \cV_{ij}} \hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})> \beta_{ij}]+\hat\lambda_{ij}^{(r)}(\beta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})=\beta_{ij}] \leq \frac{1}{2} & \forall j\\
    & (5)\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \lambda_{ij}(t_{ij},\beta_{ij}) \leq  \hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})> \beta_{ij}]+\hat\lambda_{ij}^{(r)}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\beta_{ij}] & \forall i,j,\beta_{ij}\in \cV_{ij}\\
    & (6)\quad\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}^{(r)}(\beta_{ij}, \delta_{ij}),\quad \lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}^{(n)}(\beta_{ij}, \delta_{ij}) & \forall i,j, t_{ij},\beta_{ij},\delta_{ij}\\
    %& \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) &\forall i\in[n], j \in[m] \\
    & (7)\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\ \delta_{ij} \in \Delta_i}} \delta_{ij}\cdot \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \leq d_i  & \forall i,j\\
    & (8)\quad\sum_{i\in[n]} d_i \leq 8\cdot \prev \text{\todo{Change the constant if needed.}}\\
    &(9)\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta_i}} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) = 1 & \forall i,j\\
     & w_{ij}(t_{ij})\geq 0,\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})\geq 0 & \forall i,j,t_{ij},\beta_{ij},\delta_{ij}
\end{align*}

==> program_exp.tex <==
\section{Linear Program Relaxation via Lifting}\label{sec:program}
In this section, we present the linear program relaxation for computing an approximately optimal simple mechanism. The main result of our paper is as follows:

\begin{theorem}\label{thm:main XOS-main body}
Let $T=\sum_{i,j}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance (\Cref{def:bit complexity}). %~\footnote{For any instance of our problem, define \emph{the bit complexity of the problem instance}, as the maximum bit complexity of $n$,$m$,$f_{ij}(t_{ij})$ \argyrisnote{and $\alpha_{ij}^{(k)}(t_{ij})$ for XOS bidders
%over all $i,j,t_{ij}\in \cT_{ij}$}.
%See \Cref{def:bit complexity} for more details.} For XOS bidders, 
For any $\delta>0$, there exists an algorithm that computes a RPP mechanism or a TPT mechanism, such that the revenue of the mechanism is at least $c\cdot \opt$ for some absolute constant $c>0$ with probability $1-\delta-\frac{2}{n}$.
For constrained-additive valuations, our algorithm assumes query access to a value oracle and a demand oracle of bidders' valuations. For XOS valuations, our algorithm assumes query access to a value oracle and an adjustable demand oracle. The algorithm has running time $\poly(n,m,T,b,\log (1/\delta))$.
\end{theorem}

\vspace{-.05in}
{For any matroid-rank valuation, i.e., the downward-closed feasibility constraint is a matroid, the value and demand oracle can be simulated in polynomial time using greedy algorithms. For more general constraints, it is standard to assume access to the value and demand oracle. We also show that the adjustable demand oracle (rather than a demand oracle) is necessary to obtain our XOS result. In \Cref{lem:example_adjustable_oracle}, we prove that (even an approximation of) $\adem_i$ can not be implemented in polynomial time, given access to the value oracle, demand oracle, and XOS oracle
%\footnote{An oracle that outputs the additive function that achieves the value for the input set $S$. See \Cref{sec:example_adjustable_oracle} for a formal definition.}
.}


As most of the technical barriers already exist in the constrained-additive case, for exposition purposes, we focus on constrained-additive valuations in the main body (unless explicitly stated).\footnote{The linear program for XOS valuations can be found in \Cref{fig:XOSLP} in \Cref{sec:program-XOS}.} Before stating our LP, we first provide a brief recap of the existential result by Cai and Zhao~\cite{CaiZ17} summarized in \Cref{lem:caiz17-constrained-additive}.\footnote{The statement is for constrained-additive bidders. See \Cref{appx_cai-zhao} for the statement for XOS bidders.}

%\mingfeinote{I think the current definition of CORE is confusing. It didn't show the dependence between the parameter and $\sigma$ in lemma 1. Maybe we should also mention the parameter only depends on the ex-ante probability. Otherwise it's not clear why it's enough to optimize over the marginal reduced form.}
\vspace{-.05in}

\begin{definition}\label{def:core-constrained-additive}
For any $i\in [n],j\in [m]$, %let $\cV_{ij}^0 = \{ V_{ij}(t_{ij}): t_{ij} \in \cT_{ij}\}$. For 
and any feasible interim allocation $\sigma$, and non-negative numbers {$\tilde{\vBeta}=\{\tilde{\beta}_{ij}\in \cT_{ij}\}_{i\in[n],j\in[m]}$, $\vC=\{c_i\}_{i\in[n]}$} and $\vr=\{r_{ij}\}_{i\in [n],j\in [m]}\in [0,1]^{nm}$ (referred to as the dual parameters), %~\footnote{$\tilde{\vBeta}$, $\vC$, and $r$ are the dual parameters that we refer to in the introduction.}
let $\core(\sigma,\tilde{\vBeta},\vC,\vr)$ be the welfare under allocation $\sigma$ truncated at $\tilde{\beta}_{ij}+c_i$ for every $i,j$.
~Formally, $$
\core(\sigma,\tilde{\vBeta},\vC,\vr)=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \left(\ind[t_{ij}< \tilde{\beta}_{ij}+c_i]+r_{ij}\cdot \ind[t_{ij}= \tilde{\beta}_{ij}+c_i] \right).$$
\notshow{
if the bidders have constrained-additive valuations, and
$$\core(\sigma,\tilde{\vBeta},\vC,\vr)=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}\gamma_{ij}^S(t_i)\cdot \left(\ind[V_{ij}(t_{ij})< \tilde{\beta}_{ij}+c_i]+r_{ij}\ind[V_{ij}(t_{ij})= \tilde{\beta}_{ij}+c_i] \right)$$ if the bidders have XOS valuations.
Here $\gamma_{ij}^S(t_i)=\alpha_{ij}^{k^*(t_i,S)}(t_{ij})$, where $\displaystyle k^*(t_i,S)=\arg\max_{k\in[K]}\big(\sum_{j\in S}\alpha^k_{ij}(t_{ij})\big)$.
}
\end{definition}

\begin{lemma}\cite{CaiZ17}\label{lem:caiz17-constrained-additive}
Given any BIC and IR mechanism $\cM$ with interim allocation $\sigma$,  
%\textbf{(i)} a feasible interim allocation $\sigma$,\footnote{Note that when bidders have constrained-additive valuations, it suffice to take $\sigma$ to be the interim allocation rule of $\cM$. For XOS valuations, $\sigma$ will be the interim allocation of a modified version of $\cM$. See Section~5 in~\cite{CaiZ16a} for details.} 
where $\sigma_{iS}(t_i)$ is the interim probability for bidder $i$ to receive exactly bundle $S$ when her type is $t_i$, there exist %\textbf{(i)} 
non-negative numbers {$\tilde{\vBeta}^{(\sigma)}=\{\tilde{\beta}_{ij}^{(\sigma)}\in \cT_{ij}\}_{i\in[n],j\in[m]}$, $\vC^{(\sigma)}=\{c_i^{(\sigma)}\}_{i\in[n]}$} %\argyrisnote{can we say instead $\{\tilde{\beta}_{ij}\in \cV_{ij}^0\}_{i,j}, \{c_i\}_{i\in[n]}$?}
 and $\vr^{(\sigma)}\in [0,1]^{nm}$ that satisfy\footnote{\cite{CaiZ17} provides an explicit way to calculate $\tilde{\vBeta}^{(\sigma)}, \vC^{(\sigma)}, \vr^{(\sigma)}$. We only include the crucial properties of these parameters here.} %and \textbf{(ii)} a two-part tariff mechanism $\cM_1^{(\sigma)}$ such that %\yangnote{Yang: We need to make sure all the $\tilde{\beta}_{ij}$ are in $\cV_{ij}$ and all $c_i$ are in $\Delta_i$. I think it's fine to say $\tilde{\beta}_{ij}\in \cV^0_{ij}$, and we only choose $c_i$'s such that for at least one item $j$, $\tilde{\beta}_{ij}+c_i \in \cV^0_{ij}$.}
\begin{enumerate}
    \item $\sum_{i\in[n]} \left(\Pr_{t_{ij}}[t_{ij}>\tilde\beta_{ij}^{(\sigma)}]+r_{ij}^{(\sigma)}\cdot \Pr_{t_{ij}}[t_{ij}=\tilde\beta_{ij}^{(\sigma)}]\right)\leq \frac{1}{2}$,
    \item $\frac{1}{2}\cdot\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\sigma_{iS}(t_i)\leq \Pr_{t_{ij}}[t_{ij}>\tilde\beta_{ij}^{(\sigma)}]+r_{ij}^{(\sigma)}\cdot \Pr_{t_{ij}}[t_{ij}=\tilde\beta_{ij}^{(\sigma)}],\forall i,j$,
    %\item $\rev(\cM)\leq 28\cdot \prev+4\cdot\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$.
    \item $\sum_{i\in [n]} c_i^{(\sigma)}\leq 8\cdot \prev$,
    %\item $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})\leq 64\cdot \prev + 8\cdot \rev(\cM_1^{(\sigma)})$.
\end{enumerate}
and the corresponding $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$ satisfies the following inequalities:
\begin{enumerate}\addtocounter{enumi}{3}
    \item $\rev(\cM)\leq 28\cdot \prev+4\cdot\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$,
    \item $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})\leq 64\cdot \prev + 8\cdot \rev(\cM_1^{(\sigma)})$, where $\cM_1^{(\sigma)}$ is some TPT mechanism.
\end{enumerate}
\end{lemma}


\begin{remark}\label{remark:tie-breaking}
For continuous type distributions, there exists $\tilde{\vBeta}^{(\sigma)}$ that satisfy both Property 1 and 2 of \Cref{lem:caiz17-constrained-additive} with $r_{ij}^{(\sigma)}=1,\forall i,j$ for every $\sigma$. For discrete distributions, such a $\tilde{\vBeta}^{(\sigma)}$ may not exist. This is simply a tie-breaking issue, and the role of $\vr^{(\sigma)}$ is to fix it. Roughly speaking, $r_{ij}^{(\sigma)}$ is the probability that bidder $i$ wins item $j$, when she is indifferent between purchasing or not. Readers can treat $\vr^{(\sigma)}$ as the all-one vector to get the intuition behind our approach.%\yangnote{Yang: I'm not sure if we should include the last sentence. I'm concerned that someone may think this gives an additive error, so the whole result is not multiplicative.} It can be implemented by a random rebate that loses an arbitrarily small fraction of the revenue. See~\cite{CaiZ17} for details.
%\mingfeinote{Remark about the rebate ratio r.}
\end{remark}

%\argyrisnote{I think the first two constraints are not immediately implied by the paper, but they are implied by the proof of Lemma~5 in \cite{CaiZ17}. Could this be an issue? \yangnote{That's fine.}I also think that $\sum_i c_i$ could be $8\prev + \epsilon$ since rebate might also be used there, so maybe we can relax \MarginalToGlobalConstraint to $\sum_i c_i < 9 \prev$? I also think if we change the notation of $W_i$ to be the one with the $\alpha_j^k$, we might also need to include information about them.}

By combining Property 4 and 5 of \Cref{lem:caiz17-constrained-additive}, Cai and Zhao~\cite{CaiZ17} proved that the revenue of any BIC, IR mechanism $\cM$ is bounded by a constant number of $\prev$ and the revenue of some TPT mechanism.
%for any BIC, IR mechanism $\cM$, the term $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},r^{(\sigma)})$ is bounded by a constant number of $\prev$ plus a constant times the revenue of some two-part tariff mechanisms. And thus by Property 3 of \Cref{lem:caiz17}, the optimal revenue can be bounded using $\prev$ and the revenue of two-part tariff.
Recall that $\prev$ is the optimal revenue achieved by an RPP mechanism, which is exactly the Sequential Posted Price mechanism if we restrict the bidders' valuations to unit-demand. Thus we can compute a set of posted prices that approximates $\prev$ by Chawla et al.~\cite{ChawlaHMS09}.  
%\yangnote{Yang: Let's move it to a later section. I don't think our first theorem should be something by others.}\mingfeinote{How about we change it to ``Lemma'' and move it to the beginning of Sec 3.2? I found it hard to move to after our first theorem, since the RPP mechanism in the statement is refering to this one.}
%\argyrisnote{Argyris: I think Theorem~\ref{thm:chms10} works when we only have sample-access to the agents distribution. If that is the case we should emphasize it.}\yangnote{Yang: But you need to pay an $\varepsilon H$ additive error.}

\subsection{Tour to Our Relaxation}\label{sec:tour to LP}
To facilitate our discussion about the key components and the intuition behind the relaxation, we present the development of our relaxation and along the way examine several failed attempts. In~\Cref{thm:bounding-lp-simple-mech}, we show that the optimal solution of the relaxed problem can indeed be approximated by simple mechanisms. Due to space limitations, we do not include details on the approximation analysis in this section, but focus on our intuition behind each step of our relaxation. Interested readers can find the proof of~\Cref{thm:bounding-lp-simple-mech} in~\Cref{sec:proof of bounding LP with simple mech}. We also assume $r_{ij}$ to be $1$ for every $i$ and~$j$ to keep the notation light. %We focus on the case where the bidders are constrained-additive. 

\vspace{-.18in}
\paragraph{Step 0: Replace Revenue with the Duality-Based Benchmark.}%\label{par:existing approach}
Instead of optimizing the revenue, we optimize the upper bound of revenue. As guaranteed by \Cref{lem:caiz17-constrained-additive}, for any BIC and IR mechanism $\cM=(\sigma,p)$, its revenue is upper bounded by $O(\prev+\core(\sigma,\theta(\sigma)))$, where we use $\theta(\sigma)$ to denote the set of  dual parameters $(\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)})$ guaranteed to exist by~\Cref{lem:caiz17-constrained-additive}. %$(\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$. 
Since we can approximate $\prev$, it suffices to first approximately maximize $\core(\sigma,\theta(\sigma))$ over all feasible interim allocations $\sigma$, then compute the TPT in \Cref{lem:caiz17-constrained-additive} based on the computed $\sigma$. $\core(\sigma,\theta(\sigma))$ is the truncated welfare, but the truncation depends on $\sigma$ in a complex way, causing the function to be highly non-concave in $\sigma$ (\Cref{ex:non-concave interim}). 

%Our starting point is the existential result from~\cite{CaiZ17}. With \Cref{thm:chms10}, the only non-constructive part is to compute a two-part tariff that generates high revenue.  It's unclear how to find the (approximately) optimal TPT among this class, as there are exponentially many parameters associated with a TPT and the revenue of a TPT replies on the parameters in a highly complex and non-convex way. 
%It's  not surprised that finding the best posted prices and entry fees (even if the entry fee is always 0) among this class is NP-hard. So a natural idea is to compute the particular TPT used in the proof of \Cref{lem:caiz17}. However, the parameters associated with the TPT depends on the mechanism $\cM$ (or the interim allocation $\sigma$) we are considering. Therefore, in order to compute a TPT that is approximately optimal, we need access to a mechanism $\cM$ that is itself approximately optimal.

%As we discuss in \Cref{subsec:technique}, a natural attempt is to optimize the~\core~over allocations. By Property 3 and 5 of \Cref{lem:caiz17-constrained-additive}, for any BIC, IR mechanism $\cM$ with interim allocation $\sigma$, there exists a set of dual parameters $(\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$ depending on $\sigma$, such that: (i) $O(\prev+\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)}))$ is a benchmark of $\rev(\cM)$, and (ii) it is bounded by simple mechanisms. 

%For ease of notations, we denote $\theta(\sigma)=(\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$ the set of parameters. Then to obtain a two-part tariff that achieves good revenue, one approach is to (approximately) maximize $\core(\sigma,\theta(\sigma))$ over all feasible interim allocations $\sigma$, and compute the TPT in \Cref{lem:caiz17-constrained-additive} using $\sigma$. For symmetric bidders, this optimization problem can be solved efficiently by exploiting the symmetry, but it is unclear how to solve it efficiently for asymmetric bidders~\cite{ChawlaM16, CaiZ17}. 


%Indeed, since the dual parameters $\theta$ only depend on the ex-ante allocation probabilities of $\sigma$, this approach is related to the \emph{ex-ante relaxation} technique widely used in the mechanism design literature~\cite{Alaei11,ChawlaHMS10, ChawlaM16}.~\footnote{ The ex-ante relaxation decouples the allocation problem for multiple bidders by only enforcing supply constraints over the ex-ante probabilities.} For symmetric bidders, the ex-ante relaxation can be solve efficiently by exploiting the symmetry, but it is unclear how to solve it efficiently for asymmetric bidders~\cite{ChawlaM16, CaiZ17}. % and the allocations that satisfy the ex-ante constraints. 


%\yangnote{For symmetric bidders, we can apply this observation and show that there is a single set of dual parameters that satisfies the requirements in Lemma~\ref{lem:caiz17} for the ex-ante probabilities of all symmetric allocations. As bidders are symmetric, it suffices to consider symmetric allocations, and one only needs to optimize the \core~with respect to this specific set of dual parameters.} However, for asymmetric bidders, it is unclear how to compute an (approximately) optimal ex-ante probabilities efficiently. %\mingfeinote{Here I'm referring to the discussion about ex-ante relaxation in the introduction.}      

\vspace{-.15in}
\paragraph{Step 1: Two-Stage Optimization.}
To overcome the barrier mentioned above, we consider a two-stage optimization problem (\Cref{fig:LP-fixed-parameter}) by \emph{switching the order of dependence} between the interim allocation $\sigma$ and dual parameters $\theta=(\vBeta,\vC)$. In Stage I, we optimize some function $H$ over the dual parameters $\theta=(\vBeta,\vC)$, where $H(\vBeta,\vC)$ is the optimum of the Stage II problem for every fixed set of parameters $(\vBeta,\vC)$. Constraint {\BetaConstraintFP} and {\CiConstraintFP} in the Stage I problem are due to Property 1 and 3 of \Cref{lem:caiz17-constrained-additive} respectively. In Stage II, for any fixed set of parameters $\theta=(\vBeta,\vC)$, we optimize $\core(\sigma,\theta)$ over all feasible $\sigma$ such that the tuple $(\sigma,\vBeta,\vC)$ satisfy Property 1, 2, and 3 of \Cref{lem:caiz17-constrained-additive}. We choose  the interim allocation $\sigma$ as the variables, $\core(\sigma,\vBeta,\vC)$ as the objective, and include Constraint {\WBetaConstraintFP}, which corresponds to Property 2 of \Cref{lem:caiz17-constrained-additive}. Why is the two-stage optimization a relaxation? For any interim allocation $\sigma$, (i) the corresponding set of dual parameters $\theta(\sigma)$ is a feasible solution of the first-stage optimization problem, and (ii) $\sigma$ is feasible in the second-stage optimization w.r.t. $\theta(\sigma)$, so $(\theta(\sigma),\sigma)$ is a feasible solution of the two-stage optimization problem.
%It's not hard to see that the two-stage problem is equivalent to the problem of maximizing $\core(\sigma,\theta(\sigma))$ over all feasible $\sigma$.
\vspace{-.1in}

\begin{figure}[H]
\colorbox{MyGray}{
\noindent
\begin{minipage}{.37\textwidth}
\small
\textbf{Stage I:}
$$\textbf{max } H(\vBeta,\vC)$$
\begin{align*}
\textbf{s.t.} &\quad\BetaConstraintFP\quad\sum_{i\in [n]}\Pr_{t_{ij}}[t_{ij}\geq \beta_{ij}]\leq\frac{1}{2}\qquad \forall j\\
&\quad\CiConstraintFP\quad\sum_{i\in[n]} c_i \leq 8\cdot \prev
\end{align*}
\end{minipage}
\hfill\vline\hfill

\begin{minipage}{.60\textwidth}
\small
\textbf{~~Stage II:}
$${H(\vBeta,\vC)=}\textbf{max  } \sum_{i\in [n]}\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij} + c_i]$$
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
\vspace{-.3in}
  \begin{align*}
\textbf{s.t.} &\quad\WConstraintFP \quad \text{$\sigma$ is feasible} \\
&\quad\WBetaConstraintFP\quad\frac{1}{2}\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S:j\in S}\sigma_{iS}(t_i)\leq\Pr_{t_{ij}}[t_{ij}\geq \beta_{ij}] & \forall i,j\\
\end{align*}
\end{minipage}
}
\vspace{-.15in}

\caption{Two-stage Optimization over $\theta=(\vBeta,\vC)$ and the allocation $\sigma$
%The LP to Maximize $\core$ for Fixed Parameters $\theta=(\vBeta,\vC)$ and the Constraints on $\theta$
}~\label{fig:LP-fixed-parameter}
\vspace{-.3in}
\end{figure}

%Unfortunately, we do not know how to solve the two-stage optimization problem efficiently, as the number of dual parameters is exponential in $n$ and $m$, enumerating through all possible dual parameters is not an option. To overcome this obstacle, we need ideas explained in the following step.

We now focus on the Stage II problem and try to solve it efficiently for a fixed set of parameters $\theta$. The objective is a linear function of the variables $\sigma$, yet the set of variables $\sigma=\{\sigma_{iS}(t_i)\}_{i\in [n], S\subseteq [m], t_i\in \cT_i}$ has exponential size. Luckily, the problem can be expressed more succinctly. For any interim allocation $\sigma$ and dual parameters $\theta=(\vBeta,\vC)$, the objective ($\core(\sigma,\theta)$) can be simplified as follows: 
{
\begin{equation}\label{equ:core-marginal}
\begin{aligned}
\core(\sigma,\theta)&=\sum_{\substack{i\in [n]\\ t_i\in \cT_i}}f_i(t_i) \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij}+c_i]
%\core(\sigma,\theta)&=\sum_{i\in [n]}\sum_{t_i\in \cT_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij}+c_i] \\
%\core(\sigma,\theta)&=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \left(\ind[t_{ij}< \tilde{\beta}_{ij}+c_i]+r_{ij}\cdot \ind[t_{ij}= \tilde{\beta}_{ij}+c_i] \right)\\
&=\sum_{\substack{i\in [n], j\in [m]\\t_{ij}\in \cT_{ij}}} \widehat{w}_{ij}(t_{ij})t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij}+c_i],
%&=\sum_{i\in [n]}\sum_{j\in [m]}\sum_{t_{ij}\in \cT_{ij}} \widehat{w}_{ij}(t_{ij})\cdot t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij}+c_i],
%&=\sum_i\sum_j\sum_{t_{ij}} \widehat{w}_{ij}(t_{ij})\cdot t_{ij}\cdot \left(\ind[t_{ij}< \tilde{\beta}_{ij}+c_i]+r_{ij}\cdot \ind[t_{ij}= \tilde{\beta}_{ij}+c_i] \right),
\end{aligned}
\end{equation}
}
\vspace{-.15in}

\noindent where $\widehat{w}_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sigma_{iS}(t_{ij},t_{i,-j})$ for every $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We refer to $\{\widehat{w}_{ij}(t_{ij})\}_{i\in [n],j\in [m],t_{ij}\in \cT_{ij}}$ as the \textbf{marginal reduced form} of the interim allocation rule $\sigma$. $\widehat{w}_{ij}(t_{ij})$ represents the probability that bidder $i$'s value for item $j$ is $t_{ij}$ and she receives item $j$, and the probability is taken over the randomness of the allocation, other bidders' types, as well as her own values for all the other items. Now for every fixed dual parameters $\theta$, $\core$ is expressed as a linear function of the much more succinct representation $\widehat{w}=\{\widehat{w}_{ij}(t_{ij})\}_{i, j,t_{ij}}$ that has polynomial description size. We rewrite the Stage II problem as an LP using the variables $\widehat{w}$.
Denote $\core(\hat{w},\theta)$ the last term of \Cref{equ:core-marginal}, which is the objective of the problem. By the definition of $\widehat{w}$, Constraint {\WBetaConstraintFP} is equivalent to
%For a given $\theta$, the only constraint on the allocation, i.e., Property 2 of \Cref{lem:caiz17-constrained-additive}, can also be expressed as a linear constraint on $\widehat{w}$:
\vspace{-.1in}

\begin{equation}\label{equ:constraints_on_w}
\frac{1}{2}\cdot\sum_{t_{ij}\in \cT_{ij}}\widehat{w}_{ij}(t_{ij})\leq
\Pr_{t_{ij}}[t_{ij}\geq \tilde\beta_{ij}],\qquad\forall i,j    
%\frac{1}{2}\cdot\sum_{t_{ij}\in \cT_{ij}}\widehat{w}_{ij}(t_{ij})\leq\Pr_{t_{ij}}[t_{ij}>\tilde\beta_{ij}]+r_{ij}\cdot \Pr_{t_{ij}}[t_{ij}=\tilde\beta_{ij}],\qquad\forall i,j    
\end{equation}
\vspace{-.1in}

\noindent which is a linear constraint on $\widehat{w}$. Let $\cP_1$ be the convex polytope that contains all marginal reduced forms $\widehat{w}$ that can be implemented by some feasible allocation $\sigma$ (corresponds to Constraint {\WConstraintFP}) and $\cP_2$ be the set of all  $\widehat{w}$ that satisfy all constraints in \Cref{equ:constraints_on_w}. The Stage II problem is equivalent to the LP $\max_{\widehat{w}\in \cP_1\cap \cP_2}\core(\widehat{w},\theta)$. Unfortunately, since $\cP_1$ does not have an explicit succinct description or an efficient separation oracle, it is unclear if the problem can be solved efficiently.





\notshow{

\vspace{-.15in}
\paragraph{Step 1: Optimizing over a fixed set of dual parameters $\theta$.}
To optimize $\core(\sigma,\theta(\sigma))$, %it seems natural to first obtain a good allocation $\sigma$ and then determine the corresponding dual parameters $\theta(\sigma)$ and the TPT mechanism. However, it is unclear how to find a good allocation $\sigma$ efficiently, as $\theta(\sigma)$ depends on $\sigma$ in a highly complex way.
our first insight is to \emph{switch the order of dependence}, and choose a set of dual parameters $\theta$ first then optimize over the allocation. In particular, we aim to maximize $\core(\sigma,\theta)$ for every set of dual parameters $\theta$. We notice that for any interim allocation $\sigma$ and dual parameters $\theta=(\tilde{\vBeta},\vC)$,
%$\theta=(\tilde{\vBeta},\vC,\vr)$,
$\core(\sigma,\theta)$ can be simplified as follows: 

\vspace{-.1in}
\begin{equation}\label{equ:core-marginal}
\begin{aligned}
\core(\sigma,\theta)&=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \ind[t_{ij}\leq \tilde{\beta}_{ij}+c_i] \\
%\core(\sigma,\theta)&=\sum_i\sum_{t_i}f_i(t_i)\cdot \sum_{S\subseteq [m]}\sigma_{iS}(t_i)\sum_{j\in S}t_{ij}\cdot \left(\ind[t_{ij}< \tilde{\beta}_{ij}+c_i]+r_{ij}\cdot \ind[t_{ij}= \tilde{\beta}_{ij}+c_i] \right)\\
&=\sum_i\sum_j\sum_{t_{ij}} \widehat{w}_{ij}(t_{ij})\cdot t_{ij}\cdot \ind[t_{ij}\leq \tilde{\beta}_{ij}+c_i],
%&=\sum_i\sum_j\sum_{t_{ij}} \widehat{w}_{ij}(t_{ij})\cdot t_{ij}\cdot \left(\ind[t_{ij}< \tilde{\beta}_{ij}+c_i]+r_{ij}\cdot \ind[t_{ij}= \tilde{\beta}_{ij}+c_i] \right),
\end{aligned}
\end{equation}
\vspace{-.15in}

\noindent where $\widehat{w}_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sigma_{iS}(t_{ij},t_{i,-j})$ for every $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We refer to $\{\widehat{w}_{ij}(t_{ij})\}_{i\in [n],j\in [m],t_{ij}\in \cT_{ij}}$ as the \textbf{marginal reduced form} of the interim allocation rule $\sigma$. $\widehat{w}_{ij}(t_{ij})$ represents the probability that bidder $i$'s value for item $j$ is $t_{ij}$ and she receives item $j$. The probability is taken over the randomness of the allocation, other bidders' types, as well as her own values for all the other items.

Now for every fixed dual parameters $\theta$, $\core$ can still be written as a linear function of the much more succinct representation $\widehat{w}=\{\widehat{w}_{ij}(t_{ij})\}_{i, j,t_{ij}}$ (compared to the interim allocation $\sigma$). We denote $\core(\hat{w},\theta)$ the last term of \Cref{equ:core-marginal}. For a given $\theta$, the only constraint on the allocation, i.e., Property 2 of \Cref{lem:caiz17-constrained-additive}, can also be expressed as a linear constraint on $\widehat{w}$:
\vspace{-.1in}

\begin{equation}\label{equ:constraints_on_w}
\frac{1}{2}\cdot\sum_{t_{ij}\in \cT_{ij}}\widehat{w}_{ij}(t_{ij})\leq
\Pr_{t_{ij}}[t_{ij}\geq \tilde\beta_{ij}],\qquad\forall i,j    
%\frac{1}{2}\cdot\sum_{t_{ij}\in \cT_{ij}}\widehat{w}_{ij}(t_{ij})\leq\Pr_{t_{ij}}[t_{ij}>\tilde\beta_{ij}]+r_{ij}\cdot \Pr_{t_{ij}}[t_{ij}=\tilde\beta_{ij}],\qquad\forall i,j    
\end{equation}
\vspace{-.15in}

\noindent Let $\cP_1$ be the convex polytope that contains all marginal reduced forms $\widehat{w}$ that can be implemented by some feasible allocation $\sigma$, and $\cP_2$ be the set of all  $\widehat{w}$ that satisfy all constraints in \Cref{equ:constraints_on_w}. To maximize $\core(\sigma,\theta)$, it suffices to solve $\max_{\widehat{w}\in \cP_1\cap \cP_2}\core(\widehat{w},\theta)$. Unfortunately, $\cP_1$ does not have an explicit succinct description or an efficient separation oracle. 

%use a succinct set of constraints to guarantee that $\widehat{w}$ can be implemented by a feasible allocation $\sigma$, or  %in $\cP$, a feasible $\widehat{w}$ must satisfy some constraints that are global across all bidders, to respect the ``no over-allocating'' constraint for each item, in a feasible allocation among all bidders. Thus for general constrained-additive valuations, it's unclear if there is an explicit description of $\cP$, nor if there is an efficient separation oracle using only demand queries. 

%In order to have an efficient separation oracle of the feasible region of $\widehat{w}$ using demand oracle, 


%\paragraph{Reduced Form.} The reduced form of a mechanism $\cM$ is a vector of numbers\\ $\{\bar{\sigma}_{ij}(t_i)\}_{i\in [n],j\in [m],t_i\in \cT_i}$, where $\bar{\sigma}_{ij}(t_i)$ is the probability that bidder $i$ receives item $j$ when reporting type $t_i$, over the randomness of $\cM$ and other bidders' types. Given the interim allocation $\sigma$ of $\cM$, we have $\bar{\sigma}_{ij}(t_i)=\sum_{S:j\in S}\sigma_{iS}(t_i)$. 

}


\vspace{-.15in}
\paragraph{Step 2: Marginal Reduced Form Relaxation.} To overcome this barrier, we consider a relaxation of $\cP_1$, where the feasibility constraint is only enforced on each bidder separately. 
We refer to this step as the \emph{marginal reduced~form~relaxation}. We use $\widehat{w}_i=\{\widehat{w}_{ij}(t_{ij})\}_{j\in [m],t_{ij}\in \cT_{ij}}$ to denote a feasible \emph{single-bidder marginal reduced form} for bidder $i$.  %For every $i\in [n]$, the \emph{marginal reduced form} of bidder $i$ is a vector of numbers $\widehat{w}_i=\{\widehat{w}_{ij}(t_{ij})\}_{j\in [m],t_{ij}\in \cT_{ij}}$, where $\widehat{w}_{ij}(t_{ij})$ is $f_{ij}(t_{ij})$ times the probability that bidder $i$ receives item $j$ conditioned on her value for this item being $t_{ij}$, under any feasible allocation for bidder $i$.\footnote{A feasible allocation for a single bidder $i$ is for every reported type $t_i$, returns a (random) feasible set $S\in \cF_i$.}
Formally, we define the feasible region $W_i$ of $\widehat{w}_i$ in~Definition~\ref{def:W_i-constrained-add}.  

%We notice that for any interim allocation $\sigma$ and parameters $(\tilde{\vBeta},\vC,r)$, we have


%Denote $\core(w,\theta(w))$ the last term of \Cref{equ:core-marginal}, where $\theta(w)$ is the parameter stated in \Cref{lem:caiz17} that only depends on $w$. Now it's sufficient to maximize $\core(w,\theta(w))$ over all feasible $w$, where the number of variables in the program is $\poly(n,m,\sum_{i,j}|\cT_{ij}|)$. Unfortunately, the parameters $\theta(w)$ depends on $w$ in a non-linear way and thus it's unclear how to find the optimal $w$ efficiently. 

%\vspace{-.1in}

\begin{definition}[Constrained-additive valuations: single-bidder marginal reduced form polytope]\label{def:W_i-constrained-add}
For every $i\in [n]$, suppose bidder $i$ has a constrained-additive valuation with feasibility constraint $\cF_i$. Bidder $i$'s single-bidder marginal reduced form polytope $W_i\subseteq [0,1]^{\sum_{j\in[m]}|\cT_{ij}|}$ is defined as follows: $\widehat{w}_i\in W_i$ if and only if there exists an allocation rule $\{\sigma_S(t_i)\}_{t_i\in \cT_i, S\in \cF_i}$, i.e., $\sigma_S(t_i)$ is the probability that $i$ receives set $S$ when her type is $t_i$, such that
\textbf{(i)} $\sum_{S\in \cF_i}\sigma_S(t_i)\leq 1$, $\forall t_i\in \cT_i$, and \textbf{(ii)}
$\widehat{w}_{ij}(t_{ij})=f_{ij}(t_{ij})\cdot\sum_{t_{i,-j}}f_{i,-j}(t_{i,-j})\cdot \sum_{S:j\in S}\sigma_S(t_i)$, for all $j\in[m]$ and $t_{ij}\in \cT_{ij}$.
\end{definition}

\noindent Throughout this section, we assume access to a separation oracle of $W_i$ for every bidder $i$. In \Cref{thm:multiplicative approx for constraint additive-main body}, we present an efficient separation oracle for another polytope $\widehat{W}_i$ that is a multiplicative approximation to $W_i$, i.e., $\widehat{W}_i$ is sandwiched between $c\cdot W_i$ and $W_i$ for some absolute constant $c\in(0,1)$, using only queries to bidder $i$'s demand oracle. We will argue later that we can efficiently approximate our problem with the separation oracle for $\widehat{W}_i$. 

Here is our relaxation {to the (rewritten) Stage II problem}: Instead of forcing $\widehat{w}$ to be \emph{implementable jointly} ($\widehat{w}\in \cP_1$), we consider the relaxed region $\cP'\supseteq \cP_1$: $\widehat{w}\in \cP'$ if and only if: (i) $\widehat{w}_i
%=\{\widehat{w}_{ij}(t_{ij})\}_{j\in [m],t_{ij}\in \cT_{ij}}
\in W_i$, for all bidder $i\in [n]$, and (ii) $\sum_{i}\sum_{t_{ij}}\widehat{w}_{ij}(t_{ij})\leq 1,\forall j\in [m]$. %, and (iii) $\widehat{w}$ satisfies all constraints in \Cref{equ:constraints_on_w}. 
In other words, $\cP'$ guarantees that, for every bidder $i$, $\widehat{w}_i$ is a feasible single-bidder marginal reduced form for $i$, and the supply constraint is met in terms of marginal reduced forms (rather than ex-post allocations).
%~\footnote{We show in \Cref{lem:lower bounding mu} that the analysis of Cai and Zhao~\cite{CaiZ17} is robust to this relaxation, that is, $\core(\widehat{w},\theta)$ can still be bounded with RPP and TPT mechanisms, even when $\widehat{w}$ is in the relaxed region $\cP'\cap \cP_2$. \yangnote{Yang: Do we want this sentence? We didn't talk about how to bound the Core until this point.}\mingfeinote{I would prefer to keep it here. In Lemma 1 we mentioned that in CZ, core can be bound with Properties 1-3 and here we are doing a relaxation. Readers may wonder why we can do such a relaxation. }\yangnote{Yang: Step 1 and 3 are also relaxations, but we don't talk about how to bound the Core after those relaxations.}} 

\begin{figure}[ht!]
\colorbox{MyGray}{
\noindent
\begin{minipage}{.97\textwidth}
\small
\textbf{~~Relaxed Stage II:}
$${H(\vBeta,\vC)=}\textbf{max  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}} \widehat{w}_{ij}(t_{ij})\cdot t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij} + c_i]$$
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
\vspace{-.3in}
  \begin{align*}
\textbf{s.t.} &\quad\WConstraintFP \quad \widehat{w}_i \in W_i & \forall i \\
&\quad\WBetaConstraintFP\quad\frac{1}{2}\sum_{t_{ij}}\widehat{w}_{ij}(t_{ij})\leq\Pr_{t_{ij}}[t_{ij}\geq \beta_{ij}] & \forall i,j\\
& \qquad\quad~\widehat{w}_{ij}(t_{ij})\geq 0 & \forall i,j,t_{ij}
\end{align*}
\end{minipage}
}
\caption{The Relaxed Stage II Problem over the Marginal Reduced Forms
}~\label{fig:LP-relaxed-stageii}
\vspace{-.25in}
\end{figure}

\noindent The main benefit of this relaxation is computational. Without the relaxation, we need a multiplicative approximation of $\cP_1$. \Cref{thm:multiplicative approx for constraint additive-main body} provides such an approximation if we can exactly maximizes the social welfare -- a computational task that is substantially harder than answering demand queries. Indeed, we are not aware of any efficient algorithm that exactly maximizes the social welfare with only access to demand oracles of every bidder. 
%The sampling technique from~\cite{CaiDW12b} is not suitable to approximate $\cP_1$, as it needs to efficiently maximizes the social welfare -- a task that no no such algorithm has been proposed that only requires query access~to~demand~oracles.} 
The relaxed problem $\max_{\widehat{w}\in \cP'\cap \cP_2}\core(\widehat{w},\theta)$ is captured by the LP in \Cref{fig:LP-relaxed-stageii}.\footnote{We omit the supply constraint $\sum_{i}\sum_{t_{ij}}\widehat{w}_{ij}(t_{ij})\leq 1$ as it is implied by Constraint~\BetaConstraintFP~in the Stage I problem and Constraint~\WBetaConstraintFP.}



Consider the two-stage optimization with the relaxed Stage II problem. %It is a relaxation of the original two-stage problem in \Cref{fig:LP-fixed-parameter} as well. 
For every fixed parameters $\theta$, the relaxed Stage II problem can be solved efficiently (assuming a separation oracle of $W_i$ for every $i$). Unfortunately, we do not know how to solve the two-stage optimization problem efficiently, as the number of different dual parameters is exponential in $n$ and $m$, and enumerating through all possible choices of dual parameters is not an option. To overcome this obstacle, we need ideas explained in the following step.


\notshow{
\vspace{-.15in}
\paragraph{Step 3: Two-Stage Optimization.}
In this step, we obtain a two-stage optimization problem that is a relaxation of the original problem. For a fixed set of dual parameters $\theta=(\vBeta,\vC)$, we now know that the relaxed problem $\max_{\widehat{w}\in \cP'\cap \cP_2}\core(\widehat{w},\theta)$ can be captured by a linear program shown on the RHS of \Cref{fig:LP-fixed-parameter}. This is the second-stage optimization of our problem, and we denote the optimal solution of this LP by $H(\theta)$. In the first-stage optimization, we find the optimal dual parameter $\theta$ that maximizes $H(\theta)$. To make sure this optimum can still be approximated by simple mechanisms, we need to pose certain constraints on $\theta$, that is, they need to respect Constraints \BetaConstraintFP~ and~\CiConstraintFP~corresponding to property 1 and 4 of \Cref{lem:caiz17-constrained-additive}.~\footnote{We ignore the supply constraint $\sum_{i}\sum_{t_{ij}}\widehat{w}_{ij}(t_{ij})\leq 1$ in the LP as it is implied by Constraints~\WBetaConstraintFP~and~\BetaConstraintFP.} 

%and define the set $\Theta$ of the dual parameters we need to consider. Note that these two constraints are not part of the LP, but they are necessary to guarantee that the optimum of the LP can be bounded using simple mechanisms.  In the LP, Constraint \WBetaConstraintFP~  corresponds to Property 2 of \Cref{lem:caiz17-constrained-additive}. 

%Now the relaxed problem $\max_{\widehat{w}\in \cP'\cap \cP_2}\core(\widehat{w},\theta)$ can be captured by a linear program shown in \Cref{fig:LP-fixed-parameter}.\footnote{For simplicity, we ignore the tie-breaking issue mentioned in~\Cref{remark:tie-breaking} here and assume $r_{ij}$ to be always 1 for every $i$ and $j$.} Constraints \BetaConstraintFP~ and~\CiConstraintFP~correspond to property 1 and 4 of \Cref{lem:caiz17-constrained-additive} and define the set $\Theta$ of the dual parameters we need to consider. Note that these two constraints are not part of the LP, but they are necessary to guarantee that the optimum of the LP can be bounded using simple mechanisms.  In the LP, Constraint \WBetaConstraintFP~  corresponds to Property 2 of \Cref{lem:caiz17-constrained-additive}. We ignore the supply constraint $\sum_{i}\sum_{t_{ij}}\widehat{w}_{ij}(t_{ij})\leq 1$ in the LP as it is implied by Constraints~\WBetaConstraintFP~and~\BetaConstraintFP.

\begin{figure}[ht!]
\colorbox{MyGray}{
\noindent
\begin{minipage}{.37\textwidth}
\small
\textbf{Stage I:}
$$\textbf{max } H(\vBeta,\vC)$$
\begin{align*}
s.t. &\quad\BetaConstraintFP\quad\sum_{i\in [n]}\Pr_{t_{ij}}[t_{ij}\geq \beta_{ij}]\leq\frac{1}{2}\qquad \forall j\\
&\quad\CiConstraintFP\quad\sum_{i\in[n]} c_i \leq 8\cdot \prev
\end{align*}
\end{minipage}
\hfill\vline\hfill

\begin{minipage}{.59\textwidth}
\small
\textbf{~~Stage II:}
$${H(\vBeta,\vC)=}\textbf{max  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}} \widehat{w}_{ij}(t_{ij})\cdot t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij} + c_i]$$
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
\vspace{-.3in}
  \begin{align*}
s.t. &\quad\WConstraintFP \quad \widehat{w}_i \in W_i & \forall i \\
&\quad\WBetaConstraintFP\quad\frac{1}{2}\sum_{t_{ij}}\widehat{w}_{ij}(t_{ij})\leq\Pr_{t_{ij}}[t_{ij}\geq \beta_{ij}] & \forall i,j\\
& \qquad\quad~\widehat{w}_{ij}(t_{ij})\geq 0 & \forall i,j,t_{ij}
\end{align*}
\end{minipage}
}
\caption{Two-stage Optimization over $\theta=(\vBeta,\vC)$ and the Marginal Reduced Forms
%The LP to Maximize $\core$ for Fixed Parameters $\theta=(\vBeta,\vC)$ and the Constraints on $\theta$
}~\label{fig:LP-fixed-parameter}
\vspace{-.3in}
\end{figure}

\noindent Why is the two-stage optimization a relaxation? First, for any interim allocation $\sigma$, the corresponding set of dual parameters $\theta(\sigma)$ is a feasible solution of the first-stage optimization problem. Second, for any interim allocation $\sigma$, its corresponding marginal reduced form is feasible in the second-stage optimization w.r.t. $\theta(\sigma)$. Unfortunately, we do not know how to solve the two-stage optimization problem efficiently, \argyrisnote{Argyris: Maybe writing it as "as the set of feasible dual parameter has size exponential in $n$ and $m$"} as the number of dual parameters is exponential in $n$ and $m$, enumerating through all possible dual parameters is not an option. To overcome this obstacle, we need ideas explained in the following step.

}

%For every collection of dual parameters $\theta$, denote $\optlp(\theta)$ the optimum objective of the LP in~\Cref{fig:LP-fixed-parameter}. There are two direct observations from the LP in~\Cref{fig:LP-fixed-parameter}. Firstly, for every $\theta$, with access to a separation oracle for $W_i$ for every $i$, we can solve the LP in polynomial time. Secondly, $\max_{\theta\in \Theta}\{\optlp(\theta)\}$, the highest LP optimum over all dual parameters in $\Theta$, is at least the maximum $\core(\widehat{w},\theta(\widehat{w}))$ over all feasible $\widehat{w}\in \cP$.\footnote{We slightly abuse notation here, and use $\theta(\widehat{w})$ to denote the dual parameters specified in Lemma~\ref{lem:caiz17-constrained-additive} given a marginal reduced form. Clearly, $\Theta$ contains all possible $\theta(\widehat{w})$.} It implies that if $\theta^*$ is the best dual parameters that maximizes $\optlp(\theta)$, and the variables $\hat{w}^*$ are the optimal solution that achieves $\optlp(\theta^*)$, then $\widehat{w}^*$ induces a TPT that is approximately optimal. 


%Therefore, if we can enumerate all possible parameters and find the best parameters $\theta$ and variables $w$ that enables $\max_{\theta}\{\optlp(\theta)\}$, then $w$ induces a simple mechanism that is approximately optimal. 


\vspace{-.15in}
\paragraph{Step 3: Lifting the problem to a higher dimensional space.}

Instead of enumerating all possible dual parameters $\theta$, we optimize over \emph{distributions of the parameters}. To guarantee that the number of decision variables in our program is polynomial, we focus on \emph{product distributions} over the parameters. Formally, for every $i,j$, let $\cC_{ij}$ be a distribution over $\cV_{ij}\times \Delta$, where $\cV_{ij}$ and $\Delta$ are the set of possible values of $\beta_{ij}$ and $c_i$ accordingly, after discretization 
%(see \Cref{subsec:result} for a formal definition)
(See Footnote~\ref{footnote:discretization in lp} in  Figure~\ref{fig:bigLP} for a formal definition). All $\cC_{ij}$'s are independent. In our program, we use decision variables $\{\hat{\lambda}_{ij}(\beta_{ij},\delta_{ij})\}_{i\in[n],j\in[m],\beta_{ij}\in \cV_{ij},\delta_{ij}\in \Delta}$ to represent the distribution $\cC_{ij}$, i.e., $\hat\lambda_{ij}(a,b)=\Pr_{(\beta_{ij},\delta_{ij}) \sim \cC_{ij}}[\beta_{ij} = a \land \delta_{ij} = b]$. {Notice that if the parameters are drawn from a product distribution, %the parameter $c_i$ might end up mapping to a different distribution over $\Delta$ for different item $j$. 
the parameter ``$c_i$'' may be different for each item $j$. To distinguish them, we use $\delta_{ij}$ to replace the original parameter $c_i$ in our program.  } 
%Denote $\cB_{ij}$ the marginal distribution of $\beta_{ij}$ with respect to $\cC_{ij}$.

Now we maximize the expected value of the $\core$ function over all product distributions $\times_{i,j}\cC_{ij}$ (represented by decision variables $\hat{\lambda}$) and the allocations (represented by the marginal reduced form $\widehat{w}$). {If the parameters $\theta$ and allocation $\widehat{w}$ are generated independently,} the expected $\core$ is not a linear objective, since the contributed truncated welfare in $\core$ is $\widehat{w}_{ij}(t_{ij})\cdot \hat{\lambda}_{ij}(\beta_{ij},\delta_{ij})\cdot t_{ij}\cdot \ind[t_{ij}\leq \beta_{ij}+\delta_{ij}]$ for every $t_{ij},\beta_{ij},\delta_{ij}$. \emph{To linearize the objective, we lift the problem to a higher dimensional space and consider joint distributions over the parameters and allocations.} %lift both variables $\widehat{w}\in [0,1]^{\sum_{i,j}|\cT_{ij}|}$ and $\hat{\lambda}\in \times_{i,j}(\cV_{ij}\times \Delta)$ to a higher dimension.
We do not consider arbitrary joint distributions, and only focus on the ones that correspond to the following generative process: first draw $(\beta,\delta)$ from a product distribution (according to $\hat\lambda$), then choose a feasible allocation $\widehat{w}^{(\beta,\delta)}=\{\widehat{w}^{(\beta,\delta)}_{ij}(t_{ij})\}_{i,j,t_{ij}}$  conditioned on $(\beta,\delta)$. Since there are too many parameters $(\beta,\delta)$, we certainly cannot afford to store all $\widehat{w}^{(\beta,\delta)}$'s explicitly.
\notshow{Even though we do not directly use the $\widehat{w}^{(\beta,\delta)}$'s as decision variables, they are indeed crucial for understanding many of the constraints in our LP relaxation in \Cref{fig:bigLP}. See \Cref{subsec:result} for more discussion.}
Instead, for each bidder $i$ and item $j$ we introduce a new set of decision variables $\{\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\}_{t_{ij}\in\cT_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}\in \Delta}$, where $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$ is the marginal probability for the following three events to happen simultaneously in our generative process: \textbf{(a)} $(\beta_{ij},\delta_{ij})$ are the parameters for $i$ and $j$. \textbf{(b)} Bidder $i$ receives item $j$. \textbf{(c)} Bidder $i$'s value for item $j$ is $t_{ij}$. Formally,
\vspace{-.12in}
\begin{equation}\label{equ:explain-lambda}
\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\hat{\lambda}_{ij}(\beta_{ij},\delta_{ij})\cdot\sum_{\{(\beta_{i'j'},\delta_{i'j'})\}_{(i',j')\not=(i,j)}}\left({\widehat{w}_{ij}^{(\beta,\delta)}(t_{ij})}/{f_{ij}(t_{ij})}\right)\cdot \prod_{(i',j')\not=(i,j)}\hat{\lambda}_{i'j'}(\beta_{i'j'},\delta_{i'j'})
\end{equation}
\vspace{-.15in}

\noindent With the new variables $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$'s, we can express the objective as an linear function: 
\vspace{-.12in}
$$ \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}} 
 f_{ij}(t_{ij})\cdot t_{ij}\cdot \sum_{\beta_{ij}\in \cV_{ij},\delta_{ij} \in \Delta} \lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[t_{ij}\leq \beta_{ij} + \delta_{ij}].$$
\vspace{-.15in}



%In particular, we consider a relaxation that maximizes the expected $\core$ function over the joint measure between $[0,1]^{\sum_{i,j}|\cT_{ij}|}$ and $\times_{i,j}(\cV_{ij}\times \Delta)$. For every $\beta=\{\beta_{ij}\}_{i,j}$ and $\delta=\{\delta_{ij}\}_{i,j}$, we denote $\{\widehat{w}^{(\beta,\delta)}_{ij}(t_{ij})\}_{i,j,t_{ij}}$ the marginal reduced form conditioned on the realized $(\beta,\delta)$ in the joint measure. 

\notshow{
There is a set of decision variables $\lambda$ in our program representing the marginal expected value of $\frac{\widehat{w}_{ij}^{(\beta,\delta)}(t_{ij})}{f_{ij}(t_{ij})}$ on coordinate $(\beta_{ij},\delta_{ij})$. Formally, for every $t_{ij}\in \cT_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}\in \Delta$, there is a decision variable $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$ in our program that satisfies
\begin{equation}\label{equ:explain-lambda}
\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\hat{\lambda}_{ij}(\beta_{ij},\delta_{ij})\cdot\sum_{\{(\beta_{i'j'},\delta_{i'j'})\}_{(i',j')\not=(i,j)}}\frac{\widehat{w}_{ij}^{(\beta,\delta)}(t_{ij})}{f_{ij}(t_{ij})}\cdot \prod_{(i',j')\not=(i,j)}\hat{\lambda}_{i'j'}(\beta_{i'j'},\delta_{i'j'})
\end{equation}
}
\noindent Our program can be viewed as an ``expected version'' of the the two-stage optimization, when the parameters $\theta=(\beta,\delta)\sim \bigtimes_{i,j}\cC_{ij}$. In other words, we only require the constraints to be satisfied in expectation. We discuss our relaxation in more details in \Cref{subsec:result}.% about every constraint in our program with Equations~\eqref{equ:explain-lambda} and~\eqref{equ:explain-w}.

%is essentially an ``expected version'' of the LP in \Cref{fig:LP-fixed-parameter}, when the parameter $\theta=(\beta,\delta)\sim \times_{i,j}\cC_{ij}$. Now, the marginal reduced form variables $w=\{w_{ij}(t_{ij})\}_{i,j,t_{ij}}$ can be viewed as the expectation of $\widehat{w}^{(\beta,\delta)}$:
\notshow{
\begin{equation}\label{equ:explain-w}
w_{ij}(t_{ij})=\sum_{\beta,\delta}\widehat{w}_{ij}^{(\beta,\delta)}(t_{ij})\cdot \prod_{i',j'}\hat{\lambda}_{i'j'}(\beta_{i'j'},\delta_{i'j'})\quad\forall i,j,t_{ij}\in \cT_{ij}
\end{equation}
}
 

\vspace{-.1in}
\subsection{Our LP and a Sketch of the Proof of~\Cref{thm:main XOS-main body}}\label{subsec:result}

We present a sketch of the proof of \Cref{thm:main XOS-main body} for  constrained-additive bidders and our main linear program (\Cref{fig:bigLP}). Although the LP has many constraints and may seem intimidating at first, all constraints follow quite naturally from our derivation in \Cref{sec:tour to LP}. See \Cref{sec:explain LP constraints} for more~details.

The first step of our proof is to estimate $\prev$ using \Cref{thm:chms10} from~\cite{ChawlaHMS09}. 

\vspace{-.1in}
\begin{lemma}[Theorem~14 and Appendix~F in \cite{ChawlaHMS09}]\label{thm:chms10}

There exists an algorithm that with probability at least $1-\frac{2}{n}$, computes a Rationed Posted Price mechanism $\cM$ such that $\rev(\cM) \geq \frac{1}{6.75}\left(1- \frac{2}{n}\right)\cdot\prev$. The algorithm runs in time $poly(n,m,\sum_{i,j}|\cT_{ij}|)$.
\end{lemma}
\vspace{-.1in}

 Denote $\cE$ the event that an RPP in \Cref{thm:chms10} is computed successfully. For simplicity, we will condition on the event $\cE$ for the rest of this section. Let $\estprev$ be the revenue of the RPP mechanism found in \Cref{thm:chms10}.
 
 Next, we argue that the LP in~\Cref{fig:bigLP} (or \Cref{fig:XOSLP} when the valuations are XOS) can be solved efficiently. Note that there are $\poly(n,m,\sum_{i,j}|\cT_{ij}|)$ constraints except for Constraint $\Wconstraint$, where we need to enforce the feasibility of single-bidder marginal reduced forms. It suffices to construct an efficient separation oracle for $W_i$ for every $i$. However, to the best of our knowledge, $W_i$ does not have a succinct explicit description or an efficient separation oracle. For constrained-additive valuations, we construct another polytope $\widehat{W}_i$ such that: (i) $\widehat{W}_i$ is a multiplicative approximation of $W_i$, i.e., $c\cdot W_i\subseteq \widehat{W}_i\subseteq W_i$ for some absolute constant $c\in (0,1)$, and (ii) There exists an efficient separation oracle for $\widehat{W}_i$ given access to the demand oracle. %We provide a formal statement in \Cref{thm:multiplicative approx for constraint additive-main body}.

\begin{theorem}\label{thm:multiplicative approx for constraint additive-main body}
Let $T=\sum_{i,j}|\cT_{ij}|$ and $b$ be the bit complexity of the problem instance (\Cref{def:bit complexity}). For any $i\in [n]$ and $\delta\in (0,1)$, there is an algorithm  that constructs a convex polytope $\widehat{W}_i\in [0,1]^{\sum_{j\in [m]}|\cT_{ij}|}$ using $\poly(n,m,T,\log(1/\delta))$ samples from $D_i$, such that with probability at least $1-\delta$,

\begin{enumerate}
\vspace{-.1in}
  \item $\frac{1}{12}\cdot W_i\subseteq \widehat{W}_i\subseteq W_i$, and the vertex-complexity (\Cref{def:vertex-complexity}) of $\widehat{W}_i$ is $\poly(n,m,T,b,\log(1/\delta))$.
\vspace{-.05in}
\item There exists a separation oracle $SO$ for $\widehat{W}_i$, given access to the demand oracle for bidder $i$'s valuation. The running time of $SO$ on any input with bit complexity $b'$ is $\poly(n,m,T,b,b',\log(1/\delta))$ and makes $\poly(n,m,T,b,b',\log(1/\delta))$ queries to the demand oracle.
  \end{enumerate}
  \vspace{-.1in}
The algorithm constructs the polytope and the separation oracle $SO$ in time %$\poly(n,m,T,\log(1/\delta))$ 
$\poly(n,m,T,b,\log(1/\delta))$.
\end{theorem}
  \vspace{-.02in}

\noindent Indeed, we prove a more general result regarding polytopes that can be expressed as a ``mixture of polytopes'' (\Cref{thm:special case of multiplicative approx}), which can be viewed as a generalization of the technique developed in~\cite{CaiDW12bfull} for approximating the polytope of all feasible reduced forms. 
We postpone the proof of \Cref{thm:multiplicative approx for constraint additive-main body} to \Cref{sec:mrf for constraint additive}. %Equipped with \Cref{thm:multiplicative approx for constraint additive-main body}, we continue our proof of Theorem~\ref{thm:main XOS-main body} for constrained-additive valuations. 

To solve the LP relaxation, we replace $W_i$ by $\widehat{W}_i$ in the LP in~\Cref{fig:bigLP} for every $i\in [n]$, and solve the LP in polynomial time using the ellipsoid method. Clearly, this solution is also feasible for the original LP in~\Cref{fig:bigLP}. Moreover, since $\widehat{W}_i$ contains $c\cdot W_i$, we can show that \textbf{the objective value of the solution we computed is at least $c\cdot \optlp$}, where $\optlp$ the optimum of the LP in Figure~\ref{fig:bigLP}. Our proof of \Cref{thm:multiplicative approx for constraint additive-main body} heavily relies on the fact that $W_i$ is a down-monotone polytope,\footnote{A polytope $\cP\subseteq [0,1]^d$ is down-monotone if and only if for every $\bx\in \cP$ and $\textbf{0}\leq \bx'\leq \bx$, we have $\bx'\in \cP$.}  which does not hold in the XOS case.  For XOS valuations, we construct the polytope $\widehat{W}_i$ with a weaker guarantee:
For every vector $x$ in $W_i$, there exists another vector $x'$ in $\widehat{W}_i$ such that for every coordinate $j$, $x_j/x_j'\in [a,b]$ for some absolute constant $0<a<b$, and vice versa. See \Cref{sec:mrf for xos} for a complete proof of \Cref{thm:main XOS-main body} (including the XOS case).














% Denote $\optlp$ the optimum of the LP in Figure~\ref{fig:bigLP}. 
 
 %for constrained-additive bidders and the optimum of the LP in Figure~\ref{fig:XOSLP} %(\yangnote{Add reference}) for XOS bidders.



%\argyrisnote{Note about the above lemma: Maybe we need to rebate when using the $c_i$, I think we can avoid that in the LP by relaxing the (5) constraint to be $\sum_i c_i \leq 16 \prev$? I also think we need to rethink the the argument in the proof that uses the definition of polytope $W_i$.}



%Lemma~\ref{lem:bound rev by opt} shows that the optimum of the LP in \Cref{fig:bigLP} upper bounds the \core. 
Next, we argue that the LP optimum can be approximated by simple mechanisms. \cite{CaiZ17} shows that for any BIC and IR mechanism $\cM$, $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},\vr^{(\sigma)})$ (as stated in Lemma~\ref{lem:caiz17-constrained-additive}) can be bounded by 
%the revenue of two-part tariff mechanisms.
a constant number of $\prev$ and the revenue of a TPT (see Property 5 of \Cref{lem:caiz17-constrained-additive}). 
We generalize their result by proving that for any feasible solution of the LP, its objective can be bounded by (a constant times) the revenue of a RPP or TPT mechanism, and the mechanism can be computed efficiently given the feasible~solution.

%Let $(w,\lambda,\hat\lambda, d=(d_i)_{i\in [n]})$ be any fixed feasible solution of the LP in \Cref{fig:bigLP}. We need the following definition.

%\vspace{-.02in}
\begin{definition}\label{def:Q_j}
%Given an optimal solution %$\{\lambda_{i,j}(\beta)\}_{\beta \in V_{i,j}(T_{i,j})}$,
%of the program above,
Let $(w,\lambda,\hat\lambda, \bd=(d_i)_{i\in [n]})$ be any feasible solution of the LP in \Cref{fig:bigLP}. %For every $j\in [m]$, define 
For every $j\in [m]$, define 
$Q_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot t_{ij}\cdot
    \sum_{{\beta_{ij}\in \cV_{ij}, \delta_{ij} \in \Delta}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot\ind[t_{ij}\leq \beta_{ij}+\delta_{ij}].\footnote{\text{Recall that $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$ is introduced in Step 3 of~\Cref{sec:tour to LP}. See~\Cref{fig:bigLP} for the formal definition.}}
$

%For any $i,j,\beta_{ij}\in \cV_{ij},\delta_{ij}\in \Delta_i$, define

%$$g_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})<\beta_{ij} + \delta_{ij}]+\lambda_{ij}^{(r)}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})=\beta_{ij} + \delta_{ij}]$$

%We denote by $B_{i,j} \times \Delta_{i,j}$ a coupled distribution over $V_{i,j}(T_{i,j}) \times \Delta_{i}$ such that: $\Pr_{(\beta,\delta) \sim B_{i,j} \times \Delta_{i,j}}[\beta = a \land \delta = b]= \lambda'_{i,j}(\beta_{i,j}=a, \delta_{i,j} = b)$.


%For XOS bidders, let $(\pi, w,\lambda,\hat\lambda, \bd=(d_i)_{i\in [n]})$ be any feasible solution of the LP in \Cref{fig:XOSLP}. 

%$$Q_j = \frac{1}{2}\cdot\sum_{i\in[n]}\sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
%    \sum_{\substack{\beta_{ij}\in \cV_{ij}\\\delta_{ij} \in \Delta}}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\cdot\ind[V_{ij}(t_{ij})\leq \beta_{ij}+\delta_{ij}].
%$$
\end{definition}

%\mingfeinote{Mingfei: To save some space, I suggest we remove the $Q_j$ definition for XOS bidders as we did for $\hat{Q}_j$. We will mention in the prelim that for constrained-additive, $V_{ij}(t_{ij})=t_{ij}$.}
%\yangnote{Yang: I'm ok with moving all definitions for XOS to the appendix.}

%\vspace{-0.02in}

%To bound the objective function of the LP, we construct two-part tariff mechanism $\Mtpt$ (Mechanism~\ref{def:constructed-SPEM}). 
Clearly, for any feasible solution of the LP, the objective function is $2\cdot \sum_{j\in [m]}Q_j$. We prove in \Cref{thm:bounding-lp-simple-mech} that $2\cdot \sum_{j\in [m]}Q_j$ can be bounded by the revenue of $\Mtpt$ (Mechanism~\ref{def:constructed-SPEM}) and the RPP $\Mpp$ (\Cref{thm:chms10}).  As we can efficiently compute a feasible solution whose objective is $\Omega(\optlp)$, \Cref{thm:bounding-lp-simple-mech} implies that we can compute in polynomial time a simple mechanism whose revenue is at least $\Omega(\optlp+\prev)$.




%\vspace{-.05in}
\begin{theorem}\label{thm:bounding-lp-simple-mech}
Let $(w,\lambda,\hat\lambda, \bd)$ %(or  $(\pi,w,\lambda,\hat\lambda, \bd)$) 
be any feasible solution of the LP in \Cref{fig:bigLP}.
%Then for sufficiently small $\epsilon_r$, 
Let $\Mpp$ be the rationed posted price mechanism computed in \Cref{thm:chms10}. Let $\Mtpt$ be the two-part tariff mechanism shown in Mechanism~\ref{def:constructed-SPEM} {with prices $\{Q_j\}_{j\in[m]}$}. Then the objective function of the solution $2\cdot \sum_{j\in [m]}Q_j$ is bounded by $c_1\cdot \rev(\Mpp)+c_2\cdot \rev(\Mtpt)$, for some absolute constant $c_1,c_2>0$. 
%for some \mingfeinote{restricted SPM} $\cM_1$ and some \mingfeinote{SPEM} $\cM_2$. 
Moreover, both $\Mpp$ and $\Mtpt$ can be computed in time $\poly(n,m,\sum_{i,j}|\cT_{ij}|)$ with access to the demand oracle for the bidders'~valuations. 
%(for constrained-additive valuations) or \todo{the scalable demand oracle} (for XOS valuations). 
\end{theorem}



\newpage 
The proof of \Cref{thm:bounding-lp-simple-mech} combines the ``shifted \core'' technique by Cai and Zhao~\cite{CaiZ17} with several novel ideas to handle the new challenges due to the relaxation. We postpone it to \Cref{sec:proof of bounding LP with simple mech}.

%We define and analyze the ``shifted~\core''~in~\Cref{subsec:proof_lem:Q and Q-hat}. In~\Cref{sec:proof of bounding LP with simple mech}, we prove Theorem~\ref{thm:bounding-lp-simple-mech} building on the technique developed in~\Cref{subsec:proof_lem:Q and Q-hat}.


%In the previous section, we have shown in \Cref{thm:bounding-lp-simple-mech} that given any feasible solution of our program in \Cref{fig:bigLP} (or \Cref{fig:XOSLP}), we can compute simple mechanisms efficiently whose revenue is a constant factor of the objective of the program. In this section, we discuss how to compute a \emph{multiplicative approximation} of the optimum of the LP in polynomial time. %feasible solution of the LP, whose objective is a \emph{multiplicative approximation} of the optimum objective, in polynomial time.

%To complete the proof of Theorem~\ref{thm:main XOS-main body}, 


\begin{figure}[ht!]
\colorbox{MyGray}{
\begin{minipage}{.98\textwidth}
\small
$$\quad\textbf{max  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}} 
 f_{ij}(t_{ij})\cdot t_{ij}\cdot \sum_{\substack{\beta_{ij}\in \cV_{ij},\delta_{ij} \in \Delta}} \lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[t_{ij}\leq \beta_{ij} + \delta_{ij}]$$
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
\vspace{-.3in}
  \begin{align*}
\textbf{s.t.}\\
 &\quad\textbf{Allocation Feasibility Constraints:}\\
 &\quad\Wconstraint \quad w_i \in W_i & \forall i \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
&\quad\PiConstraint \quad \sum_i\sum_{t_{ij}\in \cT_{ij}}w_{ij}(t_{ij})\leq 1 & \forall j\\  
 &\quad\textbf{Natural Feasibility Constraints:}\\
    &\quad\LambdaMarginalConstraint\quad f_{ij}(t_{ij})\cdot\sum_{\beta_{ij}\in \cV_{ij}}\sum_{\delta_{ij}\in \Delta} \lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij}) = w_{ij}(t_{ij}) & \forall i,j,t_{ij}\in \cT_{ij}\\
    &\quad\CompareMarginalConstraint\quad\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}(\beta_{ij}, \delta_{ij}) & \forall i,j, t_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}\\
    &\quad\HatLambdaDistributionConstraint\quad \sum_{\substack{\beta_{ij}\in \cV_{ij},\delta_{ij} \in \Delta}} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) = 1 & \forall i,j\\
    &\quad\textbf{Problem Specific Constraints:}\\
    &\quad\ReduceDemandConstaint \quad \sum_{i\in[n]}\sum_{\beta_{ij} \in \cV_{ij}}\sum_{\delta_{ij}\in \Delta} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[t_{ij}\geq \beta_{ij}] \leq \frac{1}{2}& \forall j\\
    %& (5)\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \lambda_{ij}(t_{ij},\beta_{ij}) \leq  \hat\lambda_{ij}(\beta_{ij}^+) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})> \beta_{ij}] & \forall i,j,\beta_{ij}\in \cV_{ij}\\
    %&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\quad+\hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})\geq\beta_{ij}]\\
    & \quad\MarginalToGlobalConstraint\quad {\frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \left(\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})+ \lambda_{ij}(t_{ij},\beta_{ij}^+,\delta_{ij})\right) \leq} \\
    &\qquad\qquad\qquad\hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \cdot \Pr_{t_{ij}}[t_{ij}\geq \beta_{ij}]+\hat\lambda_{ij}(\beta_{ij}^+,\delta_{ij}) \cdot \Pr_{t_{ij}}[t_{ij}\geq\beta_{ij}^+] & \forall i,j,\beta_{ij}\in \cV_{ij}^0,\delta_{ij}\in \Delta\\
    %& \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) &\forall i\in[n], j \in[m] \\
    &\quad\BoundMeanDeltaConstraint\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}, \delta_{ij} \in \Delta}} \delta_{ij}\cdot \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \leq d_i  & \forall i,j\\
    &\quad\BoundSumDeltaConstraint\quad\sum_{i\in[n]} d_i \leq %\yangnote{16}\cdot \prev \\
   111\cdot \estprev\\
     &\qquad\quad \lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}(\beta_{ij},\delta_{ij})\geq 0,w_{ij}(t_{ij})\geq 0,d_i\geq 0 & \forall i,j,t_{ij},\beta_{ij}\in \cV_{ij},\delta_{ij}
\end{align*}

\textbf{Variables:}~\footnote{For every $i,j$, let $\cV_{ij}^0 = \cT_{ij}$ be the set of all possible values of $t_{ij}$. To address the tie-breaking issue in \Cref{remark:tie-breaking}, let $\eps_r>0$ be an arbitrarily small number,%\todo{Fix the $\eps_r$ here.} \yangnote{Yang: What do you want to say about $\varepsilon_r$?} 
 and define $\cV_{ij}^+ = \{t_{ij} + \eps_r: t_{ij} \in \cT_{ij}\}$ and $\cV_{ij} = \cV^0_{ij} \cup \cV^+_{ij}$. Let $\Delta$ be a geometric discretization of range $[\estprev/n,55\cdot\estprev]$. Formally, $\delta\in \Delta$ if and only if $\delta=\frac{2^x}{n}\cdot \estprev$ for some integer $x$ such that $0\leq x\leq\lceil\log(55n)\rceil$. Finally, 
for each $\beta \in \cV_{ij}^0$, let $\beta^+=\beta+\eps_r\in \cV_{ij}^+$. Note that the LP  (or the LP in~\Cref{fig:XOSLP}) do not depend on the choice of $\varepsilon_r$, so we can choose $\varepsilon_r$ to be sufficiently small. In fact, let $b$ be an upper bound of the bit complexity of the problem instance, and the bit complexity of any feasible solution of our LP. Our proof works as long as $\eps_r<\min\{\frac{1}{2^{\poly(b)}},\frac{\prev}{\sum_{i,j}|\cT_{ij}|}\}$.\label{footnote:discretization in lp}}

\vspace{.1in}
- $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$, for all $i,j$ and $t_{ij}\in \cT_{ij}$, $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta$. See Step 3 of \Cref{sec:tour to LP} for an explanation of this variable.

\vspace{.1in}
- $\hat\lambda_{ij}(\beta_{ij},\delta_{ij})$, for all $i$, $j$, $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta$, denoting the distribution $\cC_{ij}$ over $\cV_{ij}\times \Delta$.

\vspace{.1in}
- $w_{ij}(t_{ij})$, for all $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$, denoting the expected marginal reduced form. We denote $w_i=\{w_{ij}(t_{ij})\}_{j\in[m],t_{ij}\in\cT_{ij}}$ the vector of all variables associated with bidder $i$.

\vspace{.1in}
- $d_i$, for all $i\in [n]$, denoting an upper bound of the expectation of $\delta_{ij}$ over distribution $\cC_{ij}$ for all $j$.
\end{minipage}
}
\caption{LP Relaxation for Constrained-Additive Bidders}~\label{fig:bigLP}
%\vspace{-.2in}

\end{figure}

\begin{algorithm}[h!]
\floatname{algorithm}{Mechanism}
%\setstretch{1.35}
%\vspace{.1in}
\begin{algorithmic}[1]
\setcounter{ALG@line}{-1}
\State Before the mechanism starts, the seller computes the \emph{price} $Q_j$ (\Cref{def:Q_j}) for every item $j$.  
\State %Bidders arrive sequentially in an arbitrary order.
Bidders arrive sequentially in the lexicographical order.
\State When bidder $i$ arrive, the seller shows her the set of available items $S_i(t_{<i})\subseteq [m]$, as well as their prices. Note that $S_i(t_{<i})$ is the set of items that are not purchased by the first $i-1$ bidders, which depends on $t_{<i}$. We use $S_1(t_{<1})$ to denote $[m]$.
\State Bidder $i$ is asked to pay an \emph{entry fee}. The seller samples a type $t_i'\sim D_i$, and sets the entry fee as: $\xi_i(S_i(t_{<i}),t_i') = \max_{S'\subseteq S_i(t_{<i})}\left(v_i(t_i',S')-\sum_{j\in S'}Q_j\right)$. The entry fee is bidder $i$'s utility for her favorite set under prices $Q_j$'s if her type is $t'_i$.
\State If bidder $i$ (with type $t_i$) agrees to pay the entry fee 
$\xi_i(S_i(t_{<i}),t_i') $, then she can enter the mechanism and take her favorite set $S^*\in\argmax_{S'\subseteq S_i(t_{<i})}\left(v_i(t_i,S')-\sum_{j\in S'}Q_j\right)$, by paying $\sum_{j\in S^*}Q_j$. Otherwise, the bidder gets nothing and pays 0. 
\end{algorithmic}
\caption{{\sf \quad Two-part Tariff Mechanism $\Mtpt$}}\label{def:constructed-SPEM}
\end{algorithm}

\begin{remark} \label{remark:lexi-order}
\Cref{thm:bounding-lp-simple-mech} indeed holds even if the bidders arrive in an arbitrary order in $\Mtpt$. We choose the lexicographical order only to keep the notation light. %Similar for Mechanism~\ref{mech:variant-tpt} and Mechanism~\ref{def:general SPEM}. 
\end{remark}

 We complete the last step of our proof by showing $\opt= O(\optlp+\prev)$ in~\Cref{lem:bound rev by opt}. More specifically, we show that for any mechanism $\cM=(\sigma,p)$, the tuple $(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},r^{(\sigma)})$ stated in \Cref{lem:caiz17-constrained-additive} corresponds to a feasible solution of the LP in~\Cref{fig:bigLP} whose objective is at least $\core(\sigma,\tilde{\vBeta}^{(\sigma)},\vC^{(\sigma)},r^{(\sigma)})$. Hence, the revenue of $\cM$ is upper bounded by $\prev$ and $\optlp$. The proof is postponed to \Cref{subsec:proof_lem:bound rev by opt}. Indeed, for both \Cref{thm:bounding-lp-simple-mech} and \Cref{lem:bound rev by opt}, we prove a general statement that applies to XOS valuations, which requires a generalized LP and definitions. See \Cref{thm:bounding-lp-simple-mech-XOS} and \Cref{lem:bound rev by opt-XOS} in \Cref{sec:appx_program} for details. %Indeed, we prove a generalization of Theorem~\ref{thm:bounding-lp-simple-mech} as Theorem~\ref{thm:bounding-lp-simple-mech-XOS} in \Cref{sec:appx_program}. 

\begin{lemma}\label{lem:bound rev by opt}
%For sufficiently small $\varepsilon_r$ \todo{fix the value $\varepsilon_r$} and 
For any BIC and IR mechanism $\cM$, $\rev(\cM)\leq 28\cdot \prev+4\cdot\optlp$.
\end{lemma}

\subsection{Interpretation of Our LP in~\Cref{fig:bigLP}.}~\label{sec:explain LP constraints} We explain our LP in this section. The objective is the expected \core, as explained in Step 3 in \Cref{sec:tour to LP}. %are going to explain every constraint in the program as well as the objective. With \Cref{equ:explain-lambda}, the objective can be viewed as $\E_{\theta}[\core(\widehat{w}^{\theta},\theta)]$, the expected $\core$ function under the marginal reduced form $\widehat{w}^{\theta}$, when the dual parameters $\theta=(\beta,\delta)$ is drawn from $\times_{i,j}\cC_{ij}$. 
%To explain the constraints, for every $i,j,t_{ij}$, we consider  
%\begin{equation}\label{equ:explain-w}
%w_{ij}(t_{ij})=\sum_{\beta,\delta}\widehat{w}_{ij}^{(\beta,\delta)}(t_{ij})\cdot \prod_{i',j'}\hat{\lambda}_{i'j'}(\beta_{i'j'},\delta_{i'j'}),
%\end{equation}
%which is the expected marginal reduced form of $\widehat{w}^{(\beta,\delta)}$ where $(\beta,\delta)\sim \times_{i,j}\cC_{ij}$. Then 
According to our definition of $\lamij$ and Constraint~\LambdaMarginalConstraint, $\{w_{ij}(t_{ij})\}_{i,j,t_{ij}}$ corresponds to the expected marginal reduced form, that is, $w_{ij}(t_{ij})$ is the expected probability for bidder $i$ to receive item $j$ and her value for item $j$ is $t_{ij}$.
Constraints~\Wconstraint~and~\PiConstraint~simply sets the feasible region of the expected marginal reduced form $w$. They follow directly from the fact that every realized $\widehat{w}^{(\beta,\delta)}$ is feasible (see Step 3 in \Cref{sec:tour to LP}).  %Constraint~\LambdaMarginalConstraint~draws the connection between $\lambda$ and $w$. It follows directly from Equations~\eqref{equ:explain-lambda} and \eqref{equ:explain-w}. 
Constraint~\CompareMarginalConstraint~follows from \Cref{equ:explain-lambda} and the fact that every ${\widehat{w}_{ij}^{(\beta,\delta)}(t_{ij})}/{f_{ij}(t_{ij})}$ is in $[0,1]$. Constraint~\HatLambdaDistributionConstraint~implies that $\{\hat\lambda_{ij}(\beta_{ij},\delta_{ij})\}_{\beta_{ij},\delta_{ij}}$ correspond to a distribution $\cC_{ij}$. 


Constraints~\ReduceDemandConstaint~-~\BoundSumDeltaConstraint~are specialized for our problem, which guarantees that the LP optimum can be bounded by simple mechanisms. Constraint~\ReduceDemandConstaint~follows from taking expectation on both sides of Constraint~\BetaConstraintFP~in \Cref{fig:LP-fixed-parameter}, over the randomness of $\beta_{ij}$. Constraints~\BoundMeanDeltaConstraint~and~\BoundSumDeltaConstraint~correspond to Constraint~\CiConstraintFP~in \Cref{fig:LP-fixed-parameter}. Here we bound the expectation of $\delta_{ij}$ by a unified upper bound $d_i$ for every $j$.\footnote{This corresponds to the fact that in \Cref{lem:caiz17-constrained-additive} (and \Cref{fig:LP-fixed-parameter}), there is a single $c_i$ that represents $\delta_{ij}$.} It is worth emphasizing Constraint~\MarginalToGlobalConstraint, which corresponds to Constraint \WBetaConstraintFP~in \Cref{fig:LP-fixed-parameter} (and \Cref{fig:LP-relaxed-stageii}). Instead of taking expectations over the dual parameters, we force the constraint to hold for every $\beta_{ij}$ and $\delta_{ij}$. %only take expectation over the $\delta_{ij}$'s.
This is an important property that is crucial in our analysis (see \Cref{fn:constraint 7} in \Cref{lem:Q and Q-hat}). Readers may notice that Constraint~\PiConstraint~is implied by Constraints {\LambdaMarginalConstraint}, {\ReduceDemandConstaint} and {\MarginalToGlobalConstraint}. We keep~Constraint~\PiConstraint~so that it is clear that the supply constraint is enforced over the (expected) marginal reduced~form. 
The Problem Specific Constraints~\ReduceDemandConstaint-\BoundSumDeltaConstraint~ in the LP in Figure~\ref{fig:bigLP} are expected versions of the constraints in the two-stage optimization problem in Figure~\ref{fig:LP-fixed-parameter}, which are directly inspired by the Properties~1, 2, and 3 in Lemma~\ref{lem:caiz17-constrained-additive}.
They are crucial to guarantee that optimal value of the LP in Figure~\ref{fig:bigLP} is still approximable by simple mechanisms.




%%%%%%%%% END of this section %%%%%%%%%%%%%%


\notshow{
\section{Backup section (only for checking)}

\begin{align*}
    (P) = 
    \max& \frac{1}{2} \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{i,j}\in T_{i,j}}  f_{i,j}(t_{i,j})\cdot V_{i,j}(t_{i,j})\cdot
    \\
    &\quad \quad\sum_{\substack{\beta\in V_{i,j}(T_{i,j}),\delta \in \Delta V_{i}}} \lambda_{i,j}(t_{i,j},\beta, \delta)\cdot \mathds{1}[V_{i,j}(t_{i,j}) \leq \beta + \delta]\\
    s.t.\quad & \pi_i \in \Pi_i  & \forall i \in[n] \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    & \sum_{\beta}\lambda_{i,j}(t_{i,j},\beta) = \pi_{i,j}(t_{i,j}) & \forall i\in[n],j\in[m],t_{i,j}\in T_{i,j}\\
    & \sum_{i\in[n]}\sum_{t_{i,j}\in T_{i,j}} f_{i,j}(t_{i,j})\cdot \pi_{i,j}(t_{i,j}) \leq 1, & \forall j \in[m] \\
    & \lambda_{i,j}(t_{i,j},\beta, \delta) \leq \lambda_{i,j}'(\beta, \delta) & \forall i\in[n], j \in[m], t_{i,j} \in T_{i,j}\\ 
    &\sum_{t_{i,j}} f_{i,j}(t_{i,j}) \lambda_{i,j}(t_{i,j},\beta) \leq \frac{1}{2}\cdot \lambda'_{i,j}(\beta) \Pr_{t_{i,j}\sim D_{i,j}}[t_{i,j} \geq \beta] & \forall \beta \in V_{i,j}(T_{i,j})\\
    & \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) \text{(Maybe not needed)} &\forall i\in[n], j \in[m] \\
    & \sum_{\delta \in \Delta V_i} \delta \lambda_{i}'(\delta) \leq \delta_i  & \forall i \in [n]\\
    & \sum_{i\in[n]} \delta_i \leq O(1) \cdot \srev \\
     & \forall i \in[n],j\in [m],t\in T_{i,j},\beta,\gamma \in V_{i,j}(t_{i,j})\\
\end{align*}
}


\notshow{


\section{Old Main Program (for reference only)}
%\argyrisnote{Do we agree that the first among the two programs is the one we are going to focus on?}

The variables in the LP are as follows:
\begin{enumerate}
    \item $\pi_{ij}(t_{ij})$, for all $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We denote $\pi_i=(\pi_{ij}(t_{ij}))_{j,t_{ij}}$ the vector of all variables associated with bidder $i$.
    \item $w_{ij}(t_{ij})$, for all $i\in [n],j\in [m],t_{ij}\in \cT_{ij}$. We denote $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}}$ the vector of all variables associated with bidder $i$.
    \item $\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij}),\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})$, for all $i,j$ and $t_{ij}\in \cT_{ij}$, $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta_i$.
    \item $\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij}), \hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$, for all $\beta_{ij}\in \cV_{ij}, \delta_{ij}\in \Delta_i$, %denoting the joint distribution over $\cV_{ij}\times \Delta_i$.
    \item $d_i$, for all $i\in [n]$.
\end{enumerate} \todo{To add some explanation of the variables.} In the LP, we will abuse the notations and let $\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})=\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})+\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})$, $\lambda_{ij}(t_{ij},\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\lambda_{ij}(t_{ij},\beta_{ij},\delta_{ij})$. Similarly, let $\hat\lambda_{ij}(\beta_{ij},\delta_{ij})=\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})+\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}^{(r)}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})$, $\hat\lambda_{ij}(\beta_{ij})=\sum_{\delta_{ij}\in\Delta_i}\hat\lambda_{ij}(\beta_{ij},\delta_{ij})$. 

%Let $W_{i}$ be the polytope of feasible normalized welfare for bidder $i$.
%That is, $w_i=(w_{ij}(t_{ij}))_{j,t_{ij}}$ is in $W_i$ if and only if there exists an allocation (for bidder $i$) $\{\sigma_{iS}(\cdot)\}_{S\subseteq [m]}$, such that $$w_{ij}(t_{ij})\cdot V_{ij}(t_{ij}) = \sum_{t_{i,-j}\in \cT_{i,-j}} f_{i,-j}(t_{i,-j})\sum_{S:j\in S}\sigma_{iS}(t_{ij},t_{i,-j})\cdot\gamma_{ij}^{S}(t_i),$$
%where $\gamma_{ij}^{S}(t_i)$ is bidder $i$'s supporting price for item $j$ with respect to set $S$. \todo{Add a definition $\gamma_{ij}^S(t_i)=\alpha_{ij}^{k(t_i,S)}$.}
%\mingfeinote{Add definition of ``supporting price''. Should be $\alpha_j^k$ instead.} \argyrisnote{I think it should be $\alpha_j^k$ instead.}

\begin{align*}
    (P)
    &\quad\text{maximize  } \sum_{i\in[n]} \sum_{j\in[m]} \sum_{t_{ij}\in \cT_{ij}}  f_{ij}(t_{ij})\cdot V_{ij}(t_{ij})\cdot
    \\
    &\sum_{\substack{\beta_{ij}\in \cV_{ij},\delta_{ij} \in \Delta_i}} \left(\lambda_{ij}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})<\beta_{ij} + \delta_{ij}]+\lambda_{ij}^{(r)}(t_{ij},\beta_{ij}, \delta_{ij})\cdot \ind[V_{ij}(t_{ij})=\beta_{ij} + \delta_{ij}]\right)\\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    s.t.\quad & (1)\quad (\pi_i,w_i) \in W_i & \forall i \\
    %s.t.\quad & (\pi_i, w_i) \in (\Pi_i,W_i)  & \forall i \in[n] \\
    & (2)\quad f_{ij}(t_{ij})\cdot\sum_{\beta_{ij}\in \cV_{ij}} \lambda_{ij}(t_{ij},\beta_{ij}) = w_{ij}(t_{ij}) & \forall i,j,t_{ij}\in \cT_{ij}\\
    &(3) \quad \sum_i\sum_{t_{ij}\in \cT_{ij}}\pi_{ij}(t_{ij})\leq 1 & \forall j\\
    &(4) \quad \sum_{i\in[n]}\sum_{\beta_{ij} \in \cV_{ij}} \hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})> \beta_{ij}]+\hat\lambda_{ij}^{(r)}(\beta_{ij}) \cdot \Pr_{t_{ij}\sim D_{ij}}[V_{ij}(t_{ij})=\beta_{ij}] \leq \frac{1}{2} & \forall j\\
    & (5)\quad \frac{1}{2}\sum_{t_{ij} \in \cT_{ij}} f_{ij}(t_{ij}) \lambda_{ij}(t_{ij},\beta_{ij}) \leq  \hat\lambda_{ij}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})> \beta_{ij}]+\hat\lambda_{ij}^{(r)}(\beta_{ij}) \cdot \Pr_{t_{ij}}[V_{ij}(t_{ij})=\beta_{ij}] & \forall i,j,\beta_{ij}\in \cV_{ij}\\
    & (6)\quad\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}^{(r)}(\beta_{ij}, \delta_{ij}),\quad \lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})\leq \hat\lambda_{ij}^{(n)}(\beta_{ij}, \delta_{ij}) & \forall i,j, t_{ij},\beta_{ij},\delta_{ij}\\
    %& \lambda_{i}'(\delta) = \sum_{\beta \in V_{i,j}(T_{i,j})} \lambda_{i,j}'(\beta, \delta) &\forall i\in[n], j \in[m] \\
    & (7)\quad \sum_{\substack{\beta_{ij}\in \cV_{ij}, \delta_{ij} \in \Delta_i}} \delta_{ij}\cdot \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) \leq d_i  & \forall i,j\\
    & (8)\quad\sum_{i\in[n]} d_i \leq 8\cdot \prev \text{\todo{Change the constant if needed.}}\\
    &(9)\quad \sum_{\substack{\beta_{ij}\in \cV_{ij},\delta_{ij} \in \Delta_i}} \hat\lambda_{ij}(\beta_{ij},\delta_{ij}) = 1 & \forall i,j\\
     & w_{ij}(t_{ij})\geq 0,\lambda_{ij}^{(r)}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\lambda_{ij}^{(n)}(t_{ij},\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}^{(r)}(\beta_{ij},\delta_{ij})\geq 0,\hat\lambda_{ij}^{(n)}(\beta_{ij},\delta_{ij})\geq 0 & \forall i,j,t_{ij},\beta_{ij},\delta_{ij}
\end{align*}



}

==> srev.tex <==
%\argyrisnote{Question: Using the result in \cite{ChawlaHMS09}, suffices to argue that we can calculate \prev, right?}

%\mingfeinote{What do you mean by $\srev$? Is it the optimal revenue achieved by sequential posted price mechanism (restricted to buy one item)?}
%\argyrisnote{Yes, I meant $\prev$}

